Robustness and Reliability When Training With Noisy Labels

Labelling of data for supervised learning can be costly and time-consuming and the risk of incorporating label noise in large data sets is imminent. When training a flexible discriminative model using a strictly proper loss, such noise will inevitably shift the solution towards the conditional distribution over noisy labels. Nevertheless, while deep neural networks have proven capable of fitting random labels, regularisation and the use of robust loss functions empirically mitigate the effects of label noise. However, such observations concern robustness in accuracy, which is insufficient if reliable uncertainty quantification is critical. We demonstrate this by analysing the properties of the conditional distribution over noisy labels for an input-dependent noise model. In addition, we evaluate the set of robust loss functions characterised by noise-insensitive, asymptotic risk minimisers. We find that strictly proper and robust loss functions both offer asymptotic robustness in accuracy, but neither guarantee that the final model is calibrated. Moreover, even with robust loss functions, overfitting is an issue in practice. With these results, we aim to explain observed robustness of common training practices, such as early stopping, to label noise. In addition, we aim to encourage the development of new noise-robust algorithms that not only preserve accuracy but that also ensure reliability.

==> background/figures/raw_figures/toy_data_2.tex <==
\addplot [draw=color0, fill=color0, mark=*, only marks, mark size=0.3pt]
table{%
x  y
-0.942162656526501 0.274101767292366
1.01032804836503 0.0858593588776655
0.629069636798295 -0.852786680645729
-0.962585238743399 0.254938251233422
0.459241896487404 -1.07926038852764
-0.878353389586699 -0.543424522095112
-1.00574075066049 0.109257569996992
0.452135008172079 -0.902483330182433
0.66123670321668 -0.817550258122285
-0.238646131889913 -0.915737105105346
-0.837921789234721 -0.431253408497801
-0.865497261096059 0.0286307173957493
0.956750158892515 -0.499475782363708
0.587808630890188 0.985407334719364
0.885692232144093 -0.439954912550586
-0.240087351823958 -0.849053086084513
-0.758135022500416 0.498228340530593
-0.639748632438833 0.727803421021586
-0.779108925011107 0.0997636966830496
-0.62111144374246 0.663722734812823
0.959112747880892 -0.127125018269938
-0.288850143792417 -0.772253317257358
1.07055805120737 0.0746811523664719
-0.285553151811158 0.927142213670946
-0.462669464949217 0.795880827258665
-0.404759489295242 1.08867009834528
0.0760578758796177 1.01424296966373
-0.838986664230144 -0.647992474792136
0.564288137860829 0.822414576872689
0.322521059629607 -0.932753986880601
0.552807934117883 -0.769052196217665
-0.702347358987449 -0.768426383917493
0.656370248317751 -0.670521879864395
-0.897345873791719 -0.0589087899406242
-0.592400287309769 0.877855916144229
-0.317794198903523 -1.14095356016334
0.89857392625225 -0.205296302386162
0.432670930004293 -0.838839052276647
-0.221341321740332 -1.03494578097382
0.416509629416294 0.654256286138151
0.975069417907422 -0.256367278179895
-1.09857663337628 0.228694392361313
-0.689369941131105 -0.646644101544268
0.234978516330792 -1.08604177220218
-0.991886841869786 -0.207947454721015
0.783749416384822 -0.721881575325639
0.374394945132161 1.05198714345382
-0.829616471791334 0.259903019642896
-0.839584730174974 -0.415714792801907
-0.293316301832894 -0.994495844494361
0.391878185107368 -1.04397941559228
0.537437567548709 -1.05983373116775
0.113969861915221 -0.912305560421795
1.32590454591806 -0.18281441909152
-1.04846252720899 -0.229672214624397
0.33549722252748 0.91791235577596
-0.590578362117747 -0.75831715373955
0.200842277463766 0.842310448506069
-0.657094256282963 -0.722960770017142
-0.848795987722546 0.542281256981053
0.848236591311093 0.340121386952154
-0.909365988464139 0.366135812130435
0.9074878725825 0.278918605477096
-0.101647895152384 -0.885295797846682
-0.926103620610067 0.16669803772085
-0.948296626196354 0.241561719120685
-0.836564628373251 -0.396601394671566
-0.737256265860596 -0.386093380391023
-0.0980404796974782 0.955602523621996
0.304802840424246 -0.819282935019926
1.02019807045207 0.0841140062153285
-0.325590828359576 -0.858837381438411
-0.108157353618195 1.03659041123672
-0.737398567042518 -0.838394268952892
-1.11423555081692 0.0393180451007706
-0.653008403177883 -0.908361612945332
-0.204957148012506 1.04453144427193
0.248333451529618 -0.804676232479934
-0.726053610399552 -0.552697204429645
0.548060431129144 -0.796843878700302
-0.949783969728249 0.645408606735096
-0.892615012725641 -0.12718585001961
-0.218170151357819 -0.942360637744711
0.413215619963067 -0.939017182545521
-0.0287420354188223 -0.831053172193317
-0.482432457775941 0.911837082085308
-1.15716103965318 0.0662520827495082
1.01519487547675 0.0879804963722468
0.464596516198935 0.756888585277477
-0.730268588761875 -0.595346945427818
0.737076509046415 0.794465567477769
-0.858711247149687 0.801524755783988
-0.779731307761601 -0.671449798816979
0.377900320875532 0.902371005155373
1.04308585453617 -0.143245392646334
-0.286242261555212 1.03965941205049
0.350207970767489 0.851342239543471
-0.306157411255627 -0.991175115894735
0.944475878807707 0.417795885223112
-0.256749583163156 -0.918059110272959
-0.571917328728672 -0.884491329447576
0.926213838505597 -0.139394108239204
0.970331942348257 -0.088267843711473
1.02631154509055 -0.0574745424227341
-0.345337109876589 0.796093352581267
-0.980817614027012 -0.140014795837656
0.156902432533322 0.878360733662936
0.861271982527608 0.575309072984635
0.000125996286252539 1.07837481731136
0.966842800761708 0.230661400555806
0.901563420388999 0.450869283781346
0.688420276120515 -0.52642861507429
-0.995652147369598 -0.268764979102355
0.628879169025923 -0.966181026034548
-0.833660570547925 0.324665282804261
-0.688782298113215 -0.802656768084899
0.668485751917936 0.839593505118995
-0.572787398963772 -0.466055324014709
0.264665289808525 -1.07010021479105
-0.979057547056223 -0.422980604968848
-0.763839756988779 -0.764491176369148
0.616458614486393 -0.981560197490571
0.544455112844303 -0.497011980315001
-0.123839653272585 1.09655252504397
0.864839088721933 -0.753025964955266
-0.422396888150641 0.857692259801657
-0.911072468608836 0.65749839357654
-0.142789490213872 0.871970672349891
0.265873263435021 -0.764953226706274
0.945595833335841 0.117680283320595
1.12095889151798 -0.277131045257717
-0.752896918239131 0.537024758484058
-1.05094823279714 -0.23915954274608
0.68279982059155 0.52503658117115
0.285462254605684 -1.1252554606062
0.371705576390842 0.979564363302467
0.669335804387258 0.762496990702516
1.01808133710277 0.202270721743584
-0.828359963611527 -0.223070853443822
0.869354964785255 -0.123559500800937
0.669535003918185 0.896077428367117
0.990114204041062 -0.474830301146038
-0.868883219026578 0.504901923187188
-0.969399942076349 0.063215501625354
0.54203090845361 -0.907493263169536
-0.914644352071408 -0.388420251301896
-0.332397679967967 1.02538827476017
0.194430780632817 -0.926406542455467
-0.75600978775583 0.669199721178253
1.13233304373971 0.184899934117355
0.794218807022704 0.412178649904334
-1.00255492611058 0.211258109667441
0.876241055815352 -0.360582318903037
0.937175723625061 -0.192943898772542
-0.0750055729115486 -0.907641005566442
0.633305080866548 -0.603810433120021
0.0989420934123382 -1.13608946258083
-0.502056832966308 -0.731075512611582
0.120750762450995 -0.986580099456386
0.289948569407856 -0.77376984838252
1.03540646679679 0.217008591766342
0.88184016839974 -0.311619779142451
1.08816679635349 -0.47936791182297
0.534942708347854 0.837150683879826
-0.142253779462648 1.04239032658887
-0.369035458815247 0.957011174863
0.959167365179029 0.230930771775072
0.590369753930598 -0.753302353844405
-0.454561174128468 -0.793463541083217
0.0546751616599945 -0.868781676570261
1.04690891535786 0.741755048212362
0.126656741181127 0.904149730372301
-1.08622690958992 -0.179994937077504
0.319226054580198 0.856770391859894
-0.563883422184768 -0.801880230883756
0.405864668290412 0.725607356849285
0.623596808631767 -0.731269348174382
0.800865996153839 -0.538054742922514
0.132102708837921 0.88230057499755
-0.256912493162814 -0.907256772585147
-0.853757437911097 -0.334497759687128
1.01926783275634 0.358669886477384
0.546976534222851 -0.793146737767892
0.00367595814368952 1.05814101378708
1.03425343190269 0.232735463038123
-0.223315556401185 0.959842507105336
0.305284005538749 -0.903429116332094
0.495174528869138 -0.72509781235551
0.697589717060091 0.654672537991059
0.221441227605729 -0.94326760814895
-0.0722673650421807 1.14856861637063
-0.763906245464052 -0.529822978759813
0.171358229249056 -1.0001662396689
-0.666702398606705 0.85304343431137
-0.821727712740723 -0.573078270034668
0.262470065276337 0.830505246224306
-0.699902558345317 -0.503981407257252
-0.56759552005156 -0.895841213124557
-0.821130158362507 0.576309427345509
-0.390198408244233 0.992881288242141
0.375779188259343 -0.993384652106964
-0.893905032230712 0.341315892150323
-0.00202891638641724 1.12333576339732
0.757473353854477 -0.507501746021891
0.503725867005059 -0.969669655490936
0.784029576989999 -0.462635799645719
1.06469444520275 -0.00479163038103913
0.950725586518318 0.493642705632546
0.1788496879217 0.971733536618481
-0.0305146112183115 1.05520087004056
0.130713710392004 0.851195503203428
-1.02059657615256 0.371004001561918
-0.821101413319643 0.25374410461738
0.778331136501906 -0.605152550677494
0.468888153754643 -1.16648829345971
-0.326272166581089 0.959408601365778
-0.408029417594748 0.903895985662936
-0.936237904320063 -0.292661003857065
-0.818435348185783 0.49537546461611
0.829658054598216 0.953533411970301
-0.612251165719383 0.731369658340788
0.60354322336752 -0.646037858976018
0.567835344906848 0.734419848225615
0.746540867521162 -0.447353154765218
0.696721068805509 -0.704633535469935
-1.00202961137308 0.00645708443784218
-0.696556437799234 0.928428907755684
0.631901466741474 0.569876543717268
-0.494394430173465 -0.851873260271787
0.56834947539439 -0.899666085157185
0.823318851302858 -0.64833747317978
-0.958571522922935 -0.198181034348753
-0.942652563621032 0.29516459090604
-0.355139197389699 -0.714973352711685
-0.106663742149397 -0.847647094517512
-0.616092979975813 0.696615515392502
0.687462886235609 0.524816850864911
-0.8029984397002 0.825967031886211
-0.84163536100257 -0.692904158872179
-0.876595863851604 -0.497685862378645
-0.465007722764661 -0.948918384944564
0.700676255150218 -0.682129246990463
0.0146429180208279 1.04743542786063
-0.91250210542249 -0.5146272215039
-0.951219252458998 0.496204641808143
-0.873457739050526 -0.54480932193322
0.127141379203352 0.694653450831573
0.973911409041166 -0.191402607159504
-0.859121640842435 0.515296758039977
-0.936539198677953 0.0204677370428533
0.61832700742467 0.88195343978224
0.900018339596911 -0.148208449964017
-0.264697167245351 -0.857462466472606
-0.227631891455912 1.03519464408207
-0.868083611998377 0.50417198697553
0.523432952977098 1.05284311103987
-0.710508321472317 0.690290351877385
0.191364373844982 -0.898954645285085
-0.737871477668773 0.113003249946894
-0.26525463559426 -1.09663906808153
-0.602417541698028 -0.640150941023232
0.822350732579447 0.357310127499703
0.816583352525739 -0.632817671250979
0.109626096938395 0.936640487477264
-1.00003991624606 -0.0117730002037091
-0.856903562394684 -0.354679866071482
0.67118278544738 -0.571195518551866
0.173560799476368 -0.994097424421379
-1.01195119149869 0.150828082289247
-0.534648356045899 0.663234316195431
0.946584154889864 0.338492755490412
0.149965625551509 -0.936070537345038
0.240624297613027 -0.942726631010963
-0.833242878006247 -0.261575242893643
0.434096116372801 -0.98664794720698
-0.721877138316209 0.505258731970489
-0.000849434320911169 1.02412111191429
0.0721079660970067 -0.914169917975321
-0.110481294988458 -0.964386943508689
0.895846827470593 -0.5890602285037
1.01994941872558 -0.484549581816229
1.09678293023166 0.164687753667146
-0.48158506028294 0.924512849301247
0.750828395642845 0.601791815366788
-0.971355886793015 -0.0605482034505227
-0.636892446532769 0.787678560959656
-0.690561140187225 0.925005121086905
-0.429661716345655 -0.977179628023817
-0.361396918658418 1.03101219778875
-0.882804596931789 -0.493432705276515
-0.987508489955458 0.680828828370542
1.01975040676275 -0.26559836169463
-0.780134020450717 0.693231837529107
-0.288674977563727 -1.00883241235736
0.773872005756771 0.0710118177286237
0.846323080047488 -0.319852875686853
-0.356665978651509 0.982797357478531
0.930459683364741 0.526132739733239
0.774713631579031 -0.718228587014652
-0.139052638953234 0.939015833947378
-0.0533586107478457 0.976067988664948
-1.085385427285 0.316564763349612
-0.131294497935728 -1.06150560751994
0.284911461712096 -0.928470872990456
0.676101041171674 -0.645689055241967
-0.279193885112486 -1.01141758369908
0.552970092912597 -0.903463300072962
1.0874867372566 0.334406665475945
0.393003070590118 0.937447405178258
-1.09459834859677 0.363792564757672
0.0667581689693657 1.10170193792457
-0.241341483838535 -0.942986800881984
-0.764938361645081 -0.492873478385092
-0.711605251403638 0.443434905913189
-0.580560720472037 0.344902927647597
-0.164023317880551 -1.03446354493607
0.0633756685361724 -0.879581303100741
-0.771165845922744 -0.70592343386018
-0.998265348603749 0.381378721707827
-0.409009799899027 -1.0331947916207
0.664161031380713 0.942266128864913
0.577892934532523 -0.733676953867419
-0.638762666686727 -0.883773380649572
0.398902644533982 0.888741287505381
-0.762128770908893 0.48063598633665
-0.682356266896996 -0.588392329353528
-1.09705880151776 0.304275075043259
0.948924187081281 -0.00973239963664288
-0.42630065680043 0.791403692147437
-0.464312495961624 0.889838376604378
-0.64033702849025 0.563267022633993
-0.423444792688782 0.788533035897198
0.805266221004734 0.826757460939287
-0.600460559423151 0.9550907540862
0.0856957920762324 1.06203737886849
-0.882473798375625 -0.318009724296119
-0.684531538653696 0.626342158293964
-0.761116017289748 -0.790778979047476
0.276402080630693 -0.776928465694536
0.367965448774529 -1.04582946340517
0.287887036247533 0.847925455504413
-0.137939012518772 -1.11259319142873
-0.813550616974412 -0.404266477217176
0.854614276675308 0.554226652350032
0.676265068422391 0.789872736602086
0.81413761587635 0.434930197589039
-0.389821620511646 0.878027789073095
-0.758150817963649 0.896987482645956
0.833101689892699 -0.771230388053035
0.671085944318986 0.609101448573698
0.78418915245602 -0.299834216382131
0.8606261758484 -0.669319445469525
-0.610236501403956 0.776102070405509
0.24362965962005 -0.98907948489133
0.332616545862149 -0.809380586249053
0.132303716932335 -1.01937393201885
0.709689626843716 0.535113371971901
0.698205087501601 -0.540561715990628
0.0133314564841247 1.06454267585376
1.26284697573805 -0.125635848654099
-0.336459127591348 0.975526298471856
-0.798100812949331 -0.421912682421294
-0.643374658226782 -0.459906960081119
0.0672855941470118 1.09426700774761
0.216566146027612 -0.986011069399091
0.614961476978424 -0.787488401558342
-0.471095709342495 -0.835526329544529
0.750346983965508 0.573050040603262
-1.01615680583055 0.261860748706626
-0.281779771311959 1.00888695553806
-0.0420703062221478 0.955099422656331
-0.888164475716764 -0.520582320666722
-0.729972912757026 -0.791974140902253
0.812828887951242 0.764742220714668
0.913668535267012 0.224416901622899
-0.715994527807108 -0.629826045020921
-0.644249777436278 -0.709100393290221
0.771958215731352 -0.685432156411496
-0.726954911899088 -0.747537425677574
-0.188590646726508 -0.951298647429721
0.794429844279929 0.672787640793456
-0.992783545784609 -0.544569087598829
-0.478139508722462 0.674864464074285
0.954495609179151 0.524530540161975
-0.966757351195104 -0.000191464368798328
0.301104820713742 -0.918526969794019
0.496852273390266 0.966712101001497
0.613378509753123 0.703899055314474
-0.660656411886208 0.72420664359395
-0.350113756105742 0.806769687137009
0.534024945285939 -0.568530784762087
-0.555577712469502 -0.711866316906939
0.0703315415507167 -0.740000871178624
-0.961563543294848 -0.371181868505964
-0.845343601821244 0.279872154641522
0.488371565759521 0.86898181832649
-0.673402482935826 -0.742004730018102
-0.974130466695204 0.293988680941532
1.14459669970693 0.0774721201061043
0.0465456499508927 -0.969236331524736
-0.588925359493317 -0.702159713598525
0.763505886732379 -0.593462056713521
-0.348692345702783 0.810699407493443
-0.125526983569969 -0.88108556009187
1.1163932398891 -0.0454160119465158
-1.11232150320616 -0.103000814825688
-0.252830823219296 1.11040760001515
-0.263173167364726 0.934817712089522
0.946174152631617 -0.532286819190405
1.03416359772894 0.324089274231786
0.688921740925811 0.776049635658796
0.425041371608273 -0.850495743020621
0.933602003292788 0.343310987739221
-0.272775217376063 -0.994572538003137
-0.700677835387205 0.695195349076998
0.183232600982559 -0.949081210426862
0.169915530750286 -1.14370643972105
0.449081213832642 0.991900295223962
-0.775756359846692 0.492857670244459
1.03847185392923 0.450329968341909
0.850643464281706 0.414049216390099
0.836571787705891 -0.179847294375143
1.12749716788469 0.104022971893639
-0.998229924773284 -0.765111118068908
0.0564907048996625 0.969756849589059
-0.3421928323864 -0.882961699823143
-1.0941963811822 -0.389359627391248
-0.366801687916676 -0.860581022776636
0.991545216481806 -0.432649367442795
-0.20033341599021 0.902690806783372
0.839096882324367 0.502734205650378
1.10296672375713 -0.105468952612251
-1.02410463190682 0.612649000305522
-0.699124003085016 0.841235672228192
-0.952201831421017 -0.0844478440845025
0.918219917841933 0.0231612555627435
-0.929020250729536 0.434415398699271
-0.075006098386596 -0.970309692714218
-0.988472849846874 -0.522177134372008
-0.988321717561769 -0.369619424641803
-0.953056362614904 -0.0313705879702243
0.718308659572094 -0.623934259797921
-0.393912588106928 -0.951801358640898
0.448358632487639 -0.891289654588119
-0.521481366695345 1.11419536015348
1.16365857098834 0.189143358804312
0.575797761417267 -0.950396340852362
0.437221396351716 -0.956106285746507
0.230158446449155 1.04490753478964
0.517845477931164 0.720199673396982
-0.789972724633825 0.656028700147559
0.249879307811363 -0.999120471836439
-0.582196166757605 0.822896648517203
0.673116482197834 0.391490369886656
-0.671296392295606 0.898108775787178
0.438045404076459 0.817044413854345
0.726452651079702 0.534903418733489
0.673710969788664 0.69148946354047
1.07676093221457 0.114319184504495
-0.601185868391459 0.994921239839576
-0.644106778350268 0.700777137874332
-0.837309573089034 0.157552378191438
0.799873179078806 -0.65425729658851
-0.0939448855139499 -1.01842733014344
-0.760285407220068 0.920099262035573
1.02740832188592 0.325086176275571
0.989015276192886 -0.374872206026202
0.636356682645788 0.90209828435793
0.896812107978313 0.50616295338016
-0.863988998506127 -0.321282299220065
0.517233885998701 1.03918502422795
-0.482567333972217 0.803793540922326
-0.66957051301189 -0.588458314705747
1.22822490293875 -0.169971869212737
-0.800275587891782 0.563202630308024
-1.12631591005403 -0.331690870770819
-0.889852643774933 -0.44670738508474
0.358044824775128 -0.805035544651649
-0.957242654730132 0.154017610809298
0.322979893704533 -0.776140620644096
-0.801287441122652 0.496509822276218
-0.987191432224156 0.267037496741464
-0.377921000838657 -1.03990740221062
-0.673695352550885 0.774698204334675
0.715465904923112 -0.620817809954345
-0.8846970366821 0.545407281077051
0.564393710238468 0.706022454824304
-0.981958950442359 -0.406619996282098
-0.695948228622535 -0.902545203364856
0.563061850002636 -0.975818843527073
0.659600477225695 -0.988281568351414
-0.0181999106628941 0.78097322067319
0.12188583599529 0.906285851701869
-0.800673807408013 -0.660191941558706
0.191635926628541 1.00898536929505
-0.445888664464746 -0.530018440456473
0.871962991626377 -0.324632731776643
0.665018527799229 0.746249305754721
0.62144979885853 0.884834502770016
-0.122456807505692 1.09945002346356
-0.603133278277297 -0.57637150808913
-0.609142240362431 -0.659407386028574
0.722451935392336 -0.597570341578678
-0.744059868093193 -0.67551624652902
-1.23413289042931 0.507225873723103
-0.874504588639056 -0.216112004849485
0.462191840430511 0.934315037963795
-0.178890689373388 0.872485873057737
-1.00899387596368 0.267348173536615
0.497245459267303 -0.666180460445101
-0.243389320252198 -0.919893174950019
0.0929039176199304 0.999451071886491
0.860822453317698 -0.657911558623716
0.901642566923236 0.303515443131745
0.840533769274677 -0.555327602970428
-0.223975252677672 -1.15043320434138
-0.142359597668953 -1.04027431772269
-0.774127355383472 0.445628825259353
0.729405331066669 0.827649784872598
-0.871199956255132 -0.592186166547032
-0.578524156165901 -0.834894313443231
-0.917162093981874 -0.532283225634315
0.646864981716705 0.750543689571783
-0.730364367151074 -0.383698411410678
-1.05003200157516 -0.149431270230626
-0.386266250728825 -0.988104989920118
-0.896100829188443 0.187210840674651
0.933958054720935 -0.439673508888917
1.06151966282535 0.0433306345824878
0.847579626722133 -0.229645330957348
-0.812569057151016 -0.844676847712679
-0.594934444134366 0.792001051143987
-0.372840730357213 -0.686572137182054
1.08989944656918 0.122386921677085
-0.445847752662239 0.721336137060721
-0.844856954341108 0.662700103108462
-0.385824483046646 -1.0148011863378
0.852820625208014 -0.699115034535949
-0.584566938318539 -0.688480496358719
0.58447350176486 -0.847064009050322
0.0948073664211559 -0.841466537923532
-0.523523050744995 0.854637504192362
-0.0191952634649783 -1.01263296110366
0.90896500998636 0.570007910472832
-0.72489354092398 -0.318990691904778
0.152941272321979 0.882387878579121
1.10497390403681 0.188719569991269
-0.840950260037329 -0.781782290576107
0.583263098342748 -0.876120659450937
0.872707801957551 0.639026344097093
0.907696352732169 -0.240976855106699
0.108583341468318 0.917435928761768
-0.277136868756048 0.936432701931825
0.211985657864055 0.88898087405219
0.10896789697733 1.18436598871453
-0.891433598972159 0.294394107161496
-1.05575451388638 0.0971681549569098
0.893310878643326 -0.488118306344218
0.730916042534131 -0.50021532880093
-1.0347322291136 -0.556516551730499
0.792851888974938 0.4870045283722
-0.25976622669194 -1.15834795344154
-0.979228854284256 0.0345735410140258
-0.798907666387803 -0.452610338500833
-0.914540530431358 0.634498342060985
-1.10655995269173 0.664740861575716
-0.422309795441952 -0.800565642917238
-0.40910390675805 -1.00518503379293
0.949815635205064 -0.648328073598462
0.327283801735199 0.978459681875635
0.814391801596316 0.0404806498163144
-0.0396926349597482 -0.834059810011403
0.666566127933954 0.812243042994002
0.779583946495667 -0.624042816843952
-0.90580468971684 -0.200339376478959
-0.214049399580344 0.987713117863418
-0.513943186744746 0.979375543998686
1.04072833479807 0.226894504048006
-0.200067489255817 0.99630652788956
0.56671030864938 -0.8208080906421
-0.746797097010264 -0.684331544644657
1.16562978733121 -0.163602390863945
-0.617148915687457 0.46023655094768
-0.443339673445732 -0.928269294987942
0.891924424903553 0.373041946551602
0.89775427143136 -0.307132119929175
0.77091727010595 0.643380852452075
-0.263269489870723 0.788736382419051
0.937210828890304 0.341459242387011
0.846389851762098 -0.284606004582023
0.110606064556147 1.06373546512484
0.86436515152196 0.114303148103428
-1.01340433491045 0.421152365765935
1.08650743364314 0.571169746876518
-0.578832834992791 -0.732831728226425
0.769663644690487 -0.620320942775693
-0.0466158436441215 0.95121630357476
-0.845884604596605 -0.348160003671072
0.981043404154848 -0.160481336727948
-0.975297850264348 -0.365898194337819
-0.799618029283593 -0.650034725648253
0.813561690815921 0.360701033575422
0.856868298270138 0.316856650972893
-0.902460185016765 0.393080106462205
0.480320084255027 -0.821503815644841
-0.795432173633317 -0.182748398968115
-1.00090475517949 -0.0866141958477189
-0.0182037726245897 0.959458009103195
1.01648715991373 0.271468526945863
-0.194150191144482 0.738299657569335
0.252355067995326 1.09044490405639
0.706109193587734 -0.620374512949383
-0.689911881812573 0.79678980485634
0.74129348092594 -0.893713504964287
-0.677691646370199 0.800115720636176
-1.06475859947716 -0.223475517108217
-0.88824328478253 -0.427350029675725
-0.921165534246506 0.0989889635547159
-0.0857114117932003 -1.00521935944063
0.350339158653549 -0.737733738646908
0.657451290277989 -0.646661945380583
0.0925553481313794 -0.801411299497479
-0.569794126685572 0.794400746761869
-0.399560379648204 0.847367177732178
-0.383373071610586 0.827660494440725
-1.1032585462975 0.117900183159635
-0.168972078772818 0.997591381040998
-1.13992502027362 0.117463765328762
-0.925900911024818 0.487795637567105
-0.0962771615695683 0.883917564199412
0.172460936841536 -1.0123008810781
-0.129001326374463 1.01939387175146
0.673524650518711 -0.757118714843408
-0.878860271622269 -0.386845745894407
0.832820403530666 0.555085495058554
0.382672118241858 1.05936023185866
-0.285753533532435 -0.92786481615227
-0.70028918804028 -0.875449941911568
0.917939400101837 0.458235483546226
0.20594747708135 0.910348544345813
-1.05818096428043 0.221031513581812
0.400184162710077 -0.626861596054934
-0.0352654313713234 -0.956294228526103
-0.725202867523603 0.798830433829398
-0.192743189735638 -0.902896285917701
-0.276922658596515 -0.966025801111007
-0.700640112610091 -0.524472705800777
-0.742732428499279 0.608466941535157
0.0647327443583237 1.07318180403967
-0.981941457408166 0.0275879255696366
0.23879467289425 0.882277386488859
-0.548979514980017 0.742774358644245
0.929649504663533 -0.509812844872964
-0.431450457480098 -0.969861245855389
-0.756645062416306 0.634055931869893
-0.103877792422083 -1.06332525216509
0.107723030939798 0.858850278331197
-0.133063449170231 1.05004308134451
-1.11851950701031 -0.179867229663255
0.95624777593076 -0.0810246809344927
-0.418977408201222 1.03828977705796
-0.150128938994023 0.878578306604606
-0.468557092172315 0.939782850297287
-0.458771674766063 0.850490757724718
-1.02769275655255 -0.0582188174511327
-1.01646565387648 0.17483198684902
0.402958577683377 0.937592102401589
0.338579538379892 -0.822345364542672
0.229524780899715 -0.997282940816697
-0.0257930513673712 1.06488306607248
0.801909149380845 0.666316221027658
-0.976603706138952 -0.365614799740513
0.366492252999776 -0.72990089303969
0.0726190724548017 0.921404147277541
0.242236627937418 -0.863426491871049
0.892157431896095 -0.67732475463266
0.684957493367945 1.01312460000116
0.323490193326136 1.0540882346
-0.633220577326754 -0.751567462313715
-1.00688008906036 -0.130442287045898
0.769759774944869 1.05524824182575
0.0874546707416418 0.984322685023646
0.789393810237097 0.421446863220701
0.904900717914599 -0.598895524994876
-0.774081296894367 -0.671853647228939
0.562283122691453 0.839444755940074
0.863494235555787 0.660979455877427
0.634772563170029 0.955353737047731
-0.660726019567145 0.436529902533796
0.941047313433946 -0.324980053684589
0.652411605364604 0.479185133171507
0.304547318336529 0.885951488122589
0.506387829846726 -0.919923146626528
0.706332127906549 0.892948384054686
0.936845712882301 0.016736283727536
-0.790154023039803 -0.641543160855217
0.750086280497257 -0.760383782368043
0.929155912413524 -0.0373693219210757
0.285017673089449 -1.05619977172644
-1.04538402220168 0.359307547886877
1.04466757336892 -0.313160742044247
0.850246934452181 -0.191839092696752
-0.0488566661670131 0.849466582021147
1.122375960786 0.279292919416923
-0.845978966213161 -0.367416998263197
-1.06968433203271 -0.216499924015773
1.06971605275057 -0.156016029294499
0.0264099090730315 -0.954724040594465
1.19680882724641 0.0520541316019766
-0.470294712993647 -0.893485094616404
0.643796008036749 -0.604936432655787
-0.649870439009119 -0.726126842973958
-0.709837320005568 -0.501844028457186
0.935159841818007 -0.0041026844390589
0.695208738664932 0.444660808486923
0.810852770639652 0.717682189409863
0.0866957914703634 0.967037795275988
0.418898600262324 0.864422743000894
-1.00534964632513 0.185583741220098
-0.684590692948676 0.777588344217244
-0.854969801535825 0.276815313020615
0.477895762114477 -0.743770001539502
-0.432164017538425 1.07864299280964
-0.909613426198707 -0.585126095638421
-0.886084639508089 -0.434338541263033
-0.0956066849592886 -0.865559447944007
-0.841275928618888 0.164687697901267
-0.0423506510152146 -1.05497692136424
-0.0989297891108046 -1.05767572380403
-0.922294876568576 -0.324263153624244
-0.614710381883472 0.670507523918786
-1.03621704990569 0.438064091476894
-0.835931924964644 -0.13061783388039
0.359355509250877 0.976624548996698
0.307502796866542 -0.86668378091893
0.368936780413148 0.864662358657135
-1.10749018529104 -0.343038831935407
0.802924707217978 0.0816198124306005
1.22641282466314 -0.105959836004639
-0.198968598644096 -0.936464332735312
1.01053847797754 0.206144699046911
0.819400268302073 -0.159093079790478
-0.188005050253629 -0.813806142016352
-1.00285948350929 -0.187413861595091
1.09250751415195 -0.0915069059271072
0.844899288909439 0.306619343794954
0.30912108517774 0.853813513272303
0.81890564258539 0.572562560023181
0.716104413800307 -0.535496174552282
0.921363273656489 -0.0947214911533193
-0.939148626627907 -0.00167683108140229
-0.107195828632914 -1.19882413909268
0.396691422714833 -1.0150679985207
-0.913003941986877 -0.520917768615624
-0.409722737771998 -0.977161185725926
0.096464988788456 0.925789420454818
1.14465954487197 0.355250729794293
-1.05348311997418 0.402841087668149
-0.921325979667724 -0.620281347917815
-1.13458785569129 0.119946858880216
0.633970984405823 -0.817995063043829
0.775431140870929 -0.659894256235613
-0.84710852247813 -0.317575626545909
-0.10688540395823 -0.866170899902095
-0.515964257322614 0.943504170387282
0.596951162308586 -0.7590999928886
0.676952491349908 -0.676147427900073
-0.798158091749463 -0.639540592862528
-0.837919877824777 0.127576812940763
0.945631838964408 -0.301807960045797
0.972198612090805 0.0181657656838048
0.137595985251759 0.971601434091767
-0.226487844778058 -1.21205946282892
-0.819344695918167 0.50555100164777
-0.126929749556003 0.933971085825493
0.20810027670064 0.960876704280198
0.800540115658858 0.534359323074879
0.174805694837235 0.989516865340845
0.651261440671759 0.88036475497776
-0.82361438137377 -0.672611069728658
-0.931196136836247 -0.673803231003525
-0.649022722516855 -0.788709231844608
0.931159191765658 0.46858898172115
0.57393395463692 0.764974465699357
0.780100095743497 -0.610082422395663
1.09752652372763 0.181520163874284
1.03216713984765 0.186020227336662
-0.846564828688074 0.594653538544934
0.662311476244863 0.669809169392507
0.469984320854998 -0.722425199117436
1.06322275509561 0.138559385439379
-0.0183844894273229 1.06932171762877
-0.364820526339948 0.851821561376929
0.677388658827796 -0.562421641747309
-1.14186482406932 0.165999357561884
-0.881626565867427 0.0123405609563397
-0.505441581211288 1.04575336232653
-0.89617319267384 -0.456046815225282
0.578392729473349 -0.959158786829776
-0.741853911144837 -0.737533301771192
-0.350073903951022 -0.923177645623475
-0.368424047133037 -0.779670462454965
0.890792195703015 -0.513506305558232
0.861855801189293 -0.0716788785289161
-0.457600440438885 -0.915963328842909
-0.937047427348226 0.235199704686041
-0.452033870563638 1.00239013410992
-0.844859959547937 0.07100687139581
0.805161601663452 0.546039056817225
-0.208205256633545 -0.889180104064589
0.762068415936737 0.461578528844144
0.933765254932013 -0.305014786887119
-0.289421080021036 1.00816298030908
0.818336542816201 -0.290924744948685
0.982664741258719 -0.261731595340918
0.76523075483406 -0.714984420174166
0.331693856817011 1.00728117886073
-0.534416848446521 -0.92066208801848
-0.589874055434762 0.864715679523049
-0.69625667018665 0.739103068128865
-1.03546733483172 0.250911389124564
-0.518385118785947 -0.826085239440095
0.912652799963277 0.389653840247408
0.257039348004878 0.856280689286791
-0.824590918501 0.587291191669545
1.0051444001399 0.0852929717096713
-0.346689978688544 1.00937197271792
-0.977110572274566 0.465684856159585
-0.840177931298103 -0.549369590485251
-0.175130437804322 -0.977329725005644
1.20630735953041 -0.323317764068056
-0.74815363163278 0.779087763185254
-0.217285086665187 0.914167883502471
-1.04743973171727 -0.128076927907774
0.478139283016301 1.11779712124438
0.28955780455428 -0.731724567217217
0.701612397193596 -0.904478676722774
1.0711227898087 -0.140514105649799
-0.646440874512557 -0.939700123871277
-0.850744250265784 -0.494052420078053
-0.61133346294189 0.755526958806182
-0.0740805686809348 1.03352473844257
-0.543575111159662 -0.754206880283213
0.690731235197672 -0.964926329154862
0.300972430361739 -0.967704427885525
-0.712118060262591 0.624043546077013
0.410863779547669 0.936894273115662
0.594002704205663 0.767725497735999
-0.244465107278775 0.96336065055251
-0.403503699220257 -0.800510689443434
-0.971906829489077 0.00255524783313968
0.295888748013196 -0.924273640234992
0.542615079626045 -0.917154411781221
-0.353008072396868 -0.922959022965897
-0.0104850303269498 -0.827969096800978
0.0439831526571717 -0.967804435537024
-0.185384507475298 -0.98526106395663
-0.410281333457322 -0.799368065157385
-0.769936724800102 -0.628059919707473
0.0209651493721859 -1.01682552314919
0.418569695213356 0.945666492720519
-0.871839645953249 0.410312804724354
-0.98969804934444 0.437128359289659
-1.10412890335946 0.164666088608822
0.261035748092121 0.811995038923993
-0.13020300893752 -1.03285514989363
-1.08412039105565 -0.21320714136164
-0.890111233545563 0.623995669025819
0.967842751595896 0.300521789433226
-0.0176754781965689 -0.98094584329479
0.432045376137433 0.851957779247652
-0.232151336489876 0.874307209876028
1.08989571507787 -0.228778502455662
0.708222384338691 -0.791080779416611
-0.853507549242179 -0.452268293536311
-0.174471214248642 0.936051622929159
-0.678554717030892 0.650992054703316
-0.635979445018167 0.698658481517905
0.329275416843938 -0.9376851240068
0.285165196355202 -1.08777949356467
0.322141611329124 -1.1124814679953
0.992042919672289 0.407450799683369
-1.09897146117258 0.157574394391766
0.556529548728507 1.08272748130502
0.802316502063568 -0.511908063059104
0.403875801864775 -0.861917168384355
-0.987372176724565 -0.289247513231198
-1.02157643121133 -0.0931475923626442
-1.03724606152758 0.174183748447037
-0.149670764143274 -0.923238380130216
-1.00986447560728 -0.0135192964295428
-0.227061268959461 -1.00559652888448
0.524164600806948 0.77096065376463
-0.162672525219661 -0.932894851010263
-0.908278743502407 -0.525276367821021
-0.942128954327372 -0.0803509386881728
-0.617302722647807 -0.659871838126428
0.133467367021569 -1.09241423597693
-0.600585538796167 -0.574858419668243
0.202466620665978 -0.994620280571597
-0.949792816430918 -0.320735249488371
-0.942198387878517 0.6218286799569
1.08527948268626 0.16866296691615
-0.657414312707039 0.707480498768702
1.16488330069167 0.296070555257291
-0.888320124291831 -0.522511516124503
-0.950086904181073 0.125654541697726
-0.0760366197048521 1.24621216650057
0.893858843816706 0.231494101152073
0.727575524652878 -0.662168009406045
-0.755582378056795 -0.748738224220384
-0.828460681639497 -0.555103422041582
-0.0461677185727001 1.15250292353789
0.865105408080302 0.548329162342464
-0.865953009692214 0.553205700904302
-1.16367337545677 -0.226629913108692
-0.675237133549203 0.620310958031623
0.825108072099047 -0.526083572377095
0.491501210232693 0.761992133677206
-0.0819373660066094 -1.00766902674575
0.820008689994918 0.599117828618169
-1.0237478609423 0.449035461594892
0.512518341955585 0.735479502059666
-0.650458907601281 -0.950631860726772
-0.880018641568364 0.538692979815593
0.805874432495208 -0.298832870043009
-0.808464866736848 -0.927501795143185
0.74929936753998 0.430123980019018
1.06288648830073 -0.458657588110202
-0.0578775111981326 1.01163790344479
0.428921116385534 -0.986356911473879
1.03947781349048 -0.180388472620262
0.88542179775785 0.425714968817089
0.537530080633334 -0.833538218227941
0.316586825079914 -1.02691036342874
0.633457125841337 -0.648483280399355
0.988146797524264 0.062423042968652
-0.308846921033295 -0.998315306261831
-0.17857310059735 -1.04459725841018
-1.03970806427252 0.204059199575703
0.389241274094065 -1.00270419563106
-0.893045937917577 -0.355444255737878
0.533470708267335 -0.963035122890002
0.649306768107768 -0.754910938496588
-0.737509904267835 -0.990507202703009
0.945724817090953 -0.461417838874058
-0.707896390523226 0.508187761150481
-0.00690046386983168 0.980237677514964
-0.131100964391095 0.919212347873557
0.357371903117763 0.89389754882227
0.946027593843046 0.626633373156204
0.894876140009887 -0.426228321936372
0.123748915608265 0.937896762385877
1.0301339264042 -0.625145609814569
0.35903092889302 0.894688699974198
-0.756046599488114 0.810926957371709
0.991468345652351 -0.236321321025122
-0.302650952324212 -0.709446680847824
0.704589678176122 0.557590988957778
-0.654579072425207 0.775973139745182
1.05655466292915 -0.118621994305179
-1.01138961412701 0.326802681967041
0.812463833598359 0.339445864647141
-0.39927254334283 -0.967195098207193
-0.852334841424256 0.724666854770063
0.956973768322176 0.129257227525634
0.822220240623064 -0.108496595891803
-0.50779558393142 0.973747067412064
-0.779191407106537 0.552289063160898
-0.194074168790306 0.886911583092511
-0.884793688089662 0.211976358973178
0.0877688425565189 1.00778164711758
0.0876827036748672 1.10097331095484
0.51600903886275 -0.796319169136201
0.540965023239412 1.01091245521146
-0.595460658437669 1.08262893874424
-0.985115970022625 -0.683706101572795
-1.00413211151815 0.0932345159921799
-0.891389066211149 0.525658576281651
-0.371064021682381 -0.896970876300153
0.464343074538117 1.01566849248456
0.690205448715124 -0.582929003764923
0.617830257728722 -0.803861481465777
0.533809990115403 -0.908229270531649
0.142851148362012 -1.00273895982974
0.237666055875931 1.17813067313441
-0.6234164085599 -0.883790954801088
0.748676785946806 0.798613304504296
-0.979904252343723 -0.462204484880885
0.128188392423465 -0.973581895929231
0.389115383693031 0.975325125757214
-0.959915188490805 -0.00817860586143796
-1.01020575224242 0.068314931299587
0.208709156542933 -0.940310586472702
0.895194600099227 -0.526585275838001
-0.718775372574356 0.731704467526361
-0.0662908880010062 -0.862609272017311
0.0969689381511978 -0.98725111209613
-0.844444321827781 -0.268975703705018
-0.801625135995328 0.518032707254582
-0.161620200508999 -1.02835102631911
-0.98907173729649 0.275299582152126
0.756693098981205 -0.487115165759501
-0.351451192938829 -0.853959503055168
0.622654143484956 -0.770656741499081
0.982054988226557 -0.451843596899608
-1.11119557511226 -0.165529018290131
0.975899971500328 -0.664823697944193
0.950328768333478 0.798457520957606
0.366149296614159 -0.876748746282688
0.511394281577542 -0.949882286464396
0.271758674616993 -1.03266904654036
0.802459620344759 0.177959402599616
-0.0769601369124126 -1.03207543929791
-1.23300324509721 0.497093186123489
1.02874687791422 0.390121176829473
0.884472900286798 -0.168746953089526
0.340469215792223 0.944438602692868
-0.200684322000586 0.906062208533571
-0.271605413322851 1.10476051117594
-0.817049519875243 0.653891352919965
0.475472316838993 1.04845593139892
0.373356666508507 -0.878903730852305
-0.505120165286089 0.711681248148893
0.32350746275868 -0.966551615406024
0.931926952324597 -0.531909478883693
-0.896375484800557 0.34680546710811
-1.10593819215339 0.0958826502785292
0.763303989706767 -0.622585030709995
-0.389033125038447 0.984631567627823
0.0230632738910341 0.854242308561997
-0.237684753779952 0.929703057854868
-0.00873480070997759 -0.892717296982551
0.0557664712216242 -0.94756545004424
-0.691194193519524 -0.885576936014461
0.342092718268212 -0.888708630608758
0.478919217367987 -0.984903432526923
-0.124963444747844 0.899141413009903
0.749438800272189 0.540486751237094
0.878944940369398 -0.157029367334655
1.05512852217942 0.1880268626715
0.313993567105171 0.860641614352202
1.01764374710454 -0.483393799994011
-0.154349980187336 -0.982988040508965
-0.144177347611205 1.00532406366729
-0.533562146151476 -0.747237809002891
0.274414078854455 -1.0235368085717
0.365356998943785 0.978965936488407
0.712544539365221 0.543605116408744
-0.979985065594057 -0.534468522821577
-0.441832393483079 -0.935156170931245
0.691539929266849 -0.801232329141074
-0.60669737331839 0.668615872132173
-0.937341727413125 0.368623183611284
-0.907548113093089 -0.331258174460468
1.14785772930825 0.336283764393451
0.353053354560075 0.942549493054624
0.541800758417764 -0.890652414426455
-0.974038818369364 0.172898030439525
0.408425882403495 -0.890285424421061
-0.317190071004244 -0.830177536688496
0.908974565257281 0.363690395162055
0.554177510913024 -0.800931283942784
0.746091102980566 0.635005007727463
0.988280130472007 0.0810435454488371
-1.11494530347558 0.152671393167811
-0.957892953437892 -0.255684985445761
0.904514911268348 0.631392678306508
-0.164173320769883 -1.03538400087359
-0.328795984150427 -0.957469368685593
-0.499872596614362 0.907342277419033
-1.11557492258397 -0.421173560606703
-0.0982799521609892 -1.02955106031333
1.02957029425648 -0.138453157161143
-0.220607624940001 1.07292681067952
0.135333948775254 0.83866070557896
-1.08190647237548 0.612748858789416
-0.809636025586078 0.517239370637704
-0.874315310129918 0.052035215247614
0.914684213342794 -0.123163479697669
0.74037054188481 0.25745343335172
-0.934453413244436 -0.0596371354532786
-0.125455685382522 1.02900827651632
-0.316694127859468 -0.940849679249479
1.14286876541745 0.415759057049757
-1.05327167395221 -0.0723840296962137
0.351073253090352 -0.990974809254132
0.393064149790644 0.777496896423048
-0.601875178280083 -0.849563071099306
0.890064185081829 -0.592021866035314
1.00672738539868 0.430107779139655
0.826067118271118 0.865566668223536
0.278283018331213 -1.11502728679247
0.932660128140344 -0.4580367366655
0.519460357090237 0.799632432975813
-1.07107168540843 -0.0818348247590802
0.953253425721328 0.490445783750402
-0.162530074946335 1.08527261703018
0.137927115973675 -0.884217973587444
0.676789421323689 0.766032129824455
0.826886384454285 -0.443557462487318
-0.0929456960109239 -1.07497257454639
0.952037561295769 0.401149021579307
1.11605736200591 -0.0756254112493581
-0.48737273036144 -0.958828653337972
-0.0118403166221014 0.916299116609766
-1.03703698939786 0.202886542139943
-0.211542827179864 0.98859948908672
1.09364170138255 -0.380249048532105
0.863792477412511 -0.264383767827147
-0.192913374653643 0.975501758918746
0.899283180479687 0.165861047457147
-0.39740437483005 0.75823034706441
1.0267361482204 0.641276394113905
0.0458345972041229 -1.13611087458448
0.688481867445706 0.841542733192231
-0.896898387078586 0.664942255415824
0.901065930468668 0.334930606598519
0.89790287074158 0.461825973524267
0.723395219513037 -0.87338717007878
0.850161264569623 -0.165858896470574
0.521824614659312 0.774997981532941
-0.407144457808491 0.952650299898238
-1.02653894679221 0.396615205865741
0.0442751491358116 -0.900687781683855
-0.530196810188809 -0.861372417183834
0.967681499268562 -0.490616800490447
0.428653580188968 -0.940000471027691
-0.939660949495398 -0.205375080761366
-0.941325707609286 -0.118512114970058
0.00731271937566253 0.99344529116911
0.355381772401625 -0.87782928529052
0.838048712706819 0.819491547716413
-0.771000371426962 0.742101388806995
-0.871247357517642 0.525769821687622
-0.839317804863643 -0.787765838911149
-0.148061883197848 0.817474707072934
-0.635953978229611 -0.885628426491338
-0.790998227247928 0.101827121922076
-0.671767392593568 0.782496988720635
0.623893515350422 0.955328870549098
-0.245550017749302 -0.992615852744501
-0.462606900532844 0.925122517489828
-0.472675670230992 0.785431912350511
-0.831556533173683 -0.284219464575102
0.949819734000224 -0.426418825875178
-0.946357229828224 0.352293148679144
0.100279307235511 -0.945461760033801
0.940282389998833 -0.291011858783714
0.192298833277706 1.00501898621332
-0.0597537408189577 0.843374169086428
-0.236168715159592 0.93836679101371
-0.885921035158206 -0.172483037890823
-0.149493363069333 1.046007346133
-0.487866202466232 0.930033612568593
0.877110444276938 0.271618827330869
0.913576816713278 0.102707095636731
0.774091473050918 0.676896800044535
0.365070302111368 0.972211428591265
-0.709858025696737 -0.568046748474687
-0.798036825862852 0.164141077521833
0.519070570511985 -0.87895155882362
0.221543907940887 0.898298865649697
0.304775617961709 0.905878268902761
-0.118004398519021 0.956584133597982
-0.865576276565048 0.536208044397534
0.865648460918954 -0.284220175086249
0.935273571876655 -0.465183491678817
0.423841302378953 1.01003625355295
-0.219971635187078 1.0882791646634
0.912556583316398 0.321425559271458
-0.20598293603368 -0.892482177439886
-0.104587359493937 -1.05218568400289
0.911710713680771 -0.230818369652966
0.86260753063027 -0.405497647128704
-0.603189902979407 -0.83533517130377
0.109097642527995 0.951170049444055
0.198746354739716 0.776953934009966
0.81131586619022 -0.451443919699028
0.968721517030831 0.218953035549922
-0.435587158097951 -0.83680316441389
0.918682447413985 -0.181594493495909
-1.16670801314234 -0.128052250286571
0.636048853423873 0.695908855579069
0.798211326407897 -0.515376742050403
0.327131522926114 0.847377919938999
-0.737921064072658 -0.705059316413799
0.982178722965924 -0.401141076787867
-1.17632240550982 -0.0626275173429802
0.0213250204797983 1.0096647121038
-0.43078505088491 0.816312998149445
-1.03684341364223 0.575648374464596
-0.981660293560756 -0.155744311722488
-0.150803722003831 0.989495385135454
0.886609955451679 -0.68229835706589
-0.595524371135614 0.789536446308633
-0.714283823580522 -0.612047179689113
-0.921295773845139 -0.121147225683279
-1.00863882624654 0.0944522154686843
-0.433393628043963 0.922458583092278
0.37452516455819 1.00494347059904
1.10106434864134 -0.132370040939091
-0.894547955747816 -0.418374092359014
-0.637448890052576 -0.912840711468506
0.0716367893755528 -1.14753777241651
0.924650816878867 -0.298762828470837
1.07254212892778 -0.0462102628543492
0.863779165729417 -0.132450602642859
1.01383006571243 -0.18478693194075
0.216448169466266 1.06697884217513
-0.77645463760024 0.0618870935940585
0.473136614406882 -0.955374174931238
0.255238663426472 -1.0869762254934
0.846522331024604 0.333208627931405
0.709728538628142 -0.838510154413089
-0.363303159256916 0.763846448075638
-0.400607915613379 -1.01999378122323
0.128560224913315 1.00085668426478
-0.574478822160155 -0.809998193591309
-0.638026566916666 -0.715539061742564
-0.899407376635901 -0.465465286942569
-0.819689185890947 0.238046486181188
-0.931885496206044 0.551120203406583
0.722635365947796 0.461692010488952
-0.65625783384806 -0.712068862112409
-0.124748476572747 -1.1433725153408
1.19519959612241 0.21368290170247
0.343162084456522 1.08532259833574
1.02096761833833 0.490709716856169
-1.02797467372843 -0.125567171286284
-0.230683763562052 0.945388725563146
1.083316466512 0.0836101404009194
0.934411094927322 0.425205149646375
0.0244647846956851 0.89863106144053
0.6760323306513 0.206191099302557
-0.847061714545163 0.672665066721704
0.330295020906748 -0.908735696899933
-0.487595806307357 1.03539343737347
0.393070606615359 -0.999995958253069
-0.649348029834684 0.913931413106319
0.872458027721378 -0.529038447132222
0.0765400159893986 1.03578758705995
-1.0161059696024 -0.311638303496301
0.801369365078244 0.533244299734137
1.00292882741543 0.00405224382066952
0.928887244976971 0.34873769756898
0.526002764518034 -0.910676565757107
-0.91536765458139 0.335387667850566
0.932427029556296 -0.322177516300246
-0.429712658129193 -0.950207555378812
-0.0153229961925081 -1.1013650741953
0.225811072560929 0.930499377510457
1.12548338945609 0.0371031730288586
0.86658944984219 -0.711553416390248
-1.0693051026381 0.281025074792706
0.539794168540661 0.932668017464718
0.393238564604388 0.937248461644354
-0.93121651580509 0.0697507442484119
-0.812672248754391 -0.556148907464021
-0.495541820114113 0.856374679455176
0.19513448222452 -1.08418687494951
0.98684694950609 -0.481701535471808
0.571862455940023 0.886680409022437
-0.371234346303911 -0.928866498778046
-0.163767532667162 1.052565904289
0.832513905725862 -0.413781663741125
0.967846791741029 0.326416090382294
0.391749785252548 0.889224034671725
-0.219669397482957 1.00545911548114
0.299164877185073 -0.731636258466194
-0.505419700697565 -0.87969594959064
-0.190579246865231 0.892148843653378
-0.231186481756781 1.0537167053237
-0.185950290596536 0.93817094741406
0.220055742443194 -0.879253545542319
0.31441994612522 1.0798586037422
0.0180317150025203 -1.0818035130956
0.0378389888447268 -0.970631615298536
-0.821308690839358 0.906019508896762
0.881128508947324 0.126644501867459
-0.382703900694909 -0.998268000187919
-0.601852156457383 -0.754442562931498
0.51339008044285 0.709449381427514
-0.79050826524708 -0.651372727006071
0.567554018389419 0.710192617279679
-0.558097768967153 -0.980515665989001
0.958100349494595 -0.355635470876855
-0.274902994704616 0.688829593576858
-0.760933245549929 -0.756100451920233
-0.773546269732279 0.534151816629913
0.133780480681038 -0.888350414799555
0.987023680792814 0.0526254080579011
0.601693375479964 -0.888147055449768
0.754676812787414 0.917756794970746
0.320161126039736 -1.04427063839455
0.168906111744836 -1.14420544830474
-0.503544330547212 0.73615975481143
-0.387584929187234 -0.946567601478746
-1.00417002154309 0.393167599849135
-0.488402335754336 0.822947662441431
-0.833505430016481 0.0693016282471565
-0.0890396404746744 1.02588465629343
1.00070566437353 -0.0395839247123544
-0.953617942210338 0.516593034895012
-0.780860378724036 -0.7871510471248
-0.684259802329543 0.234204671264425
0.990624547666479 0.270227955808429
-0.579252096810247 0.832084969789894
-0.897327509265732 0.0689385129076832
-1.0085298920767 -0.0255102969864458
-0.840861686859848 -0.194468349167787
0.858134816368102 0.63306687481409
0.587890300749595 0.787355410295736
-0.762038784468209 0.534014393443163
0.716114981328076 -0.563796311206378
0.33482671092804 -0.963878920667789
0.25123132603292 1.18294095202489
0.547763764288596 -0.927920703301377
0.812958009744238 0.356177370351941
0.689900080799215 -0.762306218319766
-0.684058174442963 0.760803672483533
-1.1099195121726 0.0157432022870759
-0.0354776898261229 -1.05392660119273
-0.873224132774476 0.576124175132346
-0.240125630749515 1.11866006756402
0.905380330486027 -0.00184477140570725
0.47883479368847 1.02852921059855
0.881932706758149 0.0431523537907126
-0.377603129312909 0.990520925827379
0.659536740220898 -0.651444117224089
-0.858497308440381 -0.158173325265237
0.727940832238948 -0.59724755285125
0.801262433758329 0.754233461592541
0.878105838523023 -0.112461227583439
0.999584550022848 0.251757453294568
-0.442694367439543 0.870726036954099
0.93196734202253 -0.428849814243385
-0.402224692884763 0.857767750771686
-0.0829580417108553 0.948131421698568
0.926186108885527 -0.236438829582517
0.974540555134878 -0.60142781636729
-0.401255764586933 0.950234120212271
1.09639566959701 0.285214128359626
-0.608260415041857 0.679004118239307
-0.508668759961908 0.968141706718966
-0.0951972466728166 1.00076038888545
-0.762351358365829 0.795056397039169
0.257286311709549 0.9882014834341
-0.286363543631471 -0.846494514356147
-0.290146831031625 -0.984878451227049
0.334528349215423 -1.03148765947362
-0.753199158594801 0.691750829030829
-0.907017073420974 -0.290372634291878
-0.547386690911312 0.778993548416986
0.92985907935021 -0.381583670610497
-0.644002583611336 0.908666103451479
0.943182562502883 0.00174917330331396
-0.677287699500648 0.677163117397323
-0.852498787862076 -0.585402160548405
0.938199265151681 0.242613335276317
-0.78052779073331 -0.88555049322251
-0.247851612171608 -1.05997189610024
-0.187327585092674 1.08117077323934
-0.316437717019136 0.876584311823898
-0.63894482090419 -1.08452069622709
0.868807018846646 -0.84150790532687
0.963641403938441 0.254988925594869
0.515769948812281 -0.871513691821249
0.503912483118094 0.819559410207033
0.693443689759706 0.495058872811066
0.871575902238644 -0.46218461275918
0.78077640324503 0.349202144708721
-0.872205955777609 0.690621533674647
-0.300385832218915 1.03553286890032
-0.35651937137136 0.89144898014885
-0.0182127660454869 1.00014889262437
-0.566349393870006 -0.733069391330484
0.976833093789243 -0.568624106857852
0.510317346429365 0.721269744744804
-0.990232921085957 -0.3563370650313
0.136027222348103 0.841051120635766
0.744305407849408 0.635645417091817
-0.279426287195809 0.898519760177644
0.371104691401309 -1.04832191845488
0.359190088749625 0.728960597502415
-0.834396757086591 -0.305526450797519
0.853028450632716 0.0247845512385805
0.977730130856125 -0.51656946889371
-0.0260395264359807 -0.864787173702144
0.273974143170519 0.933580393849039
-1.1413945683571 -0.0466668163238374
-0.141064851189732 -1.28336553488277
0.753003782597268 -0.778343817894729
-0.676373652418112 0.63102631417139
-0.405454187719286 -0.959951718634114
1.04686658949766 -0.185921077509848
0.346122027367221 0.864074701866126
0.782776182959619 -0.901506087753808
-0.3234446725757 -0.831547645385565
-0.943494336921584 0.227585017983487
0.870976463063744 -0.785108761943563
0.586995617072894 0.827021016393462
0.778589653852962 0.575593354430516
1.02968529658794 -0.168543397107239
0.169640939520749 -0.983085221337475
0.56566047802302 0.713077960296194
0.159509521087546 0.84007025227446
0.583776828898279 0.849000726991728
0.628995714761202 -0.776733904229629
0.839806020222799 0.339127090930924
0.769257256301067 -0.253337611862815
1.05254607891096 0.0902020371518007
1.12820367569218 -0.158793095469035
0.0824293270212458 1.18965604795543
0.857729825634233 -0.102710137493794
0.898885780010031 -0.594350889970355
0.0217940636983663 -1.14259493555939
0.546754973073589 0.941439072741834
-0.740318247260858 -0.623033091782521
0.487883466324722 -0.490718799345971
-0.795850303908152 0.386891307689284
0.266285731240608 0.950398061959763
-0.562187908597568 -0.69542124417454
-1.04332930979117 0.0185511279786427
-1.01945118855427 0.269406477890432
-1.03258374745566 -0.0946756930867926
0.892768745133037 -0.423809729098069
-0.844548018920536 -0.00075808445463596
-0.927365063200669 0.00758625603539306
-0.619606224367901 -0.786645561936568
-0.574406134192262 -0.858342811089782
0.0317462697149374 1.03809311679203
1.07842430028607 0.318773496504926
-0.541290549158056 -0.750510628983787
0.53910986638105 -0.861412443448879
-0.904680479141663 -0.307769489591083
0.863522476462602 -0.640786301119187
0.854911774924602 -0.567376398738457
0.650314564626054 0.653051257706552
0.0971485426478289 -0.851399641739509
0.268207505605267 0.982779818996831
-0.664189428864034 -0.677888335999917
-0.79181282815978 -0.687447299521444
-0.502815003350468 0.923149256529601
-0.191489887356062 -0.974334835985478
0.460769998267074 0.742370814557512
-0.343227238631309 -0.874800135767633
0.511700322772569 -1.09350355949904
0.749458172102619 0.717977686858299
-0.735219004239 0.781850595978416
-0.891582304738409 -0.606191320671004
-0.474536523632469 0.635650832100964
-1.13174813553718 0.00290709243995586
-0.303835711293867 1.0074364693942
0.390444652530278 0.849458058711029
0.527334285830205 -0.858371898186191
0.533382345729805 0.959393842947503
0.68328629365058 -0.786199595471957
0.808300299841726 0.779797980042565
-0.914582221210605 0.239187773502731
0.754957101256211 -0.706335279889392
0.797211432494579 0.516733272573259
0.815502121567182 -0.21138348244819
0.416754247315994 0.955475738575819
-0.926937134923401 -0.106682442719245
-0.425180830807768 0.888402875904056
-0.7205127995796 -0.688752016697814
-0.0642920353919453 -1.16522881107728
1.00681187559836 -0.128972498768988
-0.082286323180412 0.85674059379262
0.591995938475385 0.844368952699509
-0.897164120106804 -0.8056889773583
0.960546656284121 -0.143975426984401
-0.894177638479498 0.35845431338418
-0.0933495154999776 0.885467773061398
-1.06117776096841 0.432906392729743
0.915340803208782 -0.356442647777464
-1.00480684197591 0.061242679157176
0.91265687777345 0.504392614375961
-0.258027098272856 1.03540405463433
1.07664132824958 -0.0696189953032977
0.834253727806731 0.73443341537141
0.588385547085561 0.516525969507496
0.825017927289666 0.30481987300858
-0.0396165402107891 -0.953344342370712
-0.084902481945507 -1.03773125569388
1.20063757906054 0.228750851770495
-0.671621167356708 -0.685150425728977
-0.0297600139401514 -0.833435845968639
0.818203949382609 0.418567893712652
0.337449995243596 0.838510540514862
-0.504848381988729 -0.822205028326804
-0.947227503492665 0.337047247900305
1.0243123967831 -0.287871078734712
-0.0620226697528818 -0.987497807001363
0.722498332959992 0.586370801111679
0.761171514933091 -0.858235166937524
-0.900452597775055 0.486807781067401
-0.852247526890525 -0.587003321659096
-0.866581735782113 -0.391378708256583
-0.844014132402288 -0.522263799073119
1.07519827480365 -0.0475188992187942
1.00719725240931 0.125512113042886
0.250182679015123 -0.945239387652837
-0.446550780865153 0.867756349217375
0.742323913686476 -0.67587863765613
-0.827317551464018 0.768471308316235
-0.679704381720595 0.622261229813223
-0.838296764607123 -0.592692222650404
-0.716154163173888 0.360945093721816
-0.488084291792606 -0.992146494783306
0.672229854700802 0.821923243286574
0.626045433465637 0.792490397960672
-0.495918040797574 0.854976023984527
0.678873550561998 -0.856376814109761
0.835830070039957 -0.535378217894062
0.754707587978158 -0.53702254094976
0.0119084671966861 1.0430280725832
0.62444667826623 0.903377258085151
-1.00338785322005 0.181837157289116
0.348351393736823 0.984675586227901
0.953677482802044 -0.363149826604181
-0.447268015258452 0.775862476056789
-1.01787023180714 -0.423822169857407
0.87842978650974 0.599767085458011
0.840950116574503 0.979476840876326
0.984491600221895 0.18014079139476
0.579588214284765 0.724744382667755
-0.352578474988507 -0.984114679625617
0.71934906137728 0.533370286662175
0.0496823398959342 -0.938002331461042
0.0254384509432715 0.904656989082425
-0.831068995054759 0.222354030585505
-0.129683756435531 1.01507211290975
-0.821480714655936 -0.631742733279368
0.283063775575222 -0.926636812939632
-0.928443746844372 0.554662307754466
0.957460036401416 -0.0390426880648714
-0.034278139676326 -0.860759045223124
0.0579132782172723 -0.991589395723654
0.173923894237705 0.901416450254283
-0.476985750729773 -0.80531924441791
0.718380834803795 -0.654998741751925
0.282473761198807 -0.804564621346656
1.00672659849218 -0.117370243851958
-0.462665512522414 0.894592040692478
1.03970570429555 -0.299908591577989
0.402220331612505 0.980312749129386
0.943573055146572 -0.0773668637583734
1.13805921876997 0.249435596769552
0.560317634299353 -0.883969154041798
0.739408699007391 0.711061929662301
-0.976463607570015 -0.521848356622357
-0.973853934648732 -0.166368334794595
-0.473276082981271 -0.658931286919788
1.11975299104082 0.0335477751065544
0.176297712596153 1.08088611909183
0.940209013531154 -0.388198478203462
-0.474916667393557 0.742527701359522
-0.321360018152642 -1.00485953495816
1.03116688922591 -0.0574805876975965
-0.595006463850785 -0.680946883413329
0.206157872724827 -0.732073008992765
0.455274717568777 0.835559786079898
0.690040865167333 0.57146598373629
1.02864219031192 -0.29590821011545
-0.622195731750208 -0.827181626109091
1.08306122175336 0.370496775410184
0.640076195646479 -0.762030154756875
0.26368357102216 -0.981407971611216
0.870156265097206 0.381292150942851
-0.447928617487211 -0.778725340666921
0.587457044555817 0.7455925037591
-0.779711998892559 -0.50636514571045
-0.2730817073835 -0.843542091252999
-0.136774825510313 0.889657242668163
0.975136169106252 0.0190186018294899
-0.867937312393872 -0.625787461568207
1.13322665001806 0.45506092780558
0.887400037319766 -0.179351076818684
-0.0869137961409108 -0.849536591496504
-0.381960455141455 -0.945934320934028
0.967596716734537 0.0845830387991406
-0.941133594659097 -0.00157752395238608
0.013032499044231 -0.913681420506147
1.13471594820267 -0.0284142016498897
-0.944144589752312 0.598639590105822
0.48585388075164 -0.923764849814367
-0.389382027590211 0.727981348628672
0.232854795736376 -0.847429245982317
0.684242180447931 -0.787377823259509
0.442193699779022 0.821050963002863
-0.407768599782921 -0.878039840810327
-0.529038516579085 -0.925417596795151
-0.955243862079263 0.617836766158773
-0.896232183035564 -0.0163307324933128
0.0964031094607295 1.0346543555373
-0.12845909599354 1.01266261429108
-0.744251016842041 -0.583955562413588
-0.86961240177271 -0.347636292202101
0.477027901560322 -1.08428981531819
1.09910897442426 0.193085360241736
-0.379112318309057 0.953237792409893
1.06841286661291 -0.36210739700673
-0.810223645401144 0.468782089460644
0.578411441615135 -0.7700580080804
0.952963392681101 -0.0652042979269761
0.670163778843991 0.753534319606809
-0.412170476740793 -0.809560211347883
-0.619872629765951 0.940902506632526
-0.529971874151929 -0.764257145613418
1.08551534741464 0.348224973543203
0.0022941388041427 -0.750879698444394
-0.72997081582569 -0.556049652003918
0.97458511628709 0.576113469631044
0.901584824676518 -0.356184687238107
0.808040813046633 -0.442896111110101
-1.00812021346424 -0.01291709200099
-0.48590682755273 0.976749376434413
0.350338587666467 -1.10419117474668
0.608318251486226 0.819275278164645
1.03739313921478 0.277301107826861
0.416929129926392 -0.790497149163607
0.457517854817875 0.660093680019494
-0.0983205292999337 -0.93294349690366
-0.462128702751986 0.850886335926791
-0.819692567450157 -0.706538048406995
-0.955763242569168 -0.501769248445607
-0.620748615279016 -0.855915364592894
1.09265288142301 0.0724633295858258
-0.55724145889751 1.00167945409334
0.554207040802725 -0.666993200740682
-0.752891248115249 0.357405427237581
-0.638918450551766 -0.867205597264308
0.59544449975782 0.811375716755526
-1.13346660498074 -0.369617845552255
0.272727360127285 0.939131618367183
-0.859852586937531 0.494001326268081
-0.208628691127046 1.19247633725641
-0.467591232162914 0.73932307316571
1.02230673136574 0.623195720873664
-0.697573620377359 -0.600583328126642
-0.793130102038036 -0.357458114575561
-0.428525320785765 -1.01841999791571
-0.358935740742758 0.928549817916747
1.0217912791694 0.182883529042186
-0.874742227350847 0.34851592654005
0.813867043015712 -0.358725253968531
0.459249949030127 0.813170612142782
-1.06529455881998 0.146399941395212
0.721742070525703 -0.765539463703223
-0.918847746043083 -0.0318434970825043
1.00221881702112 -0.559641823546857
-0.830184288955174 -0.194123986203009
0.834856584458433 0.419932517828171
-0.182567036101344 0.941441032922987
-0.0675114584593053 -1.02278714704186
-0.79869669368087 -0.932959027999799
0.584724974132739 0.904261766247906
-0.801076547741144 -0.743995920090245
1.00456888915871 0.156975946040276
-0.491244960402165 -0.890507080997848
-0.554669498597211 -0.899209948907896
0.101258417863506 -0.969649863318671
0.227000162513104 0.887444086198789
-0.165250051335715 -1.08560752424815
0.352263292255963 0.840733813776788
-0.2388715358645 -0.958223305956449
0.928837277378425 -0.68595555993475
-0.789698883798205 -0.382663619524361
-1.02300551928182 -0.122385765102386
0.538061576616357 -0.72648077866203
-0.800319028579737 0.417119571257256
-1.00613614566852 -0.0403825253842535
0.508704866482122 0.89710635632853
0.942908569571653 -0.472881772275345
0.977817393523107 0.0880639659949341
0.472537750604794 0.946639081206872
0.491591598511428 1.08474397343867
-0.634477445172583 0.857663914989724
-0.570879030294247 0.55909343493498
-0.015064361611628 -1.11121009495501
-0.92378846175475 -0.320020892769373
-0.723588458902572 0.846701305088134
0.661645881174476 0.715723488563423
-1.00036425561341 -0.272200345414658
0.430302885702869 0.798836518340915
0.980061592656316 -0.381738861154148
-0.16535094868876 0.948928954419725
-0.627032567161906 0.657752357260804
-0.0337497198277391 -1.19202454888243
-0.452965265017377 -0.947743413453192
-0.766197436740588 0.738105781833683
0.385033239311558 1.08558410481357
0.694870503166309 -0.479826231183248
-0.935174203769052 0.564454281559419
-0.722010340486098 -0.780323619691491
-1.01749459401219 0.373702614669573
1.06337739316303 -0.137302594733292
-0.240546949196082 -0.862530309744963
-0.920780165990735 -0.630189042561956
-1.06253671728134 -0.0918932638284529
0.532928664889259 -0.855606677910354
0.000215613088034278 -1.02557400297763
0.353352941322504 0.923625621674503
0.519884265413088 0.875963226205607
-0.416720059170191 -0.880986287698085
0.791808757347474 -0.714102084925088
0.971747419407903 -0.454149799572496
-0.0717230680650669 -1.01272173256355
-1.08172866637375 -0.220356562204304
-0.329854888613483 0.931116963377478
1.09903774641826 -0.0290446747834168
-1.03088925460954 -0.449717292115975
-0.415434591146532 -0.848096550885249
0.504735200023068 -0.919502296520614
1.02872372372421 -0.242231928700482
0.986279498323867 0.546553096034792
-0.169028540647842 1.07214270406553
-0.665642756123173 -0.821546610808964
-0.937628172023551 -0.423370361804691
-0.384848561645135 0.839083613586275
-0.867477492832255 0.519027010588847
0.850352720069372 -0.416512271247327
-0.0618356988680999 0.870858498132626
-0.847475118508637 0.253157572438002
0.890133541332234 -0.391214519207645
1.12340994709722 -0.283487953845427
-0.956177309294901 0.369236942226396
-0.610665131136037 0.820953231186053
0.789836162227947 0.651569238896035
-0.802426990554562 -0.781807486346963
-0.938871940927998 0.358000816182356
-0.0567351559505022 1.1186213983754
-0.184055929149277 -0.82817631439697
-0.901996621629086 -0.0926807053472933
0.542919417935109 0.910961467698202
0.146726132368906 -0.985828195773769
-0.37215171840124 -0.90023855049908
-0.542309399645538 0.920824170761243
-1.04863500315478 -0.213996297299404
0.645743691142317 -0.500717216466371
0.596030241922633 0.732129089459624
-0.951628985195852 -0.437132356021624
-0.205259944411378 1.10586651253982
0.878644654478304 0.602161122225226
0.503347308353771 -0.825732906532414
0.511362747840103 -0.823067817417773
-0.953470580381588 -0.0886636001867441
-0.720834736488251 0.468410646965318
0.551325678382208 1.04195814390794
0.980019304023968 0.0419147263020581
0.885090745789093 0.772512534152415
0.81739172776844 -0.515590736293835
0.245929440359475 -0.837283925983367
0.863667855474652 0.0884550438731638
-0.329656583406073 -0.927943987640588
0.0231599896272923 1.05971457471571
-0.860738374088298 0.437596387179642
0.742897688774568 -0.769379119933599
-0.451516429893759 -0.831614402237326
-0.221324482174981 -0.831707031024403
0.587050174070202 0.697081340650223
0.900032694478824 0.221542358174221
-0.537894103827286 0.736847309187749
-0.889306405073753 0.150838270378425
-0.627760827132838 -0.505604562139449
-0.633908944176767 -0.782917232249299
-0.607358446667531 1.07272719196059
0.120865550692489 -0.97494533263307
0.140955855241344 0.966359961630536
-0.988204912697948 -0.076667318586425
-0.0925868127519647 -0.998098363163025
-0.90144335792297 -0.748812711018792
-0.48835560174392 0.834438933089183
-0.943136058970813 -0.000229326806648694
-0.116896109391916 0.953753205031432
-0.384582161156082 -0.769291470740434
0.737181275486837 -0.798237817205167
0.468498633481064 -0.870043806603534
-0.983582841614603 -0.412053800811783
-0.809801732360451 0.664179024286472
-0.711630378934003 -0.745006690742805
0.360452101368629 0.765554767903962
0.980856947373137 0.0955543537669227
-0.740002525011359 -0.283990936602118
0.00515213816046491 1.14040961821943
0.260591872232907 -1.03578880240774
0.763100471192413 0.61454324459852
0.89490793125971 -0.429193235221641
1.00094655539421 -0.134525092873324
-0.105441419458699 -1.0458133624064
-0.528409332396527 -0.922891487298204
-0.947856253469107 -0.633025009403026
-0.831115882281406 -0.222061139291953
1.03399315416924 0.518336775120971
-0.820270647912652 -0.297605274566825
0.183430522812407 -0.953043121354345
-0.433508437448786 0.806149766986261
-0.985826256944499 -0.300732252368899
-0.617041616319138 0.843725695535988
-1.08107375651775 0.110629290673646
-1.05798822585557 -0.496803804778586
-0.337360264597266 -1.22583776354987
-0.570781358172008 -0.679301639917868
1.03372445881788 -0.125154013577432
0.934357517340375 -0.22544859757698
-1.02010020832376 -0.296212288326049
-0.740566427882542 -0.733468636132642
0.527820784982527 -0.550735372617083
-0.137088817452121 0.91498332783646
1.01704448710406 0.134802482646058
0.806404563213492 -0.535822544660771
0.918778695933778 -0.245018565975423
0.820575217126999 0.288050956272175
0.823324399725973 -0.732281061733311
0.418404107108984 -0.871615037393475
0.885749199059911 -0.614963964888042
0.410741282430626 -0.748786660776138
0.84697653149682 0.631879368586785
-0.999423551712729 0.48960138776314
-0.639685765312801 -0.55485616614518
0.509897838947783 -1.03618299655949
-0.0905305868291113 0.856277567297865
-0.139016610627254 1.07581171266091
-0.674137144374365 0.574824120640725
0.0705918275297469 0.979264353997886
-0.451118313927201 -0.699561288606835
-1.08212745642945 0.280478680161032
-0.701128559679726 -0.438153400770112
0.120448897602453 1.05153633351583
0.0516077637779649 -1.13227921732381
-0.556505566635721 -0.903423392451253
0.874494036469729 -0.460625605107257
0.100783119262756 -0.90138440713444
0.642055759523825 -0.670218327602914
0.551255998001938 -0.876427109420625
-1.03189923260016 0.0452892345524631
-1.0003921797266 -0.0528918889646792
0.743336235518148 0.714976204051261
1.08772479465775 0.254134889306477
0.278229932899217 -0.990157046378213
0.836255863545291 -0.650475593224686
0.0800000403920769 1.09895172244192
0.0952419578261221 1.00825677786897
0.291024422728767 -0.852314742724113
-0.292365775521112 1.17229467788078
0.571503203156845 -0.877345889316697
1.02424512788445 0.701506224583338
-0.540883361986334 -1.01537041601342
0.312810305472585 0.966535536862067
0.110588015966887 0.914800654478301
-0.944961207821861 -0.338375891125646
0.575569597605361 0.84588758148918
0.584775243662099 1.09860173333397
0.537543244940035 0.743679424896784
0.652930404838122 0.846480218062473
0.722129569487689 0.403832323064195
0.792289243097096 -0.509689377299081
-1.11068416508056 0.390438512845882
-0.396506134342727 1.0758956699627
0.379844183423165 -0.767676117517972
-0.114695150457474 -0.90296773332278
0.221479217168662 0.88117390037494
-0.234274590338477 0.928241199170462
0.528670692692888 -0.828656297983518
-0.843156924166201 0.57670750237462
-0.483485695892519 -0.886930494441984
-0.616407487730679 0.714449413665655
-1.05594114652534 -0.03609982058924
0.214759480921155 0.882935412104403
0.460675363253509 1.09100293185367
1.00792614498233 -0.20211956103222
0.0643705462976979 -1.13633222463771
1.05946861883396 -0.0482966905125303
-0.578932284712805 0.800714004990431
0.972193183342608 0.455952841876287
1.02970906096244 -0.164151122744603
1.02922073278752 0.158229327393758
0.112723410539958 0.894466262205146
0.990903042252926 0.320245468240406
0.718887473909065 -0.685266081072693
0.936846408795082 -0.230844449938541
-0.746864383036189 -0.894915173434326
0.848286510570532 -0.618492603480057
-0.305503676464287 0.914365493934823
-1.06312754278138 0.0933003866627456
-0.922186122594371 0.0664263507219486
-1.04072525077191 -0.568290728327791
-1.0493918018854 0.156588466795776
-0.438043685098494 0.827329244013109
-0.848865351890669 -0.0423929904632032
-0.259977356874245 -0.870416978970418
0.084167341172838 -1.14471734836863
0.840235780359254 -0.772927480083684
-0.682982282906432 0.611761190740826
-0.627100739313357 -0.698076119338572
0.946077142216642 -0.260497971083834
-1.09886701319025 -0.362351962225563
-0.803980422680757 0.53943520902557
-0.543334592994289 0.782237718501934
0.024022474983303 -1.02440568473395
-0.905058372412717 -0.5800944392435
-0.100310359335243 0.821363421626696
-0.104246382315644 0.935811499843523
1.00156401244737 0.313835360825555
0.914029829532086 0.424457060372247
-0.750940142100502 0.396918633252309
-0.845038787851094 0.616183241787167
-0.722842246480074 0.709762275779645
-0.291825169443612 0.979423103371683
0.988829731216212 -0.321519135420829
0.11549722007581 -0.9243034912931
0.41134537071794 0.701974864761977
0.401591759752464 -1.07318064311752
1.11583074701043 0.256119618867222
-0.732916248636985 -0.41826380945816
-0.537060937364664 -0.840557968337434
-0.964257273402658 0.308991017363246
0.186437889984993 0.851033814835587
-0.85646382143049 -0.0575838156462384
1.00502462424512 -0.2180560647625
0.767032395428948 0.487529177525022
0.14901930016308 -1.02407423715771
-0.171032185760112 -0.990158219149016
1.08572059075958 0.460712210240057
1.04387863163149 -0.153078973944997
0.418540727942089 -0.819620734113676
-0.505114514645197 0.738769338004915
0.798797417070168 0.564581420824287
1.07052242642971 0.231873089060674
0.613827366270224 0.919936944475483
-1.02215559006397 -0.63398598592082
0.115128413912842 0.996801854070481
-0.839432915023848 0.658871047848087
-0.593008310876517 -0.937368751137816
-1.09155458485933 0.270708231155617
-0.838264193470276 -0.278140275017435
-0.547710470482583 1.01117421519275
0.230772539152967 -1.06136473905807
0.957545338053084 0.239148700409687
-0.36070182041127 -1.04557111569261
0.416648874370326 0.796398762599471
0.23046554751619 -0.926268011425462
-1.03620266524929 0.096716645498261
0.980319353550643 -0.323046507555075
-1.10008814952083 -0.0482013612674506
0.886130483833639 0.0683148806670505
-0.317263269405378 0.966408695401109
1.05903758164338 -0.0668948511955957
-0.488064034917179 0.881400932576456
0.250230038901046 -1.07677186055293
-0.235042693795237 1.11842255820396
-0.378394939029952 -0.933526059559312
0.511880321682493 -0.694054180094247
0.945867235480701 -0.447121136306101
0.984783858706401 -0.298429249696247
-0.974192385769985 0.458224420850953
0.840941535139759 -0.517930517915902
1.09745909595334 -0.014761528952949
-0.902345673135653 -0.243758351293299
0.351305190707662 -0.942198111297739
-0.426954907662447 -0.938941613324164
0.911465682297612 0.0433981356949652
0.784154312701619 -0.0855603171903015
-0.136169282727988 1.12980746464823
-0.271822823362933 0.694426566297266
0.662093735764309 -0.548976123784476
0.572604403541456 0.922339682791733
0.0623846621119661 -0.953255759977125
-0.992949460158525 0.26978366872506
0.919384497241354 -0.571942101064293
-0.555397334132453 -0.739990082096053
-1.05573801083974 -0.103859702045702
-0.848600800346686 0.452760395633721
-0.539212467851253 0.994633158480754
0.905950174784915 -0.260876648235857
-0.266192863479579 1.11644213188533
-0.75474800330686 0.652872990396879
0.915262081713337 0.198076624352067
-0.873524933265986 -0.305793281539644
0.930786277557642 0.0862282961122715
0.366858784982076 0.660546455817701
-0.805303050317847 0.383332984308221
-1.01060267978388 0.291988750011211
0.878590757279567 -0.671573829704058
-0.223728624289253 -1.05136160164278
-1.03675121067524 0.30771953331503
0.986242717325842 0.329840326949126
0.947462730027543 -0.21795201352376
-0.401563511343144 -1.08631875205537
-0.945630172110218 -0.526401978600161
0.583370195240724 -0.805135215233672
-0.341535933588283 0.90494675086717
0.753111400697353 0.723673580285143
0.751923705886071 -0.714753278551548
-0.532337490427423 -0.91738639852829
-1.10907562478967 -0.29664207215524
0.689118151443253 0.638276223902779
-0.353523762343898 -1.12821001906794
1.01064828106217 -0.146495543672204
-0.603790996778416 -0.808052039359069
-0.159829254582663 -1.10101669414263
-0.87412998129311 -0.138919770354857
-0.327903991122019 0.880162284630301
0.965123657352632 0.273036230242416
0.544589628624505 0.60694690190573
0.533376628816122 0.670425905651958
-0.470165156675199 -0.943518940284374
1.09375451525101 -0.598804385413235
0.994038879960034 0.345632493540943
-1.01275256751292 -0.100847721863125
0.739035138015786 0.672702708154572
0.00783344699102861 -1.17327866801184
0.99365646086228 -0.216113386143716
1.04509782253339 0.230444882734537
0.826518922370674 0.694901503030913
-0.564636305303626 -0.759244190880618
0.643954444524019 -0.922186038729047
0.933029539661358 -0.44815514992746
0.877773585518285 -0.155805212007236
0.990402742151738 0.376933392154734
-0.29628460961105 -0.923799344430308
-0.742335762711284 -0.107223324624355
0.274225743822703 -0.934820672642628
0.957854362945515 0.544880255031757
1.00206292717315 0.384750342337674
-0.827274054985196 0.0974105384055672
0.540066041854707 0.818005711502836
-0.373801199432863 0.875358683063886
-0.0319402574607512 -1.0168798017332
-0.211275145629361 0.916546020064938
0.538218722952623 -0.897681562807583
0.62616082541284 0.624514541390082
0.825502657111011 0.619656798136939
0.748737694186987 0.549809305200417
-1.01758359110524 0.514919408028978
0.731900697082831 -0.754377349876233
-0.60347036392536 0.666983509110972
-0.433956467194488 -1.08057991787923
-1.05753909530572 -0.509549694213003
0.440325327960914 0.715571754693409
-0.236408427887823 -1.12743793499471
-1.11939497877861 -0.215978814407764
-0.944680497941798 -0.528471467227604
0.528411081585962 -0.911963258672012
0.820566971411029 0.699264197408949
-1.09517112559194 -0.0995707598169075
-0.955492360258656 -0.499686861539187
0.863514229696338 0.193350168661073
0.551118733734973 -0.805171476469315
-0.982238166946846 -0.792287862406838
0.156801576341874 1.08686904128396
0.966825173476742 -0.513805594814842
-0.88327477841903 0.551755403004501
-0.960004725251944 0.401650689159621
-0.94030040115672 0.522109956380187
1.08069158108883 0.123753586189537
-0.53519503288954 -0.855160605433875
-0.108094499856464 -1.01681192657712
-0.714915704445753 -0.713483260990436
-1.29465738184034 0.0449717335619781
-0.73918095648882 -0.613911134867418
0.0346960488773179 -1.10368643914874
0.0364849874971359 0.896054723587842
0.986495200321583 0.331126409836569
-0.925486372779311 -0.236971352988265
0.709502910815796 0.880535761394246
1.0143939284973 0.198437406116837
-0.667367864323944 -0.469360953638531
-0.928145538827234 -0.149181748677137
1.00218548219777 0.13462154337897
-0.333269320235814 0.911856966864241
-0.27469190516668 -1.06271439191455
-0.322747309630728 -1.06586650720578
-0.802105355609169 -0.487763244776259
-0.912768811874126 0.247340640078896
-0.902332120138167 0.590354474657804
-0.863948384563071 0.18312518580481
-0.540228427098024 0.795818064368821
1.05522434386549 -0.120310032195843
-0.519919460077608 0.647759370381869
-0.775392961766279 -0.410344238060695
-0.74940183236983 0.518723441848271
0.562338405246811 0.825184666293605
0.447660921959209 -0.972245435845875
-0.735965572828248 0.259112736578262
0.706245358690288 -0.592438665199839
0.0686628531037455 1.0614225691045
-0.962158615490772 0.313012978902664
0.810352733374643 -0.936527842972763
-0.716497143030594 0.57805893519771
0.829564842061148 0.548018982963833
1.05630222150428 0.441741954490133
1.04040218578539 -0.214626506920999
-0.347208183805378 0.824913254399799
-0.257934460928915 1.04673659180382
-1.16372497373381 -0.258282677101064
-0.890592956069151 0.427347547221934
-0.921270308906558 0.634039906932596
-0.502494628106727 0.882229556929414
-0.866573345136246 0.0892062332095258
0.539632390027905 -0.986865705238232
-0.562084325885633 -0.808669512252223
0.285475402246604 1.03262178063378
-0.752068111973303 -0.631461066776019
-0.869029129615275 -0.283879940437403
0.888037771420603 -0.0826449860165168
-0.778468416331799 -0.743446304799647
-0.522589833531664 0.751584588771088
0.142298913291063 -0.907299870687588
0.208460287679218 1.03208823952025
-0.0475079319954868 0.921766557171127
0.338193221551231 0.871863425774187
0.639946877913243 0.825220675891896
-0.0398560115999393 1.10477170306276
-1.08202739737236 -0.553723142473367
0.3551019585202 -0.904450203260688
0.480438055265229 0.925882693883327
-0.626779017832964 0.645557286015095
-0.188031920439377 1.12114498754138
0.222178319775491 0.883072700648157
-0.971836325677129 0.225237404838006
-0.874929835936409 0.241317895412475
-0.828617632368171 0.569086927830486
0.736994727523278 0.77566149554787
0.936326938787319 0.591115347278957
-0.860882103591215 0.515586878530451
0.252957035252002 -1.21145316632931
-0.725760978062669 -0.968307288821733
0.583614119567195 0.864850696894221
-0.248708060858948 -0.982992506795453
0.482214254884382 -0.871371960497412
0.54689330741019 1.00200846084148
0.236547296335719 -0.954948101042426
0.58525464547036 -0.632690676471122
0.794351151800863 0.778441350995051
0.365936521153881 0.914960593110776
0.599516811240827 0.629179303837103
-0.830891066580777 -0.621543258741659
0.280152880827648 -0.913925438690805
0.775091805629387 0.317698488864814
1.17973335000124 -0.165694339351986
-0.381145764879318 -1.06608611959752
0.554941014774209 -0.78999952599297
-0.0762823541196276 -0.902897168104233
1.1203504267635 0.644612359962529
0.926671821216245 -0.419255090290084
0.820967554953481 0.759227045958471
0.665389659728404 -0.731001125424564
-0.685382457341267 -0.63730166891298
-0.658839051105731 0.645646506303706
-0.780705657575685 -0.536381042678701
-0.695896465970204 0.671402436156055
-1.09202313845899 -0.380172127332357
-0.632070097243776 -0.580511759034949
0.93283396314514 0.334201676400095
0.545934950389405 -0.754245351328656
0.540915739019245 0.929195894420031
-0.798785646394572 -0.860867960159842
-0.716524371880642 0.860191642675537
-0.528001129989738 0.681218020204643
0.344412195753048 -1.12495078154608
-0.852118403184633 0.400284193996875
-1.02445779978126 -0.369441115393576
-0.905289451156089 0.437883191365289
0.770993266021811 0.534793036184533
-0.943650287071538 -0.247720031692713
-0.081187952564317 -0.939406862536053
0.25983083886657 -1.0399682121751
0.679881737893788 0.402327370717055
0.817528928036804 -0.145906234900356
-0.699384148007055 -0.636662040452507
-0.345523744666994 0.864739075186045
0.512468185020926 -0.828488620884338
0.202493152077845 -1.00882126752868
0.700947031219182 0.613232991448664
-0.810519277511639 -0.634143573670765
0.724307008332395 -0.831714535044838
-0.93871858128897 0.371534135146758
0.600788476522476 -0.822430083814112
1.08079633223914 0.235103792621191
0.691310606081341 0.587480184408731
-0.986915200995189 0.309889300714816
0.565207294638462 -0.635069430472401
0.814644097465253 -0.150040743294116
0.631599940206548 0.870298972637252
0.225491731643334 -1.05334150306833
-0.519402450100142 -0.86397857009406
1.01008788209431 -0.425133683703518
1.03039621301088 0.515916610084148
0.659101403732394 -0.962180375238479
0.586763672446272 -0.927675530743255
0.409714423532738 0.890620189744889
0.879460811950546 0.588649513732508
0.0586515480524311 0.809466422225891
-0.855598687665093 0.672127889990949
0.0898191891772259 -0.907276271109594
0.238470263659837 0.951926300408562
0.872827639792514 -0.624387733552378
0.235021367111055 1.07051391260003
-0.0407980363354171 0.951257774008269
-0.950584150083918 -0.394726467193465
0.730353245499842 -0.559473545927479
0.971002900755395 0.329944602519525
0.327108572110385 0.983853047794418
-0.330260629741057 1.02023620963197
-0.452543968872859 -0.860544527842331
-0.838967676674823 0.483910581244167
0.362785586283955 0.996358182372918
0.883635547764402 -0.485196040692847
-0.935733309579544 -0.369555560089541
-1.02552926798467 0.0337198566534809
0.889530791105501 0.494530884183561
0.801318646200515 -0.41895926796836
-0.887960619742238 0.0828536276098614
0.946984157660401 -0.220966091831517
0.910754745523599 -0.572258281082878
-0.919950281695992 -0.459748266484634
1.01920215872302 -0.472678739026341
-1.00950461366562 0.549243212739056
-0.962019230170526 -0.312493422736336
1.05471024668043 0.24073553909135
-0.839726076801978 -0.614500847922503
1.09372583581221 -0.26476422147794
1.01804490366589 0.389012319835118
0.130148681041071 -1.10508729846265
-1.06780936939179 -0.027896000699636
0.940787574633177 -0.392113259286045
-0.154425408778856 1.1353116428095
0.930324794769321 -0.545019353685076
-0.0564154126663538 -0.816788797114625
0.902592144560252 -0.632770022155506
0.584495304987331 0.644447054034395
0.78872946658896 0.848563992404173
0.254927280900787 0.944551446277242
-0.729307927598481 0.244212507150482
1.04167122413573 -0.13741960098909
-0.849079091095469 -0.258636781827739
0.536782391962555 0.824364296574343
0.912081891032227 0.0265610435606899
0.746041425228116 0.837895766387747
1.01053074848346 0.237384699576112
-0.861047059649245 0.519328745748025
-0.568101312101879 0.919527642392124
-1.05075323711498 0.0130009552255608
-0.646032026587163 0.60966684594116
-0.264389069324071 0.932768768369661
-0.804573888909123 -0.564728617245703
0.949057874540166 0.445764769190143
-0.472941308434646 -0.793430966470428
0.910920048010227 -0.206163765503997
0.910032648939886 -0.232453452573165
0.311119439926632 0.76902117921092
0.787218963578601 0.656818603142374
-0.652905923613103 0.756537728541719
-0.140119990506597 0.965451235919088
-0.110225368628392 1.00118632726891
-0.0961419370855748 -1.0799276773052
1.03910380220029 0.348783568383885
0.694812507016472 0.817708946407867
1.04992240461666 0.303308198222715
0.847876482060395 0.540971332598073
-0.891062518229641 -0.299195790259526
0.573152776919841 1.00530817599201
-0.0904263131814527 0.905240795400394
0.39253557715498 0.750109356536202
0.685314695031683 0.72765590769633
0.546227127791797 -0.721131484524502
-0.84881579863017 0.365306234677712
0.0605141068070242 -1.08257815653497
-0.763926344999924 0.807170798757381
0.867059621660126 0.0662093890445906
-0.673870180782596 0.970520890200905
-1.03878402768838 0.310512592591653
0.457987539503162 -0.831523438631658
0.205494905763603 -1.01495306507628
0.211382981603414 0.913749712495518
0.970633956264656 0.599791755345576
-0.201268508629674 1.10757507876247
-1.03509446137987 0.522134113541302
-1.11365772073952 0.162750507423873
-0.429281988727745 -0.856426119827233
-0.11707176892164 -0.993236712259311
0.357033446037781 0.814533270779965
-0.845468696106323 0.497155138541845
-0.981431338827388 -0.312877418271924
-0.302898456838526 -0.887851928233912
-0.406062226205579 -0.873201812990154
-0.060857779244684 -0.957542674145515
-0.438610721126874 1.10364399977575
1.01085635194911 -0.353916630064567
0.701823959438201 0.577738355239904
-0.998956090820373 0.325339747042351
0.602144846543199 0.80287883309523
0.66256502775958 0.534469667072583
0.452245272682919 -0.79467676560194
-0.786601387137263 0.62730302212805
-0.897809317092191 0.44609323655043
0.443928456176129 -0.942405115476848
0.376060540743137 1.0730645770113
-0.594800510957042 0.73096553112629
-1.08349544751996 0.0814904097517928
-0.971923041200299 -0.229839015033386
0.861402970773352 0.237951118498738
0.98394723833338 -0.0179150114805835
-0.49862472970402 0.492447104313394
-0.594325592428547 0.696395679568865
-0.460296980542784 0.944707309041577
0.325559390749461 -0.953084885087499
1.04981593374526 0.166436306835084
-1.08377405528288 -0.0164301184424885
0.582489923942167 0.760822058251599
-0.970867744524879 -0.274687721426637
-0.969106341287608 -0.610891583345735
0.842710806730505 -0.510631115824103
-1.06243597303486 0.442472100528406
-0.105809861806668 1.09141965818708
-0.905050008785725 -0.320543709715784
-1.04436874963651 -0.0101687250638171
0.55649777536816 -0.857119234528887
0.115795758097362 -1.01605488705334
0.662442670788201 -0.0103911576001727
-0.959559604523525 -0.270041772817314
-1.15599299797327 0.172678081090696
0.689740772699122 0.526506216925577
0.812337285596758 -0.575142061538514
-0.757666542549691 0.384456440670986
-0.870249907208012 0.460300425676874
-1.04042300238794 0.508402260609187
0.940455310899877 -0.296631573013355
-0.975174111933174 -0.583263705047653
-0.192644843731432 -0.787029546523235
0.727838837698626 -0.828585333508708
-0.880081893363573 0.508170596290783
0.488897465309188 0.880655574756202
-0.691298606946936 -0.654345909098019
0.788890742125678 0.467404359995732
0.179941839413946 -0.87245682766505
0.397833045408985 0.849523611859636
0.58242442058002 -0.761336521625552
-0.852770680612626 -0.622331026509262
0.952727689272465 -0.0638068088794832
0.764627557060121 -0.29237841557757
0.162483684085613 -0.944256023585221
-0.703231051575994 0.775119215974197
-0.984896278337943 0.00536150375698507
-0.520070891603852 -0.798687853329571
0.590893235559321 0.673054545327022
-0.461633341197719 -0.891620472361851
0.076324191329053 -0.946885830752374
0.198628214609405 1.06117383878055
-0.51327498606544 -0.930059533454324
-1.01217998129065 0.101730138927929
0.0807129533590415 0.957807117895857
0.221375073363471 -0.914919725176575
-1.15423568761276 -0.00325195985659529
0.539959530261738 -0.744604075937086
0.815544278727357 0.702893825785278
1.04210152108702 0.269432841512772
-0.903477904604103 -0.66876550853708
0.976239706556259 -0.176403030309191
-0.940264677914762 -0.09415890510639
1.08602864767363 -0.186516398886117
-0.662374372224868 -0.81236874281325
-1.01734751858211 0.564549233622192
0.995092709687233 0.0180817442437673
-0.653626789973564 -0.553933363425971
1.18348086464922 -0.393202896364965
-0.326473621258759 1.02871013503594
-0.898400403993282 -0.523271934454612
-0.660747752569099 -0.617170318884027
-0.965822700411445 -0.288729359269076
0.150097377770523 1.02262578322574
-0.629027878636068 -0.923249130580839
0.414394677383013 -0.845941237475389
1.06227362094736 -0.219116674081508
0.427376231170461 -0.925870351125824
-0.863549695958705 0.546238817917172
-1.09083060617154 0.340112367736337
0.812675163719252 -0.317154110771518
1.0119142584911 -0.427691991737529
-0.0347851775966913 0.941165385356029
-0.16714100689022 1.11659992975874
-0.971703180265308 -0.357945606581798
0.933099603737124 -0.289979290333475
0.77663540428524 -0.703894715215771
0.71109583071297 -0.206850798887966
-0.604197615587674 0.842300280991124
-0.799921134270229 0.544700974809458
0.932793767318017 0.0132886045504072
-0.287323311874008 0.996546713596328
0.0191393793699811 1.00185316138603
0.418418336729681 0.924113958295017
-0.807565720022336 0.262455124651104
0.151340191543261 -0.925079657907792
0.811266177779812 -0.610067259394943
-0.651428148666758 -0.815002284156299
-0.793587904107087 -0.760646983985484
1.07891670930772 0.625357884988229
0.247714167292888 -1.0159689338163
-0.651415688815311 -0.896850589301326
-0.0323781445711271 1.03997596253702
0.0960820419278128 0.886091812344616
-0.754536620821515 0.757417447088315
0.555403010502499 -0.701405912548063
-1.08149286733368 -0.387106844519033
-0.654925480912813 0.694306378044047
-0.973115832020055 0.331822757883745
1.08757034475191 -0.500285194746428
0.897406402365036 -0.457616227372687
-0.980560680687618 0.163083752133998
0.569344239137831 -0.760333312727596
-1.02380611748639 0.426451683603944
0.504338785590637 0.905830072742643
-0.923945378729508 0.410823286660102
-0.490439667604273 0.844852038067245
-0.698889522230259 -0.618661874793055
0.728674088407386 0.625956762658624
-0.53801451797395 0.913346322817237
0.662338692966388 0.799484663818079
-0.896219624462024 0.391183953591873
0.236665120084207 -0.964710602261835
0.910283182668462 0.467858955179194
-0.369892556988086 1.00064793253338
0.3999602688137 0.958989480535162
-0.646826270821841 -0.616414931064762
0.702841843490127 0.950793197772608
-0.631109893275333 -0.853956261804783
-0.605412560655069 0.767073554277395
-0.660761356534128 -0.772024722278264
-0.295423116340081 0.787642644530959
0.813720616585016 -0.424926541733067
0.416181677073707 0.876308844653505
-0.297443034233777 0.974950816996751
-0.787464184935653 -0.5680654628494
0.937453857924967 0.640134471013603
0.40683517619611 0.799159563181371
-0.362508503184984 -1.05240129320719
0.633031843514852 0.632763600046559
-0.246249391380698 -1.04061788546239
-1.00193720998866 0.523537007923911
-0.910812798250651 -0.707450520958739
0.965551761899082 0.320662272411852
0.345982358015211 -1.07705088500653
-0.179412813896521 0.880891672360322
0.904180009843429 0.308255476797331
-0.298578969516754 0.964533406728461
-0.808322242333013 0.541517548227787
0.785552296658877 0.663735510409868
-0.919472990408303 -0.124005184934011
-0.713736683621185 0.664354682471816
0.503712390728922 0.790309742836592
1.05627584462126 -0.525315086181646
-0.742814672406195 0.178531145994378
-0.95206634967526 0.42515331862306
-0.731132456045339 0.372524421691187
-1.08744768788598 -0.110338851262776
0.635727646869094 -0.721249826616011
-1.02290986491552 0.152375384596599
0.964235345400751 0.575921831404107
0.965041641253918 0.249799019662894
-0.77926182107145 -0.538085030818358
-0.977798654075495 -0.0346908380539657
0.90536877447942 0.501379461379716
-0.707415888627153 0.639219160626687
-0.932635719474217 0.0107761578434806
0.616807700994384 -0.686046161214836
-0.69886898035821 0.521978885614544
-0.0588340116628638 -0.940908210883539
0.452096174082145 0.788263948191788
-1.05864090505525 0.292013894357238
0.808773634438458 0.536344812823029
-0.794614227004159 0.573295803443814
0.601395430409247 1.10182482514086
0.963425133487199 -0.0201938167933804
0.870705449843146 0.413628792430271
0.446295409055536 -1.03958577387876
0.972486962675401 -0.293923176585197
-0.715925364838558 0.563976360373316
0.211353095083338 0.836748983181586
-0.928738896469022 0.0724145767137153
-0.259053384481549 -0.798843146093347
-1.25586141603136 -0.303231499054859
-0.297503954389931 -0.790165072637462
0.0665759430338472 -1.08000794755258
-1.07059467860006 0.126880054735553
1.04955025411805 0.208663875369687
0.788470373343687 -0.524111166698847
0.450201509789288 -0.942232655129797
0.575410516940963 -0.816279394462692
1.00037732670464 -0.361030035250613
1.16782829957059 -0.109504725636193
-0.113478779458992 -0.914243115881143
-0.893281900592794 -0.516875090176082
-0.889835898330672 -0.315258484027986
-0.181661782406907 -0.839627275652322
-0.812689636475289 -0.693251892549371
-0.530251014305218 0.689441463972701
-0.794383094240015 0.139551945665506
};
\addlegendentry{Class 1}

\addplot [draw=color1, fill=color1, mark=*, only marks, mark size=0.3pt]
table{%
x  y
0.305940140569186 -0.467070953466366
0.13943909323927 -0.256628778947483
0.395180858049771 0.4123993898707
-0.472316848504355 -0.178792685501936
-0.412863863645507 0.0585149407547935
0.40310920035673 0.20625047900673
0.366928621997493 -0.351906760552371
0.127629689075703 -0.502878143119472
-0.0385000395086958 0.614160221534733
-0.428572769710567 0.254115342844579
-0.6644328402715 0.127202604493278
0.444920980503343 -0.26083295515121
-0.426825087824542 -0.291784096387622
-0.17359268238804 -0.550429764955415
-0.170197635952744 -0.425960750633502
0.209006347546543 0.478419270339809
-0.299009010410765 -0.510448222147144
0.24248198616134 0.444452743421531
0.281325485636556 -0.394807296496852
-0.442559073848939 -0.210059594369481
-0.451076485225953 0.0675736277848222
0.374225758945178 -0.0511316717153092
-0.323935327371667 0.435405207291669
0.0720507137718717 0.481052547704961
0.399165139385949 0.0200747985506246
-0.587939443457528 -0.0255277694149425
-0.545151732105203 0.10493930713658
0.667871594172998 0.226729609572645
-0.506829247710366 0.338556646787467
-0.226756817753164 -0.600592663324932
-0.350888951925303 -0.350876128335845
-0.0960358386434232 -0.501835864387161
-0.582779924645173 0.0131321911220882
-0.550744454502939 0.173299526180447
-0.53429274017498 0.0365068287562882
0.199668559223126 -0.32509116739106
-0.393645786566079 0.401846836389087
0.587704949252309 -0.0190856901862803
0.628921135836821 -0.030429576816084
0.185340458800411 0.571774643380267
-0.530657633927251 0.116379191031321
0.204440811551091 -0.278424114654369
0.331121505672529 0.288148087833219
0.336517364670715 0.348674262042645
-0.516538276723171 0.137123226255227
-0.461850131496365 -0.241098158286932
-0.376724940079804 -0.445124038228678
0.30937489024746 0.428024733396536
0.204792653235302 0.466047166328916
-0.630723777185899 -0.193620237478034
-0.570137107390574 0.233619110351201
0.180686430311124 -0.27199618947541
0.027213404707545 0.577466389254232
0.0840166428148452 -0.570724188557267
0.479461382598116 -0.306853767845401
-0.202067902619277 -0.312020309183771
-0.53360597668186 -0.114808650582269
0.319873227766457 -0.346165917537862
0.317109485504092 0.323325047614838
0.273188085271967 0.636164561244021
-0.464990112845635 -0.0666236663097801
-0.344919076403161 0.326417027531336
0.28263591095662 0.294324079933827
0.425734772705508 -0.539869092667379
0.363996782586346 0.237751408063717
-0.0401804326438418 -0.406433332684268
-0.298670643435694 0.284262639393217
0.500262113625359 0.0520579140014606
0.147755367737753 0.500443109065284
0.529552652798951 0.163051862904001
0.532060583827006 -0.439172100164684
-0.0596432844178217 0.729737938477468
-0.32846562256903 0.232137146863559
0.301347125927066 -0.162510736565263
0.45868082492624 0.00562041192955148
0.537529788488952 -0.0862958544609295
0.0721548736148898 0.331632960606436
0.550052666514943 0.113104687654734
0.616084311974678 0.274864423543905
-0.428791831437434 -0.251385102015259
0.320837099422068 0.32386815765607
0.413525939847625 -0.0848141156622071
0.245714467502399 -0.549266139709362
0.476727358151994 -0.0405826695921659
0.279341383405228 -0.427547405536023
-0.0696465945165025 0.59430888297905
0.607367564175189 -0.209148256001754
0.158790630462211 0.400892127826856
0.0880649876938711 -0.53174951912223
-0.463122990723869 -0.19181195450211
0.387017411708197 0.172465032386206
-0.336206330662206 -0.41548497099218
-0.218340289166631 -0.515359590603488
0.412168427151877 -0.00347199666131376
-0.00038463413933057 0.452162256429112
-0.247402177173519 -0.416727481727367
-0.501050091365218 0.0490112297652694
-0.461502069895457 -0.271218129914797
-0.543813267162086 0.143187409558797
-0.446552264210133 -0.205612865782741
-0.51491686563185 0.139131117655761
0.458238051101839 0.158161473967024
-0.269979525650662 0.0732792023393315
-0.429460731465465 -0.0542869736633871
-0.14644191845616 -0.218614803474252
-0.102012804559145 -0.568240624554873
-0.0871783403025511 -0.313928420426591
0.50205455294657 0.055757862706094
-0.0909891607756491 -0.46761758903395
0.395299699126056 -0.189386369537365
-0.432344279513567 -0.363284474410898
0.558910851649334 -0.151087440029717
0.0111923285145412 0.562104894687955
-0.532068984426632 -0.0909589795499552
-0.483414255751695 0.0786440251590557
0.315507005953863 0.400709088862538
0.186239068975158 0.383273228679176
0.239793934936708 -0.365725792315874
-0.499550453700586 -0.233645359380488
0.0729349093091742 -0.470374093440691
-0.476444910176208 0.18211486596473
-0.421765395902997 -0.448280889050856
0.6415780927927 -0.0221779104634466
-0.432565754440955 0.0899878222648172
0.0746456303759284 -0.436393287089935
-0.385739209331424 -0.269160015217079
-0.589869173808885 0.00799049572476541
0.590975045514699 -0.191445208664309
0.424145838490275 -0.125497217853758
0.191710502905255 -0.597537791422425
-0.170964558842068 0.357904715209122
0.326979030276117 0.581120957071205
-0.0519595044362832 0.488371282301899
-0.532648385481921 -0.255614587673866
0.507040073698881 0.12376301913782
-0.662429593939691 -0.0395958360866128
0.43120091603572 0.260291405386033
-0.650661571721738 0.373720763399401
-0.170952897878231 -0.437039940592555
-0.579891486937101 -0.0562448931326116
0.0865870394766725 -0.568344262285852
-0.490600325684166 0.061438066855911
0.0979196553512774 0.478119285823503
-0.701762614515431 0.297610880773472
-0.561871957822165 -0.169668518137445
0.379713984369265 -0.0101305905402454
0.514775135618838 -0.0548372695289594
-0.167708411169864 0.452432214360813
0.456467349387249 0.178054996481741
-0.0731189496624319 -0.498260535808697
0.394986015634638 0.252494394554896
0.452714559244442 -0.23104126612605
0.346034141461468 -0.250017635304144
0.248747319698955 -0.315272181726992
-0.486839220071594 -0.0292799876468016
0.440309391452006 -0.317632661467967
-0.424732789470602 0.58847004586086
-0.462160498771156 -0.338908393815333
-0.116121453757618 -0.352205842575223
0.487582114775269 0.231410392256269
-0.231667377501812 -0.40875721962099
0.628010124941346 0.113461840661119
-0.488130515203948 0.124400193340256
0.333441531781203 -0.478954138416275
-0.184760781729731 -0.371653773514089
-0.0438438396270178 -0.506350286297718
0.593688259986204 0.363958550133601
-0.398912119663283 -0.209561486105863
0.293585708764459 0.256041305038207
-0.353961694064649 -0.381961370315928
0.539991623790846 0.0506098427888744
0.168441139897555 0.479089359948774
-0.498333754992305 0.406815998366752
0.252033805565175 -0.530075420252536
0.399101863840903 -0.187778780527115
0.346183034864691 -0.327168631604131
-0.477298517270791 -0.283924972185416
0.251612569782647 0.378212604478736
-0.525435329901247 -0.284415463634605
0.041023292292747 0.494407129902506
0.157924418675846 0.174450219999599
-0.21408149099251 -0.414243012432748
-0.290706546289306 -0.461570750791147
-0.334394969154026 -0.504097323499618
-0.12017624578946 0.533028795266845
-0.250584194414902 -0.394293938951633
-0.294295650561858 0.40421114408671
-0.399876953693294 -0.118218640544951
0.3294505190834 -0.134445282984833
0.508029817519975 -0.0244479286492386
0.14673681448289 -0.485595843212568
0.644428754785152 0.142841586469801
-0.230603931348728 0.411194264117026
-0.209398791814223 -0.365405016581068
-0.419659258883773 -0.248429841159123
-0.425584292277455 0.381855621790218
-0.286526293999168 -0.396273890374913
0.312288547739133 -0.500093847574872
0.00185778309970347 0.415698089370305
-0.403169841397363 -0.453166967294661
-0.563825155656097 0.111963438477145
0.625884639026231 -0.297190574616677
0.161827966775477 -0.402006706037292
-0.340202879606446 0.30561176195296
0.541432764106314 0.214167632563532
-0.534350002352275 0.274966550610079
-0.18337594643331 0.421239454452681
-0.552824983817549 0.079560536948121
0.015477764792793 0.568985978810447
-0.411341775854922 0.315201844640088
-0.142383407662935 -0.184620725861655
-0.33193685564523 -0.427458561237343
-0.453840595601063 -0.275250316349306
-0.262509319476781 -0.26997953602153
-0.45883240323985 -0.391135744409696
-0.394683514362096 -0.0514725342182272
-0.509160635183177 -0.174870758261129
0.476847066356172 -0.0322597003512918
-0.23339591157611 0.3976053568621
0.278932494596871 -0.455913639388792
0.377801809508967 0.0745645219184055
-0.483255218002603 -0.274419646180127
-0.370691860536276 0.499806557191485
0.100757375066724 -0.389976807372348
0.122896331383957 -0.421741833614533
0.354726608885159 -0.556572502118727
0.551697168979462 0.334797030536944
0.448276009649482 -0.520041594179782
-0.0796063384170379 0.557935391077201
-0.112922862112579 0.540806396272344
-0.0952441208122311 -0.591816182834784
0.349557700152368 0.260778271109694
-0.331438595733925 -0.314881631099384
0.135064506279728 -0.510912142178652
0.386504006913542 0.413634610897338
-0.435163190210565 -0.139407824987348
-0.430533699922473 0.387957345539271
0.314401355038649 -0.449748702690405
0.350282890695632 0.32401866694945
-0.431729692845488 -0.371048238726065
0.379026628215734 0.214461052936507
0.462005273957457 0.268165869017052
-0.0142315732438316 0.49284944092289
-0.24041021338344 -0.384820955386864
-0.16275578593557 0.612444444573663
0.158345908535195 -0.609689400364066
-0.296823283135435 -0.348426262543025
0.397148286305401 0.1553272615151
-0.446892347469733 0.0141710424577544
0.10158970515779 0.475040266989679
-0.400435726903791 -0.133833432773199
-0.307786007632347 0.38399312314919
0.31387457124942 -0.446795414495553
-0.312927789767448 -0.311940409432561
0.0783147667108533 -0.549297741897075
-0.134798185852686 0.560024843341931
0.118070536798949 0.46694134740006
-0.289233384097817 0.493868991695944
-0.0874477083538038 0.620509714153054
0.0076978300773437 0.472320902059179
-0.0345749876771999 0.622702918728197
0.472676032875017 0.213617215468481
0.493330663528283 -0.0968727270817067
0.0880510659249164 -0.436999943581115
0.0728650256119761 0.545040643641817
-0.165102986115818 -0.560325598799322
-0.333626359244875 -0.20494580314407
-0.467817594496799 0.180641903722452
-0.388830620503939 0.0448920394011274
0.0301942412447017 -0.608268167119412
0.0294288272854302 0.30061584727778
0.529173292102714 -0.286118625355274
-0.125769609975546 -0.390134824318422
-0.376019204703876 -0.596024965086987
-0.34611174313273 0.197040940194047
0.0115111946568925 -0.420755700952581
0.302894746673691 -0.296853196696377
0.353160100371728 0.31578285762844
-0.385858244033721 -0.591654409183267
-0.191133233129523 -0.447211165543246
-0.120380065466597 -0.379261334179312
0.166585388011927 -0.491871587468717
-0.412782324480259 -0.13619684300988
0.363465114885212 -0.162672781537204
-0.521276051818196 0.245740994613473
0.525075980886175 0.136163677176272
0.300994952224748 0.253583452644087
0.571313781619195 -0.0487681089670129
0.480838602466533 0.01559016111173
-0.449045319416191 0.0404782386804834
0.525970728412633 0.237207253306633
0.456114882962618 -0.195693016798565
0.0540598258991689 -0.598319781655758
0.424907285792269 -0.058219043431192
-0.135926519743172 0.502635389040862
-0.198006873949941 -0.555982385955903
0.575909032938556 -0.041920366157955
0.11066673511883 -0.464207898870366
0.0445375909243031 -0.604614026558908
0.314883306570445 0.499593385640985
-0.201976946639781 -0.476222858541089
0.640447561957631 0.194130691059976
0.0039058232630494 0.249967770559023
0.406688327187075 0.330098713774943
-0.0790821204932295 -0.508140500125608
0.354160722783681 -0.229469536078155
-0.128350466450825 0.595600125302978
0.297174579900584 -0.594896546041174
0.32729011766037 0.342610587844111
-0.251854079738843 -0.271132592295145
-0.379836126624807 0.0811791947007216
0.351281419773843 0.100631677115266
-0.467610102345911 0.0403901279530716
-0.336628667002143 0.469004538123463
0.012167895775298 0.636813310638155
0.394221595451866 0.30420319731785
0.467241004508812 0.0535926569247589
-0.0736927033694288 -0.404355822690626
-0.215971140211174 0.394162879294018
-0.512807638868641 -0.0139886403338656
0.528950311943746 -0.273965621365475
-0.140100492361748 -0.577423509033863
-0.25290467426792 0.325902251557042
0.0375930260392158 0.447206374664232
-0.370894287334411 0.240786300005665
0.0138214146406718 -0.240302673706704
-0.00638006384485075 0.470753208635921
-0.280555775316888 -0.201451719128393
0.438596731077253 -0.091460288429295
-0.54467389879026 0.0840511548814344
0.327769524189714 -0.166074966115917
0.0709682862863152 0.396114319806294
0.458790954815194 -0.220761148860863
0.293862451701328 0.497596115840605
-0.491769504907367 0.0552555773127343
-0.477416007264116 0.0384538641081463
0.425069962299567 0.0174125941251855
0.387358774117216 -0.476036080436196
-0.531026744183903 -0.0596809420468456
0.158585046296625 -0.173408510785925
0.502650488891305 0.102301799454863
0.49658713317568 -0.272874313415715
0.319879372079447 0.254734700860305
-0.324413133101939 -0.219674375844935
-0.252719389088103 -0.449513132603971
0.250402221095785 0.644214790258314
-0.0988782422994305 -0.446566949718036
-0.360626527112025 -0.170984134898624
-0.555981645578322 0.152225626675151
0.0899895665437095 -0.26164616135432
-0.312333735166147 0.439009788012033
0.0372190928361407 -0.6369938128232
0.347447938440794 -0.344936638775891
0.390828453454038 0.195927371093888
-0.501820842731219 -0.236623655466704
-0.231223507341957 0.540279154894423
-0.107982265692637 0.464695348141792
0.452156760699482 0.328933898677996
-0.332302340318595 -0.766493169600571
-0.245920676436948 -0.240550792002092
0.401036977277653 -0.0397232519760422
0.155250509082073 -0.490801257766643
0.536577103363604 0.308268071172905
0.454971588173303 0.310292873999294
-0.160899425306027 -0.0273307788478989
0.36418998678329 0.0351082232008704
-0.408407437919843 0.205773130598948
-0.465866948435309 -0.282451863656959
0.303051888349076 0.455030984196731
0.289129179781126 -0.462447503465474
0.40678813042704 -0.031861636540101
-0.351904826663814 0.363251797008755
-0.328376673516365 -0.210906793646834
0.407228339870711 0.393074104774897
-0.243333024481033 0.593356909625529
0.350670433604992 -0.400188471921513
-0.269455981425575 -0.473047974563641
0.563268653553421 -0.343647316659311
-0.250365190350349 -0.419816487990175
0.197830648333287 0.354576777717107
0.400795836297218 -0.360734264766261
-0.375711297073565 0.0339348289148836
0.546225558211828 -0.112631658391475
0.201473322068901 0.476704057655095
0.48479922155128 -0.163052249292057
-0.515846049748812 -0.321902518055664
-0.474940747245003 -0.125308549416865
-0.297529108567212 -0.382585939823495
-0.145892255935 0.614518495225573
0.516844273255756 0.569644584364603
0.548157547699256 -0.272758230299313
-0.141565213619117 -0.381268570636218
-0.457517878903665 -0.0522295756731223
0.287960593117807 0.493525530545036
0.14963051954688 0.458513642212164
0.11815022772577 0.421396829474559
0.121753603125218 0.588126564536715
-0.457705389570745 -0.047057615489791
0.0911302182383127 0.364594941747524
-0.395518703359478 0.346821162331128
-0.185865005148713 0.338541207223679
0.473062260234375 0.104124830048662
-0.124618049556635 -0.46731737451156
-0.53566819940529 -0.121138029173544
-0.221419694943593 -0.166582432286656
-0.171625505982092 0.419922756090012
0.266411660891019 -0.0691861294732323
0.340658426020337 -0.377189438298131
0.1642251243539 -0.407199569295346
-0.587492545310712 0.167948908008864
-0.482287059007346 -0.193391574192951
0.512109271624828 0.183769709614487
0.240790104944342 0.572434680737868
-0.411269149634008 0.0560653905676437
-0.396087502387064 0.286117845354937
-0.2968339024744 -0.220288615946995
0.323513876420506 0.120116329817587
-0.342326677292701 -0.289932466484196
-0.00742198876889702 0.474630403843223
-0.586974983433159 0.173238225302148
-0.456466209321548 0.264784620217086
-0.116082965635472 0.495590027541705
0.536324080793185 -0.185965085964158
0.670602151475009 -0.0144844529731208
-0.255141098280054 -0.291329217994177
-0.318487618423468 0.24291116873292
-0.32129411389721 0.109217602665694
0.10300954203019 0.505281842104984
-0.197770685681096 0.671352209471705
0.46076138602338 0.531991849553423
0.192446449451671 0.463907966352702
-0.374834253460101 -0.125301399453769
0.321757931422136 0.385009907776307
0.147039787355168 -0.360029412897111
-0.307667344630003 0.510164005162867
-0.370419754204765 -0.353924395486871
0.268674437671534 0.491776382732096
-0.171994130726522 -0.534716457396787
-0.426154110821308 0.00708778269972399
-0.186964923518157 -0.293100080472335
0.21701798111164 -0.440016267501784
-0.646584637558207 -0.258536595939509
-0.292918047252631 -0.377768866923322
0.397129326971904 -0.13524885645558
-0.138311070399799 0.452457475449745
-0.325013175940896 0.215485095315095
-0.112988728362052 0.511561932941601
0.409138623260765 -0.0670108356421217
-0.139378334477814 -0.530324867553162
-0.383854608374463 -0.567041506075198
-0.32800295887796 -0.205577397936353
0.09874828808786 -0.534682535176918
-0.505571853926676 0.28025477403162
0.341825679941037 0.551564867956861
0.291023208125129 0.421371370874261
-0.517296046492922 0.0928060818519559
0.0289838482559512 0.278258949058545
0.328668666580775 0.464215092000956
0.275680811797836 0.264840216713564
-0.110444916569103 -0.478647292716119
0.407177110528308 0.038456912585276
-0.491954494784254 0.214666558662963
0.145101393619739 -0.552938925332132
0.158214590573577 -0.398436074286532
0.374374210251743 -0.267418755459703
-0.473581228555077 -0.301121602781674
-0.507017102722307 0.420061427473336
-0.217648512526336 0.336420667819175
-0.331968385234169 0.343521632883545
0.124867181840115 0.525748576146647
0.228892542057783 -0.449069503045323
-0.46888420525201 0.451153338277249
-0.580142376986349 0.0676973088567402
-0.377710918943416 -0.468456091826295
0.363431367351153 -0.480582867252533
-0.261611026025236 0.378648485476459
-0.331534943788002 -0.266462508989071
0.443326139519037 -0.291771769902135
-0.341922776503924 -0.393954968021048
-0.315131058305083 -0.443287315263216
-0.358033097898117 -0.0412739736055213
0.0876164433140768 -0.711600850348139
0.360970045535536 0.532621325228086
0.423602426266249 -0.225906235501503
-0.575684598749412 -0.465888749706272
-0.0685967875814149 0.432601684917339
-0.412483803736961 -0.266984183657062
-0.235954954784847 -0.500752054869323
0.497690938193025 0.0225269165739045
0.331414171637065 0.174310499942144
0.517129968005594 0.0654771716320457
0.275552733760246 0.328617785931783
-0.38994120631704 -0.443947205420403
-0.477276964567039 0.150484997932369
0.276708811126966 -0.349446460654513
-0.59486127587678 0.0649945481359572
0.359828016145367 -0.14863957171749
-0.289838556838619 -0.386948477873313
0.127419725084056 0.379571903032166
0.0365549966103914 0.330094887685319
-0.263629355749472 -0.33557770622691
0.385018649187647 0.050792557892927
-0.417050744502259 -0.180435577146354
-0.0370720376745002 -0.465290544804278
-0.137500173462756 -0.43173187903975
0.137978622334624 -0.379904247183909
-0.422635247912709 0.107432674081099
0.255128068607075 0.198729630688141
-0.199756902274685 -0.312211653072038
-0.0258676816965129 -0.484260607697542
0.296063189269229 -0.31574235514623
-0.121848412716095 -0.372116196242648
0.461432062091762 0.00104154990312481
-0.420193629008865 -0.419413765179781
0.539355243942542 -0.180588021895208
-0.0283189123678547 0.476239014596218
-0.333904459571554 -0.324994510938015
0.184017018904314 0.411768389633261
-0.335942832620863 -0.183100204946335
-0.400744364595967 -0.324578804261678
0.137780276400436 -0.576620369546087
-0.250444563632962 0.293138003842905
0.230180916590427 0.279590026080105
-0.0926816380677252 -0.534501950798827
-0.20673161457719 -0.524101486378032
0.679447610766911 -0.186686215005223
-0.142513431341546 -0.473353732040737
0.401978610092596 0.0374070900375606
-0.227615866797923 0.498123128831964
-0.585146306825947 -0.144648331972161
-0.301546857025825 -0.414518920919769
0.0212538949251636 -0.538920492806659
-0.270948119101524 0.442447513215488
0.506777292336602 -0.124584507978428
0.717451069424504 0.0244508648110466
-0.387162684927497 0.370207977339625
0.401161819696362 0.150884165257145
-0.10324911441772 0.4517602730771
-0.328625887269124 -0.604332147694973
-0.0975458725930557 0.541633275491105
0.0116018435180946 -0.564615709205463
-0.380740123570831 0.306639535216545
-0.00237197171195988 -0.595434962814401
-0.460444200946856 0.304166908498229
0.121565430500701 0.596011427348485
-0.579561547295023 -0.223901224166566
0.386952679681752 0.292758346814814
-0.523313153290466 0.0644943975593382
-0.271061556651345 -0.398139987533319
-0.69051923664359 0.1297442403481
0.449921186955947 -0.236060294629431
0.374139258590012 -0.399338713333467
0.351949876407517 -0.170510673694428
-0.207462314085104 -0.483752356738282
-0.2544391587885 -0.30786520203064
0.0502634646574416 -0.468748967759538
-0.384378695780432 0.329699224525064
0.00175265969727669 0.414646169772033
0.0968597290201709 0.532297631984493
-0.26577871295033 0.303959841752729
-0.487656117594901 0.154219438048293
0.445263378213572 0.475855494800548
-0.295798388286703 -0.0656620366540663
0.393307136628391 -0.0696004057078285
-0.436920360039443 -0.269156994981858
0.254688250503757 -0.556871564652549
-0.218445278009711 0.300957008357135
-0.172842739847211 0.404673502567796
-0.260188336964319 0.523892828966047
0.411501600624181 -0.387649654788731
-0.0942034663340031 0.462620406908132
-0.704485301234386 -0.228758899992657
-0.241597710611657 -0.613054913404881
-0.0162420851033796 -0.41750886522121
-0.471792682814879 -0.239523649847147
0.273174551090801 -0.484856385583698
-0.426649670816616 0.418619861807039
0.418339966472442 0.000344521582869836
-0.238900178998048 0.280867102148481
-0.0978053456854408 -0.56972100912546
0.25233388392462 -0.649633822020018
-0.542920502698672 -0.371251364177953
0.425992522278492 -0.117296181556116
0.419468476424054 -0.294824201229654
0.139276283065399 0.420614103613614
0.433923689757392 0.161210727234873
-0.309827253591544 0.461077978523485
0.595000302494982 0.0682606775380603
0.408665741049728 0.332020295630631
0.0820079295661469 -0.576087542983488
0.170233373945843 0.416616308098942
-0.21647746286146 0.412649822356312
-0.488522177385438 0.245201511095648
-0.198296001363916 0.486039246432266
0.0538016055526481 0.580021304356044
0.500619685698247 -0.0599202234193023
-0.334698627387971 -0.32397260522954
-0.39107667366322 0.32133901299862
-0.42349270622995 0.236022517188411
-0.011632975228485 -0.476312407949107
-0.46201312189821 -0.0817679708041172
0.457244236225099 -0.27017206882881
-0.512569938080178 0.109933571256708
0.427418313769864 0.366185650423716
0.71883796598079 0.124976403760582
-0.074077456553602 0.412833103956344
-0.211528337447821 0.617770690538271
0.319345036461619 0.378284971841941
-0.49041313218839 0.280461951868046
-0.326305728071924 -0.359075944714185
0.172861046500921 -0.379571089339891
0.132591479116465 -0.422483232196568
0.352982182855707 -0.345710857421754
-0.140510521109965 -0.512712663937736
-0.399636040783984 0.415072377991876
-0.325027923414104 -0.574671702490409
-0.508517263180241 -0.296962205222706
0.475825533032863 -0.0316636077421396
0.560318347941745 0.0926456872163793
-0.195987909472485 -0.422956055391246
-0.0520028769867885 -0.484395460596128
-0.613849345647998 0.139739278468169
-0.524026415608118 0.237031882107072
0.497531565650392 0.415973090027506
-0.476714828929693 -0.323577845884463
0.0812875473246569 -0.269624954088902
-0.361395575191493 -0.534389091257461
-0.4620238635127 0.28360372869886
0.220103168068015 -0.512492373841255
-0.0961330524669004 0.562977507361651
0.0413338786970621 0.463846507427504
-0.644492833374879 0.298766201953137
0.260830877355737 -0.567774558276112
-0.0798608452896962 0.571029212746134
-0.490541861082472 -0.031835607063116
0.529070504319614 -0.261765108953936
0.346646572677015 0.104929074214014
-0.24887714219893 0.434357955249882
-0.479599898862155 0.354120227624788
-0.539528578276827 0.136172249063647
0.223749822149047 -0.549242831605436
0.523656649869619 -0.0733806973690145
-0.203873071095639 0.407870822868538
-0.554752569854653 -0.108624976638138
0.440091315708111 0.38016426280761
-0.38870588120562 0.106112640781248
-0.247171429181811 -0.306848394847709
-0.390022904572335 -0.0943484482405726
0.419800422463555 0.194663530070205
0.458743567471604 0.0360248649888995
-0.462605608534101 0.062646206204503
-0.206221693992355 0.519000535516707
0.185206059749939 -0.288105948146857
0.0828927451226732 0.494200997108377
0.269852501083998 -0.362183123423141
0.527689098363356 -0.282059401368507
-0.478358719533522 0.192628796949083
0.123014796440528 -0.470041846927823
0.402556266124218 -0.312405718643164
-0.586722966672646 0.0284584564303555
0.244258984520173 0.551229220655376
-0.342719082456977 -0.495638066615149
0.460064358170597 -0.13187570202144
-0.642741069979717 -0.00969004417316754
0.230535168938351 -0.454466574954979
0.287854323612106 -0.554313167601634
-0.126775323255283 -0.5182149666524
-0.210684434386727 0.405493978864641
-0.302864449881066 0.287676222038999
-0.259916540668548 0.266642442752305
0.107726711881831 -0.428714576854844
0.280409935876978 0.525538806943923
0.510621640315556 -0.103727635634003
0.361885346873468 -0.389882046728944
0.5399892049744 0.260317839139564
0.446903879834688 0.423264498321009
-0.287594487515899 -0.600066563864592
-0.684891355713162 -0.290175929005438
0.152495287091777 -0.541832621394992
-0.442096887832904 -0.13765616710521
-0.111019107230762 -0.416165742800287
-0.0390501348799017 0.571286153492423
0.443815184997726 0.293776075258416
-0.28034149834456 0.306606393402998
0.517358431900407 -0.149972157610002
-0.476136892713476 0.102853116157482
0.051231723894206 -0.717403831243422
0.112410297803748 -0.425167672118625
-0.0230926700665245 0.4230360026528
-0.458983123565884 -0.0870787785199617
-0.233667579363843 -0.357310585034498
0.476070307432516 -0.0121504860931066
-0.544719819562809 0.282115157755216
-0.406627530591773 0.17732163053222
-0.158785336531328 -0.319805549483004
-0.17117389770901 -0.394822395474289
-0.470671390702312 0.206188374600075
-0.53080951198053 0.179060196955275
0.207494067489592 -0.246086935417704
-0.014312908080317 -0.402053655580435
0.541119622056944 0.255326414339101
0.140813738600497 0.768981956496029
0.594874780898036 -0.0982435799971521
-0.44979428851974 0.307516968590169
-0.48675145932283 0.219346275283337
0.354165572378637 0.200705044536447
0.563385626600088 -0.155645342383278
0.485939735610623 -0.286930121003992
-0.0565736727613183 0.464811792503936
-0.278519561415108 -0.481888948052563
-0.357325457094208 -0.46943559529529
0.0853343843766123 0.499585331388963
-0.300030457086612 0.295437351377888
-0.481268655018368 -0.317454194778585
0.207071334304752 0.438418646996773
0.312323547379933 -0.537643286301525
-0.265764526842989 -0.276035224590356
-0.466059105177515 -0.345776313791415
0.231445315705001 -0.489497407759101
-0.524149095192819 0.0266575322539969
0.509782931346521 0.293142122159825
-0.569122953988146 0.00271136404138984
-0.334475640001798 0.258499053230207
-0.306381856392535 -0.063268802288356
0.441967213951409 0.250892033623095
-0.0621077200812424 0.368221170049776
-0.0222893167166915 -0.536757265372262
-0.336525255069556 -0.520632087575952
0.27528057313087 0.305108539650105
-0.551489007807242 -0.193826807300288
0.223616625085983 0.670495783173712
0.280147019398697 -0.492562813434624
-0.345382618027349 -0.190820766890698
0.464599253352603 0.322270967568985
-0.524382164947411 -0.384192724478284
0.164231207703852 0.547343465234007
-0.419008575540174 0.36616829551064
-0.174123237708761 -0.378407907076008
-0.273231873949807 0.524271453242833
0.591802995418645 0.0678010049438485
0.179075804211908 -0.519533938693649
-0.350127018342188 -0.607647089642482
-0.0970357757337042 -0.475944717546248
-0.0146828855232073 0.693222550131248
0.507058504560784 0.0138308304137803
-0.193609023604912 0.546840904171865
-0.123615691237178 -0.406860286241236
0.023724685919407 -0.526056716318228
-0.0437105562096285 -0.44320504389064
0.12485939044531 -0.696605115197427
-0.365173272751227 -0.280896638690657
0.296431700901697 0.395028323473095
0.175704233071284 0.33321528240543
-0.380217912060128 0.12509190805785
0.404116269894995 -0.241494818800843
0.496387608988142 -0.171033230612984
-0.136052166374396 0.333406094542343
-0.402175968825192 -0.386541004464616
-0.198335121194731 0.352426476949304
-0.336351535593872 0.159975250663654
-0.486215573372855 0.0171729945851756
-0.487209249615397 0.246101321629904
0.134737124777038 0.470839404426002
-0.590548707372488 0.0615034701482996
0.289931849511157 0.37090092295839
0.552542778172924 0.104936909607628
0.0612417578890986 0.569171278209097
-0.420299216937981 -0.0426335052860972
-0.351947688458929 -0.520968945325042
0.51812693451209 -0.185462076321999
0.298216341711554 0.308449088886158
-0.0214175063067858 0.515547260330182
-0.40574433138583 -0.172141705395487
0.0706084115920496 -0.392549811870344
0.239274324172773 -0.435862078624291
0.50194187204942 -0.0860311085315437
0.0034453538735916 -0.60609006101983
-0.322427685126869 0.342052655806153
-0.380329212933918 0.114382761083743
0.402392006893996 -0.344409311740366
-0.308825109982711 -0.41609493594594
-0.175921484069756 -0.532343158304963
-0.489586922095321 -0.309557507084137
0.0385814982339427 -0.502183238866452
-0.405655663068316 -0.400908965366308
0.42916827071442 0.0849613847622416
0.39643795952415 0.0370665263029272
0.2261218021114 0.553052683822801
-0.573593238071454 -0.357327788695777
-0.272211529372512 -0.408753006412157
0.494253781387541 -0.203926420916758
-0.201766588372224 0.457359718560585
-0.13972793961701 0.501943237951436
0.0774550425806512 -0.359055417021544
0.551127345362191 -0.181044767908255
-0.554922349397882 -0.0565518353105405
0.365436175462957 0.0872815136409452
0.101996935800515 -0.424194814571099
0.576925187230782 -0.0747941169029737
-0.58316550637958 0.00990402527016196
0.537744640705889 0.148682191965242
0.0281024897861131 -0.462775633274617
0.467982521054584 0.343919802705248
0.344937627091607 -0.394494820309329
-0.503929418097981 -0.167260348408909
0.178065417206365 -0.649002329136517
-0.352368507680635 0.369338667755096
0.505670744947085 -0.28697619579181
-0.33333165282808 0.261980742849036
0.463770188588491 -0.0257101739394045
0.374447272548014 -0.405433463807218
0.0178382060260986 0.453661289446286
0.137168655311612 0.403793528234918
0.425859582221937 -0.379788162816376
0.348324088736407 -0.324719142913854
0.0222196862838698 -0.483482179402631
0.0680906940031901 0.58640141325194
-0.351556888102833 0.506292346163565
-0.462461247544787 0.126939962490604
0.3280467019345 0.360471911506129
-0.38887651693923 -0.258682598810724
-0.466938426714896 -0.0247607611982644
-0.000619393863356965 0.324726932898478
0.235242921946615 -0.256530578565395
-0.390810085352742 0.121251549843566
-0.425377901275616 0.206272533981029
0.318907449257181 0.348034891393833
-0.48199022998267 -0.421840801095631
0.520189980686586 0.00933337439773929
-0.654472697179734 -0.360436361889483
-0.217426979875831 0.126450192796907
-0.403128025976635 -0.0253604467783753
-0.523871071463311 0.0851886581063111
0.458550074296274 0.167716625193719
-0.54896810524544 0.13399438334252
-0.44494899783233 0.188306897265893
0.250106438122212 -0.430283860928012
-0.453065095377596 0.144201181958507
0.385206318595757 0.103084511325138
0.187528520039147 -0.606654045860549
0.399932141599938 -0.147863742762355
-0.328982053069479 0.223014699661175
0.559820984564403 0.247308475275176
0.695394648030111 0.118466232012984
-0.450881673504941 0.367194422727366
0.446592018504271 0.27143213503538
0.123919855220545 -0.268049484172504
0.177839422109281 -0.365124708086256
-0.159216509628343 0.415157841521291
0.587160380775973 -0.143543656772498
-0.434978109523665 -0.265430304538862
-0.0199957934001671 0.518477253383481
0.29292464620017 0.173922297314932
0.185027981083697 -0.435478017550518
-0.586581628517175 0.00364685658583369
-0.0908811089176889 -0.37064718761927
-0.125246162705079 0.485049712606814
0.245668855498133 0.271722428305138
-0.391915776650497 0.230838399188265
-0.109004604659603 0.334153486773582
-0.521742251351554 -0.126940079602484
-0.26575023233139 -0.317789920689431
-0.279329293198883 0.381219108544518
0.508736765437795 0.230694157948559
-0.310241409204836 -0.273659172419448
-0.0488656204589317 0.531776689354202
0.209643736368147 0.457346032767404
-0.148029258881277 -0.777580049848585
-0.335327789445578 0.339880348764239
0.434916538705938 -0.0897499437690213
0.473520165858718 -0.0733050911138046
-0.00156700954592912 0.477333068991775
0.312557430236186 -0.470665435324498
0.512909209417639 -0.0202815243898972
0.353269473262926 0.424481673175494
-0.596851885562466 -0.305826118676756
0.437708117078674 -0.0714555530321777
0.52334654589299 0.250693752737366
-0.213559348540659 -0.4425016568783
-0.000799256880658936 -0.62708844743782
0.367625896353119 -0.146740940520097
-0.388537454818137 0.353357834502427
-0.500672273672416 0.0556362718358378
0.344963224199235 0.302333252166379
0.0363873007773549 0.366454627976557
0.344459709661041 0.285569173882574
-0.398014707371202 0.0460935485588808
-0.387069270379294 0.0264086836668517
-0.211996060634315 0.501665425663775
-0.546228735173631 -0.117716508707091
0.567142604861956 -0.135504331546999
0.283086707773515 -0.197888718383684
-0.101471578475052 0.514938661253598
0.400053593797266 0.162620837865199
0.373711444914343 0.19916893315345
0.392452628796402 0.281545381236651
-0.477343260421074 0.109426974952083
0.332219073838853 0.220734232573182
0.426173775099048 0.424714447889428
0.482774438353935 -0.0918827114430104
0.185102630217221 -0.223230099506491
0.0197315885950581 0.439152669028132
-0.561990046674628 0.314352744661186
0.179429238289895 -0.366886952904499
-0.239953412672654 -0.457475158394714
-0.576701286903138 -0.0682313418975371
-0.273541985879885 0.162732274283683
-0.53165241839254 -0.0502146537236719
-0.545444651982921 0.193265591937627
0.20685656789444 0.380724239208057
-0.206776822935488 0.482707149325472
0.508310505364472 0.137958926847533
-0.359238244457529 0.0501558881471409
-0.529898364453472 0.0221472760040811
0.296657425458532 -0.482456177554341
-0.203836028265971 0.479282929678682
-0.770071177248067 0.298879381115792
-0.198035956636706 0.469974109096371
-0.2958454281538 -0.207407412091978
0.599396290780982 -0.0757205294032436
-0.0541114691710371 -0.579546437389712
-0.609823483398658 0.0480770635980505
-0.423145064193889 -0.204376956873531
-0.297928928885914 -0.291111354891323
-0.40174793215251 -0.321610083985332
-0.53260106403283 0.00370133830368555
-0.238564235240894 -0.306715719328134
0.354794748066036 -0.451706631226351
0.448412287177859 0.083628770693988
0.326597360493541 -0.310715177260339
0.456896053839283 0.38556395795536
0.394689178067687 -0.345807999550292
0.0539489881273197 0.40383195178308
0.0654062607664256 -0.544886959605629
-0.181482762058424 0.515140208371682
-0.471083624961594 -0.210793697255415
-0.340164944134964 -0.347028848498569
0.122991839625005 -0.493563667743471
0.256264614482198 0.371819561469453
-0.370972627216182 0.303756633832538
0.337892573663392 -0.72316934285426
0.58727730395885 0.270171628190122
0.496318194845454 -0.161475366487563
0.350670586545607 -0.435443350785703
0.471087534972824 0.0373807187988764
0.0900698439069439 0.333075050316347
0.244530463148365 0.301486120380866
0.248000863576076 0.490439160746
0.45056844778475 -0.375851573236822
-0.0809252535767279 0.646211773724352
0.503858348340927 -0.368657981070659
-0.0200481738760146 0.497907086564262
0.235732103259565 0.404987488826527
0.284674655276537 -0.317828210706793
0.54171013224029 -0.0299004628450421
0.476857547283873 0.180666205009448
0.175543707071481 0.337210077029212
0.65715033236294 0.0709694093671183
-0.163364576419087 -0.531781730426784
0.252428721078588 -0.483855173496759
0.0794286315904853 0.604981623067843
-0.543700206370459 -0.264752456493766
0.0616190354610894 -0.464112855569805
0.133985689127919 0.530228375077638
0.0932393143079036 -0.419323051365915
-0.336413228657638 -0.422740707291777
-0.384893376581847 -0.486450426070421
-0.48575086145294 -0.0666793054256442
0.438163672758707 0.147812891640061
0.511996151889796 -0.10996086598363
-0.367344560448834 0.429791400476067
-0.425257974718627 0.147154918102956
0.14502844341207 -0.641923941641987
0.557301780646912 0.0257997818438449
-0.54847364064532 -0.0723039137722558
0.24353415522719 0.43800827988699
0.00154697285563847 -0.33213611229654
-0.0812664635285193 -0.493703755862591
-0.336145656723598 -0.463420756054984
-0.0407287650818683 0.522883960093809
0.684700323193672 0.319568317718098
-0.375656947375512 -0.384079685231505
-0.0729258821281616 -0.565569534056151
0.426301313235251 -0.161132887190627
-0.576815179113546 0.387373657249226
0.0983045582644694 0.464948109044074
-0.378077751516968 -0.338378719402464
-0.129061758759101 -0.52425777680244
0.443188742855204 0.052929474090624
0.393212071145495 -0.181958048194864
-0.53363847963519 0.058192911131503
0.553324989598957 -0.0412940132686123
0.566577228303543 0.444871010801805
-0.240790896003035 -0.150263441405278
0.0551385588700376 0.468453365324038
-0.108720904932025 -0.609956817881014
0.210022807630025 -0.52057611355853
0.0369194350522511 0.565527444955007
-0.0753781470965849 -0.416697292539099
0.177648009299376 -0.483921470659525
0.364187256132765 -0.376678222215173
0.210282534640855 -0.441723013064841
0.414294760082443 0.0521454878701186
0.401492109122636 -0.0076774428001176
0.237270242549193 0.514603382452331
0.65831194296205 -0.12194230702744
-0.406805448982538 0.0611770157196915
-0.353413489417013 -0.326140951710452
-0.185408493744776 -0.450673445400113
-0.615970109161997 -0.276547610675718
-0.425955986440413 0.24537385302041
-0.248649374915241 0.471226977133378
-0.421207835653006 0.121142828627356
-0.494659995474286 -0.166244160406218
-0.221292390586677 -0.273984179094205
-0.100698786343832 0.398072878661258
0.137500931200125 0.302276475065423
0.203323572835298 0.0925341370505258
-0.130142630470218 -0.500785628344066
-0.0121426838240954 -0.386212520747018
0.435951541976402 0.0112767544617954
-0.496276709374292 0.369120595516156
-0.198906003667745 0.0356277108193202
0.163435645624256 -0.560464298127678
0.166521111071343 0.584963500447867
-0.0324458026473583 0.764339021360478
0.524027561307717 -0.269170184899804
0.491738327796772 0.175252920613348
0.284445837988504 0.290015786498766
-0.223116122102803 -0.323838236911677
-0.303049655446008 -0.242820921542545
0.63224533602405 -0.129231425389763
-0.0696442996066417 0.541645074537648
-0.236034821808665 0.370365578378292
-0.323615604826963 -0.273615804126685
-0.394608920396338 -0.182025972966019
0.518271136433262 -0.0918730778630867
-0.217366103341563 -0.641332178657339
-0.554238263318423 -0.320256773317602
-0.155113840204072 -0.450983846090196
0.107995685281811 -0.328529654836497
-0.0568538351607703 -0.374307401457369
-0.406073347911595 0.516368738042369
0.357598676323782 -0.137960488571039
-0.477082207194189 0.204440233639782
0.512970538472177 0.0893706257931523
-0.33158548759574 -0.239898675528984
-0.528217112189893 -0.272732285186123
0.32595872846755 -0.329826858703543
-0.14463954833103 0.566117224521376
0.216978687249071 -0.438159002156997
-0.292201621124041 -0.415153260301047
-0.0548896572613353 -0.465546381860273
0.493497817339835 0.0618591066797078
-0.360792673370375 0.570373538940932
-0.531311239857005 0.278099826619007
0.362150749265326 0.362754769271999
-0.468338188207513 0.142299115609465
-0.367261477673652 0.270022773978122
-0.43257182391381 0.27117692053756
-0.308425796038976 0.154156664449003
-0.342332450130737 -0.34395782136917
0.130456107455842 -0.242396560986628
-0.363169726941657 0.421725654993222
-0.0842708306613424 0.618291210942229
0.399810733918045 -0.385330387841149
-0.49713456474769 -0.298387271470233
-0.193601371738971 -0.339644353066227
-0.530339418769934 -0.0223667930617905
-0.544929250182861 0.222652144504971
-0.0619832705816587 0.384242859390477
0.0257840651873824 -0.609524613727098
0.0980164380935415 -0.474331148545984
-0.30731273939199 0.223653272046766
-0.0226343602292281 -0.374011543218813
0.348405977681023 -0.078060651257719
0.0919784517105331 -0.36235005377374
0.394949800042922 -0.260665476018736
0.167928561772307 -0.398276877190046
0.273432953155787 -0.355748384134347
0.39828300357197 -0.330944153000156
-0.388096269131259 0.300125085222655
0.476288763750725 0.442144492664941
0.337858143735344 -0.438225390637175
-0.313208765711352 0.436768159572368
0.00119280787069995 -0.448177620011371
0.116878248479415 -0.244990473250561
0.0533024791847692 0.570353097703067
-0.252583739755888 0.526049357912652
-0.425852609019792 0.503176169457928
-0.0363367995276982 0.488959845664106
0.727843221172546 -0.0760692142871427
0.340735858701458 -0.319652517197141
-0.46854338009664 0.0624458346059468
-0.438615583029295 -0.450870308082958
0.235321305059118 0.307516559192863
-0.0599307777705019 -0.451120315759241
0.124271535804483 -0.484300307214505
0.265339446292167 0.285014482317009
0.200295098285436 0.480423824545495
0.450526926892759 -0.133586575349283
-0.143811332481119 -0.538686897294671
-0.380314247807268 0.124683195181844
-0.0993239310118005 0.457348709941316
0.660603950063905 -0.0905641454676598
0.362601791070135 -0.378937498832563
0.506835625944091 -0.0536322743207097
-0.37224737367026 0.149928602930754
-0.336492111224054 0.489646027886647
-0.235968828050769 0.553334165058668
-0.254468524421319 0.397429865030886
-0.23292909703998 -0.450546440932356
-0.388107146873851 -0.375043370812288
0.0291677117338098 0.440638249050201
0.289521333023652 -0.311754172835688
0.358714109689869 0.271065227388719
0.404971391162471 0.231527146225563
0.265251404529336 0.452168452415411
-0.383870580898384 -0.167850558683995
-0.591792063739735 0.24546899077796
-0.273144875592614 -0.402890937729688
0.286284119854449 0.203197948448114
0.0754047839001563 -0.534721781069561
0.531667709975895 -0.239723624021988
-0.239644788334365 0.436736895145
-0.091585925861332 0.439391062167605
-0.363021888260278 0.20940221161774
-0.0518459502700863 0.402641063960803
0.153938779979805 -0.383290179054013
0.50011953336375 0.0916709769906873
0.138554196696406 0.370126018239106
-0.0594193991076753 -0.374809846178495
0.233601556091114 -0.310230569798436
0.305817373886333 -0.365657940896697
-0.0726607956951903 -0.302370859426286
-0.526608781844313 0.066176295235662
-0.219244563936807 0.54029365621028
0.203231955157495 -0.617682558935768
0.318118066224926 0.0227132593395585
-0.182733544189451 -0.282934991378175
0.314654655244123 0.436328203253494
-0.205743675757301 -0.330543137317958
-0.43375817038766 -0.184034156175146
-0.502893437830526 -0.381835152830803
0.324003325268473 -0.326700021463675
0.0120306821736758 -0.519012952217146
0.118832112052008 0.401928873806529
0.531423991116956 0.0601057620206971
0.514518857384243 0.396825579797071
0.439010081338306 0.181176993379783
0.272296824538882 -0.51997763239145
0.614639654371547 -0.10873199246882
-0.125464580077937 -0.315971093203284
-0.272431070496088 0.246710119497017
0.544850011299235 -0.285891816464592
-0.353480979632274 0.407795527202476
0.324643554916959 0.231497934426021
0.26300376665059 -0.163835563662274
0.42893145070991 0.347105884321524
0.00315874366105036 -0.440163118719176
0.126902943375348 0.572680582566047
0.243634917043785 -0.488646952812406
0.23583577601367 0.479504022121718
-0.386545269157671 0.404667815811
0.206847897816372 0.564108532935704
0.63947167387149 0.0104047314061318
-0.0770006459842211 -0.452931533974696
-0.590694358302029 0.0159442989270029
0.126091765113789 -0.569569672674915
0.561785003001701 -0.0954445167530244
0.210591572253722 -0.66953520717898
0.486228544629026 0.529523599867103
0.506066471648854 -0.0668324393005127
-0.324199538782488 -0.264366707338394
-0.433353285013461 0.44508393252766
0.255301468935691 -0.312343933391051
-0.348088966418062 0.326069740581474
-0.227109809335693 0.395410766377943
0.651923343717647 0.382192901224498
-0.265376625695591 -0.443437178124538
0.51433615038463 0.233116433188054
0.232349647571443 -0.276633307806076
0.34346869631181 0.459374014672527
-0.478401279752674 -0.0492968810866759
0.369915544153932 -0.228640777770716
0.375196283325843 -0.169524971050979
-0.00157392467305588 0.484646486586237
-0.0555878465295009 0.501463999517418
0.546825087175172 -0.229299595490034
-0.160459537311112 0.378124643667951
-0.135118129577314 0.519578405429273
0.484797084324439 -0.298163947201792
-0.33985667908192 -0.328300857571129
0.418267467150476 0.229740844451129
-0.286183964827189 -0.549325230359845
0.318113052424385 0.30695916643156
-0.339090813587151 -0.606375357890029
0.522140985706625 -0.177865897143414
0.109221812411725 0.537614982706217
0.530717087836794 -0.14276752542001
-0.438914898684429 0.154206879761444
0.362949478654557 -0.306141499617159
0.152412139956724 0.472685176488561
-0.443725312665144 5.22474702068648e-05
0.531822855151859 0.222611077794186
-0.153277915979862 0.389059313549572
0.382441744655549 0.389636355725181
-0.295318680426942 0.434446867003743
0.591675576587472 -0.323123071055569
-0.0900255318020237 0.603259765027401
0.440899622280792 0.162987856831952
-0.0384244747288071 -0.42140349216623
0.36285134911404 0.299641678513752
-0.507201375786474 -0.173306992603367
-0.0163541000808237 -0.368959828779321
0.179929151591644 0.474623743640887
0.332199669360773 0.252941563796864
-0.354230767995652 0.386936757533994
0.038196802068974 -0.453387940257799
0.486775299829726 0.166937216173174
0.0318027998928122 -0.510618770959198
0.575385876369386 -0.317341179659885
0.602237419565652 -0.0673119654603233
0.374044911442134 0.300485602728445
0.488505493027107 -0.340675106830431
0.428054805178482 -0.0304082227141913
-0.20759940005995 -0.421733876653297
0.499947949106355 -0.442003636354264
0.118282782976932 -0.480608573580628
-0.658159420549688 -0.19206062018205
-0.497510399906158 0.295440772018277
-0.282302730364822 -0.477347208489336
-0.32407688324303 0.433190982318258
-0.560322483218995 0.124960769010168
-0.0912662104674218 0.611857862168612
0.0196979412015413 -0.434626388868207
-0.34521204746635 -0.42319360925557
-0.566607770440953 0.164499514675379
0.346324474055823 -0.623667200295881
0.184088585920758 0.396219601181201
0.578694551954974 0.277896606782082
0.0978360398526969 -0.401074651843062
-0.35998625922531 -0.450201567864791
-0.122984476668586 0.551768404627466
0.310698566052851 -0.325989233159006
0.190189601480596 0.396604731418422
0.0691722691303731 0.156516972907285
-0.161404189250163 -0.199436921004803
-0.472740861690336 -0.439859374579179
-0.480791374891384 0.267415044183674
-0.498804576845445 0.053897986792085
0.404471548604411 0.38063467172672
-0.0532056635028991 0.622738174043752
0.000604932729812935 0.489307646816415
-0.219153729152023 -0.303380396773969
-0.42484399744395 0.0243470672322564
-0.475754879152587 0.193155832433617
0.305922505706727 0.403758693740781
-0.317489384838918 -0.451264968989749
-0.318420013364596 0.0813542921575217
0.238168463163345 -0.453885756864194
0.415366916683234 0.192861177959443
0.255405011104423 0.328974765564155
0.435601633216034 0.0656437165856695
0.553009492964683 -0.295240451401895
-0.462514678460245 0.25808510700504
-0.402026525442761 -0.504326070335766
-0.10653531227863 0.656573089242811
-0.0177567796355501 0.524226452592531
0.153407427549198 -0.412491062123545
0.212403856461462 -0.46111768411592
0.0613273208191983 0.362522109134484
0.458338668037309 0.385949387695338
0.13320492753803 0.298068224261448
-0.122157510879759 -0.384088504339365
0.373650755062426 0.513436907064966
0.613694604438862 -0.00930268393224801
0.494157048205806 0.209357375971833
-0.29968842080342 0.283887016915109
0.322758518481541 0.483460876290531
-0.613866064815323 -0.130360112396649
0.303720359410666 -0.121634040868571
0.267469947162014 0.201885103823736
-0.350394911117996 -0.390289948157939
-0.385593721890474 -0.213535501573451
-0.494569124548097 -0.167316344562436
0.498493604971886 -0.36380811301086
-0.207244051847759 -0.433566194865394
0.395800997614723 0.300348845550372
0.152989076121794 -0.458009784112388
0.560206712759614 0.211697629592376
-0.464726927097175 0.284782727905285
0.340957614851041 -0.363341300714919
-0.38292085311143 -0.444023055045141
-0.391275611059305 0.528340858663453
0.469192186686145 -0.182596647021597
-0.30220257963904 0.237692831268141
-0.4406727026981 -0.133947312211187
0.3076144652584 -0.349250483385029
-0.509889537036922 0.0197570162098521
-0.356243042574125 -0.48369838846645
0.125722116697204 0.541936967286285
-0.557303409607644 0.168485337759565
-0.366152439102019 -0.274528072623194
0.438320101585821 0.364287382155581
-0.471599549748932 0.0651236927222755
-0.352971134666347 -0.153846285102242
-0.313965447719873 0.135991695809426
0.119288352240501 0.63149770126338
-0.196446987171936 0.538181852077203
0.314877481062714 -0.523857538835558
0.0701586267119617 -0.501029758366357
0.334810795225123 0.389464534269482
-0.565858165609375 -0.0895611831881555
0.644391342802276 -0.10485416251453
0.318435336625697 0.287076647098728
0.183011167198266 -0.478160515230733
0.331952467543281 -0.534885863778044
-0.324454094984168 0.539139657946828
-0.231514321517788 0.4831198313365
0.477498941431438 0.499870053336703
-0.482474716969255 -0.0261821248018226
0.205883114273576 0.506307670609126
0.258778808591774 0.619833276667146
0.330408177876107 -0.41861461186999
0.216763624438463 0.571491413546178
0.440869724256736 0.513806746670792
0.524188753598677 0.0245065660027745
-0.496537735731232 -0.0635722712430038
0.399907704347418 0.0895331602817725
-0.0760415195096152 -0.497435210202797
-0.34684499110506 -0.352914569998025
0.477054100493283 -0.155382708413886
0.0982051790295014 0.532005064738506
-0.489723170473514 -0.13969508005536
-0.555098979656892 0.0113107927149313
0.341787484867836 -0.500778205533908
0.254559486903304 0.244021506931044
0.00665903785862931 -0.376099247478264
0.136849928173097 -0.534885143702446
-0.586829455638493 -0.215547424187215
-0.227281029280609 -0.506400689543
-0.381325507569911 -0.0616592197592854
0.448143474204037 0.468726166507086
0.486499777396893 -0.0313340141549166
0.319369697320115 0.392543144570775
0.342488106299301 -0.223909736058496
-0.361558197056043 0.144870688163681
-0.430202047850794 -0.244512491162056
0.469576668752671 0.129196333245781
0.604302655673628 -0.0781180135043617
0.111711098632995 0.393250779463942
0.485673851731605 -0.116112235111427
0.545297004391458 -0.0881527163213452
0.211621099085464 0.447985024161044
-0.290508180267194 0.415562726432696
0.569040057731849 -0.230434503283937
-0.549125484792119 0.239819209132945
0.330414339182141 -0.479789300317352
0.479550049476139 0.0568011409086888
0.342796846739257 -0.280243109097873
0.290809081321065 0.252689571425088
-0.310481832768293 -0.443621428188413
-0.0764224579069667 -0.57696600746244
-0.0686424828142239 0.48406679750995
0.517756315847781 0.227739960260016
-0.529858968687084 0.0348038306809163
0.220175662475261 -0.376840851006938
0.274062315782869 0.456539100039556
-0.308016154251457 -0.713877445300623
-0.466328223114511 -0.261959058482951
0.00808349290294255 0.488633013520843
0.00766791471612147 0.39288049889357
0.0506837892889762 0.638235045154696
-0.104672311154261 -0.361282382059126
-0.294347300389369 -0.0401014218879888
0.334435754165814 0.227393200130395
0.0444287194849519 0.420394356945204
0.13192308759323 0.591502027930546
-0.514373127412503 0.226283311804008
-0.411444666107899 0.16919758674413
0.114432166551318 -0.423721774691791
0.392139109674516 -0.232986009660757
-0.0885834440405968 -0.497285834452754
0.602357804676693 0.147330678155679
0.543009284832814 0.357194706853802
0.252336462978138 0.555031466276346
-0.264478257282426 -0.571339288313336
0.604592220275043 -0.00837843698374119
0.23983632640604 -0.298166014965629
-0.46572096415538 -0.31759659011354
0.440330566375832 -0.333297834621463
0.193626024546053 -0.527189986257421
-0.227011691224815 -0.468738199694617
0.256556379472597 -0.249746121229653
0.259751283986294 0.0242995858615211
0.385124536841393 -0.336045132326391
-0.0658791100252809 0.462617812671645
-0.436693615750897 0.602489297936097
-0.629450160210955 0.25967453132907
0.264727479224813 0.20663309378393
0.404758810181309 -0.0886443835602666
-0.379633949943684 0.256486760537039
-0.223858567388338 0.348207642240531
0.414069589330462 0.408768955227674
0.429946862026962 0.510551546498842
0.181816852701185 0.420652029371857
-0.278442953389486 0.0807709329221568
-0.469628948982392 0.251443985992502
-0.240817076134378 0.370785702551208
0.150894749030606 0.500277996959456
0.533873867601257 0.109593107585197
0.427448932930148 -0.190138551397556
0.519998149079823 0.476821317521454
0.271144204562589 0.376055083801017
-0.400702207961946 0.231231986329172
-0.370738275824491 -0.245772502083515
0.387882216803554 0.487644388558294
-0.522725231113125 -0.347047364254942
-0.454112576209338 -0.0625849019108906
0.0110637172691426 0.39939895554243
0.391324360187501 -0.400566379982605
0.333486385128799 -0.45613989836964
-0.165333422680291 0.334616189443102
0.252843748344772 -0.399761627070238
-0.156618013709541 -0.599765021682124
0.353439093658366 0.522561439693284
-0.380456374613143 -0.523182851362489
-0.612412648784812 0.244125120097926
-0.241201829310102 0.483793512238229
0.258872644650039 -0.0798152448284754
0.267148370781368 -0.183360310684867
-0.126054071419437 -0.222827216824345
0.239352210121278 -0.429886491072441
-0.347064851360084 -0.151240634247559
0.545498935777216 -0.141218457510854
0.220963291787239 -0.276652093061937
0.0270071181582591 -0.503835185771754
-0.548010369270751 0.263219352053843
0.264737873992389 -0.255950104421443
-0.413317113073322 -0.263806190336946
0.461973108116343 0.0467137140227455
0.317632952694165 0.655592120311055
0.182460335237394 0.5291397395811
0.605340849105078 -0.289543936552674
0.0705982415074416 0.365229742654843
0.0795469981285674 -0.505962769007975
0.309040547885617 -0.18311155053519
0.101752593650249 -0.666473426111801
-0.425094290087649 0.386913089642003
-0.0530739746492122 0.405252850449777
0.169059931463233 -0.516226434473684
-0.161176099853208 -0.531921858006988
-0.44540578557298 0.0733853381485703
0.395764650157336 0.181739051649957
-0.279182498736259 -0.291612543689961
-0.201225648147808 0.342492269390346
-0.44892204241962 0.236515434811641
-0.523498180710129 0.267311217829238
0.0108762064261434 0.576936326220468
-0.352680406357131 0.453180386250095
-0.138761422323007 -0.393894150490347
-0.0547088959482745 0.390029622494741
-0.192596827912809 0.623382050256809
-0.0557557359121135 -0.534957167699033
0.0178817659558814 -0.51930782286434
-0.188040921088047 -0.149110987998514
0.532947305623013 -0.239242041582139
-0.377538945018421 0.339681404151485
-0.366899395003671 -0.404914590408727
0.194422844865009 -0.481076356777041
0.442020049136393 -0.494377030254142
0.0961531234952401 0.404107308063069
0.233820152385566 -0.328243036022909
0.463782570775466 0.0271217394966065
0.0896747352982277 0.55918861570962
-0.230949655222178 0.381149949038593
0.100131301183151 -0.47880666973269
-0.174250010910739 -0.375349533490107
0.444456824479873 0.267650132205283
-0.0566895492353304 0.339809598716976
-0.39713638378689 -0.12320292473221
-0.308241829111955 -0.397208427374583
-0.431650282745416 0.0744218458759035
0.288863955174009 0.12103662923617
0.436045398595622 0.196464840881412
0.420862055966108 -0.113105528737618
0.621421992247552 -0.167517386851491
-0.219784021413159 -0.516125407217139
-0.328138261302683 0.251215533378357
0.0833077248095048 -0.617869211449324
-0.425504736930979 0.306876360432402
-0.280668784962637 0.499112290467715
0.11586939596611 -0.629000977259076
-0.341077320222955 0.458238153473626
0.0495114301152962 -0.350485975447874
0.100867963018309 -0.418644040992919
0.241414108139295 0.306443457780067
-0.354499000655332 0.0381891241717121
-0.350638091781267 -0.0884226583117254
0.197841035559409 0.512745355732476
-0.435509292256555 -0.0657034002172148
-0.22169960405429 0.533333633815065
-0.527824709895489 -0.217878763438903
0.723046560472355 0.122707610566721
0.32720686318182 0.230522758893486
0.408006116170699 0.0584944573850337
-0.155550165282679 0.432867033046009
0.548298531453802 0.258154942692765
-0.351127211238215 0.245109057674585
-0.375793674703915 -0.542404740819671
0.316320076185885 -0.220521167833692
-0.581058786635867 -0.0767911148487412
-0.18052629875337 0.519228974658101
-0.0491406377711122 0.308107791512101
0.491736240902191 0.0697195926303278
-0.437434712553441 -0.0117677263059165
0.409016394660463 -0.493490527929966
0.572129256971368 -0.138571867845219
0.469849631936516 0.0127829646888509
0.053454063135548 -0.257931924282823
0.582283049241954 -0.0993757816006964
-0.206034470180057 -0.517759972757323
-0.117019602734757 0.622898388951387
-0.395359834171974 -0.190672425633788
0.01723918191193 0.50161328299098
-0.320159690005212 0.339696059155883
0.404967370886974 0.419249085556732
-0.502044322082121 -0.0333438746694417
0.180000614994299 0.502334522967717
0.173170706619906 0.429845867365436
0.542180941149374 -0.147644847683724
0.255497417401424 0.356078373925493
0.448044275376755 -0.101962959072687
-0.490218360487021 -0.226296768176942
0.345945397332569 -0.290216576900181
0.327322870042921 -0.405610433487707
-0.151278840817667 0.413202552329036
-0.228850247731624 0.347743343204134
0.335105078599757 -0.443312148782182
0.484005732617579 0.200442759238843
0.0609319848863582 -0.537956548858737
-0.347159200162346 -0.467051924557347
-0.134141681762339 0.470320605804516
-0.396243120176826 0.371680053502884
-0.192025541540643 0.323167752456049
0.226221861211578 0.593949889054939
0.502911229234531 0.00300946214332831
-0.406181504896781 -0.018231696719857
-0.442311534084519 -0.104547189157301
-0.00562550745354953 -0.466804562684468
0.46799900235389 0.265762689241269
0.440434846382156 0.383888664281949
0.538965048503259 -0.258840689332986
-0.409799509339286 -0.3664216030716
0.624402634325754 -0.243977919985801
-0.118999794495304 0.568218563425653
-0.412519252842171 0.516626157421392
0.355103649266849 -0.436313851929379
0.0102123227836782 0.561258461671143
-0.158185111546182 0.42389153508255
0.132475680722723 0.277323562025368
0.30783506604155 0.604537749737726
-0.425492240764898 -0.437719027365913
-0.395073179221307 0.396968546587255
-0.657896866260448 -0.0863510984264729
-0.34790582473296 0.207687736930079
0.143401289932893 -0.428028413406015
-0.184422574358234 -0.437351628825641
-0.476526267404753 0.173462255162532
-0.35860190171595 -0.285685603932619
0.597286856089723 0.0290119404844624
-0.255891448854781 -0.279754159024265
-0.175137266079407 -0.534091094747071
-0.00958616940377961 0.559616827320523
0.0577678928295031 0.369079351884412
0.363389360860945 -0.386473116990621
-0.364032985622831 0.145278191599075
-0.421363580099693 -0.187791990352145
-0.228876120898202 0.406963775337521
-0.239521291702325 0.39111832743679
-0.239226338590968 0.502222978233745
-0.22448830970136 -0.45958299974588
0.566309249566345 -0.263200188670592
0.0637037625069466 -0.515798069560646
-0.022353778966012 0.45984523520807
0.350180448863721 0.480496226631669
-0.196557206310851 -0.547711582021558
0.247471430314091 -0.445474849982174
-0.46936959537234 0.0670517187881033
-0.536542991674156 0.113851754289699
-0.425140371605697 0.0405608325558391
0.336661346735426 0.466707125660817
-0.216840997654754 0.246542363576418
-0.535500277395108 0.147446770610341
-0.220677984764354 0.433502416067943
-0.0538351857190437 -0.679591764526103
0.0107192675076328 -0.561729344606257
-0.483403263936003 0.0114273386644611
0.569511989290161 -0.512249946481379
0.407732398348089 -0.410547534859385
0.425025985625226 -0.148263121922481
0.303422007573718 -0.186932135734968
0.315092062418105 -0.470380352453147
0.374047327941427 -0.433807134315916
-0.391420214465835 0.300003015895225
0.659375033874654 0.0201774332275706
0.548171627585449 0.276588521065241
0.378849112384144 0.161559965128754
-0.0222579255798695 0.39744280943813
-0.163329586597634 0.473905067746347
0.160919624556458 -0.426173995578024
0.443024327464977 0.318610891110892
0.0389316818664194 0.505290069708347
-0.101760573809648 -0.471309056626192
0.20285248753196 0.410424447880681
-0.266759672335734 -0.534203068790036
0.18512076026169 0.343308472667973
0.110564643212951 0.401298732507379
-0.37533308594616 -0.24508360567394
-0.0547614428004159 -0.210261768139596
-0.00142007861816512 0.635019494575554
-0.367784158536109 0.271116833703266
-0.19765041563253 0.313512584467494
-0.492610147660048 -0.00459230424474399
0.0641918868465766 0.744087523405815
-0.13789461172409 -0.59543313362158
-0.125971061985937 -0.735617891134375
0.421438697814908 0.350599460198079
-0.272294699845696 -0.216081907031224
-0.409728128407097 0.28862994538424
0.03981007027452 -0.268637298463891
0.00160040572031535 0.567293376386181
-0.341831506655382 -0.462406862770582
-0.200938263467863 -0.577807118435883
0.213605892977175 -0.510084781811755
0.268429421013208 -0.422558128345194
0.153987507332816 0.496012061272087
0.317711181411792 -0.273204799463229
0.347434007464357 0.506583333604004
-0.418624086902468 -0.0271215735268545
0.155636579351873 -0.620371809661541
0.540858104057811 0.373824497444926
0.0445447306345031 0.620979489952776
0.282648456625042 -0.369120034674319
0.0697269131937701 0.330359849584128
0.627873954580771 -0.167361702620093
0.0426357305830092 0.453326011678224
0.199342708813324 0.428503838048423
-0.460908997707291 0.255119017319386
-0.0777844019555401 -0.566392776455903
0.555557500601064 0.213704155812506
-0.0716298644213455 -0.57583110908679
-0.197585795176903 0.561781390083648
-0.452621316343142 0.505967578211162
0.450420765854019 0.249848040844515
0.0172721593250722 -0.379047783774136
-0.485197145476132 -0.217593679477808
0.475636722835582 0.104665633019773
-0.374234109920146 0.357143093430622
-0.490961787306776 0.0566956083993277
-0.354820190204408 0.227179847525415
0.492449459436583 -0.230439256612009
-0.364607886747147 0.305348631036468
-0.346516122713647 -0.371222591496249
0.13946188293772 -0.415294320803385
-0.440262039193234 -0.189917882023873
-0.293089571553626 0.206866119180966
-0.104835516597421 -0.401161735162572
0.370689636066207 0.635973454939995
-0.569821035496411 0.171530922253447
0.168396198851442 -0.318250070255182
0.0976926023814145 0.465677134833265
0.217326259403808 -0.462893987002802
-0.385290089446148 -0.385720100507466
-0.508718629413021 0.306885587314014
-0.197883011935573 0.362246803023262
-0.0809664566992639 0.438967407390125
0.549750398506657 0.105063590959614
0.233337770268824 -0.338206042708072
-0.432220079709184 -0.105342008209334
-0.108266955468302 0.478929424077069
0.542378263561503 0.138315895548077
0.144974332175462 -0.363119141255556
-0.658624944972691 0.100822115592169
0.110839397445678 -0.417489604497005
-0.16758549951741 -0.529793225121503
0.278255641903468 -0.43400308066732
-0.583504636789463 0.000446338283196679
-0.433417226005283 -0.314515334761638
-0.556577486848905 0.228650644640301
-0.55713697810095 0.0607221017755324
-0.262270628337006 -0.302346500175419
-0.0769382788267443 0.44888771835327
0.39450751430107 -0.353207402673876
0.250057838582163 -0.359796736748054
0.254647573708385 0.411975319776157
0.544722841726111 0.284579308135325
-0.362474593550141 -0.206713141606207
0.473332392106408 -0.216473260863185
-0.145402528139794 -0.488918912229856
0.557097224171055 0.0737496548623079
-0.425409110536468 -0.176464203410941
0.489198356176769 -0.0366827777521237
0.701441730078803 0.0505793712746661
-0.114003899054193 -0.424052602402755
-0.110969682838814 -0.522079715138009
0.140988144699408 0.48353235744202
-0.317343816676535 0.490812065114008
0.165500693660342 0.422415281678579
-0.346493083175512 0.371277075297856
0.424761658886006 0.338323018059806
-0.485219259657774 -0.158811188284571
-0.614936559177299 0.119170545931858
-0.301502019167128 -0.274163180419279
0.415030581339703 0.41522696369517
0.0290683640432658 0.380312123227654
-0.432166072623831 0.249562334301565
0.159612346704928 -0.490229335892219
0.489709477147753 0.0626581010032382
0.488611399647672 -0.321439731312343
-0.464465022184875 -0.209529272878083
-0.603614868064835 0.02830281124163
0.476236253971134 0.208720546259501
0.130124912850007 -0.45022384334349
0.172591658838459 0.412958004153808
-0.397085141679752 0.384667332481271
0.35040298141552 0.427270042288841
0.433901883444603 -0.305883254523694
-0.0638658694109871 0.66795545041652
0.388697984319027 -0.337402098746241
0.110133691864926 -0.447128318507153
-0.166443488579293 -0.375644510489608
-0.43811913543362 0.376663184483806
0.0497571992479098 0.521929255107068
-0.384477548340952 0.0662723242552868
-0.197802700528597 0.362738399550637
0.442937485043975 0.227453568825406
0.029103176025761 -0.544469893933952
0.399363323999811 -0.14579028588622
-0.512812509530132 0.491185064656103
-0.447910887470859 0.032973195648073
0.432670000531052 0.0994422286535654
0.0235111593994489 -0.547147294112589
0.32486173251127 0.63845978201038
0.239597636847993 0.546295372937661
0.0849934641742389 0.258406028375405
0.292334211744835 0.387307348992613
-0.359348981371482 -0.0897517156241066
-0.279527273662192 0.4070632138652
0.0349798791674681 0.508011537694748
0.402197106026678 -0.11633115329598
0.124074811258991 -0.543532290831931
0.579183357694266 -0.0533539919776933
-0.0322415297478634 0.437333434001178
-0.101111080248986 -0.523530080313069
0.573998587947018 0.136090822501112
0.12038306253643 -0.470616154029348
-0.606288459898446 -0.0286112766827914
-0.47221116230082 -0.125539192711692
0.424679669477178 0.0653476255510684
0.67627439093483 -0.209778196177365
0.451198759259587 0.135569017910581
0.20916846355965 -0.450402352708319
-0.207888475920832 -0.401345206938524
-0.0924200216574711 -0.362680854216432
0.623989507034932 0.0482807451049332
0.312554145512618 0.17676016995746
0.435609433533774 0.33235154444391
0.322139162571026 -0.488787025522924
0.561016072428813 0.2048154276223
-0.699093761494682 0.127589603818171
-0.552252059290628 -0.212127089063774
0.474472902281653 0.239588197676357
0.383075379237864 -0.51558381599977
0.157630846511985 -0.341511158137982
0.630167364558025 -0.242217178921231
-0.549103965738376 -0.0863394553120252
-0.158075134316069 0.594437838967618
0.135493511701021 0.421641470928315
-0.717698695017202 -0.303298462402768
0.223421266445591 0.411311939106585
-0.531367373451155 -0.119574015147138
0.54417885441894 0.177919292001249
0.375192017074844 -0.0706216348516562
0.0366311735161735 0.53788973399931
0.11399358401661 -0.522218118806737
-0.591024340458505 -0.354730073973519
0.629252726238917 0.12323820694723
0.177357950601917 -0.514199198757229
0.488366314210263 -0.00363687722807837
0.300579483551162 0.336299439500902
-0.386694774616714 -0.132562856063777
-0.126921474057551 -0.430478204073531
0.144791711014736 -0.382955315847838
0.230802253077133 0.356171726155408
-0.0287061947655483 0.358739918202688
-0.545366917479024 0.196179135762137
-0.704367587493663 0.0388252245051841
-0.399230707728559 0.337171267238611
-0.586914248257561 0.239781512692801
-0.411435254554927 0.201749572176621
0.0974962729592772 0.347492283782217
-0.183952496652255 -0.373357339327428
0.432481522618842 0.146407380517308
-0.251621895255796 -0.0634771215236032
0.542286247777506 -0.054036788212884
-0.485902061716414 -0.312534423066788
0.106231806551334 -0.201912508175024
-0.594591521476144 -0.0332586954645527
-0.494092742505671 0.263542825615648
0.149680404306229 0.236023298794823
-0.158953855445241 0.389278702298198
0.510906554151759 -0.0872674638187026
-0.384141575614153 -0.0153774501211066
-0.641957861863757 -0.138385453849249
-0.382611942522733 0.283559669569193
-0.499406293023794 0.0244079758716115
0.49145928123268 -0.266940544571709
0.248308428694264 -0.459335358281682
-0.0967541577907056 0.549999188772684
-0.138225842349184 0.65548215619356
0.462827317737044 -0.487045143006049
-0.43220620283001 -0.0217015061034202
-0.0830086051867787 -0.426468535689695
0.16845683674242 0.525802930840555
-0.228292184474473 -0.547360475493549
-0.382632971546761 0.459024426773195
0.751901137300731 0.200882802272128
0.412216525885519 0.246190648134084
-0.12178517612491 0.351212337168027
0.134610215975451 -0.312198493355464
-0.0490787910068601 0.547375053149299
0.633580140476201 -0.10665176347928
0.00109302379434118 0.604275867261608
0.470821021502933 -0.234531161010694
-0.233123280343875 0.352667474520225
-0.379527348030687 0.356106877988892
0.235386331927416 0.394166626539477
-0.550359058935267 0.18462386241781
-0.732051793179345 0.300454458281531
-0.452948201251071 0.135474762914792
0.431879150442324 -0.134948491224975
-0.495714551439693 0.221088762629891
0.294748620009654 0.421860007409157
0.373914127946119 -0.430955539373971
0.550539100185166 0.408809409773354
-0.347201876006579 0.386470108121439
-0.372913550309026 -0.00160406201036023
0.34710699142731 0.358753619583976
0.58188385911101 -0.241096157136027
0.45913691361334 0.191132016172602
-0.0664696864573871 -0.571118564752625
0.299858675916845 -0.410591587356745
0.203320185927614 -0.519937503817829
-0.481571129166141 0.504511080659473
-0.692852478558818 0.260945334360652
0.219978930987258 -0.420523364655428
0.179438807465269 0.460080731225156
-0.00864191311612271 0.666798730753215
0.616450982211699 0.137733036416587
0.527426105653322 0.0988670241127674
0.352682506581193 -0.285839999487323
0.443158047242716 -0.237414812276162
0.500619842145181 -0.175502603304923
-0.659355764488433 0.175390614139379
-0.140464509200005 0.521041405205742
-0.277520801397008 -0.44591205346519
0.173251303108942 0.522143715068581
-0.214162198865226 0.395445747595047
0.361300130044181 0.00514402009222506
-0.126913802960815 0.49564051925269
0.27830339044233 0.0187641796823997
0.423882656687837 -0.301951123908633
0.395941633073266 -0.341828355873042
-0.569015167496887 -0.196640296358402
-0.289958689568792 0.152746458798799
0.181596348290728 -0.366411426584387
-0.390598395539564 0.04686227539304
-0.0551776618406812 0.575503819103159
-0.438303720165156 -0.257469605561047
0.31574939918611 -0.22102599783924
0.558831079149853 -0.377421918075272
0.440890608707269 0.0935055447119736
-0.535849313550199 0.306012457351565
0.098816894562315 0.498505571749511
-0.110798893900972 0.323916927471379
-0.182610021285773 0.278790559208114
0.330443138788323 -0.323580047295606
0.455795100983961 0.127719222163118
0.415304385542165 -0.364257128389598
-0.432261894473587 -0.05984803999809
0.381890669032803 0.356494703005308
0.161577587868487 -0.478821666464164
-0.1033189029221 -0.482888808538721
0.355548921895355 -0.248091777863663
0.222461316061599 -0.28944643726216
0.356960264337719 0.19305768367281
-0.450736996819001 0.132725133158169
-0.0350013233837587 0.425335166903216
0.0157418250173836 -0.667594993125591
0.332680304607303 -0.442033259519972
-0.482284239164608 -0.32456056197205
-0.104467257754211 -0.602220075910803
-0.381513735133484 0.15076787542356
-0.12649487052828 0.555594851631228
-0.299907087647157 -0.535261315871494
-0.330090602523623 0.12843242092369
-0.345843787455493 -0.355346297853136
0.574658701521077 -0.205105479178785
-0.268282260240599 0.43701710053573
0.63196633150924 0.20305339222043
0.384918010929745 0.287310092332796
-0.230691377278688 -0.494295306764842
-0.183071942182971 0.3846618330728
0.228786342515297 -0.362584100526394
0.597052228513473 0.000907524487913931
-0.419209631055619 0.0556441887786546
-0.15832382889067 -0.580947659923459
-0.447120915744161 -0.300133361901196
-0.386805124799352 0.383826864213311
-0.517162056644773 -0.290636781144839
0.271439618140552 -0.0897734987076788
-0.470875401829945 0.557376848797419
0.461553293085415 0.295149509931116
-0.423861275274243 0.0696922980993143
-0.550633538746519 0.339920084422646
0.293939187019457 0.0888826329633406
0.405149674066711 0.352984079298619
-0.104087565769465 -0.530061023294954
0.49182253003281 -0.521112547809069
0.353679334625684 -0.462660098790425
-0.334809921072522 0.372553868918567
0.0365147288711051 0.45757531791217
-0.388672702538468 0.438884233535258
0.231769780616611 -0.59675458600214
0.30221536135683 0.508173149662648
0.444566369143089 0.0780136483997331
0.108289925826867 0.661902329418954
0.22778835654605 -0.540791050489098
-0.201100226976968 -0.371167705805525
0.364885628646458 0.280529303027317
0.360590016217418 0.308643797258393
0.402875141773483 -0.436222372483023
-0.558324266696689 -0.109666592432446
0.180442265156423 0.622203833349168
0.0423738374837007 0.382999933253934
-0.126371840897395 0.459617513561568
-0.440060236535186 -0.0388348745261372
0.518441077289197 0.389307208843207
-0.250002336059572 0.39765630955064
-0.505369022603595 -0.243082443177566
0.0850137826816006 0.423250220608491
0.252522490047618 -0.341204941048239
-0.645282878981824 0.106865023743787
-0.331725538501361 0.238381702141898
-0.191179240281921 -0.64276241885042
-0.132670994748627 0.545072782056501
0.0888958386232828 -0.354287290387332
-0.229089267203584 -0.184143691090174
0.285955478497905 0.525103008485376
0.127598714938904 -0.486629643733362
-0.170191798167634 0.513655477970084
0.188179178227028 -0.595178718585562
-0.445699343014911 -0.179706290545848
-0.150128705877467 -0.308294103873005
0.295665427660691 0.338690182526769
0.505422045860705 -0.288361794558068
0.00474087959760005 0.527195925127173
-0.262596426076626 -0.295919818480921
-0.438713790236447 0.0494385313555548
0.42216474713613 0.155674681139194
-0.615643521883596 -0.132888759087847
-0.622184016224846 -0.0357401632103637
-0.719003201971503 0.0387567927290388
0.292284266386317 -0.600474565998192
-0.452391371464299 0.177719373473692
0.130652665353598 0.499875190347449
0.0720035250210151 0.559416827066043
-0.0569086001632426 0.586185247301677
0.112372028721334 -0.537018569747554
-0.469658274879279 0.173032545390021
-0.219625584579891 -0.410148007386364
-0.477069206702859 -0.321927945316781
0.169263409730062 -0.540799559796361
-0.649124146142286 -0.328567654818725
0.287538855883322 -0.330048319791561
-0.177767502012598 -0.430645732072839
0.319616958687808 -0.348521339573375
0.317036321319972 0.270237469116057
0.37695120979966 -0.160899123798353
0.363531208603828 -0.262492154702313
-0.27124614913851 -0.293013347555235
0.324320344273642 -0.453207159311374
-0.512838962240164 -0.0437998024258031
0.361282528732022 -0.363566867776538
-0.486554426591638 0.10116211907856
-0.154391898804814 0.269239173862373
-0.517048902059342 0.393945207738496
-0.356414703390596 -0.102744350161993
0.121961406788876 0.581173132298299
0.443199583028987 0.117217663483936
0.245961774711903 0.463675038410703
0.221895898682278 -0.590463327049495
0.128380579125799 0.414816636852958
0.0411292016887732 0.371212691710095
0.470707284136561 -0.492457743873806
-0.195976603150714 -0.269625083107882
0.469911821820003 -0.485201436910602
-0.277345637256933 -0.515313947686599
0.198046053820879 0.537173942219314
-0.367749767534585 0.36742889950404
-0.51608238188217 0.23963613578577
0.424691156891267 0.0863899115788533
0.505767788265904 0.0344239374430552
0.397683557823326 0.449556995466366
0.592210422913622 0.103685023908766
-0.181421894778943 -0.388149691065405
0.417428724563931 -0.226484776456477
0.347729158476787 0.199778802358587
0.105825309454755 -0.345312327445105
0.0162589846445137 -0.329820332842534
0.417232471501025 -0.380150862412678
0.263554792451024 -0.279014677256576
-0.0211273997392213 0.509294501831005
-0.218395221003391 0.474775365966859
0.399536286543239 0.124894806039442
0.493854007068656 -0.172089790225896
-0.427791861682078 -0.0439478258867216
0.247951974732718 -0.134376632404235
0.139840554511225 0.510974453206137
0.0648931983382232 0.45032133125431
-0.405881165600956 0.143125317945622
-0.370034167372566 0.367296472888799
-0.0782148016606356 0.491542592005138
-0.413778904783947 -0.0977587088455453
-0.363033499146812 -0.428618511496954
0.358575710525913 0.475193062769338
-0.0813101241649237 0.566183662786438
-0.119364660901415 0.598973167616193
0.311083603898571 0.194927464267975
-0.10462958925057 0.711317984938563
-0.54601390485681 -0.0601910508183
-0.443923821614057 0.120856561883627
-0.433914358416741 -0.151059914073494
0.188927624521624 0.195691204884581
0.221527642578381 -0.174149144181397
-0.514841639690247 0.0646530732102412
0.288015987719799 -0.273192510017552
-0.513699317609652 -0.155485492804462
0.215516525706518 0.343456111865909
0.418984349529446 -0.0158332132007016
0.529223990624421 0.356187978291093
-0.430260913962263 0.272739180519146
-0.297632588328352 0.476419589049523
-0.387404402675046 0.258013059715109
-0.0632087221601453 0.397065920624855
0.585659345043915 0.200114989164472
-0.2919402692913 0.242139476034532
0.137470241845802 0.575533158030903
0.245676939826726 0.419917117036586
-0.219002789738259 0.468598841035761
-0.388791081738521 -0.198654884303357
0.412758070435303 -0.0392165835348443
-0.536163555150087 0.0707780239457974
0.352094086560024 -0.535217654370491
0.339293423261971 0.350048933796671
0.527999192624635 0.0934722382051431
-0.409756221569145 0.349179052474125
-0.383763981929868 0.326380926185905
0.154381365603736 -0.522981370971758
0.287536676624096 0.342308490532166
0.594322368074811 -0.133991302968403
0.390215468814612 0.235954983384501
0.532621266848175 0.22440833970138
-0.154585771529022 -0.407283981591515
0.198461192074064 0.479708546611126
0.250692124950232 -0.496483801999225
-0.292962121373329 -0.276726138641658
0.372544609191168 0.467621938880301
0.490012413701322 -0.411391439214114
0.586806730965557 0.238756994407721
0.501662126546284 -0.0163866897841472
0.501558760571475 -0.124356533796286
-0.288488828676817 0.349520492702119
0.591638171270316 -0.356039387207215
0.260104784924381 0.411776683791341
0.431943642028391 -0.402571557867973
-0.39972327402102 -0.201664991909067
-0.00650421851107469 0.462796583133191
0.625803156746498 0.159123206023864
0.576494162461947 -0.146389305810001
-0.420659006675528 0.260553021634875
-0.169423776418565 -0.478284108684363
-0.400589926902944 0.291700976944521
0.232721747578841 0.222622559609937
0.309270448704212 0.183619203184637
0.407738617320693 0.0429205915550731
0.160922714776965 -0.342935306882021
-0.504671934734593 -0.0706172004323258
-0.0606017198713432 0.467544238156209
-0.224538023642888 0.373827218533754
-0.0559090366547909 0.515021686744328
-0.276012946730025 -0.402730405658849
-0.339037291672083 -0.427546271758974
0.250793650813536 -0.368376944970942
-0.315243731617119 -0.277379232844813
0.39763825742398 -0.0874686079199279
-0.277337902419024 0.354623791982514
0.495204459412196 0.122090639769327
0.0691101936849728 -0.419051528756691
0.633595946454153 0.0313052125599256
0.224732742775894 0.370315311896052
-0.233621872110843 -0.279491632154538
-0.301348037715708 -0.257602788422254
-0.0388646502792274 -0.573768346030609
0.455508774816439 0.385449727962458
-0.164146145106092 -0.343910571747159
0.530058445172557 -0.228704763229196
0.364807362641644 -0.422514510640545
0.435676109594814 -0.0732247638053237
0.502254421447955 -0.150713312765367
-0.158034644204908 -0.39367774099283
0.208036247256488 -0.173615220786605
-0.0223422151198475 0.637352536275104
-0.117067892326764 -0.661964800561059
-0.333291176021926 -0.254197063238375
0.634900081693871 0.183065553613032
0.482432556092867 0.31102260842218
0.0137089542001257 0.329124267061045
-0.0282107308174426 -0.427163092441907
0.585512254698659 0.181443446378681
-0.14672162144536 -0.537474876843712
0.269228133538581 0.41063187863854
0.501267478524669 -0.249408789236684
0.521306878514484 -0.189309910342682
0.186680215360924 0.550993557231088
0.366859205113947 -0.229647295026025
-0.189493872884864 0.49579606566595
-0.491434356681665 -0.343197122376386
0.434646392461605 0.0832031502912406
-0.0214192696361266 0.360582560817615
0.0626545335317063 -0.48217997138892
0.46335023648911 0.0489158324078457
0.167247907136779 0.547392545542078
-0.0213144358698076 -0.559918030451737
0.486515979848471 -0.230221522374889
-0.0308251201837921 0.401017527061276
-0.0320786104158094 0.465137501802481
0.16373268403705 0.529700299204607
-0.599718532303428 -0.108535237180514
-0.134605042398219 -0.415616682415118
-0.41458784114609 -0.269690028152264
-0.308530018704789 -0.0237116899544523
0.542692469678927 -0.315027661755227
-0.304710040637066 -0.181731478994985
-0.420838732658953 -0.234047978578926
-0.611297201958266 -0.226215324647504
-0.150275456638328 0.50770288445826
-0.54618017502633 -0.123528761141385
0.551746117026652 0.0539728837366437
0.464504054834569 -0.187520043075668
0.351407244693458 0.349079950887716
-0.453335237540555 -0.36216052945639
-0.433711770596167 -0.251032575346427
0.436581339786926 -0.0617527004674107
-0.171732893101819 -0.499068318151314
0.275693857542367 -0.359725727782843
0.424035606292489 -0.499927108119873
-0.134222694570147 -0.475022106231091
-0.0691110643462938 0.654098496456345
-0.498831710869126 -0.410166339810885
-0.484221174454676 -0.40635600147006
-0.400349668802616 0.359215322447112
-0.538425942800012 0.44280653900101
-0.278659595452299 0.271625508841935
-0.0882617921706737 0.501226486193082
-0.412459694029068 -0.257473104602897
-0.475783513789754 0.0747653540894784
0.19020220353302 -0.394102787682226
0.509613462195689 -0.13747974609854
0.281797172913233 0.291281733220624
0.529190194892696 -0.134041164299182
-0.0371508150299344 -0.628744927488752
0.482876479547555 -0.0208036566907574
-0.214601864622306 -0.524926569537208
0.358174330062141 -0.109845283663382
0.543659188399606 0.279468638055161
-0.429314610941035 -0.143785750912373
0.144970146189822 0.423583281533639
0.220705961288427 -0.559290986542852
0.442498880033861 0.194764108412988
0.432981996489953 -0.494594796101796
-0.48740461632426 0.356590178759049
0.338254488073931 -0.358348159342696
-0.412018660478025 -0.0152350501146261
-0.222848374432097 -0.379513012513876
-0.530356768314804 -0.242214030180458
0.309063681711284 0.19409240942162
-0.164177094354206 0.453297690991889
-0.13767022329242 0.394100533265025
-0.398424319901931 0.502518162469089
0.215840404736243 0.300759121139268
-0.268879497084626 0.153637702923007
0.349383002174688 0.496809615116446
0.549892374025649 0.0799667281923469
-0.123829939490133 0.435114272260594
-0.474268361856033 0.0357716962036874
-0.646587480763243 -0.219594214976542
0.110362368431608 -0.345732268667796
-0.553724940685854 -0.155125731973659
-0.0668600759610034 0.471321034246695
0.267782386613508 0.509064915101577
0.362655199347001 -0.311498193705683
0.411387402538594 0.29541864178335
-0.609128029049169 0.11892628803397
-0.422091726421159 0.100431157659086
-0.210068403356338 0.360844624742739
0.211814687791418 0.4162688185051
0.606501529679284 -0.151127011361796
-0.458997889951178 0.17885874756933
-0.343618452572188 -0.462681328198656
-0.18536541234266 0.538919481826572
-0.267083515330365 0.385239844177514
-0.4422278461689 -0.277112911248985
0.466138810862589 -0.120212831688822
-0.0442612451389558 -0.515096597470398
0.495618141018324 -0.0123330135860214
-0.0246186929386839 -0.723660768376751
0.479558827941383 0.107060509580426
0.223988787569629 0.47368268018285
-0.12189404056388 0.584362435904357
0.196956881232256 0.601963522846129
0.268403357277996 0.409061433300255
-0.475873886223437 -0.171819525493092
-0.637560685972035 0.192699348171351
0.24944295430097 -0.288153559188196
-0.41661870238124 0.182181395719868
-0.207601555938646 0.366673424260585
0.0683745838642698 -0.286186637942586
0.480467454984935 0.0785819919731695
-0.258450840525091 -0.412544370798708
0.0628353252945851 -0.269795774068433
0.431822786848086 0.161599131032698
-0.453594377810562 0.0924891671095192
0.252612511898518 0.370647333358245
0.276361150228341 0.452205278844229
-0.266359694364844 -0.0685168075490342
0.359579116362363 0.0230668863873988
0.387929906183436 0.409287567481622
-0.0302996143146606 -0.658610254599892
0.496420594846919 0.315507787888864
-0.204393756270943 0.35410071512678
-0.359857265010909 0.449540450264946
0.334916606760666 0.434127284830558
0.36850784680697 5.89712891074234e-05
-0.22557144541024 0.29150250618984
0.538964265491542 -0.0818297848190963
0.121320008344019 0.548919055690194
-0.325588655305987 -0.317747123271412
0.560833859469707 0.238496680606436
0.328803958428271 0.477932233530414
0.360040826101695 0.475664951474128
0.358505930326469 -0.283469272636595
0.557634719095689 0.0943671362049456
0.0253155034892368 0.509402973451469
-0.341244558614516 0.565038475437037
0.306929044184662 0.506178486753292
0.0982923518710815 -0.61808642818759
-0.378120314648177 0.262294022367363
0.300580107933606 -0.367005755346478
-0.356959562752667 -0.0814044309417183
0.505100892033331 0.0139140952744013
0.201905484776313 -0.666149109984138
-0.317471828048833 0.58310071988629
0.642327144101007 -0.123523772308688
-0.0562380509438529 0.61281111110998
0.540115590381765 -0.120862329660969
-0.428126661205109 0.432141903202031
0.0654240467335425 -0.527055709208335
-0.223935312216881 -0.448032034699164
-0.0205244147160425 0.484415699670613
0.467780098096871 0.175785756463301
0.230714978966231 0.44118546853886
-0.113410222292677 0.503941074448889
0.357513627358345 -0.49309119271841
0.348970412594284 -0.463110265729721
0.753037172863299 0.250529932836822
-0.476604689558609 -0.121674342122082
-0.554599660726196 0.351572119594442
-0.430960254695099 -0.340593468662097
0.146256793466728 0.447482638836862
0.180589375014155 -0.433288468783537
-0.429460156870332 0.147992598323329
0.32117177650781 -0.350084635084539
-0.122208345211026 0.456540665996618
-0.367691113002475 -0.396149169939704
-0.229428311677906 -0.0969482384945651
-0.342185427428518 -0.0455006289537875
-0.434117994088126 -0.279214120015818
-0.31579661004487 -0.502034242921636
-0.306527309881809 -0.306107672660978
0.145566936303268 0.351566983213997
-0.450526760261162 -0.295351166828137
0.428755830129544 0.372074281585718
-0.277564975453605 -0.396527013863708
-0.292053839903166 0.496168432067604
0.564128590481272 0.054409464020619
0.670632988170413 0.331393221033137
-0.0638225227611708 0.533242265447673
-0.3695451919932 -0.0644415681728064
0.473202200899963 0.293717947391691
-0.0946460237856184 0.522835883344978
-0.243058009957978 -0.0762252338710816
-0.46580715849943 -0.191047484701008
-0.517747270192168 -0.12468534920288
-0.297097410005799 -0.453028299907626
-0.441196965336446 -0.0133115208436468
0.471299431567835 0.203566088788995
-0.051465197581915 0.511804429882268
0.351463102530632 -0.486904865513393
0.348340792234287 0.178302621217343
-0.0190465983681825 -0.483677154506801
-0.330111832364987 0.516052105079114
0.392971260446176 0.259886923751571
0.0863623712202173 -0.576915060584095
0.205118982721534 0.364479908135274
-0.0843297166275683 -0.683267565465375
0.585983722122448 -0.182252165410723
0.303495950694384 -0.199279408226489
0.487880550779967 -0.308588364651201
-0.293027994873903 -0.470074126178899
0.0289803848323107 0.639136032853364
0.260381854804875 0.525883338905617
-0.286827295258364 0.278369674431996
0.439008286075036 0.446596318156047
-0.534768057865252 -0.151743472253761
0.243132591985438 0.536067862554789
0.53214176725667 -0.223373972967633
0.197504759664772 0.434683250254921
-0.0206749479832579 -0.600828587834605
-0.450802777351254 0.346176945566329
-0.385437418632674 -0.315247122254874
-0.393019039670113 0.407387454206972
-0.375189901487411 -0.41198070610119
0.0580152369412027 -0.372343354076889
-0.0462908967101837 -0.580141456250303
0.394691579830127 0.289906160059099
-0.270884546492129 0.545006305204072
-0.430710703405778 0.097152564474768
0.390998918595693 0.0268172503115887
-0.193608044837987 -0.354971953965917
0.443836944412869 -0.393329666997989
0.103544572977438 -0.373703126044679
0.235899262226962 -0.333124938194722
0.327502779100172 0.390881505605721
-0.206576861808151 -0.506689178778846
-0.0920535511950847 -0.626805661501039
-0.143371623728386 -0.370808747126041
-0.0843327603629878 -0.645147306094757
0.222528703950953 0.514668514566031
0.429019945122778 -0.108943023029966
0.493265662433144 -0.068681422711857
0.418799574212017 -0.0473876669195105
-0.273217039475357 0.571130057715012
-0.0996300712397765 0.438500403085451
-0.0564782040280362 0.706873854238153
-0.353276069524669 0.347490833867532
0.00425197136282077 -0.391383553125414
0.413641958822472 -0.0212909504929675
-0.468926681609731 0.381685647063297
0.259887949845236 -0.197077889231461
-0.153870934709157 -0.420673766265942
-0.295048245757425 0.319893654364035
0.720006619053842 0.0704321989030551
0.505437181791754 -0.0493601406395091
0.182696062423845 -0.582482166824571
-0.352669879531478 0.259378859849267
-0.238999594717602 0.119804612364053
-0.504036401134316 -0.410921098477491
-0.252426020990876 0.346409830923312
0.407227518029239 0.334779444622287
-0.372151501749527 -0.238424485925228
-0.456458022994527 -0.13597808780873
0.531432967251139 -0.0625218437705367
-0.50829416684712 0.0560674506627171
0.092234190119111 -0.520323030764237
0.149107554052885 -0.444920882089844
0.53202707646777 0.0575724211525929
-0.454775413851123 0.0894157389727709
-0.583365790049323 0.0694064396227361
-0.190858093717286 0.452902719785554
-0.380953934499504 -0.478330949260321
0.146651942768558 0.583969369990677
-0.325057942628062 0.427557071489395
0.03187847517407 0.619003187044543
0.211394573667987 -0.352336308068538
-0.226239312520911 0.4912410400645
0.373855507991436 0.477266440554704
-0.127488588229167 -0.392616762020296
-0.304420866384988 -0.31511392108643
-0.318036687834423 -0.285619000223036
-0.0552353403722365 0.41685523989911
-0.317397705131187 -0.603044299846029
-0.321458780369313 0.0753740310112461
-0.356315375660538 0.200576073378276
-0.124622404223555 -0.469800262488081
0.261876148641493 -0.360950541532307
-0.13881993592241 -0.281984660286065
-0.474007401363882 -0.433946169820591
-0.49286983805463 0.320296203701078
-0.34144612023373 0.546014368235368
-0.454994571465 -0.392137118899902
0.205300040855632 -0.462600009764764
-0.0133410326106431 -0.489442890670948
-0.529103009719642 -0.0776925590243412
-0.356902619398569 -0.136199901356057
-0.570075546045202 -0.198880243899332
0.446346656066523 0.159347934531463
0.456450400978272 -0.212841903279097
0.572784097558224 0.422047587470337
0.142424144918129 -0.481949181486348
-0.578011208734588 -0.22008576706809
-0.402633335400584 0.379516453211849
0.194496025089533 -0.480350881798798
-0.370154725906058 -0.230967892889668
-0.276276191826277 0.35722618131214
-0.255247642855646 0.333948160196178
-0.345839630416853 0.0323030158493381
0.540718158235085 0.00522745642329364
0.0824220350017049 0.590822961124413
0.163201406372165 -0.347255213314656
-0.0781856196228909 0.452920898920107
-0.441173834604219 0.326460578134147
0.587619948925087 0.176845540542919
-0.279531251270546 0.145775721756054
-0.290460741750318 0.43012039162437
0.132285561424232 0.735613709692054
-0.428221169838963 -0.240622736933853
0.417035226150054 -0.156694720295775
0.164617466680964 0.364454883725263
-0.462397765625122 -0.160441564070423
0.238626364974342 -0.376763728109069
0.356092953302265 -0.420704183088197
-0.551868985913274 0.0102198599775207
0.57029582851551 0.384626123311752
-0.250593450627246 -0.606068767349413
-0.56352586023292 -0.046866124144406
0.399957584040677 -0.230543871957454
0.674759363698423 -0.123702216145201
0.384308483505981 0.0845238270232833
-0.547050949095754 0.180518991945395
0.63921374768211 0.0193526243825857
-0.550632934503122 -0.124606698110966
0.400067244900371 -0.323182074807407
0.505733007048789 0.0126180761424537
0.447841352377499 0.0171266702396127
-0.570693060048461 0.0345778899630767
0.178938244608687 0.452882463892337
0.571285811184245 -0.0287152148578778
-0.278955557328362 0.511189966097579
0.431327530519805 -0.320289522084613
0.507680673440946 -0.231759800921228
0.660398046818595 0.101643660588978
-0.411144993440451 0.599516049271225
-0.16459797698833 0.484851311627873
0.504820075516498 -0.0238028004246584
0.31753548430927 -0.406452659044909
0.322900721011058 -0.458569080887015
-0.386421183155924 0.413517310694218
0.0148489795391808 -0.56178944503547
0.423121749241213 -0.143380085115805
0.130005164945315 0.461361718983437
-0.411005219141576 0.19630547423267
-0.307927707673807 0.347697103570136
-0.16944735850482 -0.515632702245291
0.0261528405721493 -0.438097904385313
-0.342910360057714 0.342348226874299
0.404112106621508 0.181843507435474
0.307836938340197 -0.186452420734887
0.315661682775278 0.500909572837297
0.340114090470939 0.33429491135461
-0.266713761516251 -0.17644185796164
0.118999952961703 0.418838309498632
-0.29966398561714 -0.417916533704871
0.416411152199812 0.170570700393894
0.41307351045809 0.343700180226471
0.0897735294906907 0.520627706702621
-0.17797679525345 -0.34895155352597
0.370021813188669 0.206261742060509
-0.464302218920233 0.0426970075331302
0.382479753869525 -0.481763781214523
-0.414108717035251 -0.430814451108242
-0.0489137212297883 0.736374406180117
-0.480574947038865 -0.248619388078281
0.0186707447884163 -0.457258208186459
0.380237365202936 -0.470717820846587
0.0942438838394666 0.413800631568628
0.250807265233415 -0.427631619070493
-0.153202968370115 0.587186890118895
};
\addlegendentry{Class 2}




==> background/figures/toy_example.tex <==
% This file was created by tikzplotlib v0.9.8.

\tikzset{
  font={\fontsize{15pt}{12}\selectfont}}

%\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
%\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color0}{rgb}{0.5,0,0}
\definecolor{color1}{rgb}{0,0,0.5}




\begin{tikzpicture}[scale=0.5]

\begin{groupplot}[group style={group size=3 by 1, group name=toy example plots, horizontal sep =2cm,vertical sep =2cm}]
%\addplot graphics [includegraphics cmd=\pgfimage,xmin=-1.525, xmax=1.475, ymin=-1.525, ymax=1.475] {experiments/figures/raw_figures/circle_data_02.png};

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Dim 1},
xmin=-1.525, xmax=1.475,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Dim 2},
ylabel style={yshift=-0.4cm},
legend image post style={scale=8},
ymin=-1.525, ymax=1.475,
ytick style={color=black}
]

\input{background/figures/raw_figures/toy_data_2}

\nextgroupplot[
%colorbar,
%colorbar style={ylabel={}},
%colormap/viridis,
%point meta max=1,
%point meta min=0,
tick align=outside,
tick pos=left,
title={$f_0(x)$},
x grid style={white!69.0196078431373!black},
xlabel={Dim 1},
xmin=-1.525, xmax=1.475,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Dim 2},
ylabel style={yshift=-0.4cm},
ymin=-1.525, ymax=1.475,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-1.525, xmax=1.475, ymin=-1.525, ymax=1.475] {background/figures/raw_figures/uncertainty_plot_noise_0-000.png};


\nextgroupplot[
colorbar,
colorbar style={ylabel={}},
colormap/viridis,
point meta max=1,
point meta min=0,
tick align=outside,
tick pos=left,
title={$f_0(x)$},
x grid style={white!69.0196078431373!black},
xlabel={Dim 1},
xmin=-1.525, xmax=1.475,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Dim 2},
ylabel style={yshift=-0.4cm},
ymin=-1.525, ymax=1.475,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-1.525, xmax=1.475, ymin=-1.525, ymax=1.475] {background/figures/raw_figures/uncertainty_plot_noise_0.2-000.png};

\end{groupplot}
\end{tikzpicture}



==> experiments/figures/cce_0.tex <==
\addplot [semithick, color0]
table {%
0 0.0741600021719933
1 0.971560001373291
2 0.97952002286911
3 0.980359971523285
4 0.98581999540329
5 0.990960001945496
6 0.988139986991882
7 0.982659995555878
8 0.99125999212265
9 0.982900023460388
10 0.994220018386841
11 0.990819990634918
12 0.988160014152527
13 0.994260013103485
14 0.994599997997284
15 0.996840000152588
16 0.996959984302521
17 0.993920028209686
18 0.993879973888397
19 0.996900022029877
20 0.997080028057098
21 0.996900022029877
22 0.995500028133392
23 0.996659994125366
24 0.9964200258255
25 0.998579978942871
26 0.997380018234253
27 0.997399985790253
28 0.995999991893768
29 0.996720016002655
30 0.996379971504211
31 0.997420012950897
32 0.997179985046387
33 0.996840000152588
34 0.996399998664856
35 0.993539988994598
36 0.997200012207031
37 0.99592000246048
38 0.997640013694763
39 0.997680008411407
40 0.997560024261475
41 0.997219979763031
42 0.998239994049072
43 0.99345999956131
44 0.998319983482361
45 0.998920023441315
46 0.997039973735809
47 0.997420012950897
48 0.997959971427917
49 0.998820006847382
50 0.998600006103516
51 0.997820019721985
52 0.998520016670227
53 0.998300015926361
54 0.999059975147247
55 0.997099995613098
56 0.998960018157959
57 0.998440027236938
58 0.998780012130737
59 0.998099982738495
60 0.997919976711273
61 0.998860001564026
62 0.998319983482361
63 0.998820006847382
64 0.998279988765717
65 0.997560024261475
66 0.999319970607758
67 0.999019980430603
68 0.997619986534119
69 0.998619973659515
70 0.998759984970093
71 0.998799979686737
72 0.999440014362335
73 0.997820019721985
74 0.998440027236938
75 0.998480021953583
76 0.999419987201691
77 0.998080015182495
78 0.998459994792938
79 0.999180018901825
80 0.998120009899139
81 0.999239981174469
82 0.998619973659515
83 0.998799979686737
84 0.998459994792938
85 0.999080002307892
86 0.999180018901825
87 0.997659981250763
88 0.998420000076294
89 0.99728000164032
90 0.99889999628067
91 0.999400019645691
92 0.997640013694763
93 0.999440014362335
94 0.998660027980804
95 0.999379992485046
96 0.999339997768402
97 0.998820006847382
98 0.997940003871918
99 0.999279975891113
100 0.998920023441315
101 0.999300003051758
102 0.998939990997314
103 0.998679995536804
104 0.999100029468536
105 0.999520003795624
106 0.999400019645691
107 0.999239981174469
108 0.999180018901825
109 0.99915999174118
110 0.998480021953583
111 0.998359978199005
112 0.998480021953583
113 0.999440014362335
114 0.999520003795624
115 0.999700009822845
116 0.998700022697449
117 0.998160004615784
118 0.998660027980804
119 0.99975997209549
120 0.999260008335114
121 0.997659981250763
122 0.999719977378845
123 0.998759984970093
124 0.999100029468536
125 0.998939990997314
126 0.999379992485046
127 0.999199986457825
128 0.998539984226227
129 0.999239981174469
130 0.999100029468536
131 0.999339997768402
132 0.999199986457825
133 0.999520003795624
134 0.999319970607758
135 0.997879981994629
136 0.999520003795624
137 0.999180018901825
138 0.999480009078979
139 0.999180018901825
140 0.999700009822845
141 0.998099982738495
142 0.999819993972778
143 0.999260008335114
144 0.999580025672913
145 0.999620020389557
146 0.999520003795624
147 0.999419987201691
148 0.999279975891113
149 0.999679982662201
150 0.999140024185181
151 0.999080002307892
152 0.999319970607758
153 0.999360024929047
154 0.999459981918335
155 0.998979985713959
156 0.999520003795624
157 0.999459981918335
158 0.99974000453949
159 0.999339997768402
160 0.999440014362335
161 0.999499976634979
162 0.999400019645691
163 0.999360024929047
164 0.999620020389557
165 0.999700009822845
166 0.999220013618469
167 0.999480009078979
168 0.998560011386871
169 0.999719977378845
170 0.999819993972778
171 0.999719977378845
172 0.998960018157959
173 0.999239981174469
174 0.999639987945557
175 0.999939978122711
176 0.999679982662201
177 0.99888002872467
178 0.999379992485046
179 0.999559998512268
180 0.999599993228912
181 0.999719977378845
182 0.999260008335114
183 0.999319970607758
184 0.999499976634979
185 0.999800026416779
186 0.999260008335114
187 0.999719977378845
188 0.996840000152588
189 0.999260008335114
190 0.999459981918335
191 0.999679982662201
192 0.999779999256134
193 0.999559998512268
194 0.999700009822845
195 0.999559998512268
196 0.999100029468536
197 0.998780012130737
198 0.999119997024536
199 0.999599993228912
200 0.999599993228912
201 0.999700009822845
202 0.999260008335114
203 0.999880015850067
204 0.999580025672913
205 0.999620020389557
206 0.999300003051758
207 0.999660015106201
208 0.999379992485046
209 0.999700009822845
210 0.999719977378845
211 0.999059975147247
212 0.998979985713959
213 0.999639987945557
214 0.999620020389557
215 0.999679982662201
216 0.999859988689423
217 0.999719977378845
218 0.998220026493073
219 0.999620020389557
220 0.999679982662201
221 0.999899983406067
222 0.999480009078979
223 0.999800026416779
224 0.99974000453949
225 0.99915999174118
226 0.99974000453949
227 0.999639987945557
228 0.999559998512268
229 0.999960005283356
230 0.999639987945557
231 0.999199986457825
232 0.999620020389557
233 0.999599993228912
234 0.99975997209549
235 0.999279975891113
236 0.999520003795624
237 0.999800026416779
238 0.999440014362335
239 0.999840021133423
240 0.999880015850067
241 0.999559998512268
242 0.999100029468536
243 0.999859988689423
244 0.999539971351624
245 0.999779999256134
246 0.999180018901825
247 0.999520003795624
248 0.99974000453949
249 0.999679982662201
250 0.999000012874603
251 0.999440014362335
252 0.999779999256134
253 0.999920010566711
254 1
255 1
256 1
257 1
258 1
259 1
260 1
261 1
262 1
263 1
264 1
265 1
266 1
267 1
268 1
269 1
270 1
271 1
272 1
273 1
274 1
275 1
276 1
277 1
278 1
279 1
280 1
281 1
282 1
283 1
284 1
285 1
286 1
287 1
288 1
289 1
290 1
291 1
292 1
293 1
294 1
295 1
296 1
297 1
298 1
299 1
300 1
301 1
302 1
303 1
304 1
305 1
306 1
307 1
308 1
309 1
310 1
311 1
312 1
313 1
314 1
315 1
316 1
317 1
318 1
319 1
320 1
321 1
322 1
323 1
324 1
325 1
326 1
327 1
328 1
329 1
330 1
331 1
332 1
333 1
334 1
335 1
336 1
337 1
338 1
339 1
340 1
341 1
342 1
343 1
344 1
345 1
346 1
347 1
348 1
349 1
350 1
351 1
352 1
353 1
354 1
355 1
356 1
357 1
358 1
359 1
360 1
361 1
362 1
363 1
364 1
365 1
366 1
367 1
368 1
369 1
370 1
371 1
372 1
373 1
374 1
375 1
376 1
377 1
378 1
379 1
380 1
381 1
382 1
383 1
384 1
385 1
386 1
387 1
388 1
389 1
390 1
391 1
392 1
393 1
394 1
395 1
396 1
397 1
398 1
399 1
400 1
401 1
402 1
403 1
404 1
405 1
406 1
407 1
408 1
409 1
410 1
411 1
412 1
413 1
414 1
415 1
416 1
417 1
418 1
419 1
420 1
421 1
422 1
423 1
424 1
425 1
426 1
427 1
428 1
429 1
430 1
431 1
432 1
433 1
434 1
435 1
436 1
437 1
438 1
439 1
440 1
441 1
442 1
443 1
444 1
445 1
446 1
447 1
448 1
449 1
450 1
451 1
452 1
453 1
454 1
455 1
456 1
457 1
458 1
459 1
460 1
461 1
462 1
463 1
464 1
465 1
466 1
467 1
468 1
469 1
470 1
471 1
472 1
473 1
474 1
475 1
476 1
477 1
478 1
479 1
480 1
481 1
482 1
483 1
484 1
485 1
486 1
487 1
488 1
489 1
490 1
491 1
492 1
493 1
494 1
495 1
496 1
497 1
498 1
499 1
500 1
};
\addlegendentry{Train}

\addplot [semithick, color1]
table {%
0 0.0762000009417534
1 0.969099998474121
2 0.969399988651276
3 0.971000015735626
4 0.970600008964539
5 0.976000010967255
6 0.972699999809265
7 0.967000007629395
8 0.975799977779388
9 0.966499984264374
10 0.976199984550476
11 0.972299993038177
12 0.968299984931946
13 0.975399971008301
14 0.976300001144409
15 0.978900015354156
16 0.97790002822876
17 0.977299988269806
18 0.979499995708466
19 0.978999972343445
20 0.976700007915497
21 0.978200018405914
22 0.978200018405914
23 0.97869998216629
24 0.977800011634827
25 0.979900002479553
26 0.979300022125244
27 0.978200018405914
28 0.975899994373322
29 0.977199971675873
30 0.975799977779388
31 0.976700007915497
32 0.978399991989136
33 0.977100014686584
34 0.976199984550476
35 0.973599970340729
36 0.980000019073486
37 0.976999998092651
38 0.978100001811981
39 0.978999972343445
40 0.978500008583069
41 0.978799998760223
42 0.979700028896332
43 0.97460001707077
44 0.980000019073486
45 0.980599999427795
46 0.978299975395203
47 0.976599991321564
48 0.97869998216629
49 0.980099976062775
50 0.979499995708466
51 0.980599999427795
52 0.97979998588562
53 0.980400025844574
54 0.98199999332428
55 0.97869998216629
56 0.97979998588562
57 0.980300009250641
58 0.978399991989136
59 0.980300009250641
60 0.979399979114532
61 0.980099976062775
62 0.977800011634827
63 0.980099976062775
64 0.976599991321564
65 0.97759997844696
66 0.981299996376038
67 0.980400025844574
68 0.979099988937378
69 0.981100022792816
70 0.980300009250641
71 0.97979998588562
72 0.980499982833862
73 0.979700028896332
74 0.977800011634827
75 0.97979998588562
76 0.980199992656708
77 0.979099988937378
78 0.978500008583069
79 0.980199992656708
80 0.97790002822876
81 0.979900002479553
82 0.978100001811981
83 0.97869998216629
84 0.980000019073486
85 0.979499995708466
86 0.980199992656708
87 0.977699995040894
88 0.977100014686584
89 0.978200018405914
90 0.980599999427795
91 0.979200005531311
92 0.977699995040894
93 0.981800019741058
94 0.980400025844574
95 0.980400025844574
96 0.979700028896332
97 0.980300009250641
98 0.976599991321564
99 0.978399991989136
100 0.979200005531311
101 0.978100001811981
102 0.978799998760223
103 0.978200018405914
104 0.978200018405914
105 0.980099976062775
106 0.981100022792816
107 0.979600012302399
108 0.98089998960495
109 0.978799998760223
110 0.978799998760223
111 0.980000019073486
112 0.977500021457672
113 0.980400025844574
114 0.980000019073486
115 0.980799973011017
116 0.979600012302399
117 0.978500008583069
118 0.980400025844574
119 0.980700016021729
120 0.980400025844574
121 0.979700028896332
122 0.982699990272522
123 0.980099976062775
124 0.980000019073486
125 0.979499995708466
126 0.980400025844574
127 0.98089998960495
128 0.979200005531311
129 0.979700028896332
130 0.978399991989136
131 0.980599999427795
132 0.979700028896332
133 0.981100022792816
134 0.979900002479553
135 0.97759997844696
136 0.980799973011017
137 0.977699995040894
138 0.98089998960495
139 0.978500008583069
140 0.98089998960495
141 0.978900015354156
142 0.981000006198883
143 0.979700028896332
144 0.979499995708466
145 0.980400025844574
146 0.980300009250641
147 0.98089998960495
148 0.979399979114532
149 0.981400012969971
150 0.980799973011017
151 0.980099976062775
152 0.980199992656708
153 0.980599999427795
154 0.981700003147125
155 0.978500008583069
156 0.978200018405914
157 0.981000006198883
158 0.981299996376038
159 0.980499982833862
160 0.981199979782104
161 0.981199979782104
162 0.979600012302399
163 0.981100022792816
164 0.981100022792816
165 0.980599999427795
166 0.981700003147125
167 0.980700016021729
168 0.978100001811981
169 0.981500029563904
170 0.981400012969971
171 0.981800019741058
172 0.981299996376038
173 0.979600012302399
174 0.981299996376038
175 0.981700003147125
176 0.980400025844574
177 0.979300022125244
178 0.979700028896332
179 0.980099976062775
180 0.98089998960495
181 0.980300009250641
182 0.980099976062775
183 0.98089998960495
184 0.979600012302399
185 0.981000006198883
186 0.979499995708466
187 0.980700016021729
188 0.977699995040894
189 0.979600012302399
190 0.980799973011017
191 0.981100022792816
192 0.982800006866455
193 0.981199979782104
194 0.980799973011017
195 0.98089998960495
196 0.979099988937378
197 0.979399979114532
198 0.981800019741058
199 0.982500016689301
200 0.982999980449677
201 0.981400012969971
202 0.981100022792816
203 0.982699990272522
204 0.980799973011017
205 0.980799973011017
206 0.978100001811981
207 0.980799973011017
208 0.981000006198883
209 0.981299996376038
210 0.981899976730347
211 0.980000019073486
212 0.979700028896332
213 0.981100022792816
214 0.980599999427795
215 0.981400012969971
216 0.981500029563904
217 0.982200026512146
218 0.976400017738342
219 0.981199979782104
220 0.981500029563904
221 0.981700003147125
222 0.981599986553192
223 0.981000006198883
224 0.981500029563904
225 0.981400012969971
226 0.981100022792816
227 0.980700016021729
228 0.981800019741058
229 0.983200013637543
230 0.981400012969971
231 0.978399991989136
232 0.979399979114532
233 0.980700016021729
234 0.981500029563904
235 0.979900002479553
236 0.981899976730347
237 0.981800019741058
238 0.981299996376038
239 0.981500029563904
240 0.982999980449677
241 0.982699990272522
242 0.980799973011017
243 0.981800019741058
244 0.980700016021729
245 0.981800019741058
246 0.978399991989136
247 0.979200005531311
248 0.980400025844574
249 0.979900002479553
250 0.97979998588562
251 0.980099976062775
252 0.980499982833862
253 0.98089998960495
254 0.981599986553192
255 0.981500029563904
256 0.981500029563904
257 0.981500029563904
258 0.981500029563904
259 0.981500029563904
260 0.981500029563904
261 0.981500029563904
262 0.981500029563904
263 0.981500029563904
264 0.981599986553192
265 0.981599986553192
266 0.981599986553192
267 0.981599986553192
268 0.981599986553192
269 0.981599986553192
270 0.981599986553192
271 0.981599986553192
272 0.981599986553192
273 0.981599986553192
274 0.981599986553192
275 0.981599986553192
276 0.981599986553192
277 0.981599986553192
278 0.981599986553192
279 0.981599986553192
280 0.981599986553192
281 0.981599986553192
282 0.981599986553192
283 0.981599986553192
284 0.981599986553192
285 0.981599986553192
286 0.981599986553192
287 0.981599986553192
288 0.981599986553192
289 0.981599986553192
290 0.981599986553192
291 0.981599986553192
292 0.981599986553192
293 0.981599986553192
294 0.981599986553192
295 0.981599986553192
296 0.981599986553192
297 0.981599986553192
298 0.981599986553192
299 0.981599986553192
300 0.981599986553192
301 0.981599986553192
302 0.981599986553192
303 0.981599986553192
304 0.981599986553192
305 0.981599986553192
306 0.981500029563904
307 0.981500029563904
308 0.981500029563904
309 0.981500029563904
310 0.981500029563904
311 0.981500029563904
312 0.981500029563904
313 0.981500029563904
314 0.981500029563904
315 0.981500029563904
316 0.981500029563904
317 0.981500029563904
318 0.981500029563904
319 0.981500029563904
320 0.981500029563904
321 0.981500029563904
322 0.981500029563904
323 0.981500029563904
324 0.981500029563904
325 0.981500029563904
326 0.981400012969971
327 0.981400012969971
328 0.981400012969971
329 0.981400012969971
330 0.981400012969971
331 0.981400012969971
332 0.981400012969971
333 0.981400012969971
334 0.981400012969971
335 0.981400012969971
336 0.981400012969971
337 0.981400012969971
338 0.981400012969971
339 0.981400012969971
340 0.981400012969971
341 0.981400012969971
342 0.981400012969971
343 0.981400012969971
344 0.981400012969971
345 0.981400012969971
346 0.981400012969971
347 0.981400012969971
348 0.981400012969971
349 0.981400012969971
350 0.981400012969971
351 0.981400012969971
352 0.981400012969971
353 0.981400012969971
354 0.981400012969971
355 0.981400012969971
356 0.981400012969971
357 0.981400012969971
358 0.981400012969971
359 0.981400012969971
360 0.981400012969971
361 0.981400012969971
362 0.981400012969971
363 0.981400012969971
364 0.981400012969971
365 0.981400012969971
366 0.981400012969971
367 0.981400012969971
368 0.981400012969971
369 0.981400012969971
370 0.981400012969971
371 0.981400012969971
372 0.981400012969971
373 0.981400012969971
374 0.981400012969971
375 0.981400012969971
376 0.981400012969971
377 0.981400012969971
378 0.981400012969971
379 0.981400012969971
380 0.981400012969971
381 0.981400012969971
382 0.981400012969971
383 0.981400012969971
384 0.981400012969971
385 0.981400012969971
386 0.981400012969971
387 0.981400012969971
388 0.981400012969971
389 0.981400012969971
390 0.981400012969971
391 0.981400012969971
392 0.981400012969971
393 0.981400012969971
394 0.981400012969971
395 0.981400012969971
396 0.981400012969971
397 0.981400012969971
398 0.981400012969971
399 0.981400012969971
400 0.981400012969971
401 0.981400012969971
402 0.981400012969971
403 0.981400012969971
404 0.981400012969971
405 0.981400012969971
406 0.981400012969971
407 0.981400012969971
408 0.981400012969971
409 0.981400012969971
410 0.981400012969971
411 0.981400012969971
412 0.981400012969971
413 0.981400012969971
414 0.981400012969971
415 0.981400012969971
416 0.981400012969971
417 0.981400012969971
418 0.981400012969971
419 0.981400012969971
420 0.981400012969971
421 0.981400012969971
422 0.981400012969971
423 0.981400012969971
424 0.981400012969971
425 0.981400012969971
426 0.981400012969971
427 0.981400012969971
428 0.981400012969971
429 0.981400012969971
430 0.981400012969971
431 0.981400012969971
432 0.981400012969971
433 0.981400012969971
434 0.981400012969971
435 0.981400012969971
436 0.981400012969971
437 0.981400012969971
438 0.981400012969971
439 0.981400012969971
440 0.981400012969971
441 0.981400012969971
442 0.981400012969971
443 0.981400012969971
444 0.981400012969971
445 0.981400012969971
446 0.981400012969971
447 0.981400012969971
448 0.981400012969971
449 0.981400012969971
450 0.981400012969971
451 0.981400012969971
452 0.981400012969971
453 0.981400012969971
454 0.981400012969971
455 0.981400012969971
456 0.981400012969971
457 0.981400012969971
458 0.981400012969971
459 0.981400012969971
460 0.981400012969971
461 0.981400012969971
462 0.981400012969971
463 0.981400012969971
464 0.981400012969971
465 0.981400012969971
466 0.981400012969971
467 0.981400012969971
468 0.981400012969971
469 0.981400012969971
470 0.981400012969971
471 0.981400012969971
472 0.981400012969971
473 0.981400012969971
474 0.981400012969971
475 0.981400012969971
476 0.981400012969971
477 0.981400012969971
478 0.981400012969971
479 0.981400012969971
480 0.981400012969971
481 0.981400012969971
482 0.981400012969971
483 0.981400012969971
484 0.981400012969971
485 0.981400012969971
486 0.981400012969971
487 0.981400012969971
488 0.981400012969971
489 0.981400012969971
490 0.981400012969971
491 0.981400012969971
492 0.981400012969971
493 0.981400012969971
494 0.981400012969971
495 0.981400012969971
496 0.981400012969971
497 0.981400012969971
498 0.981400012969971
499 0.981400012969971
500 0.981400012969971
};
\addlegendentry{Test}

==> experiments/figures/cce_03.tex <==
\addplot [semithick, color2]
table {%
0 0.115860000252724
1 0.66482001543045
2 0.675119996070862
3 0.680060029029846
4 0.682600021362305
5 0.683000028133392
6 0.686760008335114
7 0.686760008335114
8 0.690439999103546
9 0.692340016365051
10 0.701719999313354
11 0.702899992465973
12 0.70550000667572
13 0.709280014038086
14 0.716480016708374
15 0.719879984855652
16 0.724439978599548
17 0.73445999622345
18 0.735840022563934
19 0.739759981632233
20 0.746659994125366
21 0.751439988613129
22 0.759819984436035
23 0.763620018959045
24 0.763379991054535
25 0.769620001316071
26 0.771440029144287
27 0.776419997215271
28 0.786819994449615
29 0.785179972648621
30 0.790719985961914
31 0.796459972858429
32 0.794939994812012
33 0.806739985942841
34 0.808399975299835
35 0.814459979534149
36 0.819519996643066
37 0.822099983692169
38 0.824699997901917
39 0.828140020370483
40 0.824500024318695
41 0.831820011138916
42 0.832260012626648
43 0.838540017604828
44 0.836860001087189
45 0.832199990749359
46 0.844600021839142
47 0.84332001209259
48 0.845679998397827
49 0.847679972648621
50 0.851320028305054
51 0.854160010814667
52 0.853540003299713
53 0.857940018177032
54 0.861140012741089
55 0.860580027103424
56 0.867560029029846
57 0.868260025978088
58 0.87007999420166
59 0.867079973220825
60 0.863820016384125
61 0.872039973735809
62 0.874679982662201
63 0.870980024337769
64 0.871680021286011
65 0.879859983921051
66 0.874480009078979
67 0.880620002746582
68 0.880259990692139
69 0.873820006847382
70 0.88102000951767
71 0.881619989871979
72 0.877960026264191
73 0.889980018138885
74 0.895699977874756
75 0.882879972457886
76 0.889999985694885
77 0.892899990081787
78 0.891499996185303
79 0.894079983234406
80 0.890060007572174
81 0.894559979438782
82 0.888059973716736
83 0.900240004062653
84 0.888339996337891
85 0.896019995212555
86 0.889859974384308
87 0.884859979152679
88 0.906279981136322
89 0.897539973258972
90 0.8957399725914
91 0.90122002363205
92 0.900839984416962
93 0.900439977645874
94 0.908959984779358
95 0.906859993934631
96 0.902819991111755
97 0.898060023784637
98 0.90446001291275
99 0.909699976444244
100 0.904919981956482
101 0.91158002614975
102 0.903880000114441
103 0.909479975700378
104 0.906599998474121
105 0.909600019454956
106 0.910239994525909
107 0.91567999124527
108 0.900740027427673
109 0.91346001625061
110 0.907440006732941
111 0.906080007553101
112 0.914780020713806
113 0.916299998760223
114 0.916320025920868
115 0.912580013275146
116 0.917119979858398
117 0.912559986114502
118 0.912479996681213
119 0.9132199883461
120 0.915059983730316
121 0.91509997844696
122 0.915880024433136
123 0.914260029792786
124 0.920799970626831
125 0.922720015048981
126 0.924799978733063
127 0.916459977626801
128 0.923659980297089
129 0.920220017433167
130 0.92273998260498
131 0.926100015640259
132 0.917879998683929
133 0.920700013637543
134 0.925260007381439
135 0.923740029335022
136 0.926819980144501
137 0.92246001958847
138 0.934220016002655
139 0.917779982089996
140 0.925639986991882
141 0.929000020027161
142 0.925180017948151
143 0.928619980812073
144 0.922280013561249
145 0.928359985351562
146 0.916920006275177
147 0.927219986915588
148 0.931180000305176
149 0.932780027389526
150 0.912360012531281
151 0.932380020618439
152 0.926999986171722
153 0.932739973068237
154 0.933560013771057
155 0.927799999713898
156 0.92246001958847
157 0.931079983711243
158 0.927720010280609
159 0.932479977607727
160 0.940720021724701
161 0.923720002174377
162 0.934819996356964
163 0.933640003204346
164 0.933659970760345
165 0.93010002374649
166 0.943379998207092
167 0.933340013027191
168 0.937839984893799
169 0.919539988040924
170 0.937940001487732
171 0.936879992485046
172 0.928879976272583
173 0.932600021362305
174 0.933080017566681
175 0.940559983253479
176 0.938480019569397
177 0.929139971733093
178 0.932680010795593
179 0.938740015029907
180 0.9410799741745
181 0.935519993305206
182 0.931460022926331
183 0.946879982948303
184 0.928080022335052
185 0.926060020923615
186 0.930620014667511
187 0.944419980049133
188 0.941699981689453
189 0.945119976997375
190 0.941460013389587
191 0.930819988250732
192 0.934379994869232
193 0.945259988307953
194 0.941259980201721
195 0.942099988460541
196 0.941619992256165
197 0.941500008106232
198 0.942219972610474
199 0.943639993667603
200 0.941460013389587
201 0.94021999835968
202 0.941940009593964
203 0.938300013542175
204 0.936020016670227
205 0.946020007133484
206 0.943400025367737
207 0.938920021057129
208 0.947040021419525
209 0.942120015621185
210 0.941120028495789
211 0.943679988384247
212 0.942579984664917
213 0.944180011749268
214 0.935379981994629
215 0.950020015239716
216 0.94489997625351
217 0.952419996261597
218 0.943120002746582
219 0.949079990386963
220 0.941519975662231
221 0.948279976844788
222 0.938499987125397
223 0.948920011520386
224 0.948339998722076
225 0.947099983692169
226 0.948019981384277
227 0.952359974384308
228 0.940699994564056
229 0.945800006389618
230 0.946820020675659
231 0.948599994182587
232 0.952319979667664
233 0.938260018825531
234 0.946039974689484
235 0.952939987182617
236 0.945559978485107
237 0.947359979152679
238 0.947139978408813
239 0.942499995231628
240 0.94811999797821
241 0.944079995155334
242 0.947660028934479
243 0.946039974689484
244 0.951740026473999
245 0.94514000415802
246 0.946799993515015
247 0.953140020370483
248 0.950839996337891
249 0.953239977359772
250 0.948539972305298
251 0.956439971923828
252 0.94539999961853
253 0.95253998041153
254 0.94242000579834
255 0.953339993953705
256 0.95550000667572
257 0.944920003414154
258 0.946139991283417
259 0.952960014343262
260 0.943840026855469
261 0.956520020961761
262 0.954739987850189
263 0.945339977741241
264 0.953740000724792
265 0.94378000497818
266 0.951759994029999
267 0.951799988746643
268 0.956160008907318
269 0.958440005779266
270 0.95907998085022
271 0.953599989414215
272 0.948539972305298
273 0.955219984054565
274 0.947499990463257
275 0.955699980258942
276 0.950760006904602
277 0.953199982643127
278 0.95525997877121
279 0.949079990386963
280 0.947719991207123
281 0.958079993724823
282 0.956780016422272
283 0.959999978542328
284 0.954639971256256
285 0.954919993877411
286 0.947539985179901
287 0.947700023651123
288 0.959940016269684
289 0.950839996337891
290 0.95304000377655
291 0.954180002212524
292 0.956179976463318
293 0.952979981899261
294 0.962999999523163
295 0.952499985694885
296 0.947080016136169
297 0.954320013523102
298 0.957520008087158
299 0.94760000705719
300 0.960300028324127
301 0.959360003471375
302 0.955060005187988
303 0.959020018577576
304 0.958500027656555
305 0.953480005264282
306 0.960060000419617
307 0.960600018501282
308 0.959119975566864
309 0.947499990463257
310 0.960720002651215
311 0.961080014705658
312 0.964119970798492
313 0.959219992160797
314 0.956759989261627
315 0.94651997089386
316 0.969640016555786
317 0.959379971027374
318 0.954320013523102
319 0.946979999542236
320 0.957520008087158
321 0.955799996852875
322 0.960280001163483
323 0.960200011730194
324 0.949679970741272
325 0.955699980258942
326 0.959259986877441
327 0.962119996547699
328 0.95168000459671
329 0.958920001983643
330 0.95770001411438
331 0.954299986362457
332 0.960460007190704
333 0.967559993267059
334 0.952180027961731
335 0.96205997467041
336 0.961679995059967
337 0.954720020294189
338 0.955380022525787
339 0.961820006370544
340 0.965539991855621
341 0.961880028247833
342 0.95797997713089
343 0.963739991188049
344 0.950739979743958
345 0.953580021858215
346 0.960919976234436
347 0.968159973621368
348 0.95634001493454
349 0.955959975719452
350 0.951919972896576
351 0.961359977722168
352 0.966199994087219
353 0.968360006809235
354 0.964119970798492
355 0.962679982185364
356 0.961399972438812
357 0.968819975852966
358 0.96289998292923
359 0.961960017681122
360 0.960240006446838
361 0.966300010681152
362 0.961920022964478
363 0.942799985408783
364 0.967140018939972
365 0.96833997964859
366 0.96288001537323
367 0.959819972515106
368 0.953939974308014
369 0.955680012702942
370 0.964900016784668
371 0.960539996623993
372 0.948620021343231
373 0.965680003166199
374 0.968819975852966
375 0.960739970207214
376 0.958819985389709
377 0.96204000711441
378 0.96425998210907
379 0.958739995956421
380 0.966820001602173
381 0.965279996395111
382 0.952279984951019
383 0.967480003833771
384 0.960060000419617
385 0.960640013217926
386 0.958259999752045
387 0.96095997095108
388 0.973360002040863
389 0.952740013599396
390 0.965120017528534
391 0.969579994678497
392 0.960399985313416
393 0.9689000248909
394 0.966239988803864
395 0.966880023479462
396 0.969980001449585
397 0.96644002199173
398 0.964699983596802
399 0.968659996986389
400 0.966319978237152
401 0.966840028762817
402 0.963540017604828
403 0.963580012321472
404 0.964559972286224
405 0.966759979724884
406 0.963299989700317
407 0.971000015735626
408 0.971040010452271
409 0.959479987621307
410 0.955399990081787
411 0.967360019683838
412 0.966000020503998
413 0.95958000421524
414 0.964100003242493
415 0.971180021762848
416 0.967499971389771
417 0.964760005474091
418 0.964640021324158
419 0.956979990005493
420 0.963259994983673
421 0.9721400141716
422 0.969640016555786
423 0.961660027503967
424 0.96399998664856
425 0.966380000114441
426 0.967700004577637
427 0.967719972133636
428 0.965480029582977
429 0.96780002117157
430 0.969479978084564
431 0.964179992675781
432 0.964980006217957
433 0.97163999080658
434 0.970160007476807
435 0.970399975776672
436 0.957679986953735
437 0.961860001087189
438 0.96508002281189
439 0.973360002040863
440 0.970640003681183
441 0.968100011348724
442 0.9689000248909
443 0.9685999751091
444 0.963079988956451
445 0.967779994010925
446 0.965659976005554
447 0.973439991474152
448 0.971119999885559
449 0.962979972362518
450 0.962140023708344
451 0.96917998790741
452 0.9721599817276
453 0.970459997653961
454 0.966840028762817
455 0.964439988136292
456 0.97325998544693
457 0.972840011119843
458 0.964619994163513
459 0.974640011787415
460 0.969579994678497
461 0.967180013656616
462 0.966279983520508
463 0.966920018196106
464 0.972880005836487
465 0.975780010223389
466 0.9721599817276
467 0.968819975852966
468 0.96780002117157
469 0.960479974746704
470 0.9685999751091
471 0.970439970493317
472 0.967559993267059
473 0.978760004043579
474 0.95770001411438
475 0.970220029354095
476 0.970459997653961
477 0.9685999751091
478 0.967119991779327
479 0.969560027122498
480 0.967840015888214
481 0.967400014400482
482 0.972800016403198
483 0.967440009117126
484 0.969900012016296
485 0.968519985675812
486 0.974420011043549
487 0.968219995498657
488 0.953159987926483
489 0.963739991188049
490 0.969600021839142
491 0.965979993343353
492 0.962920010089874
493 0.973819971084595
494 0.97052001953125
495 0.966579973697662
496 0.975340008735657
497 0.967499971389771
498 0.969659984111786
499 0.972479999065399
500 0.970759987831116
};
\addplot [semithick, color3]
table {%
0 0.122100003063679
1 0.941699981689453
2 0.952899992465973
3 0.95770001411438
4 0.957799971103668
5 0.950399994850159
6 0.95440000295639
7 0.947399973869324
8 0.93529999256134
9 0.931900024414062
10 0.939199984073639
11 0.933099985122681
12 0.918600022792816
13 0.918200016021729
14 0.919700026512146
15 0.911099970340729
16 0.901099979877472
17 0.893400013446808
18 0.89709997177124
19 0.878400027751923
20 0.882700026035309
21 0.871999979019165
22 0.878199994564056
23 0.860499978065491
24 0.854099988937378
25 0.850300014019012
26 0.83569997549057
27 0.843200027942657
28 0.828499972820282
29 0.822099983692169
30 0.828800022602081
31 0.814899981021881
32 0.830200016498566
33 0.83160001039505
34 0.808700025081635
35 0.811500012874603
36 0.830699980258942
37 0.820800006389618
38 0.812099993228912
39 0.802299976348877
40 0.796999990940094
41 0.794399976730347
42 0.789099991321564
43 0.790799975395203
44 0.796899974346161
45 0.77649998664856
46 0.800899982452393
47 0.787299990653992
48 0.787400007247925
49 0.793099999427795
50 0.78219997882843
51 0.771499991416931
52 0.772300004959106
53 0.785600006580353
54 0.760800004005432
55 0.767799973487854
56 0.791899979114532
57 0.785399973392487
58 0.768299996852875
59 0.761699974536896
60 0.762799978256226
61 0.77700001001358
62 0.761099994182587
63 0.756500005722046
64 0.775200009346008
65 0.767899990081787
66 0.762499988079071
67 0.746599972248077
68 0.751299977302551
69 0.745899975299835
70 0.751800000667572
71 0.7567999958992
72 0.737100005149841
73 0.755200028419495
74 0.75330001115799
75 0.743499994277954
76 0.744799971580505
77 0.737900018692017
78 0.755999982357025
79 0.736500024795532
80 0.750100016593933
81 0.740599989891052
82 0.732599973678589
83 0.737900018692017
84 0.735099971294403
85 0.726100027561188
86 0.739700019359589
87 0.731199979782104
88 0.746299982070923
89 0.725199997425079
90 0.73769998550415
91 0.740100026130676
92 0.742799997329712
93 0.730499982833862
94 0.73769998550415
95 0.748300015926361
96 0.736199975013733
97 0.712100028991699
98 0.735000014305115
99 0.728600025177002
100 0.723399996757507
101 0.736100018024445
102 0.727199971675873
103 0.717400014400482
104 0.716499984264374
105 0.74099999666214
106 0.736999988555908
107 0.737600028514862
108 0.697000026702881
109 0.730499982833862
110 0.722100019454956
111 0.720000028610229
112 0.721000015735626
113 0.732400000095367
114 0.731000006198883
115 0.725600004196167
116 0.728200018405914
117 0.716099977493286
118 0.708299994468689
119 0.721800029277802
120 0.68970000743866
121 0.706300020217896
122 0.708299994468689
123 0.715300023555756
124 0.722599983215332
125 0.71340000629425
126 0.735300004482269
127 0.70880001783371
128 0.718800008296967
129 0.711000025272369
130 0.73360002040863
131 0.725000023841858
132 0.709999978542328
133 0.710600018501282
134 0.693199992179871
135 0.731000006198883
136 0.709100008010864
137 0.720899999141693
138 0.721199989318848
139 0.716600000858307
140 0.70880001783371
141 0.723999977111816
142 0.700500011444092
143 0.706799983978271
144 0.70550000667572
145 0.710600018501282
146 0.693599998950958
147 0.71069997549057
148 0.689999997615814
149 0.717000007629395
150 0.698099970817566
151 0.703100025653839
152 0.712599992752075
153 0.694599986076355
154 0.704100012779236
155 0.703199982643127
156 0.703499972820282
157 0.709100008010864
158 0.717499971389771
159 0.704699993133545
160 0.700900018215179
161 0.697799980640411
162 0.707199990749359
163 0.700999975204468
164 0.70389997959137
165 0.715200006961823
166 0.700999975204468
167 0.702300012111664
168 0.704200029373169
169 0.682500004768372
170 0.697300016880035
171 0.706700026988983
172 0.678300023078918
173 0.715200006961823
174 0.699400007724762
175 0.709699988365173
176 0.705600023269653
177 0.702499985694885
178 0.695800006389618
179 0.704100012779236
180 0.691900014877319
181 0.68970000743866
182 0.679099977016449
183 0.711600005626678
184 0.667400002479553
185 0.699599981307983
186 0.684899985790253
187 0.695299983024597
188 0.700299978256226
189 0.707499980926514
190 0.697099983692169
191 0.682299971580505
192 0.70959997177124
193 0.703700006008148
194 0.688199996948242
195 0.69650000333786
196 0.703000009059906
197 0.703000009059906
198 0.699999988079071
199 0.699999988079071
200 0.712199985980988
201 0.709500014781952
202 0.6942999958992
203 0.686200022697449
204 0.697300016880035
205 0.695599973201752
206 0.697300016880035
207 0.699100017547607
208 0.707000017166138
209 0.711300015449524
210 0.705399990081787
211 0.690599977970123
212 0.693300008773804
213 0.697099983692169
214 0.691799998283386
215 0.706300020217896
216 0.685899972915649
217 0.697899997234344
218 0.705999970436096
219 0.689400017261505
220 0.697000026702881
221 0.69539999961853
222 0.700399994850159
223 0.691299974918365
224 0.712199985980988
225 0.689999997615814
226 0.704299986362457
227 0.693499982357025
228 0.697200000286102
229 0.689400017261505
230 0.690100014209747
231 0.690400004386902
232 0.697499990463257
233 0.685400009155273
234 0.698199987411499
235 0.708899974822998
236 0.691999971866608
237 0.690599977970123
238 0.690900027751923
239 0.685100018978119
240 0.693300008773804
241 0.706200003623962
242 0.724399983882904
243 0.706300020217896
244 0.696900010108948
245 0.672500014305115
246 0.693499982357025
247 0.697799980640411
248 0.688199996948242
249 0.697399973869324
250 0.691900014877319
251 0.693700015544891
252 0.694700002670288
253 0.693300008773804
254 0.691600024700165
255 0.692799985408783
256 0.70880001783371
257 0.693300008773804
258 0.691399991512299
259 0.694000005722046
260 0.691299974918365
261 0.68010002374649
262 0.703400015830994
263 0.689400017261505
264 0.699999988079071
265 0.683899998664856
266 0.690900027751923
267 0.681900024414062
268 0.684599995613098
269 0.68529999256134
270 0.691200017929077
271 0.697200000286102
272 0.699999988079071
273 0.699500024318695
274 0.685400009155273
275 0.689000010490417
276 0.679700016975403
277 0.687200009822845
278 0.687200009822845
279 0.685500025749207
280 0.694800019264221
281 0.686500012874603
282 0.693899989128113
283 0.69489997625351
284 0.683899998664856
285 0.687900006771088
286 0.676400005817413
287 0.677299976348877
288 0.701600015163422
289 0.674799978733063
290 0.685199975967407
291 0.676699995994568
292 0.685999989509583
293 0.689100027084351
294 0.690500020980835
295 0.692099988460541
296 0.681400001049042
297 0.676800012588501
298 0.687099993228912
299 0.681599974632263
300 0.694700002670288
301 0.686299979686737
302 0.690400004386902
303 0.700500011444092
304 0.691900014877319
305 0.682500004768372
306 0.691200017929077
307 0.703999996185303
308 0.684099972248077
309 0.690900027751923
310 0.672900021076202
311 0.691900014877319
312 0.690599977970123
313 0.682200014591217
314 0.685800015926361
315 0.665899991989136
316 0.694500029087067
317 0.694400012493134
318 0.692700028419495
319 0.68860000371933
320 0.699599981307983
321 0.6942999958992
322 0.702000021934509
323 0.693599998950958
324 0.690599977970123
325 0.685800015926361
326 0.681999981403351
327 0.682399988174438
328 0.682399988174438
329 0.686299979686737
330 0.702600002288818
331 0.673799991607666
332 0.699599981307983
333 0.699000000953674
334 0.67059999704361
335 0.679499983787537
336 0.681800007820129
337 0.705399990081787
338 0.701499998569489
339 0.688099980354309
340 0.701099991798401
341 0.676800012588501
342 0.686299979686737
343 0.68529999256134
344 0.679000020027161
345 0.679899990558624
346 0.682799994945526
347 0.691900014877319
348 0.69539999961853
349 0.691699981689453
350 0.678600013256073
351 0.680199980735779
352 0.693700015544891
353 0.685899972915649
354 0.703499972820282
355 0.693599998950958
356 0.689199984073639
357 0.670300006866455
358 0.683700025081635
359 0.663800001144409
360 0.690699994564056
361 0.68639999628067
362 0.68639999628067
363 0.65939998626709
364 0.705399990081787
365 0.68529999256134
366 0.684800028800964
367 0.667999982833862
368 0.670000016689301
369 0.6807000041008
370 0.684300005435944
371 0.67739999294281
372 0.682299971580505
373 0.689899981021881
374 0.684800028800964
375 0.697700023651123
376 0.674399971961975
377 0.688199996948242
378 0.678300023078918
379 0.686600029468536
380 0.695100009441376
381 0.712100028991699
382 0.670099973678589
383 0.681800007820129
384 0.678900003433228
385 0.67960000038147
386 0.684499979019165
387 0.667900025844574
388 0.679199993610382
389 0.676400005817413
390 0.687200009822845
391 0.684099972248077
392 0.672399997711182
393 0.689400017261505
394 0.675899982452393
395 0.672599971294403
396 0.677200019359589
397 0.67739999294281
398 0.678699970245361
399 0.676500022411346
400 0.684499979019165
401 0.685800015926361
402 0.686900019645691
403 0.675599992275238
404 0.687600016593933
405 0.685500025749207
406 0.672900021076202
407 0.681699991226196
408 0.682699978351593
409 0.682600021362305
410 0.683200001716614
411 0.685100018978119
412 0.703199982643127
413 0.682799994945526
414 0.676400005817413
415 0.690299987792969
416 0.697700023651123
417 0.676599979400635
418 0.687699973583221
419 0.675300002098083
420 0.676800012588501
421 0.696799993515015
422 0.685599982738495
423 0.667200028896332
424 0.673500001430511
425 0.684599995613098
426 0.691299974918365
427 0.685699999332428
428 0.671800017356873
429 0.678200006484985
430 0.672699987888336
431 0.675000011920929
432 0.677799999713898
433 0.686900019645691
434 0.674199998378754
435 0.68529999256134
436 0.662000000476837
437 0.65829998254776
438 0.672999978065491
439 0.684499979019165
440 0.678900003433228
441 0.679199993610382
442 0.678099989891052
443 0.672299981117249
444 0.680400013923645
445 0.669399976730347
446 0.684899985790253
447 0.678699970245361
448 0.686999976634979
449 0.697899997234344
450 0.662899971008301
451 0.67739999294281
452 0.687699973583221
453 0.688499987125397
454 0.676999986171722
455 0.666899979114532
456 0.689199984073639
457 0.688300013542175
458 0.665799975395203
459 0.694500029087067
460 0.669600009918213
461 0.680199980735779
462 0.693599998950958
463 0.666800022125244
464 0.680299997329712
465 0.676400005817413
466 0.688399970531464
467 0.672800004482269
468 0.678699970245361
469 0.673600018024445
470 0.664499998092651
471 0.677500009536743
472 0.682099997997284
473 0.688099980354309
474 0.659900009632111
475 0.695299983024597
476 0.682399988174438
477 0.675499975681305
478 0.667900025844574
479 0.681999981403351
480 0.682600021362305
481 0.690299987792969
482 0.688199996948242
483 0.666000008583069
484 0.678399980068207
485 0.672800004482269
486 0.679499983787537
487 0.670700013637543
488 0.65530002117157
489 0.659500002861023
490 0.683000028133392
491 0.665899991989136
492 0.665499985218048
493 0.681100010871887
494 0.684300005435944
495 0.676900029182434
496 0.685000002384186
497 0.680899977684021
498 0.669399976730347
499 0.672500014305115
500 0.682900011539459
};


==> experiments/figures/cce_05.tex <==
\addplot [semithick, color4]
table {%
0 0.0996600016951561
1 0.468100011348724
2 0.473720014095306
3 0.478199988603592
4 0.483339995145798
5 0.476680010557175
6 0.481920003890991
7 0.485680013895035
8 0.494280010461807
9 0.496540009975433
10 0.500460028648376
11 0.506619989871979
12 0.505620002746582
13 0.52020001411438
14 0.524339973926544
15 0.529100000858307
16 0.53659999370575
17 0.538839995861053
18 0.554820001125336
19 0.555260002613068
20 0.564719974994659
21 0.575380027294159
22 0.587660014629364
23 0.590699970722198
24 0.588379979133606
25 0.606360018253326
26 0.616060018539429
27 0.623040020465851
28 0.624899983406067
29 0.637000024318695
30 0.63782000541687
31 0.651120007038116
32 0.648959994316101
33 0.657620012760162
34 0.662440001964569
35 0.666559994220734
36 0.669560015201569
37 0.6807000041008
38 0.685079991817474
39 0.694140017032623
40 0.690779983997345
41 0.694660007953644
42 0.699360013008118
43 0.705340027809143
44 0.711139976978302
45 0.71587997674942
46 0.71832001209259
47 0.718259990215302
48 0.72188001871109
49 0.732060015201569
50 0.728619992733002
51 0.738640010356903
52 0.737500011920929
53 0.73716002702713
54 0.7360600233078
55 0.737320005893707
56 0.74915999174118
57 0.75875997543335
58 0.753480017185211
59 0.760720014572144
60 0.75084000825882
61 0.760299980640411
62 0.768700003623962
63 0.76529997587204
64 0.76775997877121
65 0.772440016269684
66 0.774680018424988
67 0.777920007705688
68 0.77209997177124
69 0.77208000421524
70 0.778699994087219
71 0.783460021018982
72 0.783800005912781
73 0.7846400141716
74 0.785520017147064
75 0.782959997653961
76 0.783379971981049
77 0.779659986495972
78 0.792800009250641
79 0.787840008735657
80 0.797020018100739
81 0.804939985275269
82 0.794860005378723
83 0.800100028514862
84 0.803300023078918
85 0.802760004997253
86 0.800180017948151
87 0.797640025615692
88 0.808700025081635
89 0.805739998817444
90 0.810540020465851
91 0.800499975681305
92 0.808659970760345
93 0.816640019416809
94 0.809400022029877
95 0.82039999961853
96 0.801320016384125
97 0.815119981765747
98 0.817340016365051
99 0.819500029087067
100 0.82397997379303
101 0.818400025367737
102 0.803300023078918
103 0.813960015773773
104 0.816020011901855
105 0.822939991950989
106 0.818599998950958
107 0.825360000133514
108 0.821780025959015
109 0.829200029373169
110 0.820599973201752
111 0.825720012187958
112 0.830659985542297
113 0.830219984054565
114 0.831219971179962
115 0.824699997901917
116 0.828779995441437
117 0.827400028705597
118 0.833840012550354
119 0.814279973506927
120 0.836419999599457
121 0.83840000629425
122 0.829519987106323
123 0.842440009117126
124 0.832579970359802
125 0.843100011348724
126 0.837339997291565
127 0.834020018577576
128 0.843559980392456
129 0.832400023937225
130 0.842739999294281
131 0.836459994316101
132 0.842960000038147
133 0.830299973487854
134 0.84960001707077
135 0.838039994239807
136 0.847880005836487
137 0.841120004653931
138 0.84307998418808
139 0.849680006504059
140 0.848119974136353
141 0.840200006961823
142 0.842960000038147
143 0.84908002614975
144 0.837679982185364
145 0.843240022659302
146 0.846979975700378
147 0.85233998298645
148 0.851320028305054
149 0.848420023918152
150 0.854960024356842
151 0.851480007171631
152 0.855080008506775
153 0.846800029277802
154 0.846300005912781
155 0.85589998960495
156 0.860159993171692
157 0.858519971370697
158 0.84934002161026
159 0.851159989833832
160 0.84281998872757
161 0.851040005683899
162 0.864579975605011
163 0.856580018997192
164 0.851779997348785
165 0.857119977474213
166 0.860740005970001
167 0.860960006713867
168 0.853380024433136
169 0.860979974269867
170 0.872699975967407
171 0.853919982910156
172 0.856939971446991
173 0.859160006046295
174 0.854920029640198
175 0.860319972038269
176 0.860960006713867
177 0.866460025310516
178 0.8575199842453
179 0.851119995117188
180 0.86327999830246
181 0.859179973602295
182 0.855799973011017
183 0.860499978065491
184 0.865679979324341
185 0.85808002948761
186 0.867039978504181
187 0.871959984302521
188 0.856440007686615
189 0.86735999584198
190 0.870239973068237
191 0.861880004405975
192 0.87992000579834
193 0.86871999502182
194 0.856660008430481
195 0.869700014591217
196 0.863600015640259
197 0.864260017871857
198 0.872820019721985
199 0.871479988098145
200 0.87338000535965
201 0.870119988918304
202 0.857779979705811
203 0.874140024185181
204 0.87007999420166
205 0.874880015850067
206 0.868499994277954
207 0.869239985942841
208 0.878939986228943
209 0.883040010929108
210 0.86734002828598
211 0.872579991817474
212 0.873960018157959
213 0.873619973659515
214 0.878340005874634
215 0.887099981307983
216 0.884339988231659
217 0.874979972839355
218 0.877659976482391
219 0.871860027313232
220 0.87992000579834
221 0.878880023956299
222 0.877160012722015
223 0.8785799741745
224 0.876399993896484
225 0.87524002790451
226 0.874580025672913
227 0.881439983844757
228 0.869679987430573
229 0.889419972896576
230 0.88238000869751
231 0.878859996795654
232 0.883819997310638
233 0.874819993972778
234 0.886900007724762
235 0.897899985313416
236 0.887279987335205
237 0.883719980716705
238 0.882219970226288
239 0.882939994335175
240 0.875880002975464
241 0.892040014266968
242 0.885919988155365
243 0.8889200091362
244 0.890619993209839
245 0.892499983310699
246 0.886619985103607
247 0.882759988307953
248 0.884940028190613
249 0.88128000497818
250 0.871519982814789
251 0.88808000087738
252 0.8817999958992
253 0.872940003871918
254 0.885280013084412
255 0.887920022010803
256 0.892939984798431
257 0.890720009803772
258 0.883059978485107
259 0.883780002593994
260 0.887960016727448
261 0.895359992980957
262 0.894420027732849
263 0.886740028858185
264 0.883840024471283
265 0.887740015983582
266 0.890100002288818
267 0.888119995594025
268 0.886080026626587
269 0.891499996185303
270 0.894980013370514
271 0.890519976615906
272 0.896740019321442
273 0.88510000705719
274 0.890860021114349
275 0.893660008907318
276 0.893700003623962
277 0.887600004673004
278 0.871840000152588
279 0.902360022068024
280 0.89326000213623
281 0.893599987030029
282 0.886420011520386
283 0.894039988517761
284 0.8817999958992
285 0.893999993801117
286 0.898639976978302
287 0.896960020065308
288 0.891420006752014
289 0.903800010681152
290 0.88672000169754
291 0.890720009803772
292 0.894159972667694
293 0.895900011062622
294 0.88647997379303
295 0.893559992313385
296 0.898320019245148
297 0.89520001411438
298 0.897459983825684
299 0.886839985847473
300 0.89657998085022
301 0.89190000295639
302 0.895359992980957
303 0.903999984264374
304 0.897300004959106
305 0.887340009212494
306 0.897520005702972
307 0.894060015678406
308 0.896520018577576
309 0.903720021247864
310 0.891019999980927
311 0.905920028686523
312 0.904600024223328
313 0.886340022087097
314 0.899659991264343
315 0.897520005702972
316 0.905099987983704
317 0.905939996242523
318 0.897040009498596
319 0.898239970207214
320 0.899860024452209
321 0.903339982032776
322 0.89410001039505
323 0.897220015525818
324 0.900240004062653
325 0.900020003318787
326 0.889739990234375
327 0.88757997751236
328 0.904980003833771
329 0.907899975776672
330 0.892159998416901
331 0.904919981956482
332 0.896719992160797
333 0.909099996089935
334 0.901639997959137
335 0.902899980545044
336 0.895160019397736
337 0.90719997882843
338 0.907620012760162
339 0.910099983215332
340 0.906379997730255
341 0.904519975185394
342 0.906799972057343
343 0.899820029735565
344 0.904760003089905
345 0.895099997520447
346 0.897220015525818
347 0.9132000207901
348 0.904320001602173
349 0.898999989032745
350 0.89766001701355
351 0.912339985370636
352 0.901859998703003
353 0.905700027942657
354 0.902180016040802
355 0.907880008220673
356 0.90473997592926
357 0.90693998336792
358 0.904020011425018
359 0.893480002880096
360 0.90421998500824
361 0.915960013866425
362 0.910719990730286
363 0.907419979572296
364 0.907100021839142
365 0.905780017375946
366 0.910340011119843
367 0.909039974212646
368 0.91346001625061
369 0.910860002040863
370 0.902440011501312
371 0.9096599817276
372 0.911960005760193
373 0.914879977703094
374 0.912419974803925
375 0.91158002614975
376 0.911920011043549
377 0.913999974727631
378 0.905399978160858
379 0.914719998836517
380 0.911300003528595
381 0.909060001373291
382 0.910380005836487
383 0.908640027046204
384 0.919340014457703
385 0.915620028972626
386 0.909619987010956
387 0.90091997385025
388 0.903779983520508
389 0.914780020713806
390 0.910459995269775
391 0.911740005016327
392 0.896920025348663
393 0.916159987449646
394 0.907079994678497
395 0.908360004425049
396 0.90446001291275
397 0.914619982242584
398 0.909940004348755
399 0.91074001789093
400 0.905239999294281
401 0.902339994907379
402 0.908339977264404
403 0.914059996604919
404 0.910979986190796
405 0.919560015201569
406 0.909780025482178
407 0.92305999994278
408 0.914640009403229
409 0.906140029430389
410 0.905499994754791
411 0.916740000247955
412 0.89793998003006
413 0.90886002779007
414 0.899460017681122
415 0.915059983730316
416 0.91100001335144
417 0.911660015583038
418 0.915300011634827
419 0.916000008583069
420 0.918099999427795
421 0.910319983959198
422 0.908119976520538
423 0.906740009784698
424 0.902960002422333
425 0.923080027103424
426 0.901279985904694
427 0.907819986343384
428 0.916499972343445
429 0.915080010890961
430 0.921199977397919
431 0.921140015125275
432 0.910679996013641
433 0.916819989681244
434 0.912079989910126
435 0.922280013561249
436 0.920340001583099
437 0.917919993400574
438 0.910660028457642
439 0.916700005531311
440 0.920719981193542
441 0.911520004272461
442 0.901560008525848
443 0.918479979038239
444 0.918280005455017
445 0.922020018100739
446 0.915539979934692
447 0.927619993686676
448 0.917439997196198
449 0.919359982013702
450 0.920979976654053
451 0.911800026893616
452 0.924139976501465
453 0.916819989681244
454 0.917119979858398
455 0.921079993247986
456 0.917999982833862
457 0.916419982910156
458 0.893540024757385
459 0.919200003147125
460 0.919860005378723
461 0.914340019226074
462 0.92874002456665
463 0.911719977855682
464 0.907480001449585
465 0.912199974060059
466 0.907100021839142
467 0.922060012817383
468 0.921500027179718
469 0.929340004920959
470 0.91430002450943
471 0.901080012321472
472 0.926620006561279
473 0.906579971313477
474 0.920920014381409
475 0.925580024719238
476 0.921180009841919
477 0.926500022411346
478 0.913940012454987
479 0.928659975528717
480 0.924899995326996
481 0.922240018844604
482 0.913320004940033
483 0.915579974651337
484 0.923340022563934
485 0.924220025539398
486 0.919719994068146
487 0.916059970855713
488 0.921000003814697
489 0.922179996967316
490 0.930639982223511
491 0.919459998607635
492 0.916700005531311
493 0.920260012149811
494 0.917240023612976
495 0.923099994659424
496 0.914919972419739
497 0.920140027999878
498 0.919839978218079
499 0.920719981193542
500 0.922940015792847
};
\addplot [semithick, color5]
table {%
0 0.089199997484684
1 0.920400023460388
2 0.926999986171722
3 0.935599982738495
4 0.938399970531464
5 0.909900009632111
6 0.913299977779388
7 0.907899975776672
8 0.920300006866455
9 0.910099983215332
10 0.907100021839142
11 0.894800007343292
12 0.872900009155273
13 0.893599987030029
14 0.876299977302551
15 0.853299975395203
16 0.848100006580353
17 0.834500014781952
18 0.819400012493134
19 0.816900014877319
20 0.791999995708466
21 0.79119998216629
22 0.788699984550476
23 0.768400013446808
24 0.746399998664856
25 0.772499978542328
26 0.766099989414215
27 0.762399971485138
28 0.736299991607666
29 0.733399987220764
30 0.710099995136261
31 0.739300012588501
32 0.688300013542175
33 0.714200019836426
34 0.6807000041008
35 0.690299987792969
36 0.689000010490417
37 0.675899982452393
38 0.672699987888336
39 0.68010002374649
40 0.655200004577637
41 0.676999986171722
42 0.676400005817413
43 0.653199970722198
44 0.673500001430511
45 0.632499992847443
46 0.651000022888184
47 0.646799981594086
48 0.639100015163422
49 0.645699977874756
50 0.620299994945526
51 0.626500010490417
52 0.619400024414062
53 0.617900013923645
54 0.61269998550415
55 0.588299989700317
56 0.604300022125244
57 0.627699971199036
58 0.605300009250641
59 0.615299999713898
60 0.607999980449677
61 0.609399974346161
62 0.610499978065491
63 0.607400000095367
64 0.588199973106384
65 0.606599986553192
66 0.618399977684021
67 0.598399996757507
68 0.583500027656555
69 0.609899997711182
70 0.586899995803833
71 0.604099988937378
72 0.604700028896332
73 0.600300014019012
74 0.579100012779236
75 0.577899992465973
76 0.574899971485138
77 0.557500004768372
78 0.582899987697601
79 0.587999999523163
80 0.575999975204468
81 0.587800025939941
82 0.567799985408783
83 0.576499998569489
84 0.562600016593933
85 0.579100012779236
86 0.570699989795685
87 0.561800003051758
88 0.579900026321411
89 0.577600002288818
90 0.571200013160706
91 0.566999971866608
92 0.569199979305267
93 0.565199971199036
94 0.554799973964691
95 0.574000000953674
96 0.550999999046326
97 0.578800022602081
98 0.565199971199036
99 0.565199971199036
100 0.562900006771088
101 0.551699995994568
102 0.539900004863739
103 0.553799986839294
104 0.570999979972839
105 0.544700026512146
106 0.53600001335144
107 0.537800014019012
108 0.564100027084351
109 0.562799990177155
110 0.542400002479553
111 0.546599984169006
112 0.536400020122528
113 0.560199975967407
114 0.553799986839294
115 0.558799982070923
116 0.552100002765656
117 0.542699992656708
118 0.536300003528595
119 0.52319997549057
120 0.548600018024445
121 0.549199998378754
122 0.546500027179718
123 0.554199993610382
124 0.54229998588562
125 0.543299973011017
126 0.543299973011017
127 0.518400013446808
128 0.532599985599518
129 0.544600009918213
130 0.538299977779388
131 0.515600025653839
132 0.538399994373322
133 0.557200014591217
134 0.549799978733063
135 0.522700011730194
136 0.541999995708466
137 0.521700024604797
138 0.539900004863739
139 0.524600028991699
140 0.524900019168854
141 0.524800002574921
142 0.510900020599365
143 0.518700003623962
144 0.514599978923798
145 0.521600008010864
146 0.524399995803833
147 0.534200012683868
148 0.530700027942657
149 0.505599975585938
150 0.524500012397766
151 0.505800008773804
152 0.535000026226044
153 0.512000024318695
154 0.521600008010864
155 0.526700019836426
156 0.52700001001358
157 0.54040002822876
158 0.498800009489059
159 0.507300019264221
160 0.529799997806549
161 0.507499992847443
162 0.529699981212616
163 0.523699998855591
164 0.515100002288818
165 0.52130001783371
166 0.51910001039505
167 0.523999989032745
168 0.518899977207184
169 0.509199976921082
170 0.516700029373169
171 0.528299987316132
172 0.512700021266937
173 0.511300027370453
174 0.518499970436096
175 0.52539998292923
176 0.497200012207031
177 0.504899978637695
178 0.517599999904633
179 0.506099998950958
180 0.514999985694885
181 0.497500002384186
182 0.502699971199036
183 0.48649999499321
184 0.500100016593933
185 0.509800016880035
186 0.509899973869324
187 0.514100015163422
188 0.494500011205673
189 0.502600014209747
190 0.519500017166138
191 0.495299994945526
192 0.528900027275085
193 0.521899998188019
194 0.486400008201599
195 0.51230001449585
196 0.516099989414215
197 0.515399992465973
198 0.492500007152557
199 0.501600027084351
200 0.517700016498566
201 0.510200023651123
202 0.498199999332428
203 0.495200008153915
204 0.499300003051758
205 0.499000012874603
206 0.500400006771088
207 0.503000020980835
208 0.522499978542328
209 0.516600012779236
210 0.507300019264221
211 0.51529997587204
212 0.513000011444092
213 0.51690000295639
214 0.503499984741211
215 0.497999995946884
216 0.515799999237061
217 0.526199996471405
218 0.496199995279312
219 0.51230001449585
220 0.517300009727478
221 0.503600001335144
222 0.500400006771088
223 0.513000011444092
224 0.52319997549057
225 0.510299980640411
226 0.495299994945526
227 0.497200012207031
228 0.496300011873245
229 0.500999987125397
230 0.508499979972839
231 0.49669998884201
232 0.51690000295639
233 0.49210000038147
234 0.519800007343292
235 0.510900020599365
236 0.505100011825562
237 0.515500009059906
238 0.504899978637695
239 0.512199997901917
240 0.505400002002716
241 0.503799974918365
242 0.507600009441376
243 0.502900004386902
244 0.528400003910065
245 0.504000008106232
246 0.514400005340576
247 0.493699997663498
248 0.493600010871887
249 0.484899997711182
250 0.486299991607666
251 0.505100011825562
252 0.489800006151199
253 0.507300019264221
254 0.485700011253357
255 0.502600014209747
256 0.506200015544891
257 0.501600027084351
258 0.499099999666214
259 0.483000010251999
260 0.502099990844727
261 0.504199981689453
262 0.491699993610382
263 0.483900010585785
264 0.476900011301041
265 0.513400018215179
266 0.480699986219406
267 0.487800002098083
268 0.476999998092651
269 0.504800021648407
270 0.493999987840652
271 0.502900004386902
272 0.513999998569489
273 0.484200000762939
274 0.48879998922348
275 0.504000008106232
276 0.49770000576973
277 0.50629997253418
278 0.487300008535385
279 0.489600002765656
280 0.500299990177155
281 0.493999987840652
282 0.488400012254715
283 0.486999988555908
284 0.496800005435944
285 0.496499985456467
286 0.506699979305267
287 0.502099990844727
288 0.485199987888336
289 0.494100004434586
290 0.489800006151199
291 0.483799993991852
292 0.48879998922348
293 0.479600012302399
294 0.468800008296967
295 0.493099987506866
296 0.483300000429153
297 0.493699997663498
298 0.492599993944168
299 0.505999982357025
300 0.482699990272522
301 0.490700006484985
302 0.508400022983551
303 0.497900009155273
304 0.491299986839294
305 0.492500007152557
306 0.501500010490417
307 0.485300004482269
308 0.495200008153915
309 0.498600006103516
310 0.478799998760223
311 0.514900028705597
312 0.501600027084351
313 0.48759999871254
314 0.488499999046326
315 0.492500007152557
316 0.513100028038025
317 0.496399998664856
318 0.491299986839294
319 0.475899994373322
320 0.474999994039536
321 0.501399993896484
322 0.456299990415573
323 0.473699986934662
324 0.469900012016296
325 0.493400007486343
326 0.472699999809265
327 0.470899999141693
328 0.473699986934662
329 0.486900001764297
330 0.481299996376038
331 0.484200000762939
332 0.479000002145767
333 0.500400006771088
334 0.482100009918213
335 0.49329999089241
336 0.467400014400482
337 0.488900005817413
338 0.475400000810623
339 0.508499979972839
340 0.485799998044968
341 0.480800002813339
342 0.488499999046326
343 0.508199989795685
344 0.498600006103516
345 0.482600003480911
346 0.48199999332428
347 0.480399996042252
348 0.491499990224838
349 0.469900012016296
350 0.475199997425079
351 0.494899988174438
352 0.476500004529953
353 0.493900001049042
354 0.489499986171722
355 0.473600000143051
356 0.483999997377396
357 0.48429998755455
358 0.47350001335144
359 0.493600010871887
360 0.462799996137619
361 0.484899997711182
362 0.480300009250641
363 0.471799999475479
364 0.473800003528595
365 0.487800002098083
366 0.48089998960495
367 0.494300007820129
368 0.486099988222122
369 0.486600011587143
370 0.480199992656708
371 0.476999998092651
372 0.480199992656708
373 0.485100001096725
374 0.485799998044968
375 0.475100010633469
376 0.489600002765656
377 0.4932000041008
378 0.488099992275238
379 0.487199991941452
380 0.472699999809265
381 0.462599992752075
382 0.492000013589859
383 0.476200014352798
384 0.488400012254715
385 0.484800010919571
386 0.472400009632111
387 0.479699999094009
388 0.472900003194809
389 0.470400005578995
390 0.493600010871887
391 0.486099988222122
392 0.460599988698959
393 0.483799993991852
394 0.470099985599518
395 0.501399993896484
396 0.490900009870529
397 0.48870000243187
398 0.459600001573563
399 0.479099988937378
400 0.458799988031387
401 0.470400005578995
402 0.479699999094009
403 0.479999989271164
404 0.476999998092651
405 0.495700001716614
406 0.491400003433228
407 0.471799999475479
408 0.490599989891052
409 0.47639998793602
410 0.473100006580353
411 0.476099997758865
412 0.462099999189377
413 0.485000014305115
414 0.486200004816055
415 0.486200004816055
416 0.477299988269806
417 0.469500005245209
418 0.461699992418289
419 0.474400013685226
420 0.479299992322922
421 0.481499999761581
422 0.474799990653992
423 0.469199985265732
424 0.469799995422363
425 0.481400012969971
426 0.481499999761581
427 0.486699998378754
428 0.491100013256073
429 0.482499986886978
430 0.475400000810623
431 0.482600003480911
432 0.476099997758865
433 0.479200005531311
434 0.478399991989136
435 0.481400012969971
436 0.500999987125397
437 0.468899995088577
438 0.474700003862381
439 0.483500003814697
440 0.473199993371964
441 0.469700008630753
442 0.473800003528595
443 0.474000006914139
444 0.485799998044968
445 0.477100014686584
446 0.472600013017654
447 0.499700009822845
448 0.473600000143051
449 0.482899993658066
450 0.481299996376038
451 0.479999989271164
452 0.474500000476837
453 0.474400013685226
454 0.473100006580353
455 0.481299996376038
456 0.465000003576279
457 0.475800007581711
458 0.469999998807907
459 0.486000001430511
460 0.470999985933304
461 0.459600001573563
462 0.495700001716614
463 0.482800006866455
464 0.452800005674362
465 0.469199985265732
466 0.452899992465973
467 0.482699990272522
468 0.465999990701675
469 0.490200012922287
470 0.488299995660782
471 0.443800002336502
472 0.48309999704361
473 0.455199986696243
474 0.490799993276596
475 0.479400008916855
476 0.44879999756813
477 0.460099995136261
478 0.465400010347366
479 0.495099991559982
480 0.469500005245209
481 0.48989999294281
482 0.449999988079071
483 0.476900011301041
484 0.492799997329712
485 0.505100011825562
486 0.475400000810623
487 0.465400010347366
488 0.469500005245209
489 0.473800003528595
490 0.475400000810623
491 0.469399988651276
492 0.470499992370605
493 0.453000009059906
494 0.47979998588562
495 0.487100005149841
496 0.47350001335144
497 0.491699993610382
498 0.469999998807907
499 0.459199994802475
500 0.469500005245209
};

==> experiments/figures/mae_ccei_0.tex <==
\addplot[semithick, color0] %x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 1
10 1
20 1
30 1
40 1
50 1
60 1
70 1
80 1
90 1
100 1
110 1
120 1
130 1
140 1
150 1
160 1
170 1
180 1
190 1
200 1
210 1
220 1
230 1
240 1
250 1
260 1
270 1
280 1
290 1
300 1
310 1
320 1
330 1
340 1
350 1
360 1
370 1
380 1
390 1
400 1
410 1
420 1
430 1
440 1
450 1
460 1
470 1
480 1
490 1
500 1
510 1
520 1
530 1
540 1
550 1
560 1
570 1
580 1
590 1
600 1
610 1
620 1
630 1
640 1
650 1
660 1
670 1
680 1
690 1
700 1
710 1
720 1
730 1
740 1
750 1
760 1
770 1
780 1
790 1
800 1
810 1
820 1
830 1
840 1
850 1
860 1
870 1
880 1
890 1
900 1
910 1
920 1
930 1
940 1
950 1
960 1
970 1
980 1
990 1
1000 1
1010 1
1020 1
1030 1
1040 1
1050 1
1060 1
1070 1
1080 1
1090 1
1100 1
1110 1
1120 1
1130 1
1140 1
1150 1
1160 1
1170 1
1180 1
1190 1
1200 1
1210 1
1220 1
1230 1
1240 1
1250 1
1260 1
1270 1
1280 1
1290 1
1300 1
1310 1
1320 1
1330 1
1340 1
1350 1
1360 1
1370 1
1380 1
1390 1
1400 1
1410 1
1420 1
1430 1
1440 1
1450 1
1460 1
1470 1
1480 1
1490 1
1500 1
1510 1
1520 1
1530 1
1540 1
1550 1
1560 1
1570 1
1580 1
1590 1
1600 1
1610 1
1620 1
1630 1
1640 1
1650 1
1660 1
1670 1
1680 1
1690 1
1700 1
1710 1
1720 1
1730 1
1740 1
1750 1
1760 1
1770 1
1780 1
1790 1
1800 1
1810 1
1820 1
1830 1
1840 1
1850 1
1860 1
1870 1
1880 1
1890 1
1900 1
1910 1
1920 1
1930 1
1940 1
1950 1
1960 1
1970 1
1980 1
1990 1
2000 1
2010 1
2020 1
2030 1
2040 1
2050 1
2060 1
2070 1
2080 1
2090 1
2100 1
2110 1
2120 1
2130 1
2140 1
2150 1
2160 1
2170 1
2180 1
2190 1
2200 1
2210 1
2220 1
2230 1
2240 1
2250 1
2260 1
2270 1
2280 1
2290 1
2300 1
2310 1
2320 1
2330 1
2340 1
2350 1
2360 1
2370 1
2380 1
2390 1
2400 1
2410 1
2420 1
2430 1
2440 1
2450 1
2460 1
2470 1
2480 1
2490 1
2500 1
2510 1
2520 1
2530 1
2540 1
2550 1
2560 1
2570 1
2580 1
2590 1
2600 1
2610 1
2620 1
2630 1
2640 1
2650 1
2660 1
2670 1
2680 1
2690 1
2700 1
2710 1
2720 1
2730 1
2740 1
2750 1
2760 1
2770 1
2780 1
2790 1
2800 1
2810 1
2820 1
2830 1
2840 1
2850 1
2860 1
2870 1
2880 1
2890 1
2900 1
2910 1
2920 1
2930 1
2940 1
2950 1
2960 1
2970 1
2980 1
2990 1
3000 1
3010 1
3020 1
3030 1
3040 1
3050 1
3060 1
3070 1
3080 1
3090 1
3100 1
3110 1
3120 1
3130 1
3140 1
3150 1
3160 1
3170 1
3180 1
3190 1
3200 1
3210 1
3220 1
3230 1
3240 1
3250 1
3260 1
3270 1
3280 1
3290 1
3300 1
3310 1
3320 1
3330 1
3340 1
3350 1
3360 1
3370 1
3380 1
3390 1
3400 1
3410 1
3420 1
3430 1
3440 1
3450 1
3460 1
3470 1
3480 1
3490 1
3500 1
3510 1
3520 1
3530 1
3540 1
3550 1
3560 1
3570 1
3580 1
3590 1
3600 1
3610 1
3620 1
3630 1
3640 1
3650 1
3660 1
3670 1
3680 1
3690 1
3700 1
3710 1
3720 1
3730 1
3740 1
3750 1
3760 1
3770 1
3780 1
3790 1
3800 1
3810 1
3820 1
3830 1
3840 1
3850 1
3860 1
3870 1
3880 1
3890 1
3900 1
3910 1
3920 1
3930 1
3940 1
3950 1
3960 1
3970 1
3980 1
3990 1
4000 1
4010 1
4020 1
4030 1
4040 1
4050 1
4060 1
4070 1
4080 1
4090 1
4100 1
4110 1
4120 1
4130 1
4140 1
4150 1
4160 1
4170 1
4180 1
4190 1
4200 1
4210 1
4220 1
4230 1
4240 1
4250 1
4260 1
4270 1
4280 1
4290 1
4300 1
4310 1
4320 1
4330 1
4340 1
4350 1
4360 1
4370 1
4380 1
4390 1
4400 1
4410 1
4420 1
4430 1
4440 1
4450 1
4460 1
4470 1
4480 1
4490 1
4500 1
4510 1
4520 1
4530 1
4540 1
4550 1
4560 1
4570 1
4580 1
4590 1
4600 1
4610 1
4620 1
4630 1
4640 1
4650 1
4660 1
4670 1
4680 1
4690 1
4700 1
4710 1
4720 1
4730 1
4740 1
4750 1
4760 1
4770 1
4780 1
4790 1
4800 1
4810 1
4820 1
4830 1
4840 1
4850 1
4860 1
4870 1
4880 1
4890 1
4900 1
4910 1
4920 1
4930 1
4940 1
4950 1
4960 1
4970 1
4980 1
4990 1
5000 1
};
%\addlegendentry{Train}
\addplot[semithick, color1] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.98199999332428
10 0.98199999332428
20 0.98199999332428
30 0.98199999332428
40 0.98199999332428
50 0.98199999332428
60 0.98199999332428
70 0.98199999332428
80 0.98199999332428
90 0.98199999332428
100 0.98199999332428
110 0.98199999332428
120 0.98199999332428
130 0.98199999332428
140 0.98199999332428
150 0.98199999332428
160 0.98199999332428
170 0.98199999332428
180 0.98199999332428
190 0.98199999332428
200 0.98199999332428
210 0.98199999332428
220 0.98199999332428
230 0.98199999332428
240 0.98199999332428
250 0.98199999332428
260 0.98199999332428
270 0.98199999332428
280 0.98199999332428
290 0.98199999332428
300 0.98199999332428
310 0.98199999332428
320 0.98199999332428
330 0.98199999332428
340 0.98199999332428
350 0.98199999332428
360 0.98199999332428
370 0.98199999332428
380 0.98199999332428
390 0.98199999332428
400 0.98199999332428
410 0.98199999332428
420 0.98199999332428
430 0.98199999332428
440 0.98199999332428
450 0.98199999332428
460 0.98199999332428
470 0.98199999332428
480 0.98199999332428
490 0.98199999332428
500 0.98199999332428
510 0.98199999332428
520 0.98199999332428
530 0.98199999332428
540 0.98199999332428
550 0.98199999332428
560 0.98199999332428
570 0.98199999332428
580 0.98199999332428
590 0.98199999332428
600 0.98199999332428
610 0.98199999332428
620 0.98199999332428
630 0.98199999332428
640 0.98199999332428
650 0.98199999332428
660 0.98199999332428
670 0.98199999332428
680 0.98199999332428
690 0.98199999332428
700 0.98199999332428
710 0.98199999332428
720 0.98199999332428
730 0.98199999332428
740 0.98199999332428
750 0.98199999332428
760 0.98199999332428
770 0.98199999332428
780 0.98199999332428
790 0.98199999332428
800 0.98199999332428
810 0.98199999332428
820 0.98199999332428
830 0.98199999332428
840 0.98199999332428
850 0.98199999332428
860 0.98199999332428
870 0.98199999332428
880 0.98199999332428
890 0.98199999332428
900 0.98199999332428
910 0.98199999332428
920 0.98199999332428
930 0.98199999332428
940 0.98199999332428
950 0.98199999332428
960 0.98199999332428
970 0.98199999332428
980 0.98199999332428
990 0.98199999332428
1000 0.98199999332428
1010 0.98199999332428
1020 0.98199999332428
1030 0.98199999332428
1040 0.98199999332428
1050 0.98199999332428
1060 0.98199999332428
1070 0.98199999332428
1080 0.98199999332428
1090 0.98199999332428
1100 0.98199999332428
1110 0.98199999332428
1120 0.98199999332428
1130 0.98199999332428
1140 0.98199999332428
1150 0.98199999332428
1160 0.98199999332428
1170 0.98199999332428
1180 0.98199999332428
1190 0.98199999332428
1200 0.98199999332428
1210 0.98199999332428
1220 0.98199999332428
1230 0.98199999332428
1240 0.98199999332428
1250 0.98199999332428
1260 0.98199999332428
1270 0.98199999332428
1280 0.98199999332428
1290 0.98199999332428
1300 0.98199999332428
1310 0.98199999332428
1320 0.98199999332428
1330 0.98199999332428
1340 0.98199999332428
1350 0.98199999332428
1360 0.98199999332428
1370 0.98199999332428
1380 0.98199999332428
1390 0.98199999332428
1400 0.98199999332428
1410 0.98199999332428
1420 0.98199999332428
1430 0.98199999332428
1440 0.98199999332428
1450 0.98199999332428
1460 0.98199999332428
1470 0.98199999332428
1480 0.98199999332428
1490 0.98199999332428
1500 0.98199999332428
1510 0.98199999332428
1520 0.98199999332428
1530 0.98199999332428
1540 0.98199999332428
1550 0.98199999332428
1560 0.98199999332428
1570 0.98199999332428
1580 0.98199999332428
1590 0.98199999332428
1600 0.98199999332428
1610 0.98199999332428
1620 0.98199999332428
1630 0.98199999332428
1640 0.98199999332428
1650 0.98199999332428
1660 0.98199999332428
1670 0.98199999332428
1680 0.98199999332428
1690 0.98199999332428
1700 0.98199999332428
1710 0.98199999332428
1720 0.98199999332428
1730 0.98199999332428
1740 0.98199999332428
1750 0.98199999332428
1760 0.98199999332428
1770 0.98199999332428
1780 0.98199999332428
1790 0.98199999332428
1800 0.98199999332428
1810 0.98199999332428
1820 0.98199999332428
1830 0.98199999332428
1840 0.98199999332428
1850 0.98199999332428
1860 0.98199999332428
1870 0.98199999332428
1880 0.98199999332428
1890 0.98199999332428
1900 0.98199999332428
1910 0.98199999332428
1920 0.98199999332428
1930 0.98199999332428
1940 0.98199999332428
1950 0.98199999332428
1960 0.98199999332428
1970 0.98199999332428
1980 0.98199999332428
1990 0.98199999332428
2000 0.98199999332428
2010 0.98199999332428
2020 0.98199999332428
2030 0.98199999332428
2040 0.98199999332428
2050 0.98199999332428
2060 0.98199999332428
2070 0.98199999332428
2080 0.98199999332428
2090 0.98199999332428
2100 0.98199999332428
2110 0.98199999332428
2120 0.98199999332428
2130 0.98199999332428
2140 0.98199999332428
2150 0.98199999332428
2160 0.98199999332428
2170 0.98199999332428
2180 0.98199999332428
2190 0.98199999332428
2200 0.98199999332428
2210 0.98199999332428
2220 0.98199999332428
2230 0.98199999332428
2240 0.98199999332428
2250 0.98199999332428
2260 0.98199999332428
2270 0.98199999332428
2280 0.98199999332428
2290 0.98199999332428
2300 0.98199999332428
2310 0.98199999332428
2320 0.98199999332428
2330 0.98199999332428
2340 0.98199999332428
2350 0.98199999332428
2360 0.98199999332428
2370 0.98199999332428
2380 0.98199999332428
2390 0.98199999332428
2400 0.98199999332428
2410 0.98199999332428
2420 0.98199999332428
2430 0.98199999332428
2440 0.98199999332428
2450 0.98199999332428
2460 0.98199999332428
2470 0.98199999332428
2480 0.98199999332428
2490 0.98199999332428
2500 0.98199999332428
2510 0.98199999332428
2520 0.98199999332428
2530 0.98199999332428
2540 0.98199999332428
2550 0.98199999332428
2560 0.98199999332428
2570 0.98199999332428
2580 0.98199999332428
2590 0.98199999332428
2600 0.98199999332428
2610 0.98199999332428
2620 0.98199999332428
2630 0.98199999332428
2640 0.98199999332428
2650 0.98199999332428
2660 0.98199999332428
2670 0.98199999332428
2680 0.98199999332428
2690 0.98199999332428
2700 0.98199999332428
2710 0.98199999332428
2720 0.98199999332428
2730 0.98199999332428
2740 0.98199999332428
2750 0.98199999332428
2760 0.98199999332428
2770 0.98199999332428
2780 0.98199999332428
2790 0.98199999332428
2800 0.98199999332428
2810 0.98199999332428
2820 0.98199999332428
2830 0.98199999332428
2840 0.98199999332428
2850 0.98199999332428
2860 0.98199999332428
2870 0.98199999332428
2880 0.98199999332428
2890 0.98199999332428
2900 0.98199999332428
2910 0.98199999332428
2920 0.98199999332428
2930 0.98199999332428
2940 0.98199999332428
2950 0.98199999332428
2960 0.98199999332428
2970 0.98199999332428
2980 0.98199999332428
2990 0.98199999332428
3000 0.98199999332428
3010 0.98199999332428
3020 0.98199999332428
3030 0.98199999332428
3040 0.98199999332428
3050 0.98199999332428
3060 0.98199999332428
3070 0.98199999332428
3080 0.98199999332428
3090 0.98199999332428
3100 0.98199999332428
3110 0.98199999332428
3120 0.98199999332428
3130 0.98199999332428
3140 0.98199999332428
3150 0.98199999332428
3160 0.98199999332428
3170 0.98199999332428
3180 0.98199999332428
3190 0.98199999332428
3200 0.98199999332428
3210 0.98199999332428
3220 0.98199999332428
3230 0.98199999332428
3240 0.98199999332428
3250 0.98199999332428
3260 0.98199999332428
3270 0.98199999332428
3280 0.98199999332428
3290 0.98199999332428
3300 0.98199999332428
3310 0.98199999332428
3320 0.98199999332428
3330 0.98199999332428
3340 0.98199999332428
3350 0.98199999332428
3360 0.98199999332428
3370 0.98199999332428
3380 0.98199999332428
3390 0.98199999332428
3400 0.98199999332428
3410 0.98199999332428
3420 0.98199999332428
3430 0.98199999332428
3440 0.98199999332428
3450 0.98199999332428
3460 0.98199999332428
3470 0.98199999332428
3480 0.98199999332428
3490 0.98199999332428
3500 0.98199999332428
3510 0.98199999332428
3520 0.98199999332428
3530 0.98199999332428
3540 0.98199999332428
3550 0.98199999332428
3560 0.98199999332428
3570 0.98199999332428
3580 0.98199999332428
3590 0.98199999332428
3600 0.98199999332428
3610 0.98199999332428
3620 0.98199999332428
3630 0.98199999332428
3640 0.98199999332428
3650 0.98199999332428
3660 0.98199999332428
3670 0.98199999332428
3680 0.98199999332428
3690 0.98199999332428
3700 0.98199999332428
3710 0.98199999332428
3720 0.98199999332428
3730 0.98199999332428
3740 0.98199999332428
3750 0.98199999332428
3760 0.98199999332428
3770 0.98199999332428
3780 0.98199999332428
3790 0.98199999332428
3800 0.98199999332428
3810 0.98199999332428
3820 0.98199999332428
3830 0.98199999332428
3840 0.98199999332428
3850 0.98199999332428
3860 0.98199999332428
3870 0.98199999332428
3880 0.98199999332428
3890 0.98199999332428
3900 0.98199999332428
3910 0.98199999332428
3920 0.98199999332428
3930 0.98199999332428
3940 0.98199999332428
3950 0.98199999332428
3960 0.98199999332428
3970 0.98199999332428
3980 0.98199999332428
3990 0.98199999332428
4000 0.98199999332428
4010 0.98199999332428
4020 0.98199999332428
4030 0.98199999332428
4040 0.98199999332428
4050 0.98199999332428
4060 0.98199999332428
4070 0.98199999332428
4080 0.98199999332428
4090 0.98199999332428
4100 0.98199999332428
4110 0.98199999332428
4120 0.98199999332428
4130 0.98199999332428
4140 0.98199999332428
4150 0.98199999332428
4160 0.98199999332428
4170 0.98199999332428
4180 0.98199999332428
4190 0.98199999332428
4200 0.98199999332428
4210 0.98199999332428
4220 0.98199999332428
4230 0.98199999332428
4240 0.98199999332428
4250 0.98199999332428
4260 0.98199999332428
4270 0.98199999332428
4280 0.98199999332428
4290 0.98199999332428
4300 0.98199999332428
4310 0.98199999332428
4320 0.98199999332428
4330 0.98199999332428
4340 0.98199999332428
4350 0.98199999332428
4360 0.98199999332428
4370 0.98199999332428
4380 0.98199999332428
4390 0.98199999332428
4400 0.98199999332428
4410 0.98199999332428
4420 0.98199999332428
4430 0.98199999332428
4440 0.98199999332428
4450 0.98199999332428
4460 0.98199999332428
4470 0.98199999332428
4480 0.98199999332428
4490 0.98199999332428
4500 0.98199999332428
4510 0.98199999332428
4520 0.98199999332428
4530 0.98199999332428
4540 0.98199999332428
4550 0.98199999332428
4560 0.98199999332428
4570 0.98199999332428
4580 0.98199999332428
4590 0.98199999332428
4600 0.98199999332428
4610 0.98199999332428
4620 0.98199999332428
4630 0.98199999332428
4640 0.98199999332428
4650 0.98199999332428
4660 0.98199999332428
4670 0.98199999332428
4680 0.98199999332428
4690 0.98199999332428
4700 0.98199999332428
4710 0.98199999332428
4720 0.98199999332428
4730 0.98199999332428
4740 0.98199999332428
4750 0.98199999332428
4760 0.98199999332428
4770 0.98199999332428
4780 0.98199999332428
4790 0.98199999332428
4800 0.98199999332428
4810 0.98199999332428
4820 0.98199999332428
4830 0.98199999332428
4840 0.98199999332428
4850 0.98199999332428
4860 0.98199999332428
4870 0.98199999332428
4880 0.98199999332428
4890 0.98199999332428
4900 0.98199999332428
4910 0.98199999332428
4920 0.98199999332428
4930 0.98199999332428
4940 0.98199999332428
4950 0.98199999332428
4960 0.98199999332428
4970 0.98199999332428
4980 0.98199999332428
4990 0.98199999332428
5000 0.98199999332428
};
%\addlegendentry{Test}

==> experiments/figures/mae_ccei_03.tex <==
\addplot[semithick, color2] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.976719975471497
10 0.960259974002838
20 0.957759976387024
30 0.959280014038086
40 0.965020000934601
50 0.963519990444183
60 0.963859975337982
70 0.955919981002808
80 0.957639992237091
90 0.959140002727509
100 0.962440013885498
110 0.964800000190735
120 0.96340000629425
130 0.96780002117157
140 0.955600023269653
150 0.955980002880096
160 0.962499976158142
170 0.959379971027374
180 0.962840020656586
190 0.95907998085022
200 0.962400019168854
210 0.959519982337952
220 0.956260025501251
230 0.954519987106323
240 0.958100020885468
250 0.958199977874756
260 0.96372002363205
270 0.96372002363205
280 0.960759997367859
290 0.962700009346008
300 0.958660006523132
310 0.954680025577545
320 0.965240001678467
330 0.950720012187958
340 0.961600005626678
350 0.964100003242493
360 0.963540017604828
370 0.9685999751091
380 0.960460007190704
390 0.956839978694916
400 0.958199977874756
410 0.96477997303009
420 0.964119970798492
430 0.962100028991699
440 0.955039978027344
450 0.967980027198792
460 0.967019975185394
470 0.955640017986298
480 0.957780003547668
490 0.964699983596802
500 0.966000020503998
510 0.948800027370453
520 0.95959997177124
530 0.957019984722137
540 0.963280022144318
550 0.952939987182617
560 0.959399998188019
570 0.958899974822998
580 0.963240027427673
590 0.95635998249054
600 0.959299981594086
610 0.960780024528503
620 0.958299994468689
630 0.962939977645874
640 0.965439975261688
650 0.969020009040833
660 0.966380000114441
670 0.958959996700287
680 0.963580012321472
690 0.96451997756958
700 0.96153998374939
710 0.96508002281189
720 0.964299976825714
730 0.96613997220993
740 0.957459986209869
750 0.969099998474121
760 0.96780002117157
770 0.969259977340698
780 0.962660014629364
790 0.958959996700287
800 0.959280014038086
810 0.96968001127243
820 0.964079976081848
830 0.967840015888214
840 0.966340005397797
850 0.958360016345978
860 0.960060000419617
870 0.961220026016235
880 0.965260028839111
890 0.961579978466034
900 0.963060021400452
910 0.962320029735565
920 0.964619994163513
930 0.963540017604828
940 0.964439988136292
950 0.956579983234406
960 0.964619994163513
970 0.964339971542358
980 0.963840007781982
990 0.963039994239807
1000 0.969940006732941
1010 0.964839994907379
1020 0.966260015964508
1030 0.967100024223328
1040 0.964119970798492
1050 0.956439971923828
1060 0.968460023403168
1070 0.968819975852966
1080 0.961480021476746
1090 0.96995997428894
1100 0.967459976673126
1110 0.96723997592926
1120 0.961899995803833
1130 0.965219974517822
1140 0.971480011940002
1150 0.970439970493317
1160 0.964879989624023
1170 0.957780003547668
1180 0.959720015525818
1190 0.967419981956482
1200 0.971379995346069
1210 0.971459984779358
1220 0.964959979057312
1230 0.963020026683807
1240 0.966080009937286
1250 0.959399998188019
1260 0.970700025558472
1270 0.970480024814606
1280 0.963360011577606
1290 0.966419994831085
1300 0.969659984111786
1310 0.964860022068024
1320 0.96399998664856
1330 0.963760018348694
1340 0.967440009117126
1350 0.968519985675812
1360 0.970000028610229
1370 0.959100008010864
1380 0.969479978084564
1390 0.965040028095245
1400 0.96508002281189
1410 0.972199976444244
1420 0.966920018196106
1430 0.970899999141693
1440 0.968659996986389
1450 0.96069997549057
1460 0.965040028095245
1470 0.961719989776611
1480 0.967859983444214
1490 0.96644002199173
1500 0.970099985599518
1510 0.96995997428894
1520 0.969380021095276
1530 0.969259977340698
1540 0.963440001010895
1550 0.969359993934631
1560 0.969799995422363
1570 0.967440009117126
1580 0.967980027198792
1590 0.966639995574951
1600 0.966180026531219
1610 0.958999991416931
1620 0.971440017223358
1630 0.971000015735626
1640 0.967400014400482
1650 0.961440026760101
1660 0.966340005397797
1670 0.969500005245209
1680 0.968360006809235
1690 0.966279983520508
1700 0.973819971084595
1710 0.966480016708374
1720 0.967140018939972
1730 0.966620028018951
1740 0.964900016784668
1750 0.966199994087219
1760 0.973919987678528
1770 0.972320020198822
1780 0.966780006885529
1790 0.968760013580322
1800 0.96995997428894
1810 0.974900007247925
1820 0.964219987392426
1830 0.9514399766922
1840 0.967140018939972
1850 0.967519998550415
1860 0.967980027198792
1870 0.966820001602173
1880 0.968559980392456
1890 0.968400001525879
1900 0.96372002363205
1910 0.959360003471375
1920 0.968140006065369
1930 0.96068000793457
1940 0.969579994678497
1950 0.973619997501373
1960 0.963060021400452
1970 0.968739986419678
1980 0.975319981575012
1990 0.97052001953125
2000 0.971419990062714
2010 0.970319986343384
2020 0.965480029582977
2030 0.966359972953796
2040 0.968540012836456
2050 0.971819996833801
2060 0.97136002779007
2070 0.969060003757477
2080 0.97325998544693
2090 0.960479974746704
2100 0.965120017528534
2110 0.976119995117188
2120 0.972959995269775
2130 0.97136002779007
2140 0.96916002035141
2150 0.967260003089905
2160 0.968640029430389
2170 0.967140018939972
2180 0.972840011119843
2190 0.967779994010925
2200 0.96942001581192
2210 0.965059995651245
2220 0.960720002651215
2230 0.972000002861023
2240 0.96968001127243
2250 0.972299993038177
2260 0.973420023918152
2270 0.973900020122528
2280 0.972639977931976
2290 0.971159994602203
2300 0.96832001209259
2310 0.964839994907379
2320 0.969460010528564
2330 0.967140018939972
2340 0.972500026226044
2350 0.972280025482178
2360 0.971679985523224
2370 0.968959987163544
2380 0.965960025787354
2390 0.976180016994476
2400 0.970399975776672
2410 0.968999981880188
2420 0.970160007476807
2430 0.977140009403229
2440 0.975199997425079
2450 0.973640024662018
2460 0.977639973163605
2470 0.97078001499176
2480 0.970200002193451
2490 0.971459984779358
2500 0.973320007324219
2510 0.95661997795105
2520 0.968519985675812
2530 0.975199997425079
2540 0.972859978675842
2550 0.967660009860992
2560 0.972760021686554
2570 0.971960008144379
2580 0.961239993572235
2590 0.962100028991699
2600 0.97053998708725
2610 0.962800025939941
2620 0.971660017967224
2630 0.975579977035522
2640 0.972320020198822
2650 0.968699991703033
2660 0.967980027198792
2670 0.964479982852936
2680 0.971239984035492
2690 0.974900007247925
2700 0.977240025997162
2710 0.970019996166229
2720 0.972559988498688
2730 0.973580002784729
2740 0.957520008087158
2750 0.970139980316162
2760 0.968259990215302
2770 0.971180021762848
2780 0.972060024738312
2790 0.968980014324188
2800 0.970480024814606
2810 0.96670001745224
2820 0.965260028839111
2830 0.971239984035492
2840 0.968640029430389
2850 0.967079997062683
2860 0.971099972724915
2870 0.972119987010956
2880 0.975799977779388
2890 0.971319973468781
2900 0.976899981498718
2910 0.969219982624054
2920 0.970740020275116
2930 0.973039984703064
2940 0.963519990444183
2950 0.970839977264404
2960 0.970579981803894
2970 0.976679980754852
2980 0.966019988059998
2990 0.971140027046204
3000 0.970380008220673
3010 0.973860025405884
3020 0.971239984035492
3030 0.974960029125214
3040 0.976119995117188
3050 0.967939972877502
3060 0.971499979496002
3070 0.974179983139038
3080 0.970740020275116
3090 0.975399971008301
3100 0.976000010967255
3110 0.973020017147064
3120 0.974439978599548
3130 0.97188001871109
3140 0.975279986858368
3150 0.970659971237183
3160 0.970860004425049
3170 0.972800016403198
3180 0.972959995269775
3190 0.974020004272461
3200 0.967999994754791
3210 0.973940014839172
3220 0.975419998168945
3230 0.971819996833801
3240 0.973999977111816
3250 0.970960021018982
3260 0.974979996681213
3270 0.974720001220703
3280 0.972639977931976
3290 0.973599970340729
3300 0.972800016403198
3310 0.967040002346039
3320 0.961660027503967
3330 0.972500026226044
3340 0.9721400141716
3350 0.976019978523254
3360 0.972320020198822
3370 0.973699986934662
3380 0.972940027713776
3390 0.95551997423172
3400 0.973339974880219
3410 0.958140015602112
3420 0.970000028610229
3430 0.974039971828461
3440 0.974799990653992
3450 0.975179970264435
3460 0.974919974803925
3470 0.96969997882843
3480 0.973580002784729
3490 0.97623997926712
3500 0.971300005912781
3510 0.976979970932007
3520 0.970560014247894
3530 0.973140001296997
3540 0.969780027866364
3550 0.972639977931976
3560 0.971319973468781
3570 0.971660017967224
3580 0.974380016326904
3590 0.968739986419678
3600 0.975059986114502
3610 0.969919979572296
3620 0.971099972724915
3630 0.971679985523224
3640 0.97136002779007
3650 0.97052001953125
3660 0.974380016326904
3670 0.976279973983765
3680 0.97298002243042
3690 0.972679972648621
3700 0.978519976139069
3710 0.973760008811951
3720 0.973060011863708
3730 0.974579989910126
3740 0.978619992733002
3750 0.973699986934662
3760 0.974740028381348
3770 0.970960021018982
3780 0.974219977855682
3790 0.973420023918152
3800 0.969560027122498
3810 0.979420006275177
3820 0.973760008811951
3830 0.970319986343384
3840 0.97272002696991
3850 0.974139988422394
3860 0.976979970932007
3870 0.976480007171631
3880 0.972220003604889
3890 0.977199971675873
3900 0.976779997348785
3910 0.972379982471466
3920 0.974960029125214
3930 0.97460001707077
3940 0.977559983730316
3950 0.980260014533997
3960 0.9757199883461
3970 0.9721599817276
3980 0.977840006351471
3990 0.977180004119873
4000 0.971459984779358
4010 0.970359981060028
4020 0.976059973239899
4030 0.978219985961914
4040 0.974720001220703
4050 0.977479994297028
4060 0.974279999732971
4070 0.976000010967255
4080 0.980180025100708
4090 0.980560004711151
4100 0.977439999580383
4110 0.973980009555817
4120 0.977360010147095
4130 0.978280007839203
4140 0.975660026073456
4150 0.976660013198853
4160 0.971419990062714
4170 0.973599970340729
4180 0.97162002325058
4190 0.973039984703064
4200 0.972039997577667
4210 0.975539982318878
4220 0.972679972648621
4230 0.975780010223389
4240 0.973999977111816
4250 0.975539982318878
4260 0.972500026226044
4270 0.979759991168976
4280 0.974560022354126
4290 0.974120020866394
4300 0.96942001581192
4310 0.97487998008728
4320 0.978519976139069
4330 0.976199984550476
4340 0.971960008144379
4350 0.970179975032806
4360 0.975059986114502
4370 0.972459971904755
4380 0.973800003528595
4390 0.978359997272491
4400 0.971979975700378
4410 0.967779994010925
4420 0.97978001832962
4430 0.971700012683868
4440 0.978240013122559
4450 0.977580010890961
4460 0.968299984931946
4470 0.977020025253296
4480 0.974039971828461
4490 0.974479973316193
4500 0.97241997718811
4510 0.973659992218018
4520 0.976679980754852
4530 0.973919987678528
4540 0.973879992961884
4550 0.971080005168915
4560 0.973640024662018
4570 0.973299980163574
4580 0.971340000629425
4590 0.975480020046234
4600 0.975040018558502
4610 0.972819983959198
4620 0.979860007762909
4630 0.974640011787415
4640 0.976700007915497
4650 0.978479981422424
4660 0.97053998708725
4670 0.97351998090744
4680 0.975759983062744
4690 0.976620018482208
4700 0.976400017738342
4710 0.973819971084595
4720 0.977119982242584
4730 0.976840019226074
4740 0.974680006504059
4750 0.973200023174286
4760 0.973640024662018
4770 0.973339974880219
4780 0.980279982089996
4790 0.977800011634827
4800 0.978460013866425
4810 0.973680019378662
4820 0.975380003452301
4830 0.97434002161026
4840 0.976040005683899
4850 0.972440004348755
4860 0.97654002904892
4870 0.9757000207901
4880 0.975480020046234
4890 0.973460018634796
4900 0.975199997425079
4910 0.974279999732971
4920 0.96916002035141
4930 0.976740002632141
4940 0.976899981498718
4950 0.979600012302399
4960 0.977439999580383
4970 0.975260019302368
4980 0.976840019226074
4990 0.976279973983765
5000 0.975019991397858
};
%\addlegendentry{Train}
\addplot[semithick, color3] %x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.678300023078918
10 0.701499998569489
20 0.684700012207031
30 0.683300018310547
40 0.684599995613098
50 0.704200029373169
60 0.683200001716614
70 0.69870001077652
80 0.686900019645691
90 0.676400005817413
100 0.690199971199036
110 0.685199975967407
120 0.699699997901917
130 0.700100004673004
140 0.702099978923798
150 0.700699985027313
160 0.687200009822845
170 0.694000005722046
180 0.688899993896484
190 0.700800001621246
200 0.6942999958992
210 0.696900010108948
220 0.693899989128113
230 0.68529999256134
240 0.667800009250641
250 0.688799977302551
260 0.687200009822845
270 0.702600002288818
280 0.674199998378754
290 0.696699976921082
300 0.695599973201752
310 0.701399981975555
320 0.687600016593933
330 0.704100012779236
340 0.687200009822845
350 0.690100014209747
360 0.694400012493134
370 0.682900011539459
380 0.682799994945526
390 0.692399978637695
400 0.687399983406067
410 0.71340000629425
420 0.697099983692169
430 0.685100018978119
440 0.690999984741211
450 0.688499987125397
460 0.692099988460541
470 0.699599981307983
480 0.692799985408783
490 0.698199987411499
500 0.688799977302551
510 0.689599990844727
520 0.686900019645691
530 0.684000015258789
540 0.681100010871887
550 0.693199992179871
560 0.69080001115799
570 0.690599977970123
580 0.695599973201752
590 0.706700026988983
600 0.690900027751923
610 0.711899995803833
620 0.678099989891052
630 0.706399977207184
640 0.681500017642975
650 0.688700020313263
660 0.692499995231628
670 0.682299971580505
680 0.688700020313263
690 0.70169997215271
700 0.678099989891052
710 0.697499990463257
720 0.707499980926514
730 0.694199979305267
740 0.684499979019165
750 0.69980001449585
760 0.679199993610382
770 0.6875
780 0.698899984359741
790 0.687699973583221
800 0.674199998378754
810 0.69379997253418
820 0.697399973869324
830 0.681800007820129
840 0.696099996566772
850 0.687600016593933
860 0.690100014209747
870 0.698800027370453
880 0.697200000286102
890 0.700200021266937
900 0.697000026702881
910 0.710600018501282
920 0.698800027370453
930 0.691399991512299
940 0.698000013828278
950 0.67059999704361
960 0.697700023651123
970 0.700699985027313
980 0.700200021266937
990 0.685199975967407
1000 0.691799998283386
1010 0.686200022697449
1020 0.702099978923798
1030 0.687699973583221
1040 0.688199996948242
1050 0.694199979305267
1060 0.690699994564056
1070 0.691399991512299
1080 0.689400017261505
1090 0.696300029754639
1100 0.683000028133392
1110 0.682799994945526
1120 0.69650000333786
1130 0.694800019264221
1140 0.692099988460541
1150 0.677500009536743
1160 0.697300016880035
1170 0.690900027751923
1180 0.685699999332428
1190 0.698800027370453
1200 0.700999975204468
1210 0.679499983787537
1220 0.696699976921082
1230 0.705299973487854
1240 0.702199995517731
1250 0.699699997901917
1260 0.702600002288818
1270 0.706499993801117
1280 0.68639999628067
1290 0.69980001449585
1300 0.691299974918365
1310 0.671800017356873
1320 0.688700020313263
1330 0.710600018501282
1340 0.691699981689453
1350 0.699699997901917
1360 0.693599998950958
1370 0.683200001716614
1380 0.697700023651123
1390 0.698000013828278
1400 0.70279997587204
1410 0.703299999237061
1420 0.69080001115799
1430 0.689899981021881
1440 0.697799980640411
1450 0.683200001716614
1460 0.703599989414215
1470 0.681400001049042
1480 0.684700012207031
1490 0.705099999904633
1500 0.697899997234344
1510 0.71340000629425
1520 0.695699989795685
1530 0.698400020599365
1540 0.703100025653839
1550 0.694599986076355
1560 0.69379997253418
1570 0.695500016212463
1580 0.689100027084351
1590 0.707199990749359
1600 0.679400026798248
1610 0.705600023269653
1620 0.689599990844727
1630 0.688799977302551
1640 0.702899992465973
1650 0.691299974918365
1660 0.707199990749359
1670 0.699299991130829
1680 0.690699994564056
1690 0.696600019931793
1700 0.690900027751923
1710 0.700999975204468
1720 0.687900006771088
1730 0.693099975585938
1740 0.685100018978119
1750 0.698300004005432
1760 0.703599989414215
1770 0.686100006103516
1780 0.694000005722046
1790 0.700200021266937
1800 0.681900024414062
1810 0.700699985027313
1820 0.685800015926361
1830 0.676500022411346
1840 0.691799998283386
1850 0.693400025367737
1860 0.704599976539612
1870 0.685599982738495
1880 0.692900002002716
1890 0.692900002002716
1900 0.693499982357025
1910 0.689599990844727
1920 0.698400020599365
1930 0.697300016880035
1940 0.677699983119965
1950 0.693700015544891
1960 0.684800028800964
1970 0.699500024318695
1980 0.703400015830994
1990 0.707799971103668
2000 0.695200026035309
2010 0.675599992275238
2020 0.693899989128113
2030 0.679499983787537
2040 0.679799973964691
2050 0.695800006389618
2060 0.699000000953674
2070 0.697200000286102
2080 0.684400022029877
2090 0.692799985408783
2100 0.676999986171722
2110 0.69650000333786
2120 0.708100020885468
2130 0.693599998950958
2140 0.699000000953674
2150 0.705399990081787
2160 0.704299986362457
2170 0.691600024700165
2180 0.69080001115799
2190 0.702700018882751
2200 0.676500022411346
2210 0.699100017547607
2220 0.694599986076355
2230 0.706099987030029
2240 0.695100009441376
2250 0.691799998283386
2260 0.688099980354309
2270 0.679899990558624
2280 0.689199984073639
2290 0.694100022315979
2300 0.700800001621246
2310 0.683300018310547
2320 0.675999999046326
2330 0.686900019645691
2340 0.690400004386902
2350 0.689499974250793
2360 0.69489997625351
2370 0.677100002765656
2380 0.658800005912781
2390 0.688300013542175
2400 0.695299983024597
2410 0.695500016212463
2420 0.685699999332428
2430 0.694100022315979
2440 0.687600016593933
2450 0.689599990844727
2460 0.691600024700165
2470 0.700399994850159
2480 0.707899987697601
2490 0.675000011920929
2500 0.694999992847443
2510 0.710799992084503
2520 0.676400005817413
2530 0.687900006771088
2540 0.674899995326996
2550 0.68860000371933
2560 0.703299999237061
2570 0.692900002002716
2580 0.676999986171722
2590 0.693099975585938
2600 0.686999976634979
2610 0.695800006389618
2620 0.691399991512299
2630 0.702700018882751
2640 0.691900014877319
2650 0.689300000667572
2660 0.687099993228912
2670 0.692499995231628
2680 0.699199974536896
2690 0.700999975204468
2700 0.693499982357025
2710 0.685800015926361
2720 0.689800024032593
2730 0.699500024318695
2740 0.660199999809265
2750 0.688199996948242
2760 0.690500020980835
2770 0.69489997625351
2780 0.684099972248077
2790 0.693300008773804
2800 0.690500020980835
2810 0.699899971485138
2820 0.70990002155304
2830 0.688199996948242
2840 0.699000000953674
2850 0.692700028419495
2860 0.702400028705597
2870 0.69080001115799
2880 0.705399990081787
2890 0.700500011444092
2900 0.678300023078918
2910 0.689000010490417
2920 0.68970000743866
2930 0.685199975967407
2940 0.681699991226196
2950 0.687799990177155
2960 0.69080001115799
2970 0.688799977302551
2980 0.682799994945526
2990 0.680800020694733
3000 0.680000007152557
3010 0.691500008106232
3020 0.680599987506866
3030 0.702300012111664
3040 0.70169997215271
3050 0.680000007152557
3060 0.688700020313263
3070 0.686600029468536
3080 0.697700023651123
3090 0.698099970817566
3100 0.701499998569489
3110 0.692099988460541
3120 0.686800003051758
3130 0.693599998950958
3140 0.678900003433228
3150 0.683399975299835
3160 0.683600008487701
3170 0.682699978351593
3180 0.685500025749207
3190 0.684499979019165
3200 0.690999984741211
3210 0.674700021743774
3220 0.682900011539459
3230 0.692399978637695
3240 0.684099972248077
3250 0.6875
3260 0.685899972915649
3270 0.688000023365021
3280 0.682299971580505
3290 0.679799973964691
3300 0.686500012874603
3310 0.693300008773804
3320 0.679400026798248
3330 0.680199980735779
3340 0.687600016593933
3350 0.692700028419495
3360 0.680800020694733
3370 0.695900022983551
3380 0.695200026035309
3390 0.694100022315979
3400 0.686800003051758
3410 0.682699978351593
3420 0.701099991798401
3430 0.681699991226196
3440 0.686200022697449
3450 0.683499991893768
3460 0.694500029087067
3470 0.694500029087067
3480 0.691799998283386
3490 0.689999997615814
3500 0.708500027656555
3510 0.695200026035309
3520 0.687399983406067
3530 0.705399990081787
3540 0.6942999958992
3550 0.675400018692017
3560 0.703299999237061
3570 0.685100018978119
3580 0.687799990177155
3590 0.691600024700165
3600 0.671299993991852
3610 0.692799985408783
3620 0.697899997234344
3630 0.689800024032593
3640 0.692499995231628
3650 0.697899997234344
3660 0.690500020980835
3670 0.686999976634979
3680 0.688700020313263
3690 0.691500008106232
3700 0.690699994564056
3710 0.69489997625351
3720 0.688899993896484
3730 0.693300008773804
3740 0.694100022315979
3750 0.703199982643127
3760 0.682799994945526
3770 0.700500011444092
3780 0.697200000286102
3790 0.711499989032745
3800 0.700399994850159
3810 0.692399978637695
3820 0.694400012493134
3830 0.681100010871887
3840 0.68529999256134
3850 0.691399991512299
3860 0.687099993228912
3870 0.702099978923798
3880 0.691600024700165
3890 0.700699985027313
3900 0.698899984359741
3910 0.703199982643127
3920 0.691699981689453
3930 0.671199977397919
3940 0.688000023365021
3950 0.699599981307983
3960 0.690900027751923
3970 0.684400022029877
3980 0.696399986743927
3990 0.696600019931793
4000 0.694999992847443
4010 0.700299978256226
4020 0.697000026702881
4030 0.680499970912933
4040 0.697700023651123
4050 0.6875
4060 0.691299974918365
4070 0.700999975204468
4080 0.696699976921082
4090 0.69080001115799
4100 0.687099993228912
4110 0.69980001449585
4120 0.695599973201752
4130 0.68529999256134
4140 0.704299986362457
4150 0.695299983024597
4160 0.681900024414062
4170 0.699699997901917
4180 0.689199984073639
4190 0.691699981689453
4200 0.689199984073639
4210 0.688300013542175
4220 0.691100001335144
4230 0.699599981307983
4240 0.697099983692169
4250 0.700200021266937
4260 0.698099970817566
4270 0.681999981403351
4280 0.670300006866455
4290 0.691900014877319
4300 0.69980001449585
4310 0.688700020313263
4320 0.691299974918365
4330 0.70169997215271
4340 0.697200000286102
4350 0.690500020980835
4360 0.691399991512299
4370 0.701399981975555
4380 0.689199984073639
4390 0.697700023651123
4400 0.683200001716614
4410 0.6942999958992
4420 0.677500009536743
4430 0.688399970531464
4440 0.68419998884201
4450 0.697300016880035
4460 0.679899990558624
4470 0.679899990558624
4480 0.700399994850159
4490 0.684000015258789
4500 0.688499987125397
4510 0.685100018978119
4520 0.684000015258789
4530 0.702199995517731
4540 0.694800019264221
4550 0.690699994564056
4560 0.685999989509583
4570 0.684899985790253
4580 0.694500029087067
4590 0.691699981689453
4600 0.694400012493134
4610 0.689800024032593
4620 0.687300026416779
4630 0.689800024032593
4640 0.696300029754639
4650 0.687099993228912
4660 0.697799980640411
4670 0.679899990558624
4680 0.682799994945526
4690 0.686299979686737
4700 0.669799983501434
4710 0.693700015544891
4720 0.688000023365021
4730 0.677799999713898
4740 0.687300026416779
4750 0.689999997615814
4760 0.693300008773804
4770 0.687799990177155
4780 0.689400017261505
4790 0.685800015926361
4800 0.696200013160706
4810 0.695299983024597
4820 0.678900003433228
4830 0.674899995326996
4840 0.69379997253418
4850 0.6807000041008
4860 0.685400009155273
4870 0.695500016212463
4880 0.681699991226196
4890 0.697799980640411
4900 0.67960000038147
4910 0.696799993515015
4920 0.677100002765656
4930 0.685599982738495
4940 0.693099975585938
4950 0.693099975585938
4960 0.702000021934509
4970 0.682799994945526
4980 0.68639999628067
4990 0.689599990844727
5000 0.684899985790253
};
%\addlegendentry{Test}

==> experiments/figures/mae_ccei_05.tex <==
\addplot[semithick, color4] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.911339998245239
10 0.913519978523254
20 0.913839995861053
30 0.905380010604858
40 0.915180027484894
50 0.90991997718811
60 0.916000008583069
70 0.909759998321533
80 0.913600027561188
90 0.919539988040924
100 0.911440014839172
110 0.9132199883461
120 0.91567999124527
130 0.917739987373352
140 0.916740000247955
150 0.915820002555847
160 0.919399976730347
170 0.921000003814697
180 0.895380020141602
190 0.917100012302399
200 0.914399981498718
210 0.914279997348785
220 0.914979994297028
230 0.919719994068146
240 0.920459985733032
250 0.919319987297058
260 0.918500006198883
270 0.911639988422394
280 0.918860018253326
290 0.903819978237152
300 0.91075998544693
310 0.916400015354156
320 0.920059978961945
330 0.904039978981018
340 0.918079972267151
350 0.921760022640228
360 0.925480008125305
370 0.909699976444244
380 0.897599995136261
390 0.923240005970001
400 0.91592001914978
410 0.91049998998642
420 0.907339990139008
430 0.916279971599579
440 0.914499998092651
450 0.913619995117188
460 0.918500006198883
470 0.903159976005554
480 0.910099983215332
490 0.925539970397949
500 0.912840008735657
510 0.922959983348846
520 0.921019971370697
530 0.917439997196198
540 0.923200011253357
550 0.924440026283264
560 0.918760001659393
570 0.915260016918182
580 0.92331999540329
590 0.924459993839264
600 0.913980007171631
610 0.914099991321564
620 0.920880019664764
630 0.914240002632141
640 0.925679981708527
650 0.917060017585754
660 0.92221999168396
670 0.91865998506546
680 0.912180006504059
690 0.919619977474213
700 0.927460014820099
710 0.919219970703125
720 0.912999987602234
730 0.927940011024475
740 0.920780003070831
750 0.917100012302399
760 0.925960004329681
770 0.921700000762939
780 0.920300006866455
790 0.919099986553192
800 0.915560007095337
810 0.924319982528687
820 0.91865998506546
830 0.922079980373383
840 0.92084002494812
850 0.92629998922348
860 0.927640020847321
870 0.921220004558563
880 0.9271399974823
890 0.922720015048981
900 0.923900008201599
910 0.920300006866455
920 0.92110002040863
930 0.916519999504089
940 0.92874002456665
950 0.91431999206543
960 0.929719984531403
970 0.925300002098083
980 0.922140002250671
990 0.922720015048981
1000 0.925679981708527
1010 0.922940015792847
1020 0.922420024871826
1030 0.918860018253326
1040 0.916480004787445
1050 0.928319990634918
1060 0.933279991149902
1070 0.930880010128021
1080 0.93478000164032
1090 0.929220020771027
1100 0.920780003070831
1110 0.929139971733093
1120 0.917840003967285
1130 0.925859987735748
1140 0.917900025844574
1150 0.92467999458313
1160 0.928560018539429
1170 0.927619993686676
1180 0.928120017051697
1190 0.925719976425171
1200 0.921720027923584
1210 0.922619998455048
1220 0.928939998149872
1230 0.920040011405945
1240 0.928780019283295
1250 0.929400026798248
1260 0.92519998550415
1270 0.930880010128021
1280 0.929359972476959
1290 0.919459998607635
1300 0.933600008487701
1310 0.925080001354218
1320 0.932919979095459
1330 0.929579973220825
1340 0.92765998840332
1350 0.923820018768311
1360 0.929660022258759
1370 0.920400023460388
1380 0.934000015258789
1390 0.9167600274086
1400 0.933120012283325
1410 0.92960000038147
1420 0.92137998342514
1430 0.921500027179718
1440 0.92765998840332
1450 0.927320003509521
1460 0.931060016155243
1470 0.92985999584198
1480 0.929359972476959
1490 0.930480003356934
1500 0.92629998922348
1510 0.928200006484985
1520 0.9307000041008
1530 0.928059995174408
1540 0.933340013027191
1550 0.927359998226166
1560 0.922800004482269
1570 0.920520007610321
1580 0.933820009231567
1590 0.924120008945465
1600 0.920660018920898
1610 0.923500001430511
1620 0.928879976272583
1630 0.924440026283264
1640 0.925599992275238
1650 0.918600022792816
1660 0.927320003509521
1670 0.918240010738373
1680 0.925520002841949
1690 0.936959981918335
1700 0.924520015716553
1710 0.925740003585815
1720 0.92960000038147
1730 0.92738002538681
1740 0.928160011768341
1750 0.926440000534058
1760 0.935479998588562
1770 0.928020000457764
1780 0.927500009536743
1790 0.936299979686737
1800 0.926819980144501
1810 0.92221999168396
1820 0.921840012073517
1830 0.921280026435852
1840 0.929139971733093
1850 0.9307000041008
1860 0.92960000038147
1870 0.936259984970093
1880 0.934419989585876
1890 0.929679989814758
1900 0.933860003948212
1910 0.925840020179749
1920 0.929820001125336
1930 0.935419976711273
1940 0.931039988994598
1950 0.934920012950897
1960 0.926460027694702
1970 0.920780003070831
1980 0.927479982376099
1990 0.919579982757568
2000 0.929040014743805
2010 0.933640003204346
2020 0.934599995613098
2030 0.920360028743744
2040 0.929199993610382
2050 0.925119996070862
2060 0.934859991073608
2070 0.936519980430603
2080 0.934759974479675
2090 0.932739973068237
2100 0.930760025978088
2110 0.927219986915588
2120 0.939379990100861
2130 0.932240009307861
2140 0.926959991455078
2150 0.937300026416779
2160 0.932179987430573
2170 0.931500017642975
2180 0.934340000152588
2190 0.935419976711273
2200 0.934300005435944
2210 0.927839994430542
2220 0.936079978942871
2230 0.933459997177124
2240 0.935140013694763
2250 0.922420024871826
2260 0.935559988021851
2270 0.926360011100769
2280 0.932879984378815
2290 0.932600021362305
2300 0.937979996204376
2310 0.934960007667542
2320 0.931699991226196
2330 0.932420015335083
2340 0.937460005283356
2350 0.935559988021851
2360 0.937120020389557
2370 0.930920004844666
2380 0.928640007972717
2390 0.941420018672943
2400 0.935679972171783
2410 0.936079978942871
2420 0.930360019207001
2430 0.934319972991943
2440 0.935620009899139
2450 0.9271399974823
2460 0.930760025978088
2470 0.936259984970093
2480 0.930360019207001
2490 0.941160023212433
2500 0.940079987049103
2510 0.931420028209686
2520 0.924019992351532
2530 0.932720005512238
2540 0.932439982891083
2550 0.929899990558624
2560 0.928539991378784
2570 0.933719992637634
2580 0.933719992637634
2590 0.934360027313232
2600 0.930260002613068
2610 0.932359993457794
2620 0.937680006027222
2630 0.931760013103485
2640 0.936900019645691
2650 0.932980000972748
2660 0.935859978199005
2670 0.919139981269836
2680 0.936559975147247
2690 0.934960007667542
2700 0.934840023517609
2710 0.938579976558685
2720 0.939800024032593
2730 0.939999997615814
2740 0.93503999710083
2750 0.930299997329712
2760 0.932519972324371
2770 0.930999994277954
2780 0.938759982585907
2790 0.935060024261475
2800 0.93206000328064
2810 0.930180013179779
2820 0.936860024929047
2830 0.93257999420166
2840 0.933600008487701
2850 0.929239988327026
2860 0.917739987373352
2870 0.933459997177124
2880 0.930499970912933
2890 0.938199996948242
2900 0.93665999174118
2910 0.932900011539459
2920 0.934319972991943
2930 0.938839972019196
2940 0.941259980201721
2950 0.932359993457794
2960 0.932799994945526
2970 0.93614000082016
2980 0.938979983329773
2990 0.939079999923706
3000 0.932200014591217
3010 0.935959994792938
3020 0.92984002828598
3030 0.938059985637665
3040 0.936439990997314
3050 0.924480020999908
3060 0.936460018157959
3070 0.940599977970123
3080 0.932079970836639
3090 0.927219986915588
3100 0.941739976406097
3110 0.939840018749237
3120 0.935459971427917
3130 0.932160019874573
3140 0.933200001716614
3150 0.943139970302582
3160 0.939180016517639
3170 0.937139987945557
3180 0.934700012207031
3190 0.936640024185181
3200 0.92493999004364
3210 0.934800028800964
3220 0.931599974632263
3230 0.94352000951767
3240 0.93834000825882
3250 0.93502002954483
3260 0.931620001792908
3270 0.945079982280731
3280 0.940680027008057
3290 0.939620018005371
3300 0.934459984302521
3310 0.937080025672913
3320 0.932120025157928
3330 0.941460013389587
3340 0.939079999923706
3350 0.931180000305176
3360 0.938319981098175
3370 0.930739998817444
3380 0.938000023365021
3390 0.939199984073639
3400 0.940140008926392
3410 0.939719974994659
3420 0.935980021953583
3430 0.940280020236969
3440 0.943099975585938
3450 0.932760000228882
3460 0.941100001335144
3470 0.938399970531464
3480 0.938139975070953
3490 0.940379977226257
3500 0.936999976634979
3510 0.938319981098175
3520 0.940039992332458
3530 0.932439982891083
3540 0.941179990768433
3550 0.943000018596649
3560 0.936179995536804
3570 0.934920012950897
3580 0.944620013237
3590 0.940240025520325
3600 0.933380007743835
3610 0.939040005207062
3620 0.944559991359711
3630 0.932600021362305
3640 0.936999976634979
3650 0.936900019645691
3660 0.939939975738525
3670 0.934279978275299
3680 0.935540020465851
3690 0.946099996566772
3700 0.935220003128052
3710 0.933399975299835
3720 0.940280020236969
3730 0.930719971656799
3740 0.940180003643036
3750 0.940739989280701
3760 0.940339982509613
3770 0.934159994125366
3780 0.925080001354218
3790 0.941640019416809
3800 0.939740002155304
3810 0.933979988098145
3820 0.940439999103546
3830 0.935500025749207
3840 0.931500017642975
3850 0.942879974842072
3860 0.93502002954483
3870 0.938120007514954
3880 0.93997997045517
3890 0.930499970912933
3900 0.936160027980804
3910 0.937560021877289
3920 0.936839997768402
3930 0.941359996795654
3940 0.937579989433289
3950 0.933979988098145
3960 0.940159976482391
3970 0.935320019721985
3980 0.939279973506927
3990 0.935739994049072
4000 0.943359971046448
4010 0.940419971942902
4020 0.930660009384155
4030 0.944079995155334
4040 0.941020011901855
4050 0.935940027236938
4060 0.943740010261536
4070 0.941820025444031
4080 0.936720013618469
4090 0.936420023441315
4100 0.938719987869263
4110 0.940280020236969
4120 0.932940006256104
4130 0.935000002384186
4140 0.938319981098175
4150 0.931320011615753
4160 0.939880013465881
4170 0.937839984893799
4180 0.939239978790283
4190 0.938780009746552
4200 0.939320027828217
4210 0.941559970378876
4220 0.942179977893829
4230 0.935760021209717
4240 0.93257999420166
4250 0.940119981765747
4260 0.943700015544891
4270 0.939540028572083
4280 0.943379998207092
4290 0.940439999103546
4300 0.936940014362335
4310 0.9410799741745
4320 0.938899993896484
4330 0.939719974994659
4340 0.937479972839355
4350 0.933239996433258
4360 0.945100009441376
4370 0.941479980945587
4380 0.944199979305267
4390 0.936160027980804
4400 0.945999979972839
4410 0.939540028572083
4420 0.938359975814819
4430 0.937439978122711
4440 0.942059993743896
4450 0.943199992179871
4460 0.941039979457855
4470 0.941479980945587
4480 0.94157999753952
4490 0.943040013313293
4500 0.933579981327057
4510 0.946619987487793
4520 0.946099996566772
4530 0.941100001335144
4540 0.939140021800995
4550 0.945219993591309
4560 0.939520001411438
4570 0.942640006542206
4580 0.93834000825882
4590 0.946160018444061
4600 0.944360017776489
4610 0.938319981098175
4620 0.947019994258881
4630 0.931760013103485
4640 0.939580023288727
4650 0.938239991664886
4660 0.933120012283325
4670 0.939899981021881
4680 0.940659999847412
4690 0.940639972686768
4700 0.937120020389557
4710 0.942640006542206
4720 0.939360022544861
4730 0.944239974021912
4740 0.939459979534149
4750 0.942799985408783
4760 0.9375
4770 0.938380002975464
4780 0.93911999464035
4790 0.93665999174118
4800 0.934580028057098
4810 0.940240025520325
4820 0.941980004310608
4830 0.942099988460541
4840 0.943840026855469
4850 0.938719987869263
4860 0.947239995002747
4870 0.939300000667572
4880 0.947019994258881
4890 0.931940019130707
4900 0.944679975509644
4910 0.944239974021912
4920 0.932160019874573
4930 0.942260026931763
4940 0.939779996871948
4950 0.934580028057098
4960 0.946080029010773
4970 0.939279973506927
4980 0.937479972839355
4990 0.939260005950928
5000 0.943660020828247
};
%\addlegendentry{Train}
\addplot[semithick, color5] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.454299986362457
10 0.522700011730194
20 0.522300004959106
30 0.510999977588654
40 0.501999974250793
50 0.510999977588654
60 0.499799996614456
70 0.526300013065338
80 0.507000029087067
90 0.519400000572205
100 0.517000019550323
110 0.510500013828278
120 0.516099989414215
130 0.519999980926514
140 0.518400013446808
150 0.516099989414215
160 0.499000012874603
170 0.500999987125397
180 0.513100028038025
190 0.495200008153915
200 0.499799996614456
210 0.500599980354309
220 0.503199994564056
230 0.513700008392334
240 0.520299971103668
250 0.513100028038025
260 0.501699984073639
270 0.50900000333786
280 0.504299998283386
290 0.511699974536896
300 0.506900012493134
310 0.515699982643127
320 0.513800024986267
330 0.500999987125397
340 0.526600003242493
350 0.513999998569489
360 0.512499988079071
370 0.50900000333786
380 0.501500010490417
390 0.512399971485138
400 0.508300006389618
410 0.521099984645844
420 0.520799994468689
430 0.510500013828278
440 0.520699977874756
450 0.509999990463257
460 0.500400006771088
470 0.483000010251999
480 0.509400010108948
490 0.518700003623962
500 0.505500018596649
510 0.508400022983551
520 0.508899986743927
530 0.521200001239777
540 0.510999977588654
550 0.505299985408783
560 0.510299980640411
570 0.513400018215179
580 0.500999987125397
590 0.504000008106232
600 0.507799983024597
610 0.511799991130829
620 0.510299980640411
630 0.520799994468689
640 0.521000027656555
650 0.504000008106232
660 0.507799983024597
670 0.515600025653839
680 0.499599993228912
690 0.509400010108948
700 0.528800010681152
710 0.504400014877319
720 0.508199989795685
730 0.509299993515015
740 0.504000008106232
750 0.530700027942657
760 0.511300027370453
770 0.516099989414215
780 0.512700021266937
790 0.509999990463257
800 0.505699992179871
810 0.509199976921082
820 0.497399985790253
830 0.512399971485138
840 0.508899986743927
850 0.511900007724762
860 0.511300027370453
870 0.508700013160706
880 0.504299998283386
890 0.505299985408783
900 0.514699995517731
910 0.508800029754639
920 0.508000016212463
930 0.521399974822998
940 0.518499970436096
950 0.50789999961853
960 0.503899991512299
970 0.504800021648407
980 0.502799987792969
990 0.498100012540817
1000 0.511300027370453
1010 0.50110000371933
1020 0.494599997997284
1030 0.516600012779236
1040 0.522599995136261
1050 0.49770000576973
1060 0.512899994850159
1070 0.508400022983551
1080 0.50330001115799
1090 0.502300024032593
1100 0.507799983024597
1110 0.50739997625351
1120 0.521000027656555
1130 0.522800028324127
1140 0.507499992847443
1150 0.513000011444092
1160 0.512700021266937
1170 0.514500021934509
1180 0.513100028038025
1190 0.525799989700317
1200 0.500800013542175
1210 0.510900020599365
1220 0.515200018882751
1230 0.507200002670288
1240 0.501699984073639
1250 0.512700021266937
1260 0.511099994182587
1270 0.505299985408783
1280 0.508599996566772
1290 0.510900020599365
1300 0.515100002288818
1310 0.500500023365021
1320 0.504599988460541
1330 0.496499985456467
1340 0.516700029373169
1350 0.495999991893768
1360 0.512899994850159
1370 0.512600004673004
1380 0.518800020217896
1390 0.489499986171722
1400 0.502499997615814
1410 0.500599980354309
1420 0.498400002717972
1430 0.509500026702881
1440 0.500400006771088
1450 0.503700017929077
1460 0.503600001335144
1470 0.503899991512299
1480 0.509800016880035
1490 0.505900025367737
1500 0.509400010108948
1510 0.516600012779236
1520 0.52240002155304
1530 0.50330001115799
1540 0.526199996471405
1550 0.504700005054474
1560 0.511300027370453
1570 0.515500009059906
1580 0.519299983978271
1590 0.512799978256226
1600 0.497299998998642
1610 0.517199993133545
1620 0.502399981021881
1630 0.507000029087067
1640 0.516700029373169
1650 0.512199997901917
1660 0.515100002288818
1670 0.487300008535385
1680 0.507700026035309
1690 0.508899986743927
1700 0.513499975204468
1710 0.519699990749359
1720 0.500500023365021
1730 0.508300006389618
1740 0.496399998664856
1750 0.509100019931793
1760 0.519500017166138
1770 0.504400014877319
1780 0.513100028038025
1790 0.51419997215271
1800 0.507300019264221
1810 0.501699984073639
1820 0.52130001783371
1830 0.490799993276596
1840 0.509299993515015
1850 0.498699992895126
1860 0.523999989032745
1870 0.511699974536896
1880 0.511799991130829
1890 0.509599983692169
1900 0.505699992179871
1910 0.515799999237061
1920 0.513700008392334
1930 0.489199995994568
1940 0.486600011587143
1950 0.510599970817566
1960 0.517799973487854
1970 0.509400010108948
1980 0.509700000286102
1990 0.506399989128113
2000 0.508099973201752
2010 0.509100019931793
2020 0.513999998569489
2030 0.520099997520447
2040 0.516700029373169
2050 0.495599985122681
2060 0.522199988365173
2070 0.510900020599365
2080 0.499599993228912
2090 0.514299988746643
2100 0.508499979972839
2110 0.51230001449585
2120 0.509199976921082
2130 0.516099989414215
2140 0.517799973487854
2150 0.507000029087067
2160 0.510900020599365
2170 0.518700003623962
2180 0.518599987030029
2190 0.505100011825562
2200 0.497099995613098
2210 0.499599993228912
2220 0.511500000953674
2230 0.501699984073639
2240 0.502799987792969
2250 0.506099998950958
2260 0.516700029373169
2270 0.528900027275085
2280 0.508899986743927
2290 0.512899994850159
2300 0.504100024700165
2310 0.500999987125397
2320 0.508499979972839
2330 0.507300019264221
2340 0.499599993228912
2350 0.509800016880035
2360 0.511300027370453
2370 0.513199985027313
2380 0.509100019931793
2390 0.517899990081787
2400 0.520299971103668
2410 0.51010000705719
2420 0.505599975585938
2430 0.49889999628067
2440 0.496899992227554
2450 0.524600028991699
2460 0.50789999961853
2470 0.513100028038025
2480 0.513800024986267
2490 0.504999995231628
2500 0.513599991798401
2510 0.503899991512299
2520 0.492500007152557
2530 0.494300007820129
2540 0.497099995613098
2550 0.488200008869171
2560 0.502499997615814
2570 0.514900028705597
2580 0.496300011873245
2590 0.502900004386902
2600 0.511399984359741
2610 0.513300001621246
2620 0.51529997587204
2630 0.521799981594086
2640 0.509199976921082
2650 0.507700026035309
2660 0.513199985027313
2670 0.509800016880035
2680 0.529999971389771
2690 0.499700009822845
2700 0.512000024318695
2710 0.50789999961853
2720 0.501299977302551
2730 0.505500018596649
2740 0.513400018215179
2750 0.485700011253357
2760 0.524699985980988
2770 0.502799987792969
2780 0.503799974918365
2790 0.504299998283386
2800 0.500899970531464
2810 0.526600003242493
2820 0.508000016212463
2830 0.50739997625351
2840 0.49329999089241
2850 0.508700013160706
2860 0.497299998998642
2870 0.501299977302551
2880 0.519800007343292
2890 0.515999972820282
2900 0.51800000667572
2910 0.50220000743866
2920 0.498499989509583
2930 0.503899991512299
2940 0.505699992179871
2950 0.497900009155273
2960 0.508499979972839
2970 0.497099995613098
2980 0.518100023269653
2990 0.49669998884201
3000 0.50789999961853
3010 0.511900007724762
3020 0.502300024032593
3030 0.508499979972839
3040 0.51639997959137
3050 0.494599997997284
3060 0.493999987840652
3070 0.520799994468689
3080 0.508700013160706
3090 0.493999987840652
3100 0.519299983978271
3110 0.506200015544891
3120 0.501900017261505
3130 0.499500006437302
3140 0.504899978637695
3150 0.513999998569489
3160 0.493600010871887
3170 0.509299993515015
3180 0.505999982357025
3190 0.502399981021881
3200 0.511500000953674
3210 0.514900028705597
3220 0.506200015544891
3230 0.509700000286102
3240 0.519200026988983
3250 0.498100012540817
3260 0.502600014209747
3270 0.504100024700165
3280 0.513999998569489
3290 0.50629997253418
3300 0.52240002155304
3310 0.507000029087067
3320 0.505699992179871
3330 0.510200023651123
3340 0.495599985122681
3350 0.520099997520447
3360 0.515399992465973
3370 0.511500000953674
3380 0.513599991798401
3390 0.52240002155304
3400 0.51529997587204
3410 0.516300022602081
3420 0.501999974250793
3430 0.51230001449585
3440 0.513700008392334
3450 0.499199986457825
3460 0.516300022602081
3470 0.504599988460541
3480 0.514400005340576
3490 0.509599983692169
3500 0.505999982357025
3510 0.501800000667572
3520 0.501800000667572
3530 0.50629997253418
3540 0.502900004386902
3550 0.497200012207031
3560 0.513400018215179
3570 0.506200015544891
3580 0.501699984073639
3590 0.493400007486343
3600 0.518299996852875
3610 0.515399992465973
3620 0.501600027084351
3630 0.499300003051758
3640 0.509400010108948
3650 0.505400002002716
3660 0.504700005054474
3670 0.496499985456467
3680 0.498299986124039
3690 0.498299986124039
3700 0.508899986743927
3710 0.517400026321411
3720 0.501299977302551
3730 0.506200015544891
3740 0.5
3750 0.503600001335144
3760 0.510900020599365
3770 0.505999982357025
3780 0.499300003051758
3790 0.511699974536896
3800 0.503499984741211
3810 0.518599987030029
3820 0.502600014209747
3830 0.512099981307983
3840 0.492500007152557
3850 0.504000008106232
3860 0.501600027084351
3870 0.522800028324127
3880 0.498199999332428
3890 0.508400022983551
3900 0.503700017929077
3910 0.491400003433228
3920 0.508800029754639
3930 0.495400011539459
3940 0.514699995517731
3950 0.499099999666214
3960 0.511900007724762
3970 0.501900017261505
3980 0.502699971199036
3990 0.486799985170364
4000 0.512600004673004
4010 0.497299998998642
4020 0.505599975585938
4030 0.496399998664856
4040 0.500899970531464
4050 0.5067999958992
4060 0.510299980640411
4070 0.514299988746643
4080 0.517400026321411
4090 0.509400010108948
4100 0.508700013160706
4110 0.505800008773804
4120 0.507600009441376
4130 0.513300001621246
4140 0.506600022315979
4150 0.506600022315979
4160 0.502799987792969
4170 0.514400005340576
4180 0.518999993801117
4190 0.504800021648407
4200 0.505599975585938
4210 0.503400027751923
4220 0.498299986124039
4230 0.501200020313263
4240 0.514500021934509
4250 0.513599991798401
4260 0.497999995946884
4270 0.506900012493134
4280 0.510699987411499
4290 0.500100016593933
4300 0.49770000576973
4310 0.499799996614456
4320 0.522899985313416
4330 0.507600009441376
4340 0.493099987506866
4350 0.496399998664856
4360 0.503899991512299
4370 0.515900015830994
4380 0.501600027084351
4390 0.509400010108948
4400 0.511799991130829
4410 0.504800021648407
4420 0.49770000576973
4430 0.509599983692169
4440 0.499300003051758
4450 0.507600009441376
4460 0.500699996948242
4470 0.507300019264221
4480 0.507499992847443
4490 0.514999985694885
4500 0.493999987840652
4510 0.496399998664856
4520 0.506600022315979
4530 0.514800012111664
4540 0.509500026702881
4550 0.499599993228912
4560 0.510800004005432
4570 0.499500006437302
4580 0.505400002002716
4590 0.500800013542175
4600 0.506600022315979
4610 0.484699994325638
4620 0.505800008773804
4630 0.511500000953674
4640 0.4966000020504
4650 0.516600012779236
4660 0.491100013256073
4670 0.500199973583221
4680 0.500500023365021
4690 0.498100012540817
4700 0.505999982357025
4710 0.51230001449585
4720 0.517099976539612
4730 0.504800021648407
4740 0.509299993515015
4750 0.506500005722046
4760 0.496399998664856
4770 0.490799993276596
4780 0.495799988508224
4790 0.498600006103516
4800 0.493999987840652
4810 0.505599975585938
4820 0.498299986124039
4830 0.494199991226196
4840 0.505900025367737
4850 0.511900007724762
4860 0.503899991512299
4870 0.500500023365021
4880 0.497299998998642
4890 0.515100002288818
4900 0.498600006103516
4910 0.50789999961853
4920 0.505999982357025
4930 0.500800013542175
4940 0.501299977302551
4950 0.496300011873245
4960 0.49669998884201
4970 0.493400007486343
4980 0.483300000429153
4990 0.499599993228912
5000 0.518400013446808
};
%\addlegendentry{Test}

==> experiments/figures/mae_ri_0.tex <==
\addplot[semithick, color0] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.092399999499321
10 0.969980001449585
20 0.975520014762878
30 0.975859999656677
40 0.971700012683868
50 0.973039984703064
60 0.981880009174347
70 0.979380011558533
80 0.981819987297058
90 0.98114001750946
100 0.982720017433167
110 0.979939997196198
120 0.978139996528625
130 0.983539998531342
140 0.983219981193542
150 0.983380019664764
160 0.981859982013702
170 0.987100005149841
180 0.976779997348785
190 0.983259975910187
200 0.985480010509491
210 0.984679996967316
220 0.988479971885681
230 0.985639989376068
240 0.985979974269867
250 0.988719999790192
260 0.98581999540329
270 0.986180007457733
280 0.98360002040863
290 0.988839983940125
300 0.986479997634888
310 0.987839996814728
320 0.987039983272552
330 0.986199975013733
340 0.98444002866745
350 0.988740026950836
360 0.989139974117279
370 0.988579988479614
380 0.988740026950836
390 0.989419996738434
400 0.988960027694702
410 0.988240003585815
420 0.983659982681274
430 0.989419996738434
440 0.990199983119965
450 0.989619970321655
460 0.988240003585815
470 0.989300012588501
480 0.989340007305145
490 0.989600002765656
500 0.989400029182434
510 0.990180015563965
520 0.990679979324341
530 0.988579988479614
540 0.991419970989227
550 0.989300012588501
560 0.989340007305145
570 0.992259979248047
580 0.988219976425171
590 0.990480005741119
600 0.990000009536743
610 0.991079986095428
620 0.989579975605011
630 0.99125999212265
640 0.989719986915588
650 0.991039991378784
660 0.990679979324341
670 0.988900005817413
680 0.991119980812073
690 0.989780008792877
700 0.990180015563965
710 0.991879999637604
720 0.990580022335052
730 0.99261999130249
740 0.989120006561279
750 0.990059971809387
760 0.990540027618408
770 0.991639971733093
780 0.989600002765656
790 0.993080019950867
800 0.992380023002625
810 0.991199970245361
820 0.991900026798248
830 0.989040017127991
840 0.990920007228851
850 0.992919981479645
860 0.993659973144531
870 0.992500007152557
880 0.993139982223511
890 0.99124002456665
900 0.99260002374649
910 0.992640018463135
920 0.993579983711243
930 0.993560016155243
940 0.991959989070892
950 0.993179976940155
960 0.991699993610382
970 0.991999983787537
980 0.992860019207001
990 0.992760002613068
1000 0.991079986095428
1010 0.993099987506866
1020 0.991219997406006
1030 0.992519974708557
1040 0.98989999294281
1050 0.992380023002625
1060 0.99234002828598
1070 0.992280006408691
1080 0.992039978504181
1090 0.992540001869202
1100 0.993260025978088
1110 0.992980003356934
1120 0.993759989738464
1130 0.990859985351562
1140 0.990920007228851
1150 0.991079986095428
1160 0.991620004177094
1170 0.991699993610382
1180 0.992479979991913
1190 0.990719974040985
1200 0.991419970989227
1210 0.992820024490356
1220 0.992079973220825
1230 0.991100013256073
1240 0.992579996585846
1250 0.99260002374649
1260 0.993099987506866
1270 0.991879999637604
1280 0.992919981479645
1290 0.990000009536743
1300 0.991400003433228
1310 0.991599977016449
1320 0.994000017642975
1330 0.990880012512207
1340 0.993219971656799
1350 0.990779995918274
1360 0.991879999637604
1370 0.993680000305176
1380 0.990559995174408
1390 0.992519974708557
1400 0.993920028209686
1410 0.99234002828598
1420 0.991360008716583
1430 0.993820011615753
1440 0.992420017719269
1450 0.991599977016449
1460 0.992560029029846
1470 0.991720020771027
1480 0.991900026798248
1490 0.993059992790222
1500 0.993759989738464
1510 0.98224002122879
1520 0.993399977684021
1530 0.993759989738464
1540 0.991500020027161
1550 0.99371999502182
1560 0.994180023670197
1570 0.992139995098114
1580 0.993120014667511
1590 0.989400029182434
1600 0.993820011615753
1610 0.993619978427887
1620 0.99456000328064
1630 0.994019985198975
1640 0.993099987506866
1650 0.99456000328064
1660 0.991159975528717
1670 0.993160009384155
1680 0.992900013923645
1690 0.993439972400665
1700 0.992240011692047
1710 0.992280006408691
1720 0.993340015411377
1730 0.991900026798248
1740 0.993300020694733
1750 0.993380010128021
1760 0.989579975605011
1770 0.993439972400665
1780 0.993380010128021
1790 0.993839979171753
1800 0.994520008563995
1810 0.994520008563995
1820 0.987720012664795
1830 0.992479979991913
1840 0.992780029773712
1850 0.992940008640289
1860 0.991400003433228
1870 0.993539988994598
1880 0.993820011615753
1890 0.993579983711243
1900 0.993420004844666
1910 0.99345999956131
1920 0.99345999956131
1930 0.992280006408691
1940 0.993619978427887
1950 0.993600010871887
1960 0.992299973964691
1970 0.991419970989227
1980 0.993399977684021
1990 0.99397999048233
2000 0.993080019950867
2010 0.993879973888397
2020 0.992919981479645
2030 0.995039999485016
2040 0.994859993457794
2050 0.994480013847351
2060 0.994480013847351
2070 0.994040012359619
2080 0.993579983711243
2090 0.991280019283295
2100 0.994740009307861
2110 0.994759976863861
2120 0.994759976863861
2130 0.994759976863861
2140 0.994759976863861
2150 0.994759976863861
2160 0.994759976863861
2170 0.994759976863861
2180 0.994759976863861
2190 0.994759976863861
2200 0.994759976863861
2210 0.994759976863861
2220 0.994759976863861
2230 0.994759976863861
2240 0.994759976863861
2250 0.994759976863861
2260 0.994759976863861
2270 0.994759976863861
2280 0.994759976863861
2290 0.994759976863861
2300 0.994759976863861
2310 0.994759976863861
2320 0.994759976863861
2330 0.994759976863861
2340 0.994759976863861
2350 0.994759976863861
2360 0.994780004024506
2370 0.994459986686707
2380 0.991460025310516
2390 0.991199970245361
2400 0.992060005664825
2410 0.994220018386841
2420 0.994880020618439
2430 0.99397999048233
2440 0.993879973888397
2450 0.994939982891083
2460 0.994939982891083
2470 0.994939982891083
2480 0.994939982891083
2490 0.994960010051727
2500 0.993099987506866
2510 0.992240011692047
2520 0.993539988994598
2530 0.993499994277954
2540 0.994920015335083
2550 0.994379997253418
2560 0.994340002536774
2570 0.994419991970062
2580 0.994099974632263
2590 0.994899988174438
2600 0.995360016822815
2610 0.994180023670197
2620 0.993799984455109
2630 0.994140028953552
2640 0.995019972324371
2650 0.987559974193573
2660 0.99397999048233
2670 0.992540001869202
2680 0.993539988994598
2690 0.993539988994598
2700 0.993439972400665
2710 0.994000017642975
2720 0.994059979915619
2730 0.992659986019135
2740 0.993120014667511
2750 0.994239985942841
2760 0.992900013923645
2770 0.99370002746582
2780 0.993499994277954
2790 0.99210000038147
2800 0.995220005512238
2810 0.994220018386841
2820 0.994539976119995
2830 0.994700014591217
2840 0.993179976940155
2850 0.995260000228882
2860 0.99506002664566
2870 0.99506002664566
2880 0.99507999420166
2890 0.99507999420166
2900 0.99507999420166
2910 0.99507999420166
2920 0.99507999420166
2930 0.99507999420166
2940 0.99507999420166
2950 0.99507999420166
2960 0.99507999420166
2970 0.99507999420166
2980 0.99507999420166
2990 0.99507999420166
3000 0.99507999420166
3010 0.99507999420166
3020 0.99507999420166
3030 0.99507999420166
3040 0.99507999420166
3050 0.99507999420166
3060 0.99507999420166
3070 0.99507999420166
3080 0.99507999420166
3090 0.99507999420166
3100 0.99507999420166
3110 0.99507999420166
3120 0.99507999420166
3130 0.99507999420166
3140 0.99507999420166
3150 0.99507999420166
3160 0.99507999420166
3170 0.99507999420166
3180 0.99507999420166
3190 0.99507999420166
3200 0.99507999420166
3210 0.99507999420166
3220 0.99507999420166
3230 0.99507999420166
3240 0.99507999420166
3250 0.99507999420166
3260 0.99507999420166
3270 0.99507999420166
3280 0.99507999420166
3290 0.99507999420166
3300 0.99507999420166
3310 0.99507999420166
3320 0.99507999420166
3330 0.99507999420166
3340 0.99507999420166
3350 0.99507999420166
3360 0.99507999420166
3370 0.99507999420166
3380 0.99507999420166
3390 0.99507999420166
3400 0.99507999420166
3410 0.99507999420166
3420 0.99507999420166
3430 0.99507999420166
3440 0.99507999420166
3450 0.99507999420166
3460 0.99507999420166
3470 0.99507999420166
3480 0.99507999420166
3490 0.99507999420166
3500 0.99507999420166
3510 0.99507999420166
3520 0.99507999420166
3530 0.99507999420166
3540 0.99507999420166
3550 0.99507999420166
3560 0.99507999420166
3570 0.99507999420166
3580 0.99507999420166
3590 0.99507999420166
3600 0.99507999420166
3610 0.99507999420166
3620 0.99507999420166
3630 0.99507999420166
3640 0.99507999420166
3650 0.99507999420166
3660 0.99507999420166
3670 0.99507999420166
3680 0.99507999420166
3690 0.99507999420166
3700 0.99507999420166
3710 0.99507999420166
3720 0.99507999420166
3730 0.99507999420166
3740 0.99507999420166
3750 0.99507999420166
3760 0.99507999420166
3770 0.99507999420166
3780 0.99507999420166
3790 0.99507999420166
3800 0.99507999420166
3810 0.99507999420166
3820 0.99507999420166
3830 0.99507999420166
3840 0.99507999420166
3850 0.99507999420166
3860 0.99507999420166
3870 0.99507999420166
3880 0.99507999420166
3890 0.99507999420166
3900 0.99507999420166
3910 0.99507999420166
3920 0.99507999420166
3930 0.99507999420166
3940 0.99507999420166
3950 0.99507999420166
3960 0.99507999420166
3970 0.99507999420166
3980 0.99507999420166
3990 0.99507999420166
4000 0.99507999420166
4010 0.99507999420166
4020 0.99507999420166
4030 0.99507999420166
4040 0.99507999420166
4050 0.99507999420166
4060 0.99507999420166
4070 0.99507999420166
4080 0.99507999420166
4090 0.99507999420166
4100 0.99507999420166
4110 0.99507999420166
4120 0.99507999420166
4130 0.99507999420166
4140 0.99507999420166
4150 0.99507999420166
4160 0.99507999420166
4170 0.99507999420166
4180 0.99507999420166
4190 0.99507999420166
4200 0.99507999420166
4210 0.99507999420166
4220 0.99507999420166
4230 0.99507999420166
4240 0.99507999420166
4250 0.99507999420166
4260 0.99507999420166
4270 0.99507999420166
4280 0.99507999420166
4290 0.99507999420166
4300 0.99507999420166
4310 0.99507999420166
4320 0.99507999420166
4330 0.99507999420166
4340 0.99507999420166
4350 0.99507999420166
4360 0.99507999420166
4370 0.99507999420166
4380 0.99507999420166
4390 0.99507999420166
4400 0.99507999420166
4410 0.99507999420166
4420 0.99507999420166
4430 0.99507999420166
4440 0.99507999420166
4450 0.99507999420166
4460 0.99507999420166
4470 0.99507999420166
4480 0.99507999420166
4490 0.99507999420166
4500 0.99507999420166
4510 0.99507999420166
4520 0.99507999420166
4530 0.99507999420166
4540 0.99507999420166
4550 0.99507999420166
4560 0.99507999420166
4570 0.99507999420166
4580 0.99507999420166
4590 0.99507999420166
4600 0.99507999420166
4610 0.99507999420166
4620 0.99507999420166
4630 0.99507999420166
4640 0.99507999420166
4650 0.99507999420166
4660 0.99507999420166
4670 0.99507999420166
4680 0.99507999420166
4690 0.99507999420166
4700 0.99507999420166
4710 0.99507999420166
4720 0.99507999420166
4730 0.99507999420166
4740 0.99507999420166
4750 0.99507999420166
4760 0.99507999420166
4770 0.99507999420166
4780 0.99507999420166
4790 0.99507999420166
4800 0.99507999420166
4810 0.99507999420166
4820 0.99507999420166
4830 0.99507999420166
4840 0.99507999420166
4850 0.99507999420166
4860 0.99507999420166
4870 0.99507999420166
4880 0.99507999420166
4890 0.99507999420166
4900 0.99507999420166
4910 0.99507999420166
4920 0.99507999420166
4930 0.99507999420166
4940 0.99507999420166
4950 0.99507999420166
4960 0.99507999420166
4970 0.99507999420166
4980 0.99507999420166
4990 0.99507999420166
5000 0.99507999420166
};
%\addlegendentry{Train}
\addplot [semithick, color1] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.0931999981403351
10 0.965699970722198
20 0.967499971389771
30 0.965300023555756
40 0.962499976158142
50 0.960600018501282
60 0.97350001335144
70 0.97189998626709
80 0.973200023174286
90 0.970399975776672
100 0.971000015735626
110 0.969200015068054
120 0.968500018119812
130 0.97189998626709
140 0.973900020122528
150 0.973999977111816
160 0.969600021839142
170 0.978500008583069
180 0.962700009346008
190 0.974699974060059
200 0.977299988269806
210 0.972599983215332
220 0.977400004863739
230 0.974900007247925
240 0.973599970340729
250 0.977699995040894
260 0.97409999370575
270 0.975499987602234
280 0.969500005245209
290 0.978500008583069
300 0.973299980163574
310 0.977999985218048
320 0.975300014019012
330 0.97299998998642
340 0.972599983215332
350 0.976999998092651
360 0.976599991321564
370 0.977100014686584
380 0.975399971008301
390 0.978500008583069
400 0.975399971008301
410 0.974699974060059
420 0.968299984931946
430 0.976499974727631
440 0.977100014686584
450 0.976400017738342
460 0.975099980831146
470 0.975099980831146
480 0.97680002450943
490 0.975799977779388
500 0.977999985218048
510 0.977800011634827
520 0.977199971675873
530 0.975799977779388
540 0.977400004863739
550 0.976899981498718
560 0.974799990653992
570 0.979200005531311
580 0.972400009632111
590 0.974699974060059
600 0.975099980831146
610 0.976899981498718
620 0.975899994373322
630 0.978100001811981
640 0.977299988269806
650 0.975600004196167
660 0.977100014686584
670 0.972400009632111
680 0.974699974060059
690 0.976599991321564
700 0.976400017738342
710 0.979900002479553
720 0.979600012302399
730 0.979099988937378
740 0.9757000207901
750 0.977199971675873
760 0.977299988269806
770 0.977500021457672
780 0.976700007915497
790 0.979099988937378
800 0.97759997844696
810 0.978600025177002
820 0.977699995040894
830 0.974300026893616
840 0.975399971008301
850 0.97790002822876
860 0.98089998960495
870 0.97979998588562
880 0.979099988937378
890 0.975199997425079
900 0.979499995708466
910 0.980099976062775
920 0.980300009250641
930 0.979099988937378
940 0.976199984550476
950 0.978600025177002
960 0.975600004196167
970 0.978500008583069
980 0.976899981498718
990 0.97979998588562
1000 0.977299988269806
1010 0.979200005531311
1020 0.976700007915497
1030 0.978399991989136
1040 0.975600004196167
1050 0.978900015354156
1060 0.977199971675873
1070 0.979300022125244
1080 0.978399991989136
1090 0.97790002822876
1100 0.979099988937378
1110 0.978299975395203
1120 0.981199979782104
1130 0.976899981498718
1140 0.976999998092651
1150 0.976400017738342
1160 0.977699995040894
1170 0.97680002450943
1180 0.978200018405914
1190 0.97759997844696
1200 0.97680002450943
1210 0.978200018405914
1220 0.976999998092651
1230 0.977199971675873
1240 0.976999998092651
1250 0.976999998092651
1260 0.977800011634827
1270 0.976899981498718
1280 0.97979998588562
1290 0.973399996757507
1300 0.975899994373322
1310 0.975499987602234
1320 0.97869998216629
1330 0.975600004196167
1340 0.978500008583069
1350 0.975799977779388
1360 0.9757000207901
1370 0.979900002479553
1380 0.976599991321564
1390 0.978299975395203
1400 0.97979998588562
1410 0.97759997844696
1420 0.977400004863739
1430 0.979600012302399
1440 0.977299988269806
1450 0.975899994373322
1460 0.976199984550476
1470 0.97680002450943
1480 0.979300022125244
1490 0.977999985218048
1500 0.978100001811981
1510 0.968400001525879
1520 0.978999972343445
1530 0.977999985218048
1540 0.976999998092651
1550 0.97759997844696
1560 0.978900015354156
1570 0.977500021457672
1580 0.979600012302399
1590 0.973900020122528
1600 0.97979998588562
1610 0.97869998216629
1620 0.979700028896332
1630 0.980400025844574
1640 0.976100027561188
1650 0.979300022125244
1660 0.97759997844696
1670 0.978999972343445
1680 0.977699995040894
1690 0.977699995040894
1700 0.977500021457672
1710 0.977699995040894
1720 0.977500021457672
1730 0.978100001811981
1740 0.979499995708466
1750 0.978500008583069
1760 0.975600004196167
1770 0.97790002822876
1780 0.979600012302399
1790 0.978799998760223
1800 0.97979998588562
1810 0.97979998588562
1820 0.974300026893616
1830 0.97759997844696
1840 0.97790002822876
1850 0.976000010967255
1860 0.976400017738342
1870 0.977699995040894
1880 0.978900015354156
1890 0.978999972343445
1900 0.979200005531311
1910 0.979300022125244
1920 0.981000006198883
1930 0.978100001811981
1940 0.977299988269806
1950 0.977699995040894
1960 0.975600004196167
1970 0.976599991321564
1980 0.975899994373322
1990 0.975799977779388
2000 0.97759997844696
2010 0.977199971675873
2020 0.976899981498718
2030 0.979600012302399
2040 0.979300022125244
2050 0.978799998760223
2060 0.97759997844696
2070 0.975600004196167
2080 0.978399991989136
2090 0.974300026893616
2100 0.978999972343445
2110 0.978999972343445
2120 0.978999972343445
2130 0.978999972343445
2140 0.978999972343445
2150 0.978900015354156
2160 0.978900015354156
2170 0.978900015354156
2180 0.978900015354156
2190 0.978900015354156
2200 0.978900015354156
2210 0.978900015354156
2220 0.978900015354156
2230 0.978900015354156
2240 0.978900015354156
2250 0.978900015354156
2260 0.978900015354156
2270 0.978900015354156
2280 0.978900015354156
2290 0.978900015354156
2300 0.978900015354156
2310 0.978900015354156
2320 0.978900015354156
2330 0.978900015354156
2340 0.978900015354156
2350 0.978900015354156
2360 0.978799998760223
2370 0.979300022125244
2380 0.975300014019012
2390 0.975499987602234
2400 0.975199997425079
2410 0.978799998760223
2420 0.97680002450943
2430 0.97759997844696
2440 0.978500008583069
2450 0.980099976062775
2460 0.980099976062775
2470 0.980099976062775
2480 0.980099976062775
2490 0.979900002479553
2500 0.976899981498718
2510 0.976499974727631
2520 0.978399991989136
2530 0.978200018405914
2540 0.981299996376038
2550 0.979399979114532
2560 0.979700028896332
2570 0.979499995708466
2580 0.977500021457672
2590 0.978900015354156
2600 0.978500008583069
2610 0.97869998216629
2620 0.978799998760223
2630 0.980099976062775
2640 0.979499995708466
2650 0.971300005912781
2660 0.97869998216629
2670 0.975899994373322
2680 0.975499987602234
2690 0.975600004196167
2700 0.978200018405914
2710 0.978200018405914
2720 0.978299975395203
2730 0.97790002822876
2740 0.978600025177002
2750 0.976700007915497
2760 0.977500021457672
2770 0.97759997844696
2780 0.976400017738342
2790 0.977999985218048
2800 0.978500008583069
2810 0.977100014686584
2820 0.975099980831146
2830 0.975300014019012
2840 0.976100027561188
2850 0.979399979114532
2860 0.979600012302399
2870 0.979600012302399
2880 0.979600012302399
2890 0.979600012302399
2900 0.979600012302399
2910 0.979600012302399
2920 0.979600012302399
2930 0.979600012302399
2940 0.979600012302399
2950 0.979600012302399
2960 0.979600012302399
2970 0.979600012302399
2980 0.979600012302399
2990 0.979600012302399
3000 0.979600012302399
3010 0.979600012302399
3020 0.979600012302399
3030 0.979600012302399
3040 0.979600012302399
3050 0.979600012302399
3060 0.979600012302399
3070 0.979600012302399
3080 0.979600012302399
3090 0.979600012302399
3100 0.979600012302399
3110 0.979600012302399
3120 0.979600012302399
3130 0.979600012302399
3140 0.979600012302399
3150 0.979600012302399
3160 0.979600012302399
3170 0.979600012302399
3180 0.979600012302399
3190 0.979600012302399
3200 0.979600012302399
3210 0.979600012302399
3220 0.979600012302399
3230 0.979600012302399
3240 0.979600012302399
3250 0.979600012302399
3260 0.979600012302399
3270 0.979600012302399
3280 0.979600012302399
3290 0.979600012302399
3300 0.979600012302399
3310 0.979600012302399
3320 0.979600012302399
3330 0.979600012302399
3340 0.979600012302399
3350 0.979600012302399
3360 0.979600012302399
3370 0.979600012302399
3380 0.979600012302399
3390 0.979600012302399
3400 0.979600012302399
3410 0.979600012302399
3420 0.979600012302399
3430 0.979600012302399
3440 0.979600012302399
3450 0.979600012302399
3460 0.979600012302399
3470 0.979600012302399
3480 0.979600012302399
3490 0.979600012302399
3500 0.979600012302399
3510 0.979600012302399
3520 0.979600012302399
3530 0.979600012302399
3540 0.979600012302399
3550 0.979600012302399
3560 0.979600012302399
3570 0.979600012302399
3580 0.979600012302399
3590 0.979600012302399
3600 0.979600012302399
3610 0.979600012302399
3620 0.979600012302399
3630 0.979600012302399
3640 0.979600012302399
3650 0.979600012302399
3660 0.979600012302399
3670 0.979600012302399
3680 0.979600012302399
3690 0.979600012302399
3700 0.979600012302399
3710 0.979600012302399
3720 0.979600012302399
3730 0.979600012302399
3740 0.979600012302399
3750 0.979600012302399
3760 0.979600012302399
3770 0.979600012302399
3780 0.979600012302399
3790 0.979600012302399
3800 0.979600012302399
3810 0.979600012302399
3820 0.979600012302399
3830 0.979600012302399
3840 0.979600012302399
3850 0.979600012302399
3860 0.979600012302399
3870 0.979600012302399
3880 0.979600012302399
3890 0.979600012302399
3900 0.979600012302399
3910 0.979600012302399
3920 0.979600012302399
3930 0.979600012302399
3940 0.979600012302399
3950 0.979600012302399
3960 0.979600012302399
3970 0.979600012302399
3980 0.979600012302399
3990 0.979600012302399
4000 0.979600012302399
4010 0.979600012302399
4020 0.979600012302399
4030 0.979600012302399
4040 0.979600012302399
4050 0.979600012302399
4060 0.979600012302399
4070 0.979600012302399
4080 0.979600012302399
4090 0.979600012302399
4100 0.979600012302399
4110 0.979600012302399
4120 0.979600012302399
4130 0.979600012302399
4140 0.979600012302399
4150 0.979600012302399
4160 0.979600012302399
4170 0.979600012302399
4180 0.979600012302399
4190 0.979600012302399
4200 0.979600012302399
4210 0.979600012302399
4220 0.979600012302399
4230 0.979600012302399
4240 0.979600012302399
4250 0.979600012302399
4260 0.979600012302399
4270 0.979600012302399
4280 0.979600012302399
4290 0.979600012302399
4300 0.979600012302399
4310 0.979600012302399
4320 0.979600012302399
4330 0.979600012302399
4340 0.979600012302399
4350 0.979600012302399
4360 0.979600012302399
4370 0.979600012302399
4380 0.979600012302399
4390 0.979600012302399
4400 0.979600012302399
4410 0.979600012302399
4420 0.979600012302399
4430 0.979600012302399
4440 0.979600012302399
4450 0.979600012302399
4460 0.979600012302399
4470 0.979600012302399
4480 0.979600012302399
4490 0.979600012302399
4500 0.979600012302399
4510 0.979600012302399
4520 0.979600012302399
4530 0.979600012302399
4540 0.979600012302399
4550 0.979600012302399
4560 0.979600012302399
4570 0.979600012302399
4580 0.979600012302399
4590 0.979600012302399
4600 0.979600012302399
4610 0.979600012302399
4620 0.979600012302399
4630 0.979600012302399
4640 0.979600012302399
4650 0.979600012302399
4660 0.979600012302399
4670 0.979600012302399
4680 0.979600012302399
4690 0.979600012302399
4700 0.979600012302399
4710 0.979600012302399
4720 0.979600012302399
4730 0.979600012302399
4740 0.979600012302399
4750 0.979600012302399
4760 0.979600012302399
4770 0.979600012302399
4780 0.979600012302399
4790 0.979600012302399
4800 0.979600012302399
4810 0.979600012302399
4820 0.979600012302399
4830 0.979600012302399
4840 0.979600012302399
4850 0.979600012302399
4860 0.979600012302399
4870 0.979600012302399
4880 0.979600012302399
4890 0.979600012302399
4900 0.979600012302399
4910 0.979600012302399
4920 0.979600012302399
4930 0.979600012302399
4940 0.979600012302399
4950 0.979600012302399
4960 0.979600012302399
4970 0.979600012302399
4980 0.979600012302399
4990 0.979600012302399
5000 0.979600012302399
};
%\addlegendentry{Test}


==> experiments/figures/mae_ri_03.tex <==
\addplot[semithick, color2] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.0842799991369247
10 0.674300014972687
20 0.669120013713837
30 0.683239996433258
40 0.680379986763
50 0.685500025749207
60 0.680599987506866
70 0.669579982757568
80 0.68665999174118
90 0.686839997768402
100 0.685259997844696
110 0.685779988765717
120 0.686699986457825
130 0.685959994792938
140 0.684899985790253
150 0.688239991664886
160 0.689639985561371
170 0.683780014514923
180 0.689019978046417
190 0.689920008182526
200 0.689400017261505
210 0.68588000535965
220 0.684759974479675
230 0.684700012207031
240 0.687539994716644
250 0.682120025157928
260 0.680920004844666
270 0.689400017261505
280 0.678860008716583
290 0.686559975147247
300 0.690100014209747
310 0.686779975891113
320 0.688440024852753
330 0.685220003128052
340 0.688979983329773
350 0.688440024852753
360 0.690079987049103
370 0.691479980945587
380 0.685259997844696
390 0.690880000591278
400 0.685959994792938
410 0.68996000289917
420 0.692740023136139
430 0.690240025520325
440 0.690779983997345
450 0.689599990844727
460 0.690419971942902
470 0.691380023956299
480 0.687780022621155
490 0.692600011825562
500 0.691139996051788
510 0.690060019493103
520 0.686360001564026
530 0.684700012207031
540 0.691340029239655
550 0.693340003490448
560 0.686179995536804
570 0.692099988460541
580 0.693139970302582
590 0.690460026264191
600 0.692300021648407
610 0.693220019340515
620 0.692239999771118
630 0.685379981994629
640 0.692120015621185
650 0.692279994487762
660 0.691540002822876
670 0.692659974098206
680 0.692359983921051
690 0.693379998207092
700 0.692560017108917
710 0.693939983844757
720 0.686739981174469
730 0.691619992256165
740 0.690439999103546
750 0.691760003566742
760 0.688820004463196
770 0.685140013694763
780 0.692319989204407
790 0.694719970226288
800 0.69157999753952
810 0.694019973278046
820 0.694379985332489
830 0.694639980792999
840 0.693880021572113
850 0.694419980049133
860 0.695119976997375
870 0.694459974765778
880 0.69352000951767
890 0.694140017032623
900 0.69216001033783
910 0.695020020008087
920 0.694280028343201
930 0.689620018005371
940 0.692399978637695
950 0.691299974918365
960 0.691460013389587
970 0.694620013237
980 0.69293999671936
990 0.695659995079041
1000 0.695680022239685
1010 0.695699989795685
1020 0.691680014133453
1030 0.692139983177185
1040 0.692979991436005
1050 0.692979991436005
1060 0.695640027523041
1070 0.694440007209778
1080 0.69539999961853
1090 0.692219972610474
1100 0.694920003414154
1110 0.694419980049133
1120 0.6910799741745
1130 0.694060027599335
1140 0.693979978561401
1150 0.694540023803711
1160 0.696439981460571
1170 0.696099996566772
1180 0.693840026855469
1190 0.694999992847443
1200 0.690999984741211
1210 0.694700002670288
1220 0.696699976921082
1230 0.690100014209747
1240 0.697080016136169
1250 0.697179973125458
1260 0.696600019931793
1270 0.696460008621216
1280 0.694779992103577
1290 0.696340024471283
1300 0.694760024547577
1310 0.695760011672974
1320 0.694840013980865
1330 0.694079995155334
1340 0.693539977073669
1350 0.693340003490448
1360 0.695659995079041
1370 0.694859981536865
1380 0.693859994411469
1390 0.695819973945618
1400 0.694180011749268
1410 0.696319997310638
1420 0.69650000333786
1430 0.69650000333786
1440 0.69650000333786
1450 0.692860007286072
1460 0.69515997171402
1470 0.696219980716705
1480 0.696739971637726
1490 0.696439981460571
1500 0.697080016136169
1510 0.696579992771149
1520 0.695620000362396
1530 0.693819999694824
1540 0.696020007133484
1550 0.695860028266907
1560 0.69539999961853
1570 0.696820020675659
1580 0.696460008621216
1590 0.696820020675659
1600 0.694859981536865
1610 0.695940017700195
1620 0.695940017700195
1630 0.692139983177185
1640 0.69650000333786
1650 0.696200013160706
1660 0.696399986743927
1670 0.695479989051819
1680 0.697120010852814
1690 0.696699976921082
1700 0.69760000705719
1710 0.697459995746613
1720 0.696699976921082
1730 0.696600019931793
1740 0.695020020008087
1750 0.696039974689484
1760 0.695559978485107
1770 0.697120010852814
1780 0.69379997253418
1790 0.694739997386932
1800 0.694939970970154
1810 0.696699976921082
1820 0.694320023059845
1830 0.695259988307953
1840 0.695259988307953
1850 0.691919982433319
1860 0.697480022907257
1870 0.697939991950989
1880 0.697040021419525
1890 0.697059988975525
1900 0.693920016288757
1910 0.696619987487793
1920 0.694620013237
1930 0.695959985256195
1940 0.697239995002747
1950 0.698040008544922
1960 0.690419971942902
1970 0.696979999542236
1980 0.697279989719391
1990 0.696640014648438
2000 0.697640001773834
2010 0.698300004005432
2020 0.696940004825592
2030 0.698080003261566
2040 0.697820007801056
2050 0.695620000362396
2060 0.69598001241684
2070 0.698580026626587
2080 0.69844001531601
2090 0.695680022239685
2100 0.698899984359741
2110 0.697399973869324
2120 0.698480010032654
2130 0.697440028190613
2140 0.697579979896545
2150 0.697440028190613
2160 0.697440028190613
2170 0.695860028266907
2180 0.699020028114319
2190 0.696659982204437
2200 0.698019981384277
2210 0.698740005493164
2220 0.698059976100922
2230 0.699240028858185
2240 0.697300016880035
2250 0.696219980716705
2260 0.69871997833252
2270 0.696539998054504
2280 0.697979986667633
2290 0.697920024394989
2300 0.697239995002747
2310 0.694500029087067
2320 0.69651997089386
2330 0.696460008621216
2340 0.696080029010773
2350 0.696380019187927
2360 0.697059988975525
2370 0.697539985179901
2380 0.699440002441406
2390 0.697700023651123
2400 0.698639988899231
2410 0.698639988899231
2420 0.698660016059875
2430 0.698660016059875
2440 0.698660016059875
2450 0.697319984436035
2460 0.697839975357056
2470 0.698099970817566
2480 0.698379993438721
2490 0.698400020599365
2500 0.698400020599365
2510 0.698400020599365
2520 0.698400020599365
2530 0.697420001029968
2540 0.697539985179901
2550 0.698840022087097
2560 0.698319971561432
2570 0.696699976921082
2580 0.699699997901917
2590 0.695840001106262
2600 0.698880016803741
2610 0.699440002441406
2620 0.699440002441406
2630 0.699440002441406
2640 0.699440002441406
2650 0.694679975509644
2660 0.695519983768463
2670 0.694019973278046
2680 0.69871997833252
2690 0.693099975585938
2700 0.695919990539551
2710 0.697520017623901
2720 0.699000000953674
2730 0.699060022830963
2740 0.699000000953674
2750 0.698639988899231
2760 0.698019981384277
2770 0.698599994182587
2780 0.699020028114319
2790 0.69844001531601
2800 0.698199987411499
2810 0.698199987411499
2820 0.697960019111633
2830 0.699119985103607
2840 0.699060022830963
2850 0.699379980564117
2860 0.698260009288788
2870 0.699400007724762
2880 0.69811999797821
2890 0.699320018291473
2900 0.697459995746613
2910 0.698740005493164
2920 0.696820020675659
2930 0.699199974536896
2940 0.699060022830963
2950 0.698740005493164
2960 0.696979999542236
2970 0.699500024318695
2980 0.697700023651123
2990 0.695039987564087
3000 0.699039995670319
3010 0.698880016803741
3020 0.699339985847473
3030 0.697920024394989
3040 0.698059976100922
3050 0.70033997297287
3060 0.700299978256226
3070 0.70032000541687
3080 0.700439989566803
3090 0.700439989566803
3100 0.700439989566803
3110 0.700439989566803
3120 0.700439989566803
3130 0.700439989566803
3140 0.700439989566803
3150 0.700439989566803
3160 0.700439989566803
3170 0.700439989566803
3180 0.698319971561432
3190 0.697939991950989
3200 0.699400007724762
3210 0.69922000169754
3220 0.698580026626587
3230 0.698580026626587
3240 0.698599994182587
3250 0.698159992694855
3260 0.69811999797821
3270 0.691919982433319
3280 0.696420013904572
3290 0.697200000286102
3300 0.698260009288788
3310 0.698679983615875
3320 0.698679983615875
3330 0.698679983615875
3340 0.698679983615875
3350 0.698679983615875
3360 0.698679983615875
3370 0.699079990386963
3380 0.698780000209808
3390 0.697579979896545
3400 0.696539998054504
3410 0.699339985847473
3420 0.699339985847473
3430 0.699379980564117
3440 0.699379980564117
3450 0.694519996643066
3460 0.696120023727417
3470 0.697740018367767
3480 0.696539998054504
3490 0.697640001773834
3500 0.699140012264252
3510 0.69896000623703
3520 0.698740005493164
3530 0.699940025806427
3540 0.699379980564117
3550 0.698040008544922
3560 0.69760000705719
3570 0.698759973049164
3580 0.699620008468628
3590 0.698539972305298
3600 0.69734001159668
3610 0.70032000541687
3620 0.699360013008118
3630 0.699039995670319
3640 0.699039995670319
3650 0.698899984359741
3660 0.698599994182587
3670 0.6978600025177
3680 0.69844001531601
3690 0.698520004749298
3700 0.699259996414185
3710 0.699320018291473
3720 0.696680009365082
3730 0.698140025138855
3740 0.699259996414185
3750 0.699299991130829
3760 0.699299991130829
3770 0.699299991130829
3780 0.699299991130829
3790 0.699299991130829
3800 0.698279976844788
3810 0.69844001531601
3820 0.69844001531601
3830 0.698459982872009
3840 0.693740010261536
3850 0.697960019111633
3860 0.697820007801056
3870 0.69897997379303
3880 0.698660016059875
3890 0.698040008544922
3900 0.698099970817566
3910 0.698639988899231
3920 0.699500024318695
3930 0.699559986591339
3940 0.698880016803741
3950 0.697939991950989
3960 0.700119972229004
3970 0.699919998645782
3980 0.699919998645782
3990 0.699919998645782
4000 0.696039974689484
4010 0.696080029010773
4020 0.696600019931793
4030 0.696860015392303
4040 0.696860015392303
4050 0.696680009365082
4060 0.699119985103607
4070 0.698580026626587
4080 0.696280002593994
4090 0.699360013008118
4100 0.699180006980896
4110 0.699779987335205
4120 0.698639988899231
4130 0.699679970741272
4140 0.700399994850159
4150 0.700299978256226
4160 0.700280010700226
4170 0.698660016059875
4180 0.700500011444092
4190 0.699460029602051
4200 0.699100017547607
4210 0.699999988079071
4220 0.699880003929138
4230 0.70007997751236
4240 0.700540006160736
4250 0.698419988155365
4260 0.70033997297287
4270 0.700420022010803
4280 0.700439989566803
4290 0.698220014572144
4300 0.698740005493164
4310 0.700240015983582
4320 0.700240015983582
4330 0.700240015983582
4340 0.700240015983582
4350 0.695640027523041
4360 0.700540006160736
4370 0.699540019035339
4380 0.699339985847473
4390 0.700619995594025
4400 0.700420022010803
4410 0.697160005569458
4420 0.698279976844788
4430 0.699840009212494
4440 0.700160026550293
4450 0.699699997901917
4460 0.697160005569458
4470 0.700940012931824
4480 0.697979986667633
4490 0.699460029602051
4500 0.700500011444092
4510 0.699639976024628
4520 0.700760006904602
4530 0.700860023498535
4540 0.700860023498535
4550 0.700860023498535
4560 0.700860023498535
4570 0.700879991054535
4580 0.700879991054535
4590 0.700879991054535
4600 0.700879991054535
4610 0.700879991054535
4620 0.700879991054535
4630 0.700879991054535
4640 0.700879991054535
4650 0.700879991054535
4660 0.700879991054535
4670 0.700879991054535
4680 0.700879991054535
4690 0.700879991054535
4700 0.700879991054535
4710 0.700879991054535
4720 0.700879991054535
4730 0.700879991054535
4740 0.700879991054535
4750 0.700879991054535
4760 0.700879991054535
4770 0.700879991054535
4780 0.700879991054535
4790 0.700879991054535
4800 0.700879991054535
4810 0.700879991054535
4820 0.700879991054535
4830 0.700879991054535
4840 0.700879991054535
4850 0.700879991054535
4860 0.700879991054535
4870 0.700879991054535
4880 0.700879991054535
4890 0.700879991054535
4900 0.700879991054535
4910 0.700879991054535
4920 0.700879991054535
4930 0.700879991054535
4940 0.700879991054535
4950 0.700879991054535
4960 0.700879991054535
4970 0.700879991054535
4980 0.700879991054535
4990 0.700879991054535
5000 0.700879991054535
};
%\addlegendentry{Train}
\addplot[semithick, color3] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.0710999965667725
10 0.952499985694885
20 0.940400004386902
30 0.962000012397766
40 0.958899974822998
50 0.964699983596802
60 0.95880001783371
70 0.943199992179871
80 0.962700009346008
90 0.966300010681152
100 0.964699983596802
110 0.963299989700317
120 0.963599979877472
130 0.962000012397766
140 0.961300015449524
150 0.967199981212616
160 0.969799995422363
170 0.958199977874756
180 0.967999994754791
190 0.968800008296967
200 0.965399980545044
210 0.960200011730194
220 0.962599992752075
230 0.960399985313416
240 0.964399993419647
250 0.955200016498566
260 0.958899974822998
270 0.967999994754791
280 0.950900018215179
290 0.96450001001358
300 0.966400027275085
310 0.963199973106384
320 0.967199981212616
330 0.959999978542328
340 0.96560001373291
350 0.965900003910065
360 0.968400001525879
370 0.971599996089935
380 0.961700022220612
390 0.967199981212616
400 0.959800004959106
410 0.96670001745224
420 0.971300005912781
430 0.965200006961823
440 0.967499971389771
450 0.967499971389771
460 0.96780002117157
470 0.970899999141693
480 0.962100028991699
490 0.971599996089935
500 0.967599987983704
510 0.96450001001358
520 0.961499989032745
530 0.959100008010864
540 0.969399988651276
550 0.972000002861023
560 0.960799992084503
570 0.970099985599518
580 0.969299972057343
590 0.968500018119812
600 0.967299997806549
610 0.970099985599518
620 0.969299972057343
630 0.95959997177124
640 0.969099998474121
650 0.969200015068054
660 0.968699991703033
670 0.968999981880188
680 0.967400014400482
690 0.969799995422363
700 0.968100011348724
710 0.969799995422363
720 0.961000025272369
730 0.965799987316132
740 0.96560001373291
750 0.96780002117157
760 0.962199985980988
770 0.960200011730194
780 0.967499971389771
790 0.972400009632111
800 0.966499984264374
810 0.971800029277802
820 0.972400009632111
830 0.972899973392487
840 0.970200002193451
850 0.970000028610229
860 0.973299980163574
870 0.97299998998642
880 0.971800029277802
890 0.968699991703033
900 0.964999973773956
910 0.971199989318848
920 0.969399988651276
930 0.963100016117096
940 0.968200027942657
950 0.965499997138977
960 0.963800013065338
970 0.972100019454956
980 0.966899991035461
990 0.973699986934662
1000 0.973699986934662
1010 0.973699986934662
1020 0.966899991035461
1030 0.96670001745224
1040 0.966099977493286
1050 0.967199981212616
1060 0.971199989318848
1070 0.969200015068054
1080 0.971400022506714
1090 0.966199994087219
1100 0.969399988651276
1110 0.969299972057343
1120 0.966199994087219
1130 0.971499979496002
1140 0.970200002193451
1150 0.971099972724915
1160 0.972400009632111
1170 0.972599983215332
1180 0.967400014400482
1190 0.970899999141693
1200 0.967700004577637
1210 0.970300018787384
1220 0.972100019454956
1230 0.96450001001358
1240 0.971000015735626
1250 0.972400009632111
1260 0.97189998626709
1270 0.971000015735626
1280 0.969600021839142
1290 0.972599983215332
1300 0.968800008296967
1310 0.969799995422363
1320 0.973299980163574
1330 0.96780002117157
1340 0.969299972057343
1350 0.966199994087219
1360 0.9689000248909
1370 0.970399975776672
1380 0.969099998474121
1390 0.971099972724915
1400 0.970600008964539
1410 0.970600008964539
1420 0.971199989318848
1430 0.971199989318848
1440 0.971199989318848
1450 0.9689000248909
1460 0.970200002193451
1470 0.971800029277802
1480 0.97409999370575
1490 0.972100019454956
1500 0.973200023174286
1510 0.969399988651276
1520 0.969799995422363
1530 0.966400027275085
1540 0.971199989318848
1550 0.968699991703033
1560 0.969799995422363
1570 0.973100006580353
1580 0.971000015735626
1590 0.970200002193451
1600 0.968500018119812
1610 0.971300005912781
1620 0.972599983215332
1630 0.965099990367889
1640 0.969900012016296
1650 0.970899999141693
1660 0.971400022506714
1670 0.967999994754791
1680 0.971499979496002
1690 0.971000015735626
1700 0.972500026226044
1710 0.970600008964539
1720 0.971000015735626
1730 0.970099985599518
1740 0.969799995422363
1750 0.971400022506714
1760 0.970600008964539
1770 0.971800029277802
1780 0.965499997138977
1790 0.967400014400482
1800 0.970000028610229
1810 0.969799995422363
1820 0.966799974441528
1830 0.968299984931946
1840 0.969799995422363
1850 0.964200019836426
1860 0.970200002193451
1870 0.971800029277802
1880 0.970600008964539
1890 0.97079998254776
1900 0.967100024223328
1910 0.96969997882843
1920 0.9689000248909
1930 0.966600000858307
1940 0.96969997882843
1950 0.972100019454956
1960 0.959699988365173
1970 0.967700004577637
1980 0.969200015068054
1990 0.97079998254776
2000 0.972199976444244
2010 0.972199976444244
2020 0.969799995422363
2030 0.972899973392487
2040 0.971800029277802
2050 0.969299972057343
2060 0.971800029277802
2070 0.97409999370575
2080 0.973299980163574
2090 0.968699991703033
2100 0.97409999370575
2110 0.971300005912781
2120 0.971300005912781
2130 0.970000028610229
2140 0.968200027942657
2150 0.969099998474121
2160 0.969099998474121
2170 0.968500018119812
2180 0.973200023174286
2190 0.971400022506714
2200 0.970499992370605
2210 0.971300005912781
2220 0.973599970340729
2230 0.972800016403198
2240 0.968400001525879
2250 0.970499992370605
2260 0.973900020122528
2270 0.969900012016296
2280 0.972400009632111
2290 0.970899999141693
2300 0.970499992370605
2310 0.962800025939941
2320 0.96969997882843
2330 0.967000007629395
2340 0.968400001525879
2350 0.966199994087219
2360 0.970000028610229
2370 0.971099972724915
2380 0.971400022506714
2390 0.970899999141693
2400 0.972800016403198
2410 0.972800016403198
2420 0.972800016403198
2430 0.972800016403198
2440 0.972800016403198
2450 0.970499992370605
2460 0.970200002193451
2470 0.971800029277802
2480 0.972599983215332
2490 0.973200023174286
2500 0.973200023174286
2510 0.973200023174286
2520 0.973200023174286
2530 0.971400022506714
2540 0.970200002193451
2550 0.972800016403198
2560 0.971400022506714
2570 0.969399988651276
2580 0.975899994373322
2590 0.9685999751091
2600 0.972800016403198
2610 0.971300005912781
2620 0.971300005912781
2630 0.971300005912781
2640 0.971300005912781
2650 0.965699970722198
2660 0.967000007629395
2670 0.963900029659271
2680 0.971300005912781
2690 0.962999999523163
2700 0.969200015068054
2710 0.96780002117157
2720 0.970000028610229
2730 0.969900012016296
2740 0.969900012016296
2750 0.968800008296967
2760 0.967599987983704
2770 0.969500005245209
2780 0.970899999141693
2790 0.96969997882843
2800 0.968999981880188
2810 0.968999981880188
2820 0.970000028610229
2830 0.971300005912781
2840 0.971000015735626
2850 0.970399975776672
2860 0.971300005912781
2870 0.973100006580353
2880 0.96560001373291
2890 0.969099998474121
2900 0.969900012016296
2910 0.970899999141693
2920 0.967299997806549
2930 0.971000015735626
2940 0.972800016403198
2950 0.970399975776672
2960 0.968299984931946
2970 0.972199976444244
2980 0.967499971389771
2990 0.964399993419647
3000 0.97079998254776
3010 0.971300005912781
3020 0.971599996089935
3030 0.967599987983704
3040 0.969299972057343
3050 0.97299998998642
3060 0.97299998998642
3070 0.973100006580353
3080 0.97299998998642
3090 0.973100006580353
3100 0.973100006580353
3110 0.973100006580353
3120 0.973100006580353
3130 0.973100006580353
3140 0.973100006580353
3150 0.973100006580353
3160 0.973100006580353
3170 0.973100006580353
3180 0.970000028610229
3190 0.969200015068054
3200 0.97409999370575
3210 0.969600021839142
3220 0.969799995422363
3230 0.969799995422363
3240 0.969799995422363
3250 0.968999981880188
3260 0.968100011348724
3270 0.958899974822998
3280 0.969099998474121
3290 0.972299993038177
3300 0.970600008964539
3310 0.972000002861023
3320 0.972000002861023
3330 0.972000002861023
3340 0.972000002861023
3350 0.972000002861023
3360 0.97189998626709
3370 0.972400009632111
3380 0.974699974060059
3390 0.971800029277802
3400 0.97079998254776
3410 0.972699999809265
3420 0.972699999809265
3430 0.972699999809265
3440 0.972699999809265
3450 0.965399980545044
3460 0.971499979496002
3470 0.970399975776672
3480 0.970899999141693
3490 0.971199989318848
3500 0.972199976444244
3510 0.971800029277802
3520 0.972599983215332
3530 0.972899973392487
3540 0.972699999809265
3550 0.969299972057343
3560 0.969500005245209
3570 0.970600008964539
3580 0.971800029277802
3590 0.969200015068054
3600 0.969099998474121
3610 0.973200023174286
3620 0.971199989318848
3630 0.971800029277802
3640 0.971800029277802
3650 0.971099972724915
3660 0.969600021839142
3670 0.967000007629395
3680 0.969600021839142
3690 0.971499979496002
3700 0.972299993038177
3710 0.972599983215332
3720 0.965300023555756
3730 0.968400001525879
3740 0.970000028610229
3750 0.972100019454956
3760 0.972199976444244
3770 0.972199976444244
3780 0.972100019454956
3790 0.972000002861023
3800 0.971400022506714
3810 0.972199976444244
3820 0.972199976444244
3830 0.972199976444244
3840 0.963900029659271
3850 0.968699991703033
3860 0.968200027942657
3870 0.969900012016296
3880 0.971499979496002
3890 0.970399975776672
3900 0.970099985599518
3910 0.969900012016296
3920 0.972599983215332
3930 0.97079998254776
3940 0.967999994754791
3950 0.969399988651276
3960 0.971800029277802
3970 0.96969997882843
3980 0.96969997882843
3990 0.96969997882843
4000 0.968299984931946
4010 0.966000020503998
4020 0.968100011348724
4030 0.966899991035461
4040 0.966899991035461
4050 0.967400014400482
4060 0.970099985599518
4070 0.967499971389771
4080 0.967199981212616
4090 0.96969997882843
4100 0.971400022506714
4110 0.972800016403198
4120 0.968999981880188
4130 0.972899973392487
4140 0.973599970340729
4150 0.97350001335144
4160 0.972800016403198
4170 0.97079998254776
4180 0.97189998626709
4190 0.970099985599518
4200 0.969399988651276
4210 0.970499992370605
4220 0.972000002861023
4230 0.97350001335144
4240 0.970899999141693
4250 0.968299984931946
4260 0.973900020122528
4270 0.972699999809265
4280 0.972699999809265
4290 0.97079998254776
4300 0.971599996089935
4310 0.973599970340729
4320 0.973599970340729
4330 0.973599970340729
4340 0.973599970340729
4350 0.968100011348724
4360 0.970399975776672
4370 0.970700025558472
4380 0.971199989318848
4390 0.973800003528595
4400 0.971400022506714
4410 0.970099985599518
4420 0.970200002193451
4430 0.971499979496002
4440 0.971099972724915
4450 0.971199989318848
4460 0.969399988651276
4470 0.972100019454956
4480 0.968800008296967
4490 0.969200015068054
4500 0.970899999141693
4510 0.972500026226044
4520 0.972599983215332
4530 0.97079998254776
4540 0.97079998254776
4550 0.97079998254776
4560 0.97079998254776
4570 0.97079998254776
4580 0.97079998254776
4590 0.97079998254776
4600 0.97079998254776
4610 0.97079998254776
4620 0.97079998254776
4630 0.97079998254776
4640 0.97079998254776
4650 0.97079998254776
4660 0.97079998254776
4670 0.97079998254776
4680 0.97079998254776
4690 0.97079998254776
4700 0.97079998254776
4710 0.97079998254776
4720 0.97079998254776
4730 0.97079998254776
4740 0.97079998254776
4750 0.97079998254776
4760 0.97079998254776
4770 0.97079998254776
4780 0.97079998254776
4790 0.97079998254776
4800 0.97079998254776
4810 0.97079998254776
4820 0.97079998254776
4830 0.97079998254776
4840 0.97079998254776
4850 0.97079998254776
4860 0.97079998254776
4870 0.97079998254776
4880 0.97079998254776
4890 0.97079998254776
4900 0.97079998254776
4910 0.97079998254776
4920 0.97079998254776
4930 0.97079998254776
4940 0.97079998254776
4950 0.97079998254776
4960 0.97079998254776
4970 0.97079998254776
4980 0.97079998254776
4990 0.97079998254776
5000 0.97079998254776
};
%\addlegendentry{Test}

==> experiments/figures/mae_ri_05.tex <==
\addplot[semithick, color4] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.0917000025510788
10 0.465079993009567
20 0.481119990348816
30 0.482520014047623
40 0.47503998875618
50 0.47843998670578
60 0.485159993171692
70 0.483819991350174
80 0.482520014047623
90 0.486939996480942
100 0.480300009250641
110 0.48633998632431
120 0.487879991531372
130 0.484219998121262
140 0.489340007305145
150 0.488440006971359
160 0.477539986371994
170 0.482820004224777
180 0.488579988479614
190 0.489300012588501
200 0.489340007305145
210 0.489939987659454
220 0.488719999790192
230 0.488880008459091
240 0.491380006074905
250 0.487320005893707
260 0.489659994840622
270 0.488660007715225
280 0.487780004739761
290 0.486059993505478
300 0.488640010356903
310 0.485260009765625
320 0.490619987249374
330 0.491400003433228
340 0.491239994764328
350 0.491459995508194
360 0.49261999130249
370 0.492040008306503
380 0.493499994277954
390 0.492839992046356
400 0.49252000451088
410 0.491140007972717
420 0.492080003023148
430 0.478100001811981
440 0.491279989480972
450 0.488400012254715
460 0.493499994277954
470 0.485760003328323
480 0.492879986763
490 0.492940008640289
500 0.488999992609024
510 0.490220010280609
520 0.486440002918243
530 0.490139991044998
540 0.491540014743805
550 0.488719999790192
560 0.492500007152557
570 0.492060005664825
580 0.481240004301071
590 0.490599989891052
600 0.491059988737106
610 0.486400008201599
620 0.491239994764328
630 0.489859998226166
640 0.492260009050369
650 0.492419987916946
660 0.488920003175735
670 0.492500007152557
680 0.493440002202988
690 0.488040000200272
700 0.491459995508194
710 0.491059988737106
720 0.493739992380142
730 0.493220001459122
740 0.485179990530014
750 0.492720007896423
760 0.493479996919632
770 0.493400007486343
780 0.494439989328384
790 0.493099987506866
800 0.494540005922318
810 0.494619995355606
820 0.495180010795593
830 0.49549999833107
840 0.488840013742447
850 0.494480013847351
860 0.49210000038147
870 0.49575999379158
880 0.49524000287056
890 0.495099991559982
900 0.496080011129379
910 0.493479996919632
920 0.494940012693405
930 0.488860011100769
940 0.496120005846024
950 0.496100008487701
960 0.494100004434586
970 0.492700010538101
980 0.495099991559982
990 0.495059996843338
1000 0.490220010280609
1010 0.491899996995926
1020 0.496039986610413
1030 0.493239998817444
1040 0.494879990816116
1050 0.491780012845993
1060 0.495539993047714
1070 0.497000008821487
1080 0.492000013589859
1090 0.497440010309219
1100 0.496280014514923
1110 0.493999987840652
1120 0.495180010795593
1130 0.494159996509552
1140 0.494839996099472
1150 0.494019985198975
1160 0.496199995279312
1170 0.497900009155273
1180 0.494500011205673
1190 0.495480000972748
1200 0.49524000287056
1210 0.496259987354279
1220 0.49388000369072
1230 0.494159996509552
1240 0.493959993124008
1250 0.492500007152557
1260 0.49397999048233
1270 0.49439999461174
1280 0.496160000562668
1290 0.491719990968704
1300 0.497339993715286
1310 0.494899988174438
1320 0.49125999212265
1330 0.496380001306534
1340 0.497599989175797
1350 0.49753999710083
1360 0.495119988918304
1370 0.495939999818802
1380 0.494679987430573
1390 0.491580009460449
1400 0.495059996843338
1410 0.49711999297142
1420 0.49702000617981
1430 0.494960010051727
1440 0.497519999742508
1450 0.493580013513565
1460 0.49796000123024
1470 0.496879994869232
1480 0.49277999997139
1490 0.495880007743835
1500 0.497359991073608
1510 0.4966000020504
1520 0.498059988021851
1530 0.497740000486374
1540 0.493160009384155
1550 0.495799988508224
1560 0.496540009975433
1570 0.493840008974075
1580 0.496560007333755
1590 0.49779999256134
1600 0.497900009155273
1610 0.496960014104843
1620 0.497420012950897
1630 0.498279988765717
1640 0.496360003948212
1650 0.495299994945526
1660 0.496360003948212
1670 0.496879994869232
1680 0.498320013284683
1690 0.498180001974106
1700 0.499240010976791
1710 0.496800005435944
1720 0.49617999792099
1730 0.49524000287056
1740 0.49711999297142
1750 0.498140007257462
1760 0.496580004692078
1770 0.498140007257462
1780 0.499599993228912
1790 0.499779999256134
1800 0.492659986019135
1810 0.499020010232925
1820 0.498439997434616
1830 0.496100008487701
1840 0.498059988021851
1850 0.494960010051727
1860 0.4966000020504
1870 0.4966000020504
1880 0.4966000020504
1890 0.496160000562668
1900 0.497339993715286
1910 0.497900009155273
1920 0.498780012130737
1930 0.498780012130737
1940 0.498780012130737
1950 0.498320013284683
1960 0.496919989585876
1970 0.499199986457825
1980 0.498320013284683
1990 0.497599989175797
2000 0.497599989175797
2010 0.497599989175797
2020 0.497599989175797
2030 0.495719999074936
2040 0.49481999874115
2050 0.491200000047684
2060 0.496499985456467
2070 0.495319992303848
2080 0.496820002794266
2090 0.494280010461807
2100 0.493660002946854
2110 0.495819985866547
2120 0.498439997434616
2130 0.497060000896454
2140 0.497680008411407
2150 0.4966000020504
2160 0.499099999666214
2170 0.499179989099503
2180 0.499179989099503
2190 0.499179989099503
2200 0.499199986457825
2210 0.499220013618469
2220 0.499220013618469
2230 0.496560007333755
2240 0.495539993047714
2250 0.49821999669075
2260 0.49821999669075
2270 0.49821999669075
2280 0.49821999669075
2290 0.49821999669075
2300 0.498199999332428
2310 0.496160000562668
2320 0.496639996767044
2330 0.496320009231567
2340 0.494580000638962
2350 0.498679995536804
2360 0.498679995536804
2370 0.498699992895126
2380 0.49601998925209
2390 0.495539993047714
2400 0.498580008745193
2410 0.498580008745193
2420 0.496560007333755
2430 0.491959989070892
2440 0.496320009231567
2450 0.497079998254776
2460 0.498299986124039
2470 0.495660006999969
2480 0.499099999666214
2490 0.499220013618469
2500 0.498979985713959
2510 0.498439997434616
2520 0.497940003871918
2530 0.499119997024536
2540 0.496520012617111
2550 0.496320009231567
2560 0.495779991149902
2570 0.500280022621155
2580 0.497260004281998
2590 0.499900013208389
2600 0.499379992485046
2610 0.49702000617981
2620 0.49702000617981
2630 0.49702000617981
2640 0.49702000617981
2650 0.500760018825531
2660 0.49533998966217
2670 0.499220013618469
2680 0.499000012874603
2690 0.499240010976791
2700 0.494800001382828
2710 0.498679995536804
2720 0.499799996614456
2730 0.499000012874603
2740 0.497759997844696
2750 0.500660002231598
2760 0.499119997024536
2770 0.499119997024536
2780 0.495939999818802
2790 0.499139994382858
2800 0.500159978866577
2810 0.500779986381531
2820 0.499980002641678
2830 0.496939986944199
2840 0.499520003795624
2850 0.501219987869263
2860 0.500379979610443
2870 0.49932000041008
2880 0.500580012798309
2890 0.500580012798309
2900 0.500580012798309
2910 0.500580012798309
2920 0.494899988174438
2930 0.496939986944199
2940 0.49838000535965
2950 0.499020010232925
2960 0.495180010795593
2970 0.499040007591248
2980 0.50084000825882
2990 0.498659998178482
3000 0.500620007514954
3010 0.498840004205704
3020 0.500800013542175
3030 0.499500006437302
3040 0.499819993972778
3050 0.498800009489059
3060 0.500280022621155
3070 0.499500006437302
3080 0.500720024108887
3090 0.500720024108887
3100 0.499339997768402
3110 0.497940003871918
3120 0.499020010232925
3130 0.496580004692078
3140 0.498959988355637
3150 0.495840013027191
3160 0.499179989099503
3170 0.498259991407394
3180 0.497900009155273
3190 0.498780012130737
3200 0.498519986867905
3210 0.49889999628067
3220 0.498620003461838
3230 0.498620003461838
3240 0.498620003461838
3250 0.498400002717972
3260 0.498580008745193
3270 0.499819993972778
3280 0.500819981098175
3290 0.500519990921021
3300 0.496239989995956
3310 0.496239989995956
3320 0.496239989995956
3330 0.495599985122681
3340 0.4998399913311
3350 0.500299990177155
3360 0.495880007743835
3370 0.498840004205704
3380 0.499720007181168
3390 0.499720007181168
3400 0.499720007181168
3410 0.499720007181168
3420 0.499819993972778
3430 0.500379979610443
3440 0.498400002717972
3450 0.496219992637634
3460 0.500379979610443
3470 0.500060021877289
3480 0.498499989509583
3490 0.497060000896454
3500 0.499419987201691
3510 0.496619999408722
3520 0.499639987945557
3530 0.496619999408722
3540 0.498019993305206
3550 0.501420021057129
3560 0.499960005283356
3570 0.492659986019135
3580 0.500940024852753
3590 0.500999987125397
3600 0.499419987201691
3610 0.500440001487732
3620 0.500440001487732
3630 0.499440014362335
3640 0.499000012874603
3650 0.501659989356995
3660 0.493140012025833
3670 0.500980019569397
3680 0.499379992485046
3690 0.498299986124039
3700 0.496060013771057
3710 0.499359995126724
3720 0.499779999256134
3730 0.498140007257462
3740 0.500779986381531
3750 0.498360008001328
3760 0.496060013771057
3770 0.499980002641678
3780 0.499920010566711
3790 0.499480009078979
3800 0.499639987945557
3810 0.498939990997314
3820 0.498860001564026
3830 0.499900013208389
3840 0.500440001487732
3850 0.500440001487732
3860 0.500440001487732
3870 0.500440001487732
3880 0.49915999174118
3890 0.500419974327087
3900 0.499339997768402
3910 0.499339997768402
3920 0.499339997768402
3930 0.497359991073608
3940 0.500039994716644
3950 0.500199973583221
3960 0.50135999917984
3970 0.499779999256134
3980 0.500760018825531
3990 0.501860022544861
4000 0.501860022544861
4010 0.501860022544861
4020 0.501860022544861
4030 0.500100016593933
4040 0.497839987277985
4050 0.497839987277985
4060 0.497839987277985
4070 0.497839987277985
4080 0.497920006513596
4090 0.498879998922348
4100 0.501900017261505
4110 0.498540014028549
4120 0.500880002975464
4130 0.501579999923706
4140 0.501579999923706
4150 0.501579999923706
4160 0.501579999923706
4170 0.501579999923706
4180 0.501579999923706
4190 0.501579999923706
4200 0.501579999923706
4210 0.501579999923706
4220 0.501579999923706
4230 0.501579999923706
4240 0.501579999923706
4250 0.501579999923706
4260 0.501579999923706
4270 0.501579999923706
4280 0.501579999923706
4290 0.501579999923706
4300 0.501579999923706
4310 0.501579999923706
4320 0.501579999923706
4330 0.501579999923706
4340 0.501579999923706
4350 0.501579999923706
4360 0.501579999923706
4370 0.501579999923706
4380 0.501579999923706
4390 0.501579999923706
4400 0.501579999923706
4410 0.501579999923706
4420 0.501579999923706
4430 0.501579999923706
4440 0.501579999923706
4450 0.501579999923706
4460 0.501579999923706
4470 0.501579999923706
4480 0.501579999923706
4490 0.501579999923706
4500 0.501579999923706
4510 0.501579999923706
4520 0.501579999923706
4530 0.501579999923706
4540 0.501579999923706
4550 0.501579999923706
4560 0.501579999923706
4570 0.501579999923706
4580 0.501579999923706
4590 0.501579999923706
4600 0.501579999923706
4610 0.501579999923706
4620 0.501579999923706
4630 0.501579999923706
4640 0.501579999923706
4650 0.501579999923706
4660 0.501579999923706
4670 0.501579999923706
4680 0.501579999923706
4690 0.501579999923706
4700 0.501579999923706
4710 0.501579999923706
4720 0.501579999923706
4730 0.501579999923706
4740 0.501579999923706
4750 0.501579999923706
4760 0.501579999923706
4770 0.501579999923706
4780 0.501579999923706
4790 0.501579999923706
4800 0.501579999923706
4810 0.501579999923706
4820 0.501579999923706
4830 0.501579999923706
4840 0.501579999923706
4850 0.501579999923706
4860 0.501579999923706
4870 0.501579999923706
4880 0.501579999923706
4890 0.501579999923706
4900 0.501579999923706
4910 0.501579999923706
4920 0.501579999923706
4930 0.501579999923706
4940 0.501579999923706
4950 0.501579999923706
4960 0.501579999923706
4970 0.501579999923706
4980 0.501579999923706
4990 0.501579999923706
5000 0.501579999923706
};
%\addlegendentry{Train}
\addplot[semithick, color5] % x filter/.code={\pgfmathparse{#1*0.1}\pgfmathresult}
table {%
0 0.0812000036239624
10 0.907000005245209
20 0.942099988460541
30 0.943199992179871
40 0.92739999294281
50 0.934599995613098
60 0.949199974536896
70 0.944599986076355
80 0.942399978637695
90 0.952899992465973
100 0.93639999628067
110 0.949999988079071
120 0.951200008392334
130 0.946300029754639
140 0.956099987030029
150 0.954999983310699
160 0.929499983787537
170 0.9375
180 0.949000000953674
190 0.95440000295639
200 0.95550000667572
210 0.957300007343292
220 0.947899997234344
230 0.953599989414215
240 0.957499980926514
250 0.950800001621246
260 0.955999970436096
270 0.948300004005432
280 0.951099991798401
290 0.947099983692169
300 0.948099970817566
310 0.942600011825562
320 0.953700006008148
330 0.958299994468689
340 0.954900026321411
350 0.953999996185303
360 0.957899987697601
370 0.957199990749359
380 0.958100020885468
390 0.959200024604797
400 0.95990002155304
410 0.953199982643127
420 0.956499993801117
430 0.923799991607666
440 0.95880001783371
450 0.951099991798401
460 0.960399985313416
470 0.94489997625351
480 0.958000004291534
490 0.961099982261658
500 0.949000000953674
510 0.95550000667572
520 0.943700015544891
530 0.949999988079071
540 0.951399981975555
550 0.950900018215179
560 0.959999978542328
570 0.956900000572205
580 0.936200022697449
590 0.954900026321411
600 0.955799996852875
610 0.944500029087067
620 0.953599989414215
630 0.952600002288818
640 0.953499972820282
650 0.955799996852875
660 0.947799980640411
670 0.958100020885468
680 0.960900008678436
690 0.944599986076355
700 0.953299999237061
710 0.952099978923798
720 0.958700001239777
730 0.956900000572205
740 0.942399978637695
750 0.955099999904633
760 0.957599997520447
770 0.956499993801117
780 0.957099974155426
790 0.953299999237061
800 0.958999991416931
810 0.959500014781952
820 0.961000025272369
830 0.962000012397766
840 0.94870001077652
850 0.958899974822998
860 0.952000021934509
870 0.959999978542328
880 0.957899987697601
890 0.95959997177124
900 0.962400019168854
910 0.954999983310699
920 0.956700026988983
930 0.945500016212463
940 0.961099982261658
950 0.960500001907349
960 0.953999996185303
970 0.952099978923798
980 0.961300015449524
990 0.958599984645844
1000 0.947099983692169
1010 0.953700006008148
1020 0.959699988365173
1030 0.955200016498566
1040 0.954100012779236
1050 0.947499990463257
1060 0.954800009727478
1070 0.955999970436096
1080 0.949500024318695
1090 0.95990002155304
1100 0.959699988365173
1110 0.956300020217896
1120 0.954500019550323
1130 0.955399990081787
1140 0.955699980258942
1150 0.954299986362457
1160 0.960099995136261
1170 0.960799992084503
1180 0.954900026321411
1190 0.958500027656555
1200 0.954299986362457
1210 0.957099974155426
1220 0.953499972820282
1230 0.955799996852875
1240 0.951600015163422
1250 0.950999975204468
1260 0.950600028038025
1270 0.954100012779236
1280 0.958999991416931
1290 0.94870001077652
1300 0.961000025272369
1310 0.95169997215271
1320 0.951600015163422
1330 0.95880001783371
1340 0.959800004959106
1350 0.961300015449524
1360 0.955999970436096
1370 0.95660001039505
1380 0.950699985027313
1390 0.949000000953674
1400 0.955999970436096
1410 0.956200003623962
1420 0.958700001239777
1430 0.958400011062622
1440 0.959200024604797
1450 0.948599994182587
1460 0.956799983978271
1470 0.955900013446808
1480 0.945599973201752
1490 0.955099999904633
1500 0.956799983978271
1510 0.952899992465973
1520 0.959999978542328
1530 0.955099999904633
1540 0.94870001077652
1550 0.956099987030029
1560 0.956099987030029
1570 0.951600015163422
1580 0.957499980926514
1590 0.960500001907349
1600 0.959800004959106
1610 0.960399985313416
1620 0.959200024604797
1630 0.960200011730194
1640 0.956200003623962
1650 0.95440000295639
1660 0.958299994468689
1670 0.955699980258942
1680 0.958000004291534
1690 0.955799996852875
1700 0.95959997177124
1710 0.95770001411438
1720 0.953700006008148
1730 0.951900005340576
1740 0.955900013446808
1750 0.957499980926514
1760 0.956399977207184
1770 0.958599984645844
1780 0.959399998188019
1790 0.95880001783371
1800 0.945599973201752
1810 0.960900008678436
1820 0.95660001039505
1830 0.953700006008148
1840 0.958700001239777
1850 0.954299986362457
1860 0.955699980258942
1870 0.955699980258942
1880 0.955699980258942
1890 0.953299999237061
1900 0.955999970436096
1910 0.957899987697601
1920 0.958500027656555
1930 0.958500027656555
1940 0.958500027656555
1950 0.956399977207184
1960 0.956799983978271
1970 0.960099995136261
1980 0.957300007343292
1990 0.956799983978271
2000 0.956799983978271
2010 0.956799983978271
2020 0.956799983978271
2030 0.950800001621246
2040 0.951900005340576
2050 0.943400025367737
2060 0.956499993801117
2070 0.954500019550323
2080 0.958599984645844
2090 0.950200021266937
2100 0.947000026702881
2110 0.950200021266937
2120 0.956099987030029
2130 0.955299973487854
2140 0.958100020885468
2150 0.95550000667572
2160 0.958599984645844
2170 0.958500027656555
2180 0.958500027656555
2190 0.958500027656555
2200 0.958500027656555
2210 0.958400011062622
2220 0.958299994468689
2230 0.95550000667572
2240 0.951900005340576
2250 0.957300007343292
2260 0.957300007343292
2270 0.957300007343292
2280 0.957199990749359
2290 0.957300007343292
2300 0.957400023937225
2310 0.955299973487854
2320 0.953199982643127
2330 0.957799971103668
2340 0.949899971485138
2350 0.959399998188019
2360 0.959399998188019
2370 0.959399998188019
2380 0.95440000295639
2390 0.951099991798401
2400 0.957300007343292
2410 0.957300007343292
2420 0.955699980258942
2430 0.946099996566772
2440 0.949999988079071
2450 0.95440000295639
2460 0.958400011062622
2470 0.954999983310699
2480 0.958599984645844
2490 0.959299981594086
2500 0.955200016498566
2510 0.958199977874756
2520 0.957199990749359
2530 0.956200003623962
2540 0.95389997959137
2550 0.95169997215271
2560 0.949299991130829
2570 0.9617999792099
2580 0.953999996185303
2590 0.960600018501282
2600 0.960099995136261
2610 0.954599976539612
2620 0.954599976539612
2630 0.954599976539612
2640 0.954500019550323
2650 0.961499989032745
2660 0.952099978923798
2670 0.958400011062622
2680 0.959200024604797
2690 0.95990002155304
2700 0.949000000953674
2710 0.954800009727478
2720 0.95959997177124
2730 0.957599997520447
2740 0.955799996852875
2750 0.961600005626678
2760 0.958299994468689
2770 0.958299994468689
2780 0.951900005340576
2790 0.958199977874756
2800 0.95990002155304
2810 0.961099982261658
2820 0.960099995136261
2830 0.952499985694885
2840 0.959999978542328
2850 0.962000012397766
2860 0.960600018501282
2870 0.960200011730194
2880 0.960300028324127
2890 0.960300028324127
2900 0.960300028324127
2910 0.960300028324127
2920 0.950999975204468
2930 0.958100020885468
2940 0.95959997177124
2950 0.957000017166138
2960 0.951900005340576
2970 0.957400023937225
2980 0.961899995803833
2990 0.956399977207184
3000 0.960300028324127
3010 0.958199977874756
3020 0.960600018501282
3030 0.957400023937225
3040 0.95959997177124
3050 0.957599997520447
3060 0.959299981594086
3070 0.95660001039505
3080 0.959399998188019
3090 0.959399998188019
3100 0.959299981594086
3110 0.955299973487854
3120 0.955999970436096
3130 0.951300024986267
3140 0.956499993801117
3150 0.951399981975555
3160 0.957499980926514
3170 0.957000017166138
3180 0.954699993133545
3190 0.95660001039505
3200 0.958000004291534
3210 0.958599984645844
3220 0.95770001411438
3230 0.95770001411438
3240 0.957799971103668
3250 0.95660001039505
3260 0.956499993801117
3270 0.960500001907349
3280 0.960900008678436
3290 0.958999991416931
3300 0.94980001449585
3310 0.94980001449585
3320 0.94980001449585
3330 0.954599976539612
3340 0.958999991416931
3350 0.960200011730194
3360 0.951200008392334
3370 0.957199990749359
3380 0.957099974155426
3390 0.957099974155426
3400 0.957099974155426
3410 0.957099974155426
3420 0.962599992752075
3430 0.956799983978271
3440 0.957099974155426
3450 0.950699985027313
3460 0.961600005626678
3470 0.95880001783371
3480 0.956399977207184
3490 0.954999983310699
3500 0.956499993801117
3510 0.950500011444092
3520 0.957000017166138
3530 0.951200008392334
3540 0.955999970436096
3550 0.962599992752075
3560 0.959800004959106
3570 0.944000005722046
3580 0.961600005626678
3590 0.96069997549057
3600 0.957499980926514
3610 0.961000025272369
3620 0.961000025272369
3630 0.956099987030029
3640 0.955600023269653
3650 0.961700022220612
3660 0.943499982357025
3670 0.960399985313416
3680 0.959500014781952
3690 0.954500019550323
3700 0.954200029373169
3710 0.959200024604797
3720 0.960099995136261
3730 0.953100025653839
3740 0.958299994468689
3750 0.954299986362457
3760 0.950500011444092
3770 0.959399998188019
3780 0.958999991416931
3790 0.959299981594086
3800 0.958899974822998
3810 0.957400023937225
3820 0.955999970436096
3830 0.958100020885468
3840 0.958400011062622
3850 0.958400011062622
3860 0.958400011062622
3870 0.958400011062622
3880 0.958199977874756
3890 0.959299981594086
3900 0.957599997520447
3910 0.957599997520447
3920 0.957599997520447
3930 0.952199995517731
3940 0.95770001411438
3950 0.959200024604797
3960 0.962599992752075
3970 0.959299981594086
3980 0.959999978542328
3990 0.960099995136261
4000 0.960099995136261
4010 0.960099995136261
4020 0.960099995136261
4030 0.958100020885468
4040 0.953999996185303
4050 0.953999996185303
4060 0.953999996185303
4070 0.953999996185303
4080 0.95550000667572
4090 0.955699980258942
4100 0.962499976158142
4110 0.957099974155426
4120 0.960099995136261
4130 0.961899995803833
4140 0.961899995803833
4150 0.961899995803833
4160 0.962100028991699
4170 0.962100028991699
4180 0.962100028991699
4190 0.962100028991699
4200 0.962100028991699
4210 0.962100028991699
4220 0.962100028991699
4230 0.962100028991699
4240 0.962100028991699
4250 0.962100028991699
4260 0.962100028991699
4270 0.962100028991699
4280 0.962100028991699
4290 0.962100028991699
4300 0.962100028991699
4310 0.962100028991699
4320 0.962100028991699
4330 0.962100028991699
4340 0.962100028991699
4350 0.962100028991699
4360 0.962100028991699
4370 0.962100028991699
4380 0.962100028991699
4390 0.962100028991699
4400 0.962100028991699
4410 0.962100028991699
4420 0.962100028991699
4430 0.962100028991699
4440 0.962100028991699
4450 0.962100028991699
4460 0.962100028991699
4470 0.962100028991699
4480 0.962100028991699
4490 0.962100028991699
4500 0.962100028991699
4510 0.962100028991699
4520 0.962100028991699
4530 0.962100028991699
4540 0.962100028991699
4550 0.962100028991699
4560 0.962100028991699
4570 0.962100028991699
4580 0.962100028991699
4590 0.962100028991699
4600 0.962100028991699
4610 0.962100028991699
4620 0.962100028991699
4630 0.962100028991699
4640 0.962100028991699
4650 0.962100028991699
4660 0.962100028991699
4670 0.962100028991699
4680 0.962100028991699
4690 0.962100028991699
4700 0.962100028991699
4710 0.962100028991699
4720 0.962100028991699
4730 0.962100028991699
4740 0.962100028991699
4750 0.962100028991699
4760 0.962100028991699
4770 0.962100028991699
4780 0.962100028991699
4790 0.962100028991699
4800 0.962100028991699
4810 0.962100028991699
4820 0.962100028991699
4830 0.962100028991699
4840 0.962100028991699
4850 0.962100028991699
4860 0.962100028991699
4870 0.962100028991699
4880 0.962100028991699
4890 0.962100028991699
4900 0.962100028991699
4910 0.962100028991699
4920 0.962100028991699
4930 0.962100028991699
4940 0.962100028991699
4950 0.962100028991699
4960 0.962100028991699
4970 0.962100028991699
4980 0.962100028991699
4990 0.962100028991699
5000 0.962100028991699
};
%\addlegendentry{Test}


==> experiments/figures/overfitting_test_acc.tex <==
\tikzset{font={\fontsize{15pt}{12}\selectfont}}

\input{experiments/figures/omega_0_acc}
\input{experiments/figures/omega_03_acc}
\input{experiments/figures/omega_05_acc}
